ViWiD: Leveraging WiFi for Robust and Resource-Efficient SLAM

Recent interest towards autonomous navigation and exploration robots for indoor applications has spurred research into indoor Simultaneous Localization and Mapping (SLAM) robot systems. While most of these SLAM systems use Visual and LiDAR sensors in tandem with an odometry sensor, these odometry sensors drift over time. To combat this drift, Visual SLAM systems deploy compute and memory intensive search algorithms to detect `Loop Closures', which make the trajectory estimate globally consistent. To circumvent these resource (compute and memory) intensive algorithms, we present ViWiD, which integrates WiFi and Visual sensors in a dual-layered system. This dual-layered approach separates the tasks of local and global trajectory estimation making ViWiD resource efficient while achieving on-par or better performance to state-of-the-art Visual SLAM. We demonstrate ViWiD's performance on four datasets, covering over 1500 m of traversed path and show 4.3x and 4x reduction in compute and memory consumption respectively compared to state-of-the-art Visual and Lidar SLAM systems with on par SLAM performance.

==> ViWiD SLAM_arx/abstract/abstract1.tex <==
% !TEX root = root.tex

\begin{abstract}
% A recent spur of interest in indoor robotics has increased the importance of robust simultaneous localization and mapping algorithms in indoor scenarios. This robustness is typically provided by the use of multiple sensors which can correct each others' deficiencies. In this vein, exteroceptive sensors, like cameras and LiDARs, employed for fusion are capable of correcting the drifts accumulated by wheel odometry or inertial measurement units (IMU's). However, these exteroceptive sensors suffer their own deficiencies in highly structured environments and dynamic lighting conditions. This paper will present WiFi as a robust and straightforward sensing modality capable of circumventing these issues. Specifically, we make three contributions. First, we will understand the necessary features to be extracted from WiFi signals. Second, we characterize the quality of these measurements. Third, we integrate these features with odometry into a state-of-art GraphSLAM backend. We present our results in a $25 \times 30$ m and $50 \times 40$ environment and robustly test the system by driving the robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $6 \times$ with respect to odometry-only estimation and perform on par with one of the state-of-the-art Visual-based SLAM. 

WiFi infrastructure is ubiquitous in most indoor settings and thus can be leveraged as a sensor for indoor mapping and navigation. In this paper, we present \name, which incorporates WiFi as a bearing sensor and densely fuses it with visual features from a monocular camera and odometry sensors. The sensor fusion proposed in \name provides accurate and accessible localization and mapping capabilities scalable to large indoor environments. To showcase these claims, \name is deployed in two real-world environments, spanning $25 \times 30$ m and $50 \times 40$ m, and robustly tested by driving the robot a cumulative distance of over $1225$ m. In these evaluations, \name shows an improvement of $xx \times$ and $xx \times$ over solely using odometry and visual-inertial odometry respectively. \name is further showcased by deploying an application which autonomously navigates an office space to deliver packages to specific rooms. 
\end{abstract}

==> ViWiD SLAM_arx/abstract/abstract2.tex <==
% !TEX root = root.tex

\begin{abstract}
    Recent interest towards autonomous navigation and exploration robots for Indoor applications has spurred research into deploying Simultaneous Localization and Mapping (SLAM) systems for Indoor applications.
    While most of these SLAM systems use Visual and LiDAR sensors in tandem with a Odometer sensor, these Odometer sensors drift over time.
    This leads to the Visual SLAM systems to use compute and memory intensive algorithms to correct for this drift and perform SLAM.
    In this paper, we present \name, which integrates WiFi and Visual (camera) sensors in a dual-layered system.
    This Dual-layered approach provides independent tasks to each layer making \name memory and compute efficient while achieving comparable performance to state-of-the-art Visual SLAM.
    We demonstrate \name's performance on a dataset we have collected, spanning $25 \times 30$ m, and robustly tested by driving the robot a cumulative distance of over $1000$m.
    Wherein we show that we consume 5$\times$ less compute and 3$\times$ less memory on average compared to state-of-the-art Visual SLAM system.
\end{abstract}

==> ViWiD SLAM_arx/abstract/abstract3.tex <==
% !TEX root = root.tex

\begin{abstract}
    Recent interest towards autonomous navigation and exploration robots for indoor applications has spurred research into indoor Simultaneous Localization and Mapping (SLAM) robot systems.
    While most of these SLAM systems use Visual and LiDAR sensors in tandem with an odometry sensor, these odometry sensors drift over time.
    To combat this drift, Visual SLAM systems deploy compute and memory intensive search algorithms to detect `Loop Closures', which make the trajectory estimate globally consistent.
    To circumvent these resource (compute and memory) intensive algorithms, we present \name, which integrates WiFi and Visual sensors in a dual-layered system.
    This dual-layered approach separates the tasks of local and global trajectory estimation making \name resource efficient while achieving on-par or better performance to state-of-the-art Visual SLAM.
    We demonstrate \name's performance on four datasets, covering over $1500$ m of traversed path and show 4.3$\times$ and 4$\times$ reduction in compute and memory consumption respectively compared to state-of-the-art Visual and Lidar SLAM systems with on par SLAM performance.
    
    \textit{Keywords} -- Sensor Fusion; SLAM; Localization

\end{abstract}

==> ViWiD SLAM_arx/background/background1.tex <==
\section{Background and Motivation}

To robustly solve the SLAM problem requires two parts -- the sensing front-end and the optimization back-end. Consider a simple monocular camera sensor, the sensing front end would consist of two parts -- identifying robust feature keypoints in the images, and matching them across different camera image frames based on their unique descriptions. These keypoints are generally comprised of corners or edges in an image and are matched across frames by using their unique feature descriptions. A similar ideology is applied for LiDAR's or RGBD/Stereo cameras. Once a set unique keypoints, or landmarks, have been identified and matched, they are passed on to the optimization backend. In parallel, relative changes in orientation and translations are fed back to the optimization backend by the odometry sensors and GPS.

% next, the backend optimization does ...
The main purpose of the backend optimization is to take these incoming measurements from the sensing front end, collate them and provide a location estimate and create a map of the environment. To collate the information from different sensors, we need to formally define the behavior of these sensors. Each of the visual or odometry sensors are governed by observation functions, which given the current state of the robot (its position, orientation, velocity, noise and other bias parameters) and the map, can predict the potential measurement coming from the respective sensor. By design if the observation function is given an accurate state of the robot and map, it would perfectly predict the measurement from a sensor. And inversely, if we poorly predict an incoming measurement, it means an incorrect estimate of the state. In fact, this inconsistency between the predicted measurement and the true measurement can serve as an error function upon which to estimate our current state. Given multiple measurements over time and across different sensors, the backend optimizer can use this error function to converge towards an accurate state for the system. 

% NOTE: Push erroneous sensor measurements to later, maybe background and motivation ... 
To correct the former is the job of the backend optimizer; whereas the latter is a failure on part of the sensor which would hurt our state's estimation. Unfortunately, it is not easy to discern between an erroneous state estimation or a sensor's failure and depending on the environment, different sensors better serve as an accurate predictor of our state. For instance in a well lit and static environment, the landmarks extracted from a camera front-end is stable and consistent, and serve as a strong predictor of the state of our system. Hence, it falls upon the backend optimizer to keep track of ...

==> ViWiD SLAM_arx/background/background2.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system that overcomes the current SLAM systems, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of both the Visual Inertial Odometry (VIO) SLAM systems and existing Graph SLAM approaches that utilize WiFi bearing measurements. 

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}

Firstly, we describe the operations of the VIO based SLAM algorithms. 
In The existing VIO-SLAM algorithms, we take VINS-MONO~\cite{qin2018vins} as characteristic example but the understanding could be easily extended to any other systems like ORB-SLAM, RTABMap, or cartographer~\cite{orbslam,Labb2018RTABMapAA,cartographer}.

A typical VIO-SLAM that uses a monocular camera in tandem with an inertial odometry measurement has three major components that contribute towards their global pose estimation and the environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since, it is very memory intensive to store all the images for each frame, the VIO-SLAM first identifies appropriate features for each frame~\cite{swift}. 
These features are then tracked across frames to assign a fixed landmark label to consistent features, thus updating the local map of features and their identifiers, which are dubbed as `landmarks'.

\noindent(2) \textbf{Local Feature Mapping:} The multiple frames that have these landmarks are tracked across, are dubbed as `keyframes'.
These landmarks tracked across the keyframes in tandem with the inertial odometry measurements provide for a joint estimate of where these landmarks are in the 3D space and also the robot poses that have enabled this mapping. 
Thus both local robot pose and the local map are simultaneously optimized using these landmarks and odometry measurements.

Both of these above measurements do not require either large memory or heavy compute. 
This is because both of these operations need to have an active memory of last few seconds of keyframes and their landmarks that are tracked and searched within. 
Thus, they are low-compute and low-latency operations.
So, the robot continues to perform local loop-closures for every few frames to generate and incrementally build the map and estimating the robot's pose.

\noindent(3) \textbf{Global Loop Closures:}  However in the long run the robot poses and the map that has been built accrues errors. 
A few of the reasons this happens due to the drift accrued in the inertial odometer measurement and camera's turn estimated incorrectly. 
This can be avoided if let us say the camera can see very old keyframe features and correct for the accumulated drift and back-propagate this error through all the existing poses and the map.
This global drift correction is what is called global loop closure. 

However, to perform these global loop closures the SLAM algorithm needs to maintain a memory consuming dictionary of the past key frames amongst which it has to continuously search for global loop-closures, which in itself is memory and compute intensive process. Additionally, a global loop-closure detected has to optimize for the entire graph which is again a time and compute consuming operation.

We can see that cameras as a sensor are very capable to provide accurate and detailed information of local robot poses and maps. 
However, they cannot perform accurate global pose estimation and map generation in memory and compute efficient fashion. 
We observe that the global loop-closure requirements arise due to accumulated drifts and errors in the inertial odometer measurements reported to the VINS-MONO optimizer.
So if there is a sensor that can give optimized global poses for the robot without any accumulated drifts or errors.
This can be used in tandem with camera, that can handle local pose estimation and mapping and avoid the global loop-closures.

\subsection{WiFi GraphSLAM}\label{sec:back-wifi}

Now that we have established a requirement of a low-cost `Oracle' system that can provide global poses to the camera local feature tracker we can achieve low-compute and adaptable SLAM for indoor robotics. To this extend, we make few interesting observations. (i) all robots are equipped with a WiFi transceiver (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is a relatively cheap sensor modality, and (iv) there has been a couple of decades of research in WiFi based localization and tracking. Owing to these reasons we utilize WiFi as the low-cost `Oracle' sensor that can report global robot poses to the camera graph optimizer.

To that extent, we have observed that bearing measurements have been widely used as the WiFi measurements used for WiFi based SLAM algorithms in the recent past~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot}. Inspired from these system, in \name we utilize WiFi as a bearing measurement sensor.
In contrast to the existing works that either depend on the APs reporting their measurements~\cite{arun2022p2slam} or end-to-end optimization~\cite{arun2022p2slam,zhang2020robot}. 
In \name we only use the bearings measured at the robot's end and enable real-time graph optimization using  the factor graph optimization technique, incremental SAM implementation (iSAM)~\cite{gtsam} as further detailed in ~\cref{sec:design}.

A key thing to observe here is that these WiFi sensors provide low-compute global poses because they do not need time-taking, and memory and compute consuming global loop closure searches for landmark matching. The main reason for this is because each WiFi AP acts as a unique landmark that also has a consistent unique identifier called the hardware MAC address. This removes the need for landmark search making the global pose estimations of WiFi graph low-compute, low-power and accurate.

% To robustly solve the SLAM problem requires two parts -- the sensing front-end and the optimization back-end. Consider a simple monocular camera sensor, the sensing front end would consist of two parts -- identifying robust feature keypoints in the images, and matching them across different camera image frames based on their unique descriptions. These keypoints are generally comprised of corners or edges in an image and are matched across frames by using their unique feature descriptions. A similar ideology is applied for LiDAR's or RGBD/Stereo cameras. Once a set unique keypoints, or landmarks, have been identified and matched, they are passed on to the optimization backend. In parallel, relative changes in orientation and translations are fed back to the optimization backend by the odometry sensors and GPS.

% % next, the backend optimization does ...
% The main purpose of the backend optimization is to take these incoming measurements from the sensing front end, collate them and provide a location estimate and create a map of the environment. To collate the information from different sensors, we need to formally define the behavior of these sensors. Each of the visual or odometry sensors are governed by observation functions, which given the current state of the robot (its position, orientation, velocity, noise and other bias parameters) and the map, can predict the potential measurement coming from the respective sensor. By design if the observation function is given an accurate state of the robot and map, it would perfectly predict the measurement from a sensor. And inversely, if we poorly predict an incoming measurement, it means an incorrect estimate of the state. In fact, this inconsistency between the predicted measurement and the true measurement can serve as an error function upon which to estimate our current state. Given multiple measurements over time and across different sensors, the backend optimizer can use this error function to converge towards an accurate state for the system. 

% % NOTE: Push erroneous sensor measurements to later, maybe background and motivation ... 
% To correct the former is the job of the backend optimizer; whereas the latter is a failure on part of the sensor which would hurt our state's estimation. Unfortunately, it is not easy to discern between an erroneous state estimation or a sensor's failure and depending on the environment, different sensors better serve as an accurate predictor of our state. For instance in a well lit and static environment, the landmarks extracted from a camera front-end is stable and consistent, and serve as a strong predictor of the state of our system. Hence, it falls upon the backend optimizer to keep track of ...

==> ViWiD SLAM_arx/background/background3.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system that overcomes the current SLAM systems, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of both the Visual Inertial Odometry (VIO) SLAM systems and existing Graph SLAM approaches that utilize WiFi bearing measurements. 

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}

Firstly, to describe the operations of the existing VIO based SLAM algorithms, we take VINS-MONO~\cite{qin2018vins} as characteristic example but the similar understanding could be easily extended to any other systems like ORB-SLAM, RTABMap, or cartographer~\cite{orbslam,Labb2018RTABMapAA,cartographer}.
Wherein, a typical VIO-SLAM that uses a monocular camera in tandem with an inertial odometry measurement has three major components that contribute towards their global pose estimation and the environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since, it is very memory intensive to store all the images for each frame, the VIO-SLAM first identifies appropriate features for each frame~\cite{swift}. 
These features are then tracked across frames to assign a fixed landmark label to consistent features, thus updating the local map of features and their identifiers, which are dubbed as `landmarks'.

\noindent(2) \textbf{Local Feature Mapping:} The multiple frames that have these landmarks are tracked across, are dubbed as `keyframes'.
These landmarks tracked across the keyframes in tandem with the inertial odometry measurements provide for a joint estimate of where these landmarks are in the 3D space and also the robot poses that have enabled this mapping. 
Thus both local robot pose and the local map are simultaneously optimized using these landmarks and odometry measurements.

Both of these above measurements do not require either large memory or heavy compute. 
This is because both of these operations need to have an active memory of last few seconds of keyframes and their landmarks that are tracked and searched within. 
Thus, they are low-compute and low-latency operations.
So, the robot continues to perform local loop-closures for every few frames to generate and incrementally build the map and estimating the robot's pose.

\noindent(3) \textbf{Global Loop Closures:}  However in the long run the robot poses and the map that has been built accrues errors. 
A few of the reasons this happens due to the drift accrued in the inertial odometer measurement and camera's turn estimated incorrectly. 
This can be avoided if let us say the camera can see very old keyframe features and correct for the accumulated drift and back-propagate this error through all the existing poses and the map.
This global drift correction is what is called global loop closure. 

However, to perform these global loop closures the SLAM algorithm needs to maintain a memory consuming dictionary of the past key frames amongst which it has to continuously search for global loop-closures, which in itself is memory and compute intensive process. Additionally, a global loop-closure detected has to optimize for the entire graph which is again a time and compute consuming operation.

We can see that cameras as a sensor are very capable to provide accurate and detailed information of local robot poses and maps. 
However, they cannot perform accurate global pose estimation and map generation in memory and compute efficient fashion. 
We observe that the global loop-closure requirements arise due to accumulated drifts and errors in the inertial odometer measurements reported to the VINS-MONO optimizer.
So if there is a sensor that can give optimized global poses for the robot without any accumulated drifts or errors.
This can be used in tandem with camera, that can handle local pose estimation and mapping and avoid the global loop-closures.

\subsection{WiFi GraphSLAM}\label{sec:back-wifi}

Now that we have established a requirement of a low-cost `Oracle' system that can provide global poses to the camera local feature tracker we can achieve low-compute and adaptable SLAM for indoor robotics. To that extent, we have observed that in the recent past~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} that bearing based WiFi sensor measurements have been widely used for global pose estimation without the need for global loop-closures. 
Most of these bearing based SLAM algorithms utilize factor graph optimization techniques like GTSAM, an open-sourced GraphSLAM framework~\cite{gtsam}, to obtain the robot poses in 2D~\cite{arun2022p2slam,zhang2020robot}.
%  Inspired from these system, in \name we utilize WiFi as a bearing measurement sensor.
% In contrast to the existing works that either depend on the APs reporting their measurements~\cite{arun2022p2slam} or end-to-end optimization~\cite{arun2022p2slam,zhang2020robot}. 
% In \name we only use the bearings measured at the robot's end and enable real-time graph optimization using the factor graph optimization technique, incremental SAM implementation (iSAM)~\cite{gtsam}.

To formally define and understand how the how the GraphSLAM approach is used for WiFi based global 2D pose estimation, we first assume that we have the readings from the wheel odometry of the robot like any other SLAM system. 
Typically, it is the wheel odometry and gyroscope sensors that provide relative pose measurements of the robots across time steps. 
Now, let us say that these relative pose measurement provided is $z_i$ with a diagonal covariance matrix $\Sigma_i \in \mathbb{R}^3$. 
This covariance is usually estimated by empirically modeling the noise in the odometer and gyroscope beforehand~\cite{lesson1966simple} which are reported by the manufacturer.
We can then define a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \;|\; \Vec{p}_i = (p^x_i, p^y_i, p^\theta_i) \in SE(2), \; \forall i \in [1, N]\}$, where each $p_i$ belongs to the Special Euclidean group ($SE(2)$). 
Next we need to define the measurement model for the odometer factors or the in-between factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$. The measurement model can be shown to be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(-p^\theta_i) [p^x_{i+1} - p^x_{i},\; p^y_{i+1} - p^y_{i}]^T\\
                    (p^\theta_{i+1} - p^\theta_i)
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(2)$ is the rotation matrix. This prediction function now allows us to constrain two consecutive robot poses via a between factor within GraphSLAM \cite{gtsam} and defines an error function between the measurement and prediction as $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$. 
Similarly, one can define the factor graph for the bearing measurements $\hat{z}^{AP}_{ij}(p_i, x_j)$ as well:
\begin{align}\label{eq:ping-pred}
    \hat{z}^{AP}_{ij}(p_i, x_j) = R(-p_i^\theta)\mathrm{atan}2(x^x_i - p^x_i, x^y_i - p^y_i)
\end{align}
where, $\{p_i \; \forall i \in [1, N]\}\ \bigcup\ \{x_j \; \forall j \in [1, N_{ap}]\}$, for $N$ number of robot poses and $N_{ap}$ WiFi AP poses as we do not want to usually assume the pose of the APs in the environment. 
$\mathrm{atan}2(\cdot)$ is the ``2-argument'' inverse tangent function. 
The rotation $R(-p_i^\theta)$ brings the bearing of the access point into the local coordinate frame of the robot. 
This bearing measurement is made on the robot's WiFi sensor from the WiFi access points in the environment.
While, the authors in $\mathrm{P^2}$SLAM assume the WiFi access points coordination in reporting the bearing measured at the access point from the robot we neglect those measurements as this coordination is not practical.

With the factor graph thus constructed, we can then define optimization function to find a set of values $S_{opt}$ such that the total error between our predictions and actual measurements is minimized
\todo{update the $S_{opt}$ equation}
\begin{align}\label{eq:graph-optim-head}
    & S_{opt} =  \argmin_{S} \sum_{i=1}^N \sum_{j=1}^{N_{ap}}  \rho\left(\frac{\big(e^{bearing}_{ij}\big)^2}{\sigma^{bearing}};c\right) \\
         & + \sum_{i=1}^N  \big(e^{odom}_i\big)^T \Sigma_i^{-1} e^{odom}_i.\nonumber 
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$. Thus providing for optimized global robot poses $\{p_i \; \forall i \in [1, N]\}$ without needing any memory and compute demanding global loop-closures. These global robot poses can now be sent over to the 

A key thing to observe here is that these WiFi sensors based factor graph optimization provide low-compute global poses because they do not need time-taking, and memory and compute consuming global loop closure searches for landmark matching. 
The main reason for this is because each WiFi AP acts as a unique landmark that also has a consistent unique identifier called the hardware MAC address. 
This removes the need for landmark search making the global pose estimations of WiFi graph low-compute, low-power and accurate, unlike the VIO-SLAM systems.
On the flip-side, while these WiFi graph SLAM frameworks provide optimized global pose estimations, there is not context of what the environment is and how the robot can navigate through this environment.
We can thus see that both these systems have their respective shortcomings, but have their own strengths.
That is we can use the optimized global pose estimates can be used as `Oracle' Odometer measurements for the camera graph which can provide the map of the environment, adding context to the environment the robot is exploring.
This is where we provide \name, which utilizes these advantages and creates a `Dual-graph' layered solution to provide a deployable and scalable SLAM system.





% Similarly, to incorporate for the WiFi bearing measurements into the factor graph, we first note that in \name we do not assume the initial position of the WiFi APs, and thus need to optimize for their poses as well as the robot's poses. To thus incorporate that, we append the poses of $Q$ WiFi APs ($x$) to our state space. The complete state space would then become $\{p_i \; \forall i \in [1, P]\}\ \bigcup\ \{x_j \; \forall j \in [1, Q]\}$.
% We thus define our prediction function to obtain the angle subtended by access point $x_j$ at robot pose $p_i$ as
% \begin{align}\label{eq:ping-pred}
%     \hat{z}^{AP}_{ij}(p_i, x_j) = R(-p_i^\theta)\mathrm{atan}2(x^x_i - p^x_i, x^y_i - p^y_i)
% \end{align}
% where $\mathrm{atan}2(\cdot)$ is the ``2-argument'' inverse tangent function. The rotation $R(-p_i^\theta)$ brings the bearing of the access point into the local coordinate frame of the robot. This bearing measurement is made when the WiFi radio receives the `pong' acknowledgement from the WiFi access points. 
% Finally, to anchor the robot to a fixed global frame of reference and align it with the ground truth trajectory and map generated by Cartographer~\cite{cartographer}, we further provide an initial prior, $p_0$, to the first pose. 

% With the factor graph constructed, we can then define optimization function to find a set of values $S_{opt}$ such that the total error between our predictions and actual measurements is minimized
% \todo{update the $S_{opt}$ equation}
% \begin{align}\label{eq:graph-optim-head}
%     & S_{opt} =  \argmin_{S} \sum_{i=1}^P \sum_{j=1}^Q  \rho\left(\frac{\big(e^{bearing}_{ij}\big)^2}{\sigma^{bearing}};c\right) \\
%          & + \sum_{i=1}^P  \big(e^{odom}_i\big)^T \Sigma_i^{-1} e^{odom}_i.\nonumber 
% \end{align}
% where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$. To further strengthen the optimization to outliers, we use a Huber cost function, $\rho(\cdot, c)$~\cite{zhang1997parameter}, for which
% we find through our experiments the threshold $c = 1.345$ provides the best estimate. This function is easily minimized in linear time proportional to the number of nodes initialized, i.e. $N+M$, via Levenberg-Marquadt \cite{gtsam}.

==> ViWiD SLAM_arx/background/background4.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of existing visual-inertial odometry (VIO) SLAM systems, and graph SLAM approaches that utilize WiFi bearing measurements. 

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}
Let us first understand the operations of existing Visual Inertial Odometry (VIO) based SLAM algorithms like ORB-SLAM, RTABMap, or Kimera~\cite{orbslam,Labb2018RTABMapAA,rosinol2021kimera}.
A typical VIO-SLAM system that uses a monocular camera in tandem with an inertial odometry measurement unit has three major components that contribute towards global pose estimation and environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since it is very memory intensive to store the entire camera image for each frame, the VIO-SLAM system first identifies appropriate features for each frame~\cite{shi1994good}. 
These features are then tracked across frames by assigning a fixed identity label to consistent features, and updating a local map of features and their identifiers, which are dubbed as `landmarks'. Additionally, camera frames which have a large number of new landmarks are stored in memory and are dubbed `keyframes'. These keyframes will be later used for global drift corrections to the robot's trajectory.  

\noindent(2) \textbf{Local Feature Mapping:} Out of the landmarks tracked, some are judged stable and consistent, and are integrated into the map. 
These landmarks are localized in 3D space by jointly optimizing over the distinct robot positions at which the landmarks were observed. 
Thus, both local robot pose and the local map can be simultaneously optimized using these landmarks and odometry measurements.

It is important to note that both feature tracking and local mapping operations are low in memory and compute because these operations need to have an active memory of only the last few seconds of camera frames, observed landmarks and odometry measurements. 
So, the robot continues to perform local drift corrections for every few frames to incrementally build the map and estimate the robot's pose.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/WiViD_overview.pdf}
    \caption{\name's layered approach: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time.}
    \label{fig:layered-arch}
\end{figure*}

\noindent(3) \textbf{Global Loop Closures:}  However, in the long run the robot poses and the map that has been built accrue errors as drifts in inertial odometry measurements cannot be accurately cancelled via local corrections only.
These long-term drifts can are corrected by employing global loop closures. Specifically, if the robot revisits a space and the camera can find previously seen keyframe features, it can constrain the current robot's pose to the previously estimated pose at this keyframe and re-optimize the robot's trajectory considering this additional constraint. These large drift corrections, which affect a large number of nodes in the robot's pose, are called global loop closures. 

In order to perform these global loop closures, the SLAM algorithm needs to maintain a dictionary of all the past key frames, amongst which it has to continuously search for global loop closures. This buffer of keyframes and continuous search is a very memory and compute intensive process.  Additionally, a global loop closure detection triggers a re-optimization of the entire robot trajectory which is again a time and compute intensive operation. Furthermore, the required memory and search-time scales linearly with the size of the environment, reducing the scalability of the system as well.

In short, cameras as a sensor are capable of providing accurate and detailed information of local robot poses and maps. 
However, they cannot perform accurate global pose estimation and map generation in a memory and compute efficient fashion. 
We observe that requirements for global loop closures arise due to accumulated drifts and errors in the inertial odometry measurements reported to the optimizer.
Hence, there is a requirement for a sensor to provide these global `Oracle' poses for the robot, free of accumulated drifts and errors in a compute and memory-light fashion, so that the camera can coherently map and understand the environment.  
% So if a sensor that can give optimized global poses for the robot without any accumulated drifts or errors.
% This can be used in tandem with camera, that can handle local pose estimation and mapping and avoid the global loop closures.

\subsection{\name's design Motivation}\label{sec:back-wifi}

Now that we have established a requirement of a low-cost `Oracle' system that can provide global poses to the local feature tracker, we have a path to low-compute and adaptable SLAM for indoor robotics. 

We have observed that in the recent past~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot}, bearing based WiFi sensor measurements have been widely used for global pose estimation without the need for global loop closures. 
Most of these bearing based SLAM algorithms utilize factor graph optimization techniques like GTSAM, an open-sourced GraphSLAM framework~\cite{gtsam}, to obtain the robot and AP poses~\cite{arun2022p2slam,zhang2020robot}.

A key observation is these WiFi-sensor based GraphSLAM approaches provide low-compute global pose estimates, as they do not rely on memory and compute consuming global loop closure searches for landmark matching. 
While in camera SLAM, an increasing number of `landmarks' are needed to be kept in active memory to identify and perform loop closures, WiFi has fixed a number of `landmarks' in the form of WiFi Access Points deployed in the environment.
Furthermore, while camera-landmarks are unique features in a frame, they are vulnerable to ambiguities, resulting in false-positive loop closures in homogeneous spaces.
On the other hand, in WiFi SLAM each WiFi AP acts as a unique landmark that also has a consistent discernible identifier (hardware MAC address) removing any room for instability in the system. 
These consistently identifiable landmarks allow for global pose corrections sans global loop closures providing low-compute, low-power and accurate `Oracle' pose updates.
On the flip-side, while these WiFi graph SLAM frameworks provide optimized global pose estimations, they lack context of the environment, essential for autonomous robot navigation in any environment.

Thus both sensors have their advantages and disadvantages, and we present \name that amalgamates both the sensors to bring out the best of both camera and WiFi sensor capabilities. 
\if 0
We first present \name's dual-graph design  as shown in Figure~\ref{fig:layered-arch} in ~\cref{sec:design}, that demonstrates the scalability of \name's design. We then describe the challenges in estimating accurate measurements for camera and WiFi sensors in ~\cref{sec:design-measure}. We go on to detail implementation and deployment of \name in ~\cref{sec:implementation} and demonstrate \name's performance and a detailed analysis in ~\cref{sec:eval}. 
% Additionally, we showcase simple application where the robot autonomously navigates to a given room number to deliver a package in ~\cref{sec:showcase}.
Finally in ~\cref{sec:conclusion}, we present the limitations that hinder our current implementation of \name and future directions that our research in \name opens.
\fi

==> ViWiD SLAM_arx/background/background5.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of existing visual-inertial odometry (VIO) SLAM systems, and graph SLAM approaches that utilize WiFi bearing measurements. 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/viwid_overview-crop.pdf}
    \caption{\name's Dual layered Design: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time. \todo{Fix numbers}}
    \label{fig:layered-arch}
\end{figure*}

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}
Let us first understand the operations of existing Visual Inertial Odometry (VIO) based SLAM algorithms like ORB-SLAM, RTABMap, or Kimera~\cite{mur2015orb,Labb2018RTABMapAA,rosinol2021kimera}.
A typical VIO-SLAM system that uses a monocular camera in tandem with an inertial odometry measurement unit has three major components that contribute towards global pose estimation and environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since it is very memory intensive to store the entire camera image for each frame, the VIO-SLAM system first identifies appropriate features for each frame~\cite{shi1994good}. 
These features are then tracked across frames by assigning a fixed identity label to consistent features, and updating a local map of features and their identifiers, which are dubbed as `landmarks'. Additionally, camera frames that have a large number of new landmarks are stored in memory and are dubbed `keyframes'. These keyframes will be later used for global drift corrections to the robot's trajectory.  

\noindent(2) \textbf{Local Feature Mapping:} Out of the landmarks tracked, some are judged stable and consistent, and are integrated into the map. 
These landmarks are localized in 3D space by jointly optimizing over the distinct robot positions at which the landmarks were observed. 
Thus, both the local robot pose and the local map can be simultaneously optimized using these landmarks and odometry measurements.

\noindent(3) \textbf{Global Loop Closures:}  However, in the long run, the robot poses and the map built accrue errors as drifts in inertial odometry measurements cannot be accurately canceled via local corrections alone.
These long-term drifts can are corrected by employing global loop closures. Specifically, if the robot revisits a space and the camera can find previously seen keyframe features, it can constrain the current robot's pose to the previously estimated pose at this keyframe and re-optimize the robot's trajectory considering this additional constraint. These large drift corrections, which affect a large number of robot poses, are called global loop closures. 

To perform these global loop closures, the SLAM algorithm needs to maintain a dictionary of all the past keyframes, amongst which it has to continuously search for global loop closures. This buffer of keyframes and continuous search is very memory and compute-intensive process~\cite{semenova2022quantitative}.  Additionally, a global loop closure detection triggers a re-optimization of the entire robot trajectory which is again a time and compute-intensive operation. Furthermore, the required memory and search times scale linearly with the size of the environment, reducing the scalability of the system.

\subsection{\name's design Motivation}\label{sec:back-wifi}

In short, cameras as a sensor are capable of providing accurate and detailed information of local robot poses and maps with low compute and memory resources. 
However, they cannot perform accurate global pose estimation and map generation in memory and compute efficient fashion. 
We observe that requirements for global loop closures arise due to accumulated drifts and errors in the inertial odometry measurements reported to the optimizer.
Hence, if the camera has access to global poses of the robot, free of accumulated drifts and errors in a compute and memory-light fashion, the camera SLAM can coherently map and understand the environment.
Now, this approach of abstraction of tasks similar to network layer abstraction~\cite{session1994it5} has pioneered the research and development of current data networks. This motivates the Dual-layer design of \name.

Inspired by this intuition, we observe recent SLAM development into WiFi sensor-based global pose estimation without the need for global loop closures~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot}.
So these WiFi-sensor-based SLAM approaches provide low-compute global pose estimates, as they do not rely on memory and compute consuming global loop closure searches for landmark matching. 
Thus, we use the WiFi-sensor-based SLAM systems as our drift-free pose estimation system that can provide poses of the robot to the camera SLAM can coherently map and understand the environment.
This leads to the Visual-WiFi Dual-layered SLAM design of \name that is described in ~\cref{sec:design}.

==> ViWiD SLAM_arx/background/background6.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of existing visual-inertial odometry (VIO) SLAM systems, and graph SLAM approaches that utilize WiFi bearing measurements. 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/viwid_overview-crop.pdf}
    \caption{\name's Dual layered Design: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time. \todo{Fix numbers}}
    \label{fig:layered-arch}
\end{figure*}

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}
Let us first understand the operations of existing Visual Inertial Odometry (VIO) based SLAM algorithms like ORB-SLAM, RTABMap, or Kimera~\cite{mur2015orb,Labb2018RTABMapAA,rosinol2021kimera}.
A typical VIO-SLAM system that uses a monocular camera in tandem with an inertial odometry measurement unit has three major components that contribute towards global pose estimation and environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since it is very memory intensive to store the entire camera image for each frame, the VIO-SLAM system first identifies appropriate features for each frame~\cite{shi1994good}. 
These features are then tracked across frames by assigning a fixed identity label to consistent features, and updating a local map of features and their identifiers, which are dubbed as `landmarks'. Additionally, camera frames that have a large number of new landmarks are stored in memory and are dubbed `keyframes'. These keyframes will be later used for global drift corrections to the robot's trajectory.  

\noindent(2) \textbf{Local Feature Mapping:} Out of the landmarks tracked, some are judged stable and consistent, and are integrated into the map. 
These landmarks are localized in 3D space by jointly optimizing over the distinct robot positions at which the landmarks were observed. 
Thus, both the local robot pose and the local map can be simultaneously optimized using these landmarks and odometry measurements.

\noindent(3) \textbf{Global Loop Closures:}  However, in the long run, the robot poses and the map built accrue errors as drifts in inertial odometry measurements cannot be accurately canceled via local corrections alone.
These long-term drifts are corrected by employing global loop closures. Specifically, if the robot revisits a space and the camera can find previously seen keyframe features, it can constrain the current robot's pose to the previously estimated pose at this keyframe and re-optimize the robot's trajectory considering this additional constraint. These large drift corrections, which affect a large number of robot poses, are called global loop closures. 

To perform these global loop closures, the SLAM algorithm needs to maintain a dictionary of all the past keyframes, amongst which it has to continuously search for global loop closures. This buffer of keyframes and continuous search is very memory and compute-intensive process~\cite{semenova2022quantitative}.  Additionally, a global loop closure detection triggers a re-optimization of the entire robot trajectory which is again a time and compute-intensive operation. Furthermore, the required memory and search times scale linearly with the size of the environment, reducing the scalability of the system.

\subsection{\name's Design Motivation}\label{sec:back-wifi}

In short, cameras as a sensor are capable of providing accurate and detailed information of local robot poses and maps with low compute and memory resources. 
However, they cannot perform accurate global pose estimation and map generation in memory and compute efficient fashion. 
We observe that requirements for global loop closures arise due to accumulated drifts and errors in the inertial odometry measurements reported to the optimizer.
Hence, if the camera has access to global poses of the robot, free of accumulated drifts and errors in a compute and memory-light fashion, the camera SLAM can coherently map and understand the environment.
Now, this approach of abstraction of tasks similar to network layer abstraction~\cite{session1994it5} has pioneered the research and development of current data networks. This motivates the Dual-layer design of \name.

Inspired by this intuition, we observe recent SLAM development into WiFi sensor-based global pose estimation without the need for global loop closures~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot}.
So these WiFi-sensor-based SLAM approaches provide low-compute global pose estimates, as they do not rely on memory and compute consuming global loop closure searches for landmark matching. 
Thus, we use the WiFi-sensor-based SLAM systems as our drift-free pose estimation system that can provide poses of the robot to the camera SLAM can coherently map and understand the environment.
This leads to the Visual-WiFi Dual-layered SLAM design of \name that is described in ~\cref{sec:design}.

==> ViWiD SLAM_arx/design/design1.tex <==
% !TEX root = root.tex
\section{Design}\label{sec:design}

Assuming we have robust and accurate bearing measurements, we first detail \name's Dual-graph solution for a scalable SLAM system using the WiFi and camera sensors, describing each individual layer first and how they are connected with each other.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

To this extent, we make few interesting observations. (i) all robots are equipped with a WiFi transceiver (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is a relatively cheap sensor modality, and (iv) there has been a couple of decades of research in WiFi based localization and tracking. Owing to these reasons we utilize WiFi as the low-cost `Oracle' sensor that can report global robot poses to the camera graph optimizer.

To formally define and understand how the how the GraphSLAM approach is used for WiFi based global 2D pose estimation, we first assume that we have the readings from the wheel odometry of the robot like any other SLAM system. 
Typically, it is the wheel odometry and gyroscope sensors that provide relative pose measurements of the robots across time steps. 
Now, let us say that these relative pose measurement provided is $z_i$ with a diagonal covariance matrix $\Sigma_i \in \mathbb{R}^3$. 
This covariance is usually estimated by empirically modeling the noise in the odometer and gyroscope beforehand~\cite{lesson1966simple} which are reported by the manufacturer.
We can then define a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \;|\; \Vec{p}_i = (p^x_i, p^y_i, p^\theta_i) \in SE(2), \; \forall i \in [1, N]\}$, where each $p_i$ belongs to the Special Euclidean group ($SE(2)$). 
Next we need to define the measurement model for the odometer factors or the in-between factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$. The measurement model can be shown to be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(-p^\theta_i) [p^x_{i+1} - p^x_{i},\; p^y_{i+1} - p^y_{i}]^T\\
                    (p^\theta_{i+1} - p^\theta_i)
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(2)$ is the rotation matrix. This prediction function now allows us to constrain two consecutive robot poses via a between factor within GraphSLAM \cite{gtsam} and defines an error function between the measurement and prediction as $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$. 
Similarly, one can define the factor graph for the bearing measurements $\hat{z}^{AP}_{ij}(p_i, x_j)$ as well:
\begin{align}\label{eq:ping-pred}
    \hat{z}^{AP}_{ij}(p_i, x_j) = R(-p_i^\theta)\mathrm{atan}2(x^x_i - p^x_i, x^y_i - p^y_i)
\end{align}
where, $\{p_i \; \forall i \in [1, N]\}\ \bigcup\ \{x_j \; \forall j \in [1, N_{ap}]\}$, for $N$ number of robot poses and $N_{ap}$ WiFi AP poses as we do not want to usually assume the pose of the APs in the environment. 
$\mathrm{atan}2(\cdot)$ is the ``2-argument'' inverse tangent function. 
The rotation $R(-p_i^\theta)$ brings the bearing of the access point into the local coordinate frame of the robot. 
This bearing measurement is made on the robot's WiFi sensor from the WiFi access points in the environment.
While, the authors in $\mathrm{P^2}$SLAM assume the WiFi access points coordination in reporting the bearing measured at the access point from the robot we neglect those measurements as this coordination is not practical.

With the factor graph thus constructed, we can then define optimization function to find a set of values $S_{opt}$ such that the total error between our predictions and actual measurements is minimized
\todo{update the $S_{opt}$ equation}
\begin{align}\label{eq:graph-optim-head}
    & S_{opt} =  \argmin_{S} \sum_{i=1}^N \sum_{j=1}^{N_{ap}}  \rho\left(\frac{\big(e^{bearing}_{ij}\big)^2}{\sigma^{bearing}};c\right) \\
         & + \sum_{i=1}^N  \big(e^{odom}_i\big)^T \Sigma_i^{-1} e^{odom}_i.\nonumber 
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$. Thus providing for optimized global robot poses $\{p_i \; \forall i \in [1, N]\}$ without needing any memory and compute demanding global loop-closures.



Highlight that we use only measurements at the robot, making it in dependant of the environment and can be deployed even in the cases of distaster relief where the WiFi AP Locations are not known apriori.

The rest would be a description of p2slam's graphslam framework and optimization with intuitions.

then talk about how iSAM works and is different from end-to-end slam, and how it is more difficult and much more important for real-world deployments.

A key thing to observe here is that these WiFi sensors provide low-compute global poses because they do not need time-taking, and memory and compute consuming global loop closure searches for landmark matching. The main reason for this is because each WiFi AP acts as a unique landmark that also has a consistent unique identifier called the hardware MAC address. This removes the need for landmark search making the global pose estimations of WiFi graph low-compute, low-power and accurate.

\subsection{Camera Factor Graph}\label{sec:design-graph2}

The camera graph now utilizes the global optimized pose estimates outputted from the WiFi factor graph in real-time and uses them as the odometer factors for its graph optimization.

What are the exact outputs from the WiFi factor graph to the camera factor graph. Is it just locations? If so, how delayed are they and what happens when they are updated?

We make smart choices as to when to update them and how frequently to avoid the camera graph from breaking.

It then performs local mapping and pose corrections, providing with global optimized pose and map for the frames of data collected so far without the requirement of compute heavy graphslam.

\subsection{Accurate Bearing Measurements}\label{sec:design-bearing}

While existing works use end-to-end optimization, we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for real-time local updates. This demands that the bearing measurements made are accurate, more dense and do not have any ambiguities.

Thus to solve these problems in \name we make few innovations on the bearing estimation end.

Firstly to remove the ambiguities of the half-plane in the typically deployed ULAs in the literature, we use square antenna array with $3\lambda/8$ side length of the square, which has unique solution for theta in the full-space.

Next to increase the accuracy and density of bearing measurements to the WiFi access points in the environment while maintaining real time estimates we get inspired from the Spoti/MUSIC though are high compute and latency. 
We cannot simple averaging across FFT profiles, as each measurement has unique random phase offset that changes across time due to timing mismatches between the transmitting AP and the receiving WiFi sensor on the robot
In contrast, in \name the averaging is done by performing eigen or singular decomposition over a collated measurements both across time and if there multiple antennas on the transmitting AP, then across these antennas as well.

We then identify the component with strongest singular value, which corresponds to the direct path in most of the cases and perform a simple 2D FFT on it as mentioned/detailed in ~\cite{ayyalasomayajula2018bloc}. And from this we pick the global maxima to obtain cleaned, more accurate and denser bearing measurements if and when we perform a moving window averaging on these WiFi measurements.

Thus, \name solves for getting accurate and dense bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

Thus we have seen how the layered approach in bifurcating the tasks between the WiFi and camera sensors to utilize them for what they are best at brings the best of both the sensors. This WiFi and Visual Dual factor graph SLAM solution thus makes \name-SLAM, low-cost, low-compute, accurate and adaptable SLAM system. Thus enabling scalable and deployable robotics using \name-SLAM's design.

==> ViWiD SLAM_arx/design/design2.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

% \begin{figure*}[ht]
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/placeholder.pdf}
%         \subcaption{}
%     \end{minipage}
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/placeholder.pdf}
%         \subcaption{}
%     \end{minipage}
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/placeholder.pdf}
%         \subcaption{}
%     \end{minipage}
%     \caption{\name's design: (a) Shows the layered design where the inputs to and outputs from each layer are detailed. (b) Shows the details of the implementation of the WiFi graph (c) Details on how the camera graph uses the WiFi Odometry measurements for Mapping.}
%     \label{fig:design-overview}
% \end{figure*}

The existing VIO SLAM and WiFi SLAM systems have their respective shortcomings and strengths as described in ~\cref{sec:background}.
To overcome the limitations of these existing systems, and make use of the best use of these two individual sensors, we propose \name a `Dual-graph' layered solution to provide a deployable and scalable SLAM system.
We detail \name's `Dual-graph' design in this section where we first assume that we have accurate real-time bearings available for robots poses and define the WiFi graph optimization in ~\cref{sec:design-graph1} that provides optimized robot poses. 
These WiFi-optimized robot poses are then smartly fed to the camera graph which is described in ~\cref{sec:design-graph2}, to jointly optimize for the robot positions and the various visual landmarks observed in the environment.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

Firstly, to identify the sensor modality to use within the first graph that provides for the optimized global pose estimates to the second graph, we make few interesting observations:
(i) all robots are equipped with a WiFi transceiver (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is an inexpensive sensing modality, and (iv) WiFi based localization and tracking~\cite{ma2019wifi} is well studied which can be exploited for the global pose estimation. Owing to these four reasons, we utilize WiFi as the low-cost `Oracle' sensor that can be used to build the first SLAM module to provide global robot poses to the second Camera-based graph optimizer.

\noindent\textbf{Bearings as Robust WiFi Measurements:} To enable this `dual-graph' idea, the WiFi SLAM module should take the WiFi measurements at multiple robot poses from access points deployed in the environment as shown in Figure~\ref{fig:wifi-factor}a and optimize for global pose estimates.
To demonstrate that in \name, these WiFi measurements are integrated with the widely deployed GraphSLAM~\cite{gtsam} approach.
This GraphSLAM approach lays down these WiFi measurements, $z_{ij}^\mathrm{bot}$, as factors in a factor graph, connecting the access points' pose estimates, $ \Vec{x}_j$ to the robot pose, $ \Vec{p}_i$, across frames. 
These robot pose estimates are further connected with the wheel-encoder and gyroscope measurements which provide relative odometry measurements, $z_i^\mathrm{odom}$ between two consecutive pose estimates.
Once we lay down these WiFi measurements and relative odometry measurements as shown in Figure~\ref{fig:wifi-factor}b, it can be optimized to estimate accurate global poses.

With the high-level factor graph laid out, we have to choose the appropriate WiFi-based measurements which provide the necessary global pose corrections.
Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} have shown that bearing measurements are one of the most robust estimates that can be used for Indoor localization and tracking.
Inspired from these works we utilize bearings as the WiFi measurements to be integrated into our WiFi factor graph's definition.
These bearing measurements can be estimated either at the robot's WiFi device or at the WiFi access points in the environment using the channel state information (CSI) measured while receiving WiFi signal~\cite{arun2022p2slam,spotfi,arraytrack}.

Unfortunately, these implementations either assume the apriori pose of the WiFi access points in the environment~\cite{spotfi} or assume the CSI measurements at the WiFi APs are reported back to the robot~\cite{arun2022p2slam}. These assumptions reduce the deployability of the WiFi-SLAM system, requiring fine-grained measurements of AP's locations or cooperation from infrastructure. 
In  \name's WiFi factor graph, we break away from these assumptions, and do not require any knowledge of the environment including the AP poses or collaboration between the AP's and the robot.
Thus in \name, we utilize the bearing estimates, $z_{ij}^{bot}$ made only at the robot's end with respect to the AP's in the environment as can also be seen in the factor graph shown in Figure~\ref{fig:wifi-factor}.
The final requirement for real-time wide-deployability is to provide timely global pose updates to the Camera-graph and ensure accurate mapping of the environment.
These timely global pose estimates demands that the bearing measurements be real-time and accurate, which poses its unique challenges that we solve as discussed later in ~\cref{sec:design-bearing}. For the sake of brevity we first assume that we have these accurate real-time bearing measurements and describe \name's WiFi factor graph implementation.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across various robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}

\noindent\textbf{Building and Optimizing the WiFi-Graph:}
To formally define and understand how the GraphSLAM approach is used for WiFi based global 4DoF pose estimation, we first assume that we have the readings from the wheel odometry and gyroscope measurements from the robot like any other SLAM system. 
Typically, these sensors provide relative pose measurements of the robots across time steps. 
Now, let us say that these relative pose measurement provided is $z_i$ with a diagonal covariance matrix $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$. 
This covariance is usually estimated by empirically modeling the noise in the odometer and gyroscope beforehand~\cite{lesson1966simple} which are reported by the manufacturer.
We can then define a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \;|\; \Vec{p}_i = (p^x_i, p^y_i, p^z_i, q^x_i, q^y_i, q^z_i) \in SE(3), \; \forall i \in [1, N]\}$, where each $p_i$ belongs to the Special Euclidean group ($SE(3)$). Specifically, each $\Vec{p}_i$ has two components, the translation in space, $p^t_i = (p^x_i, p^y_i, p^z_i)$, and the quaternion representing its rotation, $p^q_i(q^x_i, q^y_i, q^z_i, 1 - ||(q^x_i, q^y_i, q^z_i)||^2)$.
Next we need to define the measurement model for the odometer factors or the in-between factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$. The measurement model can be shown to be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion~\cite{diebel2006representing}. This prediction function now allows us to constrain two consecutive robot poses via a between factor within GraphSLAM \cite{gtsam} and defines an error function between the measurement and prediction as $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$. 
Similarly, one can define the factor graph for the bearing measurements of AP $j$ at robot position $x_i$ as $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$:
\begin{align}\label{eq:ping-pred}
    &\hat{z}^{bot}_{ij}(p_i, x_j) = \mathrm{Local}(\mathrm{TransformTo}(x_j, p_i), p_i) \\
                                &= \mathrm{Local}([\cos(\phi)\cos(\theta), \cos(\phi)\sin(\theta), \sin(\phi)]^T, p_i) \nonumber
\end{align}
where, $\{p_i \; \forall i \in [1, N]\}\ \bigcup\ \{x_j \; \forall j \in [1, N_{ap}]\}$, for $N$ number of robot poses and $N_{ap}$ WiFi AP poses. Furthermore, \textit{TransformTo}$(\cdot)$ transforms the coordinates of the AP $x_j$ to the coordinate system provided by the robot at $p_i$, in which the AP subtends an elevation angle of $\phi$ and an azimuth angle of $\theta$. \textit{Local}$(\cdot)$ projects this bearing measurement to the tangent plane defined by the current pose of the robot, $p_i$. 

At this point, we are faced with an interesting choice. As mentioned previously, the angle of arrival of signal from an access point is the measurement of choice. We can consider extracting both the elevation and azimuth angle given a 2D antenna array as opposed to just the azimuth angle. Unfortunately this comes with two challenges, (1) it doubles the state-space of the optimization, (2) most WiFi clients have four or fewer antennas~\cite{quantenna}, resulting in poor resolution and incorrect estimation of elevation angles. Hence, we set $\phi = 0$, regardless of the height of the access point, and only extract the azimuth angle, $\theta$. \todo{bringing out elevation sucks, only azimuth, confirm here}. Finally, we also define the covariance of these bearing measurements, $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$. 

With the factor graph thus constructed, we can define optimization function to find a set of values $S_{opt}$ such that the total error between our predictions, $\hat{z}$'s, and actual measurements, $z$'s, is minimized. 
Unlike the existing WiFi SLAM architectures~\cite{arun2022p2slam,ferris2007wifi} we do not perform end-to-end optimization, we instead use the incremental smoothing and mapping (iSAM) implementation of the GraphSLAM approach~\cite{gtsam}.
At a high level, GTSAM framework optimizes for all the variables, $\{p_i \; \forall i \in [1, N]\}\ \bigcup\ \{x_j \; \forall j \in [1, N_{ap}]\}$, end-to-end considering all the measurements, $\{z_i^{odom},\hat{z}^{AP}_{ij}(p_i, x_j)\} \forall i \in [1, N]$ and $\forall j \in [1, N_{ap}]\}$ together and optimizing for them as a post processing step.
On the other hand, in iSAM, the graph is optimized every time a new measurement is added to the factor graph. 
This might lead to incredibly high compute and memory requirements as the factor graph gets bigger with each new measurement coming in.
In order to avoid this, in iSAM~\cite{gtsam}, the authors determine which of the past poses are effected by the new incoming measurement and only those subset of pose estimates are optimized.
Specifically, given $I={p_i,x_j: i<n, \forall j \in [1, N_{ap}]}$, where $n$ is the current time instance when a new measurement is added to the factor graph, only a subset of the factors $I_{sub} \subseteq I$ are optimized.
We can estimate the optimized robot poses $S_{opt}^n$ for time instance $n$ by minimizing the total error between our predictions and actual measurements for the subset $I_{sub}$, i.e.
\begin{align}\label{eq:graph-optim-head}
    S_{opt}^n = \argmin_{S} \sum_{i\in I_{sub}} \sum_{j\in I_{sub}}  & \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. Thus providing for optimized global robot poses $\{p_i \; \forall i \in I_{sub}\}$ without needing any memory and compute demanding global loop closures.

\noindent\textbf{Initialization of Factors:} Finally, we also need to initialize each of the $N$ robot positions and $N_{ap}$ AP positions for the optimizer. 
Like any other SLAM system, we initialize the robot positions using the relative odometry measurements. But it is important to note that these priors will be affected by drift accumulated by the odometer. 
We also do not assume apriori location of the AP's in the environment, but unlike for the end-to-end optimization scenario, real-time incremental optimizations we cannot initialize all the AP poses at the origin at the beginning of the optimization.
This is because many of these APs have not yet been discovered or are not effected by the current incoming bearing measurements, thus making the optimization problem ill-defined. Furthermore, AP's which have been discovered may not have enough bearing measurements to strongly constrain the system. This makes the optimization unstable and converge to poor estimates. Thus, we need to initialize the APs in a smart fashion considering the most probable bearing measurement factors when getting added that effect the AP and robot poses.

To solve for the indeterminate solution due to incorrect WiFi AP initialization, we draw from the intuition of WiFi signal propagation characteristics.
More specifically WiFi received signal signal strength (RSSI) statistics, which have been studied in the past for localization.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's translation $p^t_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maxima among all the robots poses $p_i \forall i \in [1,n]$ measured at $n^{th}$ time instance.
We can then initialize $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation.
Once all the APs in the environment are detected and initialized in this fashion the factor graph optimization system is no more indeterminate or ill-defined.
Thus solving all the challenges for the \name's WiFi graph optimization, which can now provide accurate and real-time global pose estimates for the camera graph to consume.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/camera_factor.pdf}
    \caption{Shows the details of the implementation of the Camera Factor graph}
    \label{fig:cam-factor}
\end{figure}

\subsection{Camera Factor Graph}\label{sec:design-graph2}

As we described in ~\cref{sec:back-vio}, a typical Visual Inertial Odometer based SLAM system needs camera features and Odometer measurements. 
To extract, track and map the camera features we utilize the Shi-Tomasi features~\cite{shi1994good} from the VINS-MONO implementation~\cite{qin2018vins}.
These camera features are undistorted and then mapped onto a unit sphere to get an approximate estimate of the 3D point cloud projections.
These projections are then laid down as the map projections or `landmarks' in the factor graph for a fixed set of local frames. 
These `landmarks' now in tandem with the Odometer measurements could jointly optimize to perform local pose corrections. 
These local corrections ensure accurate 3D mapping of the `landmark' point clouds in the environment as shown in Figure~\ref{fig:cam-factor}

% We detail on how we extract robust camera measurements in ~\cref{sec:design-camera}, where we go into further details on how we use the feature extraction provided by the VINS-MONO feature extractor and tracker~\cite{qin2018vins}.
In addition to this, these VIO-SLAM systems trigger global loop closures for two distinct reasons (i) because of the drift accrued in the robot pose estimates provided by the Inertial Odometry sensors for long runs, and (ii) the homogeneity of the visual features based landmarks that demands constant trigger for feature matching and thus large memory cache of all the landmarks.
In \name, we overcome both of these issues using the global pose estimates provided by the WiFi graph as the `Oracle' robot pose measurements for the camera graph.
Since, these WiFi global pose estimates can be made with low-compute and in real-time with high-accuracy we can eliminate the need for global loop closure in the camera features based VIO-SLAM systems.

\begin{algorithm}[t]
\caption{Implementation of the buffered WiFi Pose updates to the Camera Odometry factors.\todo{The algo is not correct, correct it!!!!!!!}}
\label{algo:pose-buffer}
    \SetAlgoLined
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    % \SetKwData{Circular}{circularCache_w}
    \Input{Pose threshold $t$, stability threshold size $st$, moving window size $w$}
    initialization Circular Cache $C_0 \leftarrow \{\}$, Buffer $V \leftarrow \{\} $, Pose Updates $S_{opt}^0\leftarrow \{\} $, Cache size $Vs \gets 0$ \\
    
    \For{$n \gets 1$ \KwTo $N$}{
        Estimate $S_{opt}^n$ from Eq~\ref{eq:graph-optim-head}\\
        $N_n \gets |S_{opt}^n|$ \\
        \eIf{$C_{n-1} > st$ }{
            $C_n \gets \mathrm{circularCache}_w\{C_{n-1}, N_n\}$ \\
            }{}
        
        \eIf{$RMSE(C_n - C_{n-1}) \leq t$}{
            $V \gets S_{opt}^n$ \\
            Push $V$ as pose updates
          }{
          $V \gets V+S_{opt}^n$ \\
          $Vs \gets Vs + N_n$ \\
              \If{$Vs \geq ct$}{
                  Push $V$ as pose updates
              }
          }
    }
\end{algorithm}

So these WiFi global pose estimates could be sent to the camera graph as camera's Odometer measurements for every frame of the WiFi measurement.

\textbf{Smart Pose Update Buffering:}
However, numerous and large updates to the odometry measurements in the camera graph would trigger frequent graph optimization for large number of camera factors.
These camera factors will keep increasing as the number of robot poses keep increasing, leading to updates in the camera graph which becomes memory intensive.
Thus we cannot naively send each and every WiFi graph's pose updates to the camera graph and observe that these WiFi frames usually are updated at a rate of ~100Hz while camera frames are only fed at ~2-10Hz.
With this observation, \name's WiFi graph's pose updates are maintained in a buffer that is continuously updated when there are frequent large updates.
This buffer of pose-updates are pushed as odometer updates to the camera graph only when these global pose updates are lesser than a threshold as described in Algorithm~\ref{algo:pose-buffer}.
This buffer-based updates avoids frequent global camera graph optimization avoiding high compute and memory demanding operations. \todo{this needs to be corrected}

From the Algorithm~\ref{algo:pose-buffer} we can see that the Pose updates buffer $V$, can create significant delay between the WiFi graph and camera graph. To avoid such significant delays we limit the size of the number of pose updates that can be held in the buffer $V$, thus avoiding any observable delays in the camera graph optimization.

Finally, once the camera factor graph receives the pose updates from the WiFi graph, they are used as `Oracle' pose measurements.
These measurements are used to constrain the camera locations where certain camera frames features have been detected and mapped.
We utilize VINS-MONO~\cite{qin2018vins} features extractor for feature extraction and feature matching across various frames. Once the feature matching across local frames has been performed they are then mapped into the 3D space as point clouds which are then optimized for in tandem with the WiFi global pose updates for optimized mapping and local pose corrections of the robot. \todo{add more information about SmartProjectionPoseFactors from GTSAM}
Thus \name solves for low-cost, low-compute, and context-aware SLAM system using a `Dual-graph' layered approach.

\section{Measurements For factor Graphs}\label{sec:design-measure}
To further demonstrate and deploy \name on COTS devices, we need to estimate accurate measurements for each factor graph.
So in this section, we present our solution for estimating accurate and robust WiFi bearing and camera measurements for the WiFi graph in ~\cref{sec:design-bearing} and camera graph in ~\cref{sec:design-camera}.

\subsection{Accurate \& Robust WiFi Measurements}\label{sec:design-bearing}

Finally, while existing works use end-to-end optimization, in \name we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for map-building. 
This demands that the bearing measurements made are real-time, robust and accurate.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reasons for inaccuracies in the bearing measurements for indoors are multipath and Non-Line of Sight issues that have been well-studied~\cite{spotfi,arraytrack,ayyalasomayajula2020deep,ma2019wifi,soltanaghaei2018multipath} in the literature. 
It is known that the WiFi signal is broadcasted and at the receiver a combination of all these different paths called `multipath' is measured as shown in Figure~\ref{fig:wifi-meas}.
Additionally, the receiver measures a complex, channel state information (CSI) whose phase values are the accumulation of delays along each individual direction. 
Wherein, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are cause for erroneous bearing estimates.
Additionally, since each antenna is physically at a farther distance, the phase accumulates for the extra distance travelled to each antenna on the access point.

With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna for $n^{th}$ frequency component, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m, n} = \underbrace{\Big[H^{m, n}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m, n}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{arraytrack,spotfi} are vulnerable to aliasing, as there is no distinction between signals coming from opposite sides of the array.
Since we need to resolve this ambiguity in order to estimate the true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. We incorporate this into our CSI model from Eq~\ref{eq:sensor_model1} as:
$$
    H^{m, n}_i = a_i \exp\left({\textstyle -\iota 2 \pi \frac{f_0}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right) \exp \left({\textstyle -\iota 2\pi  \frac{f_n}{c} l_i}\right)
$$
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{spotfi, vasisht2016decimeter}.


Individual CSI measurements are vulnerable to noise and transient multipath, meaning that some of the bearings we measure will be erroneous.
Systems in the past\cite{spotfi} have typically employed a two-stage solution of (i) principle component analysis (PCA) based temporal packet averaging, followed by a\todo{reword} (ii) super-resolution algorithm to deal with multipath accurately and separate the direct path from the reflected paths.
However, these super-resolution algorithms are very compute intensive and thus cannot be deployed in real time in a scalable manner. So, we instead rely just on temporal CSI smoothing to remove this noise from our measured channel. To this end, we observe that reflected paths are much less consistent across packets than the direct path\cite{arraytrack}. So, we combine multiple channel measurements into a matrix $M = \begin{bmatrix}M_0,&M_1,&...\end{bmatrix}$ to estimate the true channel $H$ from the measured channels. Assuming the robot does not move too much in between measurements, the true channel should remain consistent. Additionally, most devices transmitting WiFi signals transmit on multiple antennas, allowing us to make multiple channel measurements per transmission. With these dense measurements, we can now use PCA to estimate the true channel. We assume that noise and multipath is much less correlated across measurements than the direct path. Under this assumption, our distribution of channel measurements has greatest variance along an axis $V$ corresponding to our true channel. In particular, it maximises 
$$
H\approx\argmax_{V}\sum_{i}(|\langle M_i,V \rangle|)^2
$$.
This largest principle component $V$ of the measurement matrix M is commonly known to be the eigenvector corresponding to the largest eigenvalue of $MM^\dag$, where $\dag$ is the conjugate transpose operator. We compute this vector by singular value decomposition of $M$, where $V$ will be the first basis vector in the left subspace. Thus, we have implemented a CSI smoothing method that filters erroneous measurements and attenuates multipath, without using a high-compute super-resolution algorithm. In most cases, this channel will correspond to the direct path, and from here a simple 2D FFT can be used to identify the bearing of the direct path as detailed in ~\cite{ayyalasomayajula2018bloc,xie2019md}.

Thus, \name solves for getting accurate and dense bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

\subsection{Accurate Camera Measurements}\label{sec:design-camera}

In \name we utilize the camera feature extractor and tracker functionalities of the VINS-MONO implementation~\cite{qin2018vins}, wherein they extract the Shi-Tomasi features~\cite{shi1994good} for each frame. 
But as the robot moves some of the older frames and thus the features go out of view.
These out of frame features are replaced by a new set of features identified in the current frame so as to maintain a constant number of detected features in each frame.
This also avoids placing any features behind the camera's FOV and creating chirality issues. \todo{lacks clarity here}
The fixed number of camera points is a tunable parameter and in \name we use \todo{xx} number of features to be detected in each frame as `landmarks' mapped in the environment.
These `landmarks' aid in the local-pose corrections and mapping of the environment as discussed in ~\cref{sec:design-graph2}.

Thus we have seen how the layered approach in bifurcating the tasks between the WiFi and camera sensors to utilize them for what they are best at brings the best of both the sensors. This Visual and WiFi Dual factor graph SLAM solution thus makes \name-SLAM, low-cost, low-compute, accurate and adaptable SLAM system. Thus enabling scalable and deployable robotics using \name-SLAM's design.

==> ViWiD SLAM_arx/design/design3.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

We have seen how existing Visual (camera) SLAM algorithms are compute and memory intensive, due to the accumulated drifts of the odometry that needs to be corrected. 
As discussed in ~\cref{sec:back-wifi}, we solve this by designing a dual-layered solution, as demonstrated in Figure~\ref{fig:intro-fig}.
The robot, mounted with WiFi and camera sensors, navigates in the environment, while \name's WiFi layer combines WiFi and odometry measurements to provide for accurate pose estimates that are drift free. 
This design removes the need for compute and memory heavy correlation (`loop-closure') operations. We first describe this drift-free pose generation in ~\cref{sec:design-graph1}.
These drift-free poses are fed to the \name visual layer that consumes these poses via a smart real-time buffer, along with camera frames, which we further detail in ~\cref{sec:design-graph2}.
In ~\cref{sec:design-measure}, we specify \name's methods for integrating these measurements into the \name WiFi and visual layers.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

Firstly, to identify the sensor modality to use within the \name WiFi layer that provides for drift-free pose estimates, we make a few interesting observations:
(i) All robots are equipped with a WiFi transceiver, (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is an inexpensive sensing modality, and (iv) WiFi based localization and tracking~\cite{ma2019wifi} is well studied and can be exploited for global pose estimation. Owing to these reasons, we utilize WiFi as a low-compute and low-memory sensor that can be used to build a SLAM system capable of providing drift-free robot poses to the Visual SLAM system.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}

\noindent\textbf{Angle of Arrival at Robot as WiFi Measurements:}
Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearing measurements are a robust WiFi-based estimation method for indoor localization and tracking.
Inspired from these works, we measure the Angle of Arrival (AoAs) of incoming signals at the robot,  thus not needing collaboration with WiFi access points (APs) in the environment. These are the WiFi measurements to be integrated into \name WiFi layer.
AoA measurements can be estimated at the robot's WiFi device with respect to WiFi transmitters in the environment using the Channel State Information, (CSI) measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi,arraytrack}.

\noindent\textbf{Unknown AP Locations and Robot Poses:}
Most current localization algorithms use AoA measurements with respect to multiple APs to locate the transmitting device. 
Unfortunately, we do not know the locations of these APs in the environment, as in a SLAM scenario we cannot assume any a priori information about the environment.
Thus, we cannot get accurate robot poses using existing localization algorithms~\cite{spotfi,soltanaghaei2018multipath,ayyalasomayajula2020deep,xie2019md}.
There are solutions that use robot pose to estimate the WiFi AP locations~\cite{ayyalasomayajula2020locap}, by tracking AoA measured from an AP across multiple known poses of the robot.
However, the authors of LocAP~\cite{ayyalasomayajula2020locap} need accurate robot poses to do this, which they achieve using a LiDAR based SLAM (Cartographer~\cite{cartographer}). This algorithm is memory and compute inefficient.
So, we need to somehow jointly solve for both the robot poses and the AP locations in the environment with the AoA measurements between them as the only known information.

We observe that GraphSLAM~\cite{gtsam} is capable of jointly solving these multi-variate optimization problems as long as these variables are connected by some measurements. This method uses a graph-based representation of the estimation problem to compute the most likely state of the system (robot poses and landmark locations) given a probabilistic model of the measurements.
So, we define the Wi-Fi facotr graph with odometry readings($z_I^{Odom}$) as measurements connecting two continuous robot poses $p_i,p_{i-1}$, and the Wi-Fi AoA estiamtes ($z_ij^{bearing}$) as measurements connecting the robot's current pose $p_i$ with each AP's position $x_j$ the AoA corresponds to as shown in Figure~\ref{fig:wifi-factor}.
Now that we have defined these variables and measurements, we can compute the most likely robot poses $p_i \forall i\in \{1,2,\cdots,n\}$ where $n$ is the current position of the robot and $n=[1 N]$, where $N$ are the total robot poses in the entirety of time and AP locations $x_j \forall j\in \{1,2,\cdots,N_{ap}\}$, where $N_{ap}$ are the number of APs in the environment.

\noindent\textbf{Building and Optimizing the WiFi-Graph:}
At a high level, the GraphSLAM algorithm defines a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \; \forall i \in [1, N]\}$, where each $\Vec{p}_i$ belongs to the Special Euclidean group ($SE(3)$). 
We can the define the measurement model for the odometry factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$ which would be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion~\cite{diebel2006representing}.
Similarly, one can define the factor graph for the bearing measurements of AP $j$ with AP position $x_j$ as $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$.

Unlike the existing WiFi SLAM architectures~\cite{arun2022p2slam,ferris2007wifi} we do not perform end-to-end optimization, we instead use the incremental smoothing and mapping (iSAM) implementation of the GraphSLAM approach~\cite{gtsam}.
So, once we have defined the measurement models we can estimate the optimized robot poses $S_{opt}^n$ for time instance $n$ by minimizing the total error between our predictions and actual measurements for the subset $I_{sub}$, i.e.
\begin{align}\label{eq:graph-optim-head}
    S_{opt}^n = \argmin_{S} \sum_{i\in I_{sub}} \sum_{j\in I_{sub}}  & \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and AoA measurements respectively. In iSAM, one step of optimization is performed every time a new measurement is added.
Upon a new addition to the graph, we want to optimize $\{p_i \; \forall i \in I_{sub}\}$ for given $I={p_i,x_j: i<n, \forall j \in [1, N_{ap}]}$, where $n$ is the next step of optimization. Only a subset of the factors $I_{sub} \subseteq I$ are optimized, according to the iSAM algorithm, without needing any memory and compute demanding global loop closures. Please refer Appendix~\ref{sec:appendix} for a more formal definitions of each of the variables and understanding the operation of incremental GraphSLAM (iSAM~\cite{gtsam}) which is an open-sourced solver.

\noindent\textbf{Initialization of Factors:} Now that we have defined our graph and the optimization problem, like for any other optimization algorithm we also need to initialize each of the $N$ robot positions and $N_{ap}$ AP positions for the optimizer. 
Like any other SLAM system, we initialize the robot positions using the relative odometry measurements, which have drift accumulated in them. This is the drift we are trying to remove.
Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
While one could naively initialize all known APs in the environment at the origin, some APs may start too far away as to estimate their position at all, as there may be no incoming measurements when the optimizer is started.

Since these APs have no measurements attached to them, the loss associated with them is ill-defined and the optimization problem is unsolvable.
Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this indeterminacy due to poor a poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been study extensively in the bast for localization~\cite{ez}.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's translation $p^t_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maximum among all current robot's poses $p_i \forall i \in [1,n]$ measured at $n^{th}$ time instance, with the intuition that this is where the robot passed closest to the AP.
We can then initialize $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation.
Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
Givem good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/camera_factor.pdf}
    \caption{Shows the details of the implementation of the Camera Factor graph. While a typical camera based SLAM would also correct for the robot poses, but since we do not optimize for robot poses in \name camera SLAM, we can thro these nodes away as shown in the figure.}
    \label{fig:cam-factor}
\end{figure}

\subsection{Camera Factor Graph}\label{sec:design-graph2}

As we described in ~\cref{sec:back-vio}, a Visual-Inertial Odometry based SLAM system needs camera features and odometry measurements. 
To extract, track and map the camera features we utilize  Shi-Tomasi features~\cite{shi1994good} from the VINS-MONO implementation~\cite{qin2018vins}.
These camera features are then mapped onto a unit sphere to get an approximate estimate of the 3D locations of the measured features.
These projections are then projected into the map as `landmarks' in the factor graph for a fixed set of local frames. 
The positions of these `landmarks' and the odometry measurements can now be jointly optimized to correct the robot's trajectory. 
These local corrections ensure accurate 3D mapping of the `landmark' point clouds in the environment as shown in Figure~\ref{fig:cam-factor}.
While a typical camera based SLAM would need to simultaneously correct for the robot poses, in \name, we strongly constrain the robot's poses to discourage optimizing over them, instead estimating them in \name's WiFi SLAM layer.

% We detail on how we extract robust camera measurements in ~\cref{sec:design-camera}, where we go into further details on how we use the feature extraction provided by the VINS-MONO feature extractor and tracker~\cite{qin2018vins}.
In addition to this, these VIO-SLAM systems require global loop closures to cancel the drift accrued in the robot pose estimates provided by the robot's inertial odometry. However, the homogeneity of these visual feature based landmarks demands constant feature matching operations, and requires a large memory cache of all the landmarks.
\name sidesteps this issue by using the global pose estimates provided by the WiFi graph, which do not drift over time, as the robot pose measurements for the camera graph.
Since these WiFi global pose estimates can be made in real time with high-accuracy, we can eliminate the need for global loop closure in these visual feature-based VIO-SLAM systems.

\begin{algorithm}[t]
\caption{Implementation of WiFi pose update buffering to the Visual Odometry graph.}
\label{algo:pose-buffer}
    \SetAlgoLined
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input{Pose threshold $\Delta P$, stability threshold size $N_{thresh}$, max size of circular cache $N_{cache}$}
    initialization circular cache $C_{update} \leftarrow \{\}$;
    Buffer $V_{update} \leftarrow \{\} $;
    Pose Updates $P_{opt}^0\leftarrow \{\} $ \\
    \For{$t \gets 1$ \KwTo $T$}{
        Estimate $P_{opt}^t$ from Eq~\ref{eq:graph-optim-head}
        \begin{flalign}
        P_{filt}^t &= \{p^t - p^{t-1} > \Delta P \;|\; p^t \in P_{opt}^t; p^{t-1} \in P_{opt}^{t-1}\}&&\nonumber\\
                    & \cup \; \{p \;|\; p \in  P_{opt}^t; p \not\in P_{opt}^{t-1}\}&&\nonumber
        \end{flalign}\\
        $N_t \gets |P_{filt}^t|$ \\
        $C_{update} \gets append(C_{update}, N_t)$ \\
        $V_{update} \gets append(V_{update}, P_{filt}^t)$ \\
        \If{$ n < N_{thresh}, \; \forall n \in C_{update} $}{
            Flushes the buffer, $V$ as pose updates
        }
    }
\end{algorithm}

So, these WiFi global pose estimates can be sent to the camera graph as odometry measurements when the WiFi graph updates.

\textbf{Smart Pose Update Buffering:}
However, numerous and large updates to the odometry measurements in the camera graph would trigger frequent graph optimization for large number of camera factors.
These camera factors will keep increasing as the number of robot poses keep increasing, leading to updates in the camera graph which becomes memory intensive.
Thus we cannot naively send each and every WiFi graph's pose updates to the camera graph and observe that these WiFi frames usually are updated at a rate of ~100Hz while camera frames are only fed at ~2-10Hz.
With this observation, \name WiFi graph's pose updates are maintained in a buffer ($V_{update}$) that is continuously updated when there are frequent large updates. A large update to the robot pose is defined with respect to the pose threshold, $\Delta P$ in Algorithm~\ref{algo:pose-buffer}.
This poses in $V_{update}$ are pushed as pose updates to the camera graph only when the WiFi-graph is stable, i.e., when the total number of updates in the past $N_{cache}$ optimization steps is less than $N_{thresh}$.
Effectively, by tuning $N_{cache}$ and $N_{thresh}$, we can define the sensitivity of stability. 
For example, by increasing $N_{cache}$ and decreasing $N_{thresh}$, we wait longer for the WiFi-graph robot poses to stabilize. 
Additionally, by tuning $\Delta P$, we can re-define what we mean by an update to reduce the number of the updates sent to the camera graph. 
By incorporating this smart buffer \name avoids frequent global camera graph optimization avoiding high compute and memory demanding operations. 

Finally, once the camera factor graph receives the pose updates from the WiFi graph, they are used as drift-free pose measurements.
These measurements are used to constrain the camera locations where certain camera features have been detected and mapped.
We utilize VINS-MONO~\cite{qin2018vins} features tracker for feature extraction and feature matching across various frames. 
Once the feature matching across local frames has been performed they are then mapped into the 3D space as point clouds which are then optimized for in tandem with the WiFi global pose updates for optimized mapping and local pose corrections of the robot. 
Thus \name solves for  compute and memory efficient SLAM system using a `Dual-graph' layered approach.

\section{Measurements For factor Graphs}\label{sec:design-measure}
To further demonstrate and deploy \name on COTS devices, we need to estimate accurate measurements for each factor graph.
So in this section, we present our solution for estimating accurate and robust WiFi bearing and camera measurements for the WiFi graph in ~\cref{sec:design-bearing} and camera graph in ~\cref{sec:design-camera}.

\subsection{Accurate \& Robust WiFi Measurements}\label{sec:design-bearing}

Finally, while existing works use end-to-end optimization, in \name we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for map-building. 
This demands that the bearing measurements made are real-time, robust and accurate.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reasons for inaccuracies in the bearing measurements for indoors are multipath and Non-Line of Sight issues that have been well-studied~\cite{spotfi,arraytrack,ayyalasomayajula2020deep,ma2019wifi,soltanaghaei2018multipath} in the literature. 
It is known that the WiFi signal is broadcasted and at the receiver a combination of all these different paths called `multipath' is measured as shown in Figure~\ref{fig:wifi-meas}.
Additionally, the receiver measures a complex, channel state information (CSI) whose phase values are the accumulation of delays along each individual direction. 
Wherein, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are cause for erroneous bearing estimates.
Additionally, since each antenna is physically at a farther distance, the phase accumulates for the extra distance travelled to each antenna on the access point.

With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna for $n^{th}$ frequency component, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m, n} = \underbrace{\Big[H^{m, n}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m, n}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{arraytrack,spotfi} are vulnerable to aliasing, as there is no distinction between signals coming from opposite sides of the array.
Since we need to resolve this ambiguity in order to estimate the true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. We incorporate this into our CSI model from Eq~\ref{eq:sensor_model1} as:
$$
    H^{m, n}_i = a_i \exp\left({\textstyle -\iota 2 \pi \frac{f_0}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right) \exp \left({\textstyle -\iota 2\pi  \frac{f_n}{c} l_i}\right)
$$
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{spotfi, vasisht2016decimeter}.

\todo{connect the english in this paragraph to the channel model build in 2}
Individual CSI measurements are vulnerable to noise and transient multipath, meaning that some of the bearings we measure will be erroneous.
Systems in the past\cite{spotfi} have typically employed a two-stage solution of (i) principle component analysis (PCA) based temporal packet averaging, followed by a (ii) super-resolution algorithm to deal with multipath accurately and separate the direct path from the reflected paths.
However, these super-resolution algorithms are very compute intensive and thus cannot be deployed in real time in a scalable manner. So, we instead rely just on temporal CSI averaging to remove this noise from our measured channel. To this end, we observe that reflected paths are much less consistent across packets than the direct path\cite{arraytrack}. So, we combine multiple channel measurements into a matrix $M = \begin{bmatrix}M_0,&M_1,&...\end{bmatrix}$ to estimate the true channel $H$ from the measured channels. Assuming the robot does not move too much in between measurements, the true channel should remain consistent. Additionally, most devices transmitting WiFi signals transmit on multiple antennas, allowing us to make multiple channel measurements per transmission. With these dense measurements, we can now use PCA to estimate the true channel. We assume that noise and multipath is much less correlated across measurements than the direct path. Under this assumption, our distribution of channel measurements has greatest variance along an axis $V$ corresponding to our true channel, that we call principle component channel or PC-CSI. In particular, it maximises 
$$
H\approx\argmax_{V}\sum_{i}(|\langle M_i,V \rangle|)^2.
$$
This largest principle component $V$ of the measurement matrix M is commonly known to be the eigenvector corresponding to the largest eigenvalue of $MM^\dag$, where $\dag$ is the conjugate transpose operator. We compute this vector by singular value decomposition of $M$, where $V$ will be the first basis vector in the left subspace. Thus, we have implemented a principle component CSI method that filters erroneous measurements and attenuates multipath, without using a high-compute super-resolution algorithm. In most cases, this channel will correspond to the direct path, and from here a simple 2D FFT can be used to identify the bearing of the direct path as detailed in ~\cite{ayyalasomayajula2018bloc,xie2019md}.

Thus, \name solves for getting accurate and dense bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

\subsection{Accurate Camera Measurements}\label{sec:design-camera}

In \name we utilize the camera feature extractor and tracker functionalities of the VINS-MONO implementation~\cite{qin2018vins}, \\wherein they extract the Shi-Tomasi features~\cite{shi1994good} for each frame. 
But as the robot moves some of the older frames and thus the features go out of view.
These out of frame features are replaced by a new set of features identified in the current frame so as to maintain a constant number of detected features in each frame.
This also avoids placing any features behind the camera's FOV and creating chirality issues.
The fixed number of camera points is a tunable parameter and in \name we use 50 number of features to be detected in each frame as `landmarks' mapped in the environment.
These `landmarks' aid in the local-pose corrections and mapping of the environment as discussed in ~\cref{sec:design-graph2}.

Thus we have seen how the layered approach in bifurcating the tasks between the WiFi and camera sensors to utilize them for what they are best at brings the best of both the sensors. This Visual and WiFi Dual factor graph SLAM solution thus makes \name-SLAM, low-memory, low-compute, accurate and adaptable SLAM system. Thus enabling scalable and deployable robotics using \name-SLAM's design.

==> ViWiD SLAM_arx/design/design4.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

We have seen how existing Visual (camera) SLAM algorithms are compute and memory intensive, due to the accumulated drifts of the odometry that needs to be corrected. 
As discussed in ~\cref{sec:back-wifi}, we solve this by designing a dual-layered solution, as demonstrated in Figure~\ref{fig:intro-fig}.
The robot, mounted with WiFi and camera sensors, navigates in the environment, while \name's WiFi layer combines WiFi and odometry measurements to provide for accurate pose estimates that are drift free. 
This design removes the need for compute and memory heavy correlation (`loop-closure') operations. We first describe this drift-free pose generation in ~\cref{sec:design-graph1}.
These drift-free poses are fed to the \name visual layer that consumes these poses via a smart real-time buffer, along with camera frames, which we further detail in ~\cref{sec:design-graph2}.
In ~\cref{sec:design-measure}, we specify \name's methods for integrating these measurements into the \name WiFi and visual layers.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

Firstly, to identify the sensor modality to use within the \name WiFi layer that provides for drift-free pose estimates, we make a few interesting observations:
(i) All robots are equipped with a WiFi transceiver, (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is an inexpensive sensing modality, and (iv) WiFi based localization and tracking~\cite{ma2019wifi} is well studied and can be exploited for global pose estimation. Owing to these reasons, we utilize WiFi as a low-compute and low-memory sensor that can be used to build a SLAM system capable of providing drift-free robot poses to the Visual SLAM system.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}

\noindent\textbf{Angle of Arrival at Robot as WiFi Measurements:}
Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearing measurements are a robust WiFi-based estimation method for indoor localization and tracking.
Inspired from these works, we measure the Angle of Arrival (AoAs) of incoming signals at the robot,  thus not needing collaboration with WiFi access points (APs) in the environment. These are the WiFi measurements to be integrated into \name WiFi layer.
AoA measurements can be estimated at the robot's WiFi device with respect to WiFi transmitters in the environment using the Channel State Information, (CSI) measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi,arraytrack}.

\noindent\textbf{Unknown AP Locations and Robot Poses:}
Most current localization algorithms use AoA measurements with respect to multiple APs to locate the transmitting device. 
Unfortunately, we do not know the locations of these APs in the environment, as in a SLAM scenario we cannot assume any a priori information about the environment.
Thus, we cannot get accurate robot poses using existing localization algorithms~\cite{spotfi,soltanaghaei2018multipath,ayyalasomayajula2020deep,xie2019md}.
There are solutions that use robot pose to estimate the WiFi AP locations~\cite{ayyalasomayajula2020locap}, by tracking AoA measured from an AP across multiple known poses of the robot.
However, the authors of LocAP~\cite{ayyalasomayajula2020locap} need accurate robot poses to do this, which they achieve using a LiDAR based SLAM (Cartographer~\cite{cartographer}). This algorithm is memory and compute inefficient.
So, we need to somehow jointly solve for both the robot poses and the AP locations in the environment with the AoA measurements between them as the only known information.

We observe that GraphSLAM~\cite{gtsam} is capable of jointly solving these multi-variate optimization problems as long as these variables are connected by some measurements. This method uses a graph-based representation of the estimation problem to compute the most likely state of the system (robot poses and landmark locations) given a probabilistic model of the measurements.
So, we define the Wi-Fi facotr graph with odometry readings($z_I^{Odom}$) as measurements connecting two continuous robot poses $p_i,p_{i-1}$, and the Wi-Fi AoA estiamtes ($z_ij^{bearing}$) as measurements connecting the robot's current pose $p_i$ with each AP's position $x_j$ the AoA corresponds to as shown in Figure~\ref{fig:wifi-factor}.
Now that we have defined these variables and measurements, we can compute the most likely robot poses $p_i \forall i\in \{1,2,\cdots,n\}$ where $n$ is the current position of the robot and $n=[1 N]$, where $N$ are the total robot poses in the entirety of time and AP locations $x_j \forall j\in \{1,2,\cdots,N_{ap}\}$, where $N_{ap}$ are the number of APs in the environment.

\noindent\textbf{Building and Optimizing the WiFi-Graph:}
At a high level, the GraphSLAM algorithm defines a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \; \forall i \in [1, N]\}$, where each $\Vec{p}_i$ belongs to the Special Euclidean group ($SE(3)$). 
We can the define the measurement model for the odometry factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$ which would be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion~\cite{diebel2006representing}.
Similarly, one can define the factor graph for the bearing measurements of AP $j$ with AP position $x_j$ as $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$.

Unlike the existing WiFi SLAM architectures~\cite{arun2022p2slam,ferris2007wifi} we do not perform end-to-end optimization, we instead use the incremental smoothing and mapping (iSAM) implementation of the GraphSLAM approach~\cite{gtsam}.
So, once we have defined the measurement models we can estimate the optimized robot poses $S_{opt}^n$ for time instance $n$ by minimizing the total error between our predictions and actual measurements for the subset $I_{sub}$, i.e.
\begin{align}\label{eq:graph-optim-head}
    S_{opt}^n = \argmin_{S} \sum_{i\in I_{sub}} \sum_{j\in I_{sub}}  & \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and AoA measurements respectively. In iSAM, one step of optimization is performed every time a new measurement is added.
Upon a new addition to the graph, we want to optimize $\{p_i \; \forall i \in I_{sub}\}$ for given $I={p_i,x_j: i<n, \forall j \in [1, N_{ap}]}$, where $n$ is the next step of optimization. Only a subset of the factors $I_{sub} \subseteq I$ are optimized, according to the iSAM algorithm, without needing any memory and compute demanding global loop closures. Please refer Appendix~\ref{sec:appendix} for a more formal definitions of each of the variables and understanding the operation of incremental GraphSLAM (iSAM~\cite{gtsam}) which is an open-sourced solver.

\noindent\textbf{Initialization of Factors:} Now that we have defined our graph and the optimization problem, like for any other optimization algorithm we also need to initialize each of the $N$ robot positions and $N_{ap}$ AP positions for the optimizer. 
Like any other SLAM system, we initialize the robot positions using the relative odometry measurements, which have drift accumulated in them. This is the drift we are trying to remove.
Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
While one could naively initialize all known APs in the environment at the origin, some APs may start too far away as to estimate their position at all, as there may be no incoming measurements when the optimizer is started.

Since these APs have no measurements attached to them, the loss associated with them is ill-defined and the optimization problem is unsolvable.
Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this indeterminacy due to poor a poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been study extensively in the bast for localization~\cite{ez}.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's translation $p^t_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maximum among all current robot's poses $p_i \forall i \in [1,n]$ measured at $n^{th}$ time instance, with the intuition that this is where the robot passed closest to the AP.
We can then initialize $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation.
Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
Given good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.

\subsection{Accurate \& Robust WiFi Measurements}\label{sec:design-bearing}

Finally, while existing works use end-to-end optimization, in \name we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for map-building. 
This demands that the bearing measurements made are real-time, robust and accurate.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reasons for inaccuracies in the bearing measurements for indoors are multipath and Non-Line of Sight issues that have been well-studied~\cite{spotfi,arraytrack,ayyalasomayajula2020deep,ma2019wifi,soltanaghaei2018multipath} in the literature. 
It is known that the WiFi signal is broadcasted and at the receiver a combination of all these different paths called `multipath' is measured as shown in Figure~\ref{fig:wifi-meas}.
Additionally, the receiver measures a complex, channel state information (CSI) whose phase values are the accumulation of delays along each individual direction. 
Wherein, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are cause for erroneous bearing estimates.
Additionally, since each antenna is physically at a farther distance, the phase accumulates for the extra distance travelled to each antenna on the access point.

With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna for $n^{th}$ frequency component, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m, n} = \underbrace{\Big[H^{m, n}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m, n}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{arraytrack,spotfi} are vulnerable to aliasing, as there is no distinction between signals coming from opposite sides of the array.
Since we need to resolve this ambiguity in order to estimate the true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. We incorporate this into our CSI model from Eq~\ref{eq:sensor_model1} as:
$$
    H^{m, n}_i = a_i \exp\left({\textstyle -\iota 2 \pi \frac{f_0}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right) \exp \left({\textstyle -\iota 2\pi  \frac{f_n}{c} l_i}\right)
$$
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{spotfi, vasisht2016decimeter}.

\todo{connect the english in this paragraph to the channel model build in 2}
Individual CSI measurements are vulnerable to noise and transient multipath, meaning that some of the bearings we measure will be erroneous.
Systems in the past\cite{spotfi} have typically employed a two-stage solution of (i) principle component analysis (PCA) based temporal packet averaging, followed by a (ii) super-resolution algorithm to deal with multipath accurately and separate the direct path from the reflected paths.
However, these super-resolution algorithms are very compute intensive and thus cannot be deployed in real time in a scalable manner. So, we instead rely just on temporal CSI averaging to remove this noise from our measured channel. To this end, we observe that reflected paths are much less consistent across packets than the direct path\cite{arraytrack}. So, we combine multiple channel measurements into a matrix $M = \begin{bmatrix}M_0,&M_1,&...\end{bmatrix}$ to estimate the true channel $H$ from the measured channels. Assuming the robot does not move too much in between measurements, the true channel should remain consistent. Additionally, most devices transmitting WiFi signals transmit on multiple antennas, allowing us to make multiple channel measurements per transmission. With these dense measurements, we can now use PCA to estimate the true channel. We assume that noise and multipath is much less correlated across measurements than the direct path. Under this assumption, our distribution of channel measurements has greatest variance along an axis $V$ corresponding to our true channel, that we call principle component channel or PC-CSI. In particular, it maximises 
$$
H\approx\argmax_{V}\sum_{i}(|\langle M_i,V \rangle|)^2.
$$
This largest principle component $V$ of the measurement matrix M is commonly known to be the eigenvector corresponding to the largest eigenvalue of $MM^\dag$, where $\dag$ is the conjugate transpose operator. We compute this vector by singular value decomposition of $M$, where $V$ will be the first basis vector in the left subspace. Thus, we have implemented a principle component CSI method that filters erroneous measurements and attenuates multipath, without using a high-compute super-resolution algorithm. In most cases, this channel will correspond to the direct path, and from here a simple 2D FFT can be used to identify the bearing of the direct path as detailed in ~\cite{ayyalasomayajula2018bloc,xie2019md}.

Thus, \name solves for getting accurate and dense bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

==> ViWiD SLAM_arx/design/design5.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

\todo{Start by describing your design... }

We have seen that loop closures can be memory and compute intensive at best or at worst can detrimentally affect the quality of the pose prediction during incorrect keyframe matching. \todo{have you? read your DLOC design intro... }
To circumvent loop-closures entirely, we design a real time \todo{is it just WiFi graph??} Wifi-graph as demonstrated in Figure~\ref{fig:wifi-factor} to take advantage of existing WiFi access points in the environment and provide correction to drift accommodated by Visual-intertial or Lidar-inertial SLAM systems.

The robot, mounted with WiFi and camera (or Lidar) sensors, navigates in the environment. Through local feature matching (or scan matching) and the inertial measurements from IMU (or wheel encoder), the SLAM algorithm provides accurate pose measurements for the robot in real time. These pose updates from the local-odometry are fed into the Wifi-graph which incorporates the bearing of the incoming WiFi signal to track a deployed WiFi access point (AP) in an environment. In effect, the AP is treated as a stationary and unique landmark. Furthermore, since the incoming WiFi signal identifies the access point it originated from, this design removes the need for compute and memory heavy correlation (`loop-closure') operations. 

We first formulate and describe this drift-free pose generation in ~\cref{sec:design-graph1} assuming we have the local-odometry from VIO/LIO.
We then detail on how to get accurate WiFi measurements for the WiFi graph's real-time optimization in ~\cref{sec:design-bearing}. We finally describe how the system is built and optimized along with the Visual-graph in ~\cref{sec:design-camera}.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

Firstly, to motivate the use of WiFi as the sensor modality to use, we make a few interesting observations:
(i) All robots are equipped with a WiFi transceiver, (ii) It is ubiquitously deployed in indoor environments, (iii) It is an inexpensive sensing modality, and (iv) WiFi based localization and tracking~\cite{ma2019wifi} is well studied and can be exploited for global pose estimation. Owing to these reasons, we utilize WiFi as a low-compute and low-memory sensor that can be used to build a SLAM system capable of providing drift-free robot poses to the Visual (or Lidar) SLAM systems. \todo{make sure you don't under-estimate your contribution to A+B, if WiFi is already low-compute and low-memory what did you do? }

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}

\noindent\textbf{Angle of Arrival at Robot as WiFi Measurements:}
Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearing measurements are a robust WiFi-based estimation method for indoor localization and tracking.
Inspired from these works, we use the bearing of the incoming signals at the robot as our WiFi measurements, thus not needing collaboration with WiFi access points (APs) in the environment.
Bearing measurements can be estimated at the robot's WiFi device with respect to WiFi transmitters in the environment using the Channel State Information, CSI, measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi}.

Unfortunately, we do not know the locations of these APs in the environment a-prioiri, as is typically required~\cite{spotfi}.
So, we need to jointly solve for both the robot poses and the AP locations in the environment with the AoA measurements between them as the only known information.

We observe that GraphSLAM~\cite{gtsam} is capable of jointly solving these multi-variate optimization problems as long as these variables are connected by some measurements. This method uses a graph-based representation of the estimation problem to compute the most likely state of the system (robot poses and landmark locations) given a probabilistic model of the measurements.
So, we define the Wi-Fi factor graph with odometry readings($z_i^{odom}$) as measurements connecting two continuous robot poses $p_i,p_{i+1}$, and the Wi-Fi AoA estimates ($z_{ij}^{Bearing}$) as measurements connecting the robot's current pose $p_i$ with each AP's position $x_j$ as shown in Figure~\ref{fig:wifi-factor} (left).
Here we assume a generic in-between odometry reading, which can be provided by the VIO/LIO \textit{without} their loop-closure modules or a simple wheel encoder.
Now that we have defined these variables and measurements, we can compute the most likely robot poses $p_i \forall i\in \{1,2,\cdots,n\}$ where $n$ is the current position of the robot and $n=[1 N]$, where $N$ are the total robot poses in the entirety of time and AP locations $x_j \forall j\in \{1,2,\cdots,N_{ap}\}$, where $N_{ap}$ are the number of APs in the environment.

\noindent\textbf{Building and Optimizing the WiFi-Graph:}
Unlike prior work~\cite{arun2022p2slam, ferris2007wifi}, we do not use end-end optimization and instead opt to use the incremental smoothing and mapping (iSAM)~\cite{gtsam} to provide real-time pose estimates. At a high level, the state space at time $t$, $S_t$, is a set of robot poses and access point locations over $t$ time steps in our graph, $S_t = \{\Vec{p}_i \; \forall i \in [1, t]\} \cup \{\Vec{x}_j \; \forall j \in [1, N]\}$, with the robot pose, $\Vec{p}_i \in SE(3)$ and the $N$ access points positions observed till time $t$, $x_i \in \mathbb{R}^3$. 
We can the define odometry measurements (from VIO/LIO or wheel encoders) between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps as:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion~\cite{diebel2006representing}.
Similarly, one can define the factor graph for the bearing measurements of AP $j$ with AP position $x_j$ as $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$. \todo{add this factor defn here as well}

So, once we have defined the measurement models we can estimate the optimized robot poses $S^{opt}_t$ for time instance $t$ by minimizing the total error between our predictions and actual measurements,
\begin{align}\label{eq:graph-optim-head}
    S^{opt}_t = \argmin_{S_t} & \sum_{i \leq t} \sum_{j \leq N}  \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and bearing measurements respectively. 

\noindent\textbf{Initialization of Factors:} Next to ensure convergence of our optimization, we need to initialize each of the $t$ robot positions and $N$ AP positions for the optimizer. 
Similar to prioir works~\cite{arun2022p2slam}, the robot positions are initialized using the relative odometry measurements. These poses have accumulated drift over time which we seek to correct.
A naive initialization for the AP's would be to place them at the origin and allow the optimizer to place them appropriately in the environment. Unfortunately, the iSAM optimizer, given the limited number of measurements it has seen up until time $t$, can fail to converge with this naive initialization. 

% Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
% While one could naively initialize all known APs in the environment at the origin, some APs may not be receiving any signals at all as they are actually very far from the robot's origin, thus might be too far away when the optimizer is started.

% Since these faraway APs have no measurements attached to them, the cost associated with them is ill-defined and the optimization problem is unsolvable.
% Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this in-determinancy due to poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been study extensively in the past for localization~\cite{ez}.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's pose $p_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maximum among all current robot's poses $p_i \forall i \in [1,t]$, with the intuition that this is where the robot passed closest to the AP.
We can then initialize the $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation. This random perturbation is added to avoid in-determinancy with the optimizer. 
% Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
% Given good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.

\subsection{Accurate \& Unambiguous WiFi Measurements}\label{sec:design-bearing}

Finally, while existing works use end-to-end optimization, in \name we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for map-building. 
This demands that the bearing measurements made are real-time, unambiguous and accurate.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reasons for inaccuracies in the bearing measurements for indoors are multipath and Non-Line of Sight issues that have been well-studied~\cite{spotfi,arraytrack,ayyalasomayajula2020deep,ma2019wifi,soltanaghaei2018multipath} in the literature. 
It is known that the WiFi signal is broadcasted and at the receiver a combination of all these different paths called `multipath' is measured as shown in Figure~\ref{fig:wifi-meas}.
Additionally, the receiver measures a complex, channel state information (CSI) whose phase values are the accumulation of delays along each individual direction. 
Wherein, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are cause for erroneous bearing estimates.
Additionally, since each antenna is physically at a farther distance, the phase accumulates for the extra distance travelled to each antenna on the access point.

With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna for $n^{th}$ frequency component, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m, n} = \underbrace{\Big[H^{m, n}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m, n}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/eval_ral/aoa-err-boxplot.pdf}
    \caption{ \todo{complete, }}
    \label{fig:aoa-array}
    \vspace{-0.1in}
\end{figure}


\noindent\textbf{Unambiguous Measurements:} However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{arraytrack,spotfi} can resolve only half-plane of the horizontal plane. Thus these linear arrays are vulnerable to aliasing in the full-horizontal plane, as there is no distinction between signals coming from opposite half-planes of the array. Further, as shown in Figure~\ref{fig:aoa-array}(bottom) the errors in bearing measurements increase as the actual bearings are farther from $0^{\circ}$ for the datasets of $\mathrm{P^2}$SLAM.
Since we need to resolve this ambiguity in order to estimate the accurate and true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. 
This can be further seen from Figure~\ref{fig:aoa-array}(top) for the dataset we have collected with the square array. We can see that a square array can resolve more accurately without ambiguity between $-170^{\circ}$ to $180^{\circ}$.
So, we incorporate this into our CSI model from Eq~\ref{eq:sensor_model1} as:
\begin{align}
    H^{m, n}_i = a_i * & \exp\left({\textstyle -\iota 2 \pi \frac{f_0}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right)  \notag\\ &  * \exp \left({\textstyle -\iota 2\pi  \frac{f_n}{c} l_i}\right)
\end{align}
    
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{spotfi, vasisht2016decimeter}.

\todo{connect the english in this paragraph to the channel model build in 2}

\noindent\textbf{Accurate and Real-time bearing measurements:} In order to identify the direct signal's path among the multiple reflected paths, past Wi-Fi systems\cite{spotfi} have used algorithms that super-resolve the measured signal using principle component analysis (PCA) as well as information across different frequency bins to measure the relative time offset between different signal paths. This allows identification of the direct path, as it must have traveled the least distance of all paths and thus arrives before the other reflections

However, these super-resolution algorithms are very compute intensive, because they need to consider each antenna's CSI at each subcarrier frequency independently, and because they have added another dimension to the search space of signals. So, in \name we employ a sliding-window PCA based algorithm to efficiently combine information across subcarriers to estimate the direct path without having to identify and separate all of the reflected paths present in the signal.

We observe that the direct path signal has a property that the reflected paths typically do not: as it has traveled in a straight line, we can expect its contribution to the measured channel $H$ to be much better described by the model \ref{eq:sensor_model1} than the reflected paths. Intuitively, the direct path channel $H_0$ is relatively simple, while the reflected path channels $H_{1...n}$ to estimate the true channel $H$ from the measured channels. Assuming the robot does not move too much in between measurements, the true channel should remain consistent. Additionally, most devices transmitting WiFi signals transmit on multiple antennas, allowing us to make multiple channel measurements per transmission. With these dense measurements, we can now use PCA to estimate the true channel. We assume that noise and multipath is much less correlated across measurements than the direct path. Under this assumption, our distribution of channel measurements has greatest variance along an axis $V$ corresponding to our true channel, that we call principle component channel or PC-CSI. In particular, it maximises 
$$
H\approx\argmax_{V}\sum_{i}(|\langle M_i,V \rangle|)^2.
$$
This largest principle component $V$ of the measurement matrix M is commonly known to be the eigenvector corresponding to the largest eigenvalue of $MM^\dag$, where $\dag$ is the conjugate transpose operator. We compute this vector by singular value decomposition of $M$, where $V$ will be the first basis vector in the left subspace. Thus, we have implemented a principle component CSI method that filters erroneous measurements and attenuates multipath, without using a high-compute super-resolution algorithm. In most cases, this channel will correspond to the direct path, and from here a simple 2D FFT can be used to identify the bearing of the direct path as detailed in ~\cite{ayyalasomayajula2018bloc,xie2019md}.

\noindent\textbf{RSSI Filtering:} Finally, the measurements averaged across time in PC-FFT might note have direct-path which would lead to the dominant path being the reflected path or a noisy measurement. To avoid this, based on the intuition that the signal without the direct path or a weak direct path has very weak received signal strength (RSSI) we set an empirically verified RSSI threshold of $-65$dBm. This leads to the PC-FFT based bearing measurements are accurate.

Thus, \name solves for getting real-time, unambiguous and accurate bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

\begin{figure*}[pt]
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem-interframetime.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation_no_lc.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/aoa_err.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\textbf{Microbenchmarks}: \textbf{(a) Kimera:} Shows the trade-off between memory consumption(red) and the accuracy(blue) for various interframe rates. \textbf{(b) Cartographer:} Shows the trade-off between compute required(red) and the accuracy(blue) for various scan-matching thresholds. \textbf{(c) Odometry-Graph:} Shows the comparison on how various odometry inputs to the WiFi graph look before optimization.\textbf{(d) Bearing Measurement Algorithms:} Comparison between 2D-FFT from $\mathrm{P^2}$SLAM, PC-2D-FFT and our proposed PC-FFT. \todo{avg cpu: 2dfft: 5.6, pc-2dfft: 4.7, pc-fft: 0.11}}
    \label{fig:micro}
    \vspace{-0.1in}
\end{figure*}

\subsection{Dual Graph Integration}\label{sec:design-camera}
Thus we have seen on how the WiFi graph optimizes for accurate and real-time 3-DoF robot poses without requiring any loop-closures when provided with the odometry measurements.
These Odometry can simply come from a wheel encoder and gyroscope of the wheeled robot but it will not have any visual context to be able to provide any human-readable maps.
In contrast, in \name-SLAM's design, we utilize a dual graph approach, wherein we utilize existing VIO/LIO SLAM systems without their loop closure detection and corrections enabled.
So, while these VIO/LIO systems can correct for local drifts in the wheel encoders or the IMUs, they cannot perform global corrections.
These locally corrected robots 3-DoF poses are used to provide the Odometry measurements for the WiFi-graph that we have built in ~\cref{sec:design-graph1}.

The advantage with turning off the loop closure detection and corrections though is that the rate of memory of consumption and compute required is minimized.
Thus, the `VIO/LIO graph` can map the environment while providing locally corrected odometry measurements to the `WiFi-graph`.
The WiFi-graph thus then performs global corrections without the need of loop-closure detection thus enabling \name-SLAM to be an accurate, real-time robot navigation system that can minimizing the rate of memory consumption and the amount of compute.

==> ViWiD SLAM_arx/design/design6.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

A robot, mounted with WiFi and camera (or Lidar) sensors, navigates in the environment. Through local feature matching (or scan matching) and the inertial measurements from IMU (or wheel encoder), the SLAM algorithm provides accurate local pose measurements for the robot in real time. These pose updates from the local-odometry are fed into the WiFi-graph (described in ~\cref{sec:design-graph1}) which incorporates the bearing of the incoming WiFi signal (described in ~\cref{sec:design-bearing}) to track a deployed WiFi access point (AP) in an environment. In effect, the AP is treated as a stationary and unique landmark. Furthermore, since the incoming WiFi signal identifies the access point it originated from, this design removes the need for compute and memory heavy correlation (`loop-closure') operations. Finally, it is imperative to initialize our access points optimally to ensure stability of the convergence (described in~\cref{sec:design-init}). 

% We first formulate and describe this drift-free pose generation in ~\cref{sec:design-graph1} assuming we have the local-odometry from VIO/LIO.
% We first detail on how to get accurate WiFi measurements for the WiFi graph's real-time optimization in ~\cref{sec:design-bearing}. 

\subsection{Providing accurate and real-time WiFi measurements}\label{sec:design-bearing}

Firstly, to motivate the use of WiFi as the sensor modality to use, we make a few interesting observations:
(i) All robots are equipped with a WiFi transceiver, (ii) It is ubiquitously deployed in indoor environments, and (iii) WiFi based localization and tracking~\cite{ma2019wifi, spotfi} is well studied and can be exploited for global pose estimation. Owing to these reasons, we utilize WiFi as a promising sensor to build a SLAM system capable of providing drift-free robot poses to the Visual (or Lidar) SLAM systems. 

Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearing measurements are a robust WiFi-based estimation method for indoor localization and tracking.
Inspired from these works, we use the bearing of the incoming signals at the robot as our WiFi measurements (as shown in Figure~\ref{fig:wifi-meas}). This moves away from prior work~\cite{arun2022p2slam} which required bearings to be measured at the access point as well and removes the need to collaborate with WiFi access points (APs) in the environment.
Specifically, these bearing measurements, providing the direction of the WiFi AP's in the environment in the robot's local coordinate frame, can be estimated using the Channel State Information, CSI, measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi}. But there are important challenges which need to be overcome to ensure these bearing measurements are accurate and unambiguous to allow for real-time global drift corrections.  

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reason for inaccuracies in the bearing measurements for indoors is multipath~\cite{spotfi,ayyalasomayajula2020deep,ma2019wifi}. 
A WiFi signal is broadcasted, and multiple reflections of the signal (\textit{mulitpath}) along with the direct path, impinge at the receiver as shown in Figure~\ref{fig:wifi-meas}. Clearly, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are the cause for erroneous bearing estimates. The receiver measures complex-valued channel state information (CSI) describing the phase delay and attenuation between each transmitter-receiver pair.
Since each antenna is at a different location, different phases accumulate between antennas depending on the incoming angle. With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m} = \underbrace{\Big[H^{m}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/eval_ral/aoa-err-boxplot.pdf}
    \caption{Bearing errors are accumulated in steps of $10^\circ$ for the the square antenna array (\textit{Top}) and linear array (\textit{Bottom}).}
    \label{fig:aoa-array}
    \vspace{-0.1in}
\end{figure}

\noindent\textbf{Unambiguous Measurements:} However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{spotfi, arun2022p2slam} are vulnerable to aliasing - they can only measure bearings in a $180^\circ$ range(i.e. the top half plane in Figure~\ref{fig:wifi-meas}) at a time, as there is no distinction between signals coming from opposite sides of the array. Furthermore, as shown in Figure~\ref{fig:aoa-array}(bottom) these arrays have low resolution of signals travelling mostly parallel to the array. The datasets in $\mathrm{P^2}$SLAM utilize a linear array, but since we need to resolve this ambiguity in order to estimate the true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. 
This can be further seen from Figure~\ref{fig:aoa-array}(top) for the dataset we have collected with the square array -- \name's finds a good trade-off between resolution and aliasing, able to resolve angles from $-160^{\circ}$ to $160^{\circ}$.
This array allows us to calculate the channel model in Eq~\ref{eq:sensor_model1} as:
\begin{align}
    H^{m}_i (\theta_i, l_i) = a_i \times & \exp\left({\textstyle -\iota 2 \pi \frac{f}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right)  \notag\\ &  \times \exp \left({\textstyle -\iota 2\pi  \frac{f}{c} l_i}\right)
\end{align}
    
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{ma2019wifi}.

% \todo{connect the english in this paragraph to the channel model build in 2}

\noindent\textbf{Accurate and Real-time bearing measurements:} In order to identify the direct signal's path among the multiple reflected paths, past Wi-Fi systems\cite{ma2019wifi} have used algorithms that `super-resolve' the measured signal using information across the $N$ different frequency bins to measure the relative time offset between different signal paths. This allows identification of the direct path, as it must have traveled the least distance of all paths and thus arrives before the other reflections.

However, these super-resolution algorithms are very compute intensive because they have added another dimension to the search space of signals. 
So, in \name we employ a sliding-window PCA based algorithm to efficiently combine information across subcarriers to estimate the direct path without identifying all of the reflected paths present in the signal, which we refer to as PCAB (Principle Component Analysis based Bearing). This begs the question, how can we perform adequate bearing estimation despite mulitpath corruption? 

The wireless channel in Eq~\ref{eq:sensor_model1} can be extended to incorporate the $L \geq 1$ transmitters' channel response. $H_f$, an $m\times l$ sub-matrix of the channel values for a particular subcarrier frequency $f$, can be decomposed~\cite{fukushima} by singular value decomposition into
$$H_f=U\Sigma\Bar{V}.$$
The left eigenvectors, $U$, form an orthogonal basis for the signals measured at the receiver, and similarly, the rows of $\bar{V}$ form a basis for signals transmitted from the transmitter. 

We identify a property that the direct path signal has which the others do not: since the direct path has traveled in a straight line, the columns of the direct path channel $H_{0}$ will be very highly correlated over time instances and subcarrier frequencies. However, reflected paths in general are much more susceptible to small changes in transmitter position and frequency, as real-world reflections can take many continuous reflected paths and create complex constructive and destructive interference. Thus, we expect that the strongest principle component of $H$, $U_0$ should correspond to the direct path signal and the multipath can be effectively averaged out.

Specifically, in PCAB, our goal is to get the best estimate of the responses at the receivers ($U_0$). Hence, we treat the channels response for each subcarrier-transmitter pair independently to create a stacked channel matrix at time $i$ as $H_i \in \mathbb{C}^{N \times ML}$, and compute the autocorrelation matrix $H_i\bar{H_i}$. Furthermore, we combine the most recent $T$ matrices across a period of 0.5 seconds and compute $U_0$ as:

% and  instead of working with each receiver-subcarrier pair independently to super-resolve the measured signal, we treat each transmitter-subcarrier pair as a separate transmitter. Thus we can combine the auto-correlation matrices across the $p$ most recent packets and $t$ transmitters to get a very good estimate of $U_0$
$$
U_0 = \boldsymbol{\lambda_0}(\sum_{i= t-T}^t H_{i}\Bar{H}_{i}),
$$
Where $\boldsymbol{\lambda_0}(\cdot)$ denotes the largest eigenvector, which is trivial to compute for our $N \times  N$ autocorrelation matrix. From here, our direct path signal $U_0$ can be mapped to a bearing by a coarse search over the space of possible bearings. This method allows us to achieve similar bearing estimation performance to the standard 2D-FFT algorithm~\cite{arun2022p2slam} at just a fraction of the compute, as PCAB only has to perform a one-dimensional search across possible bearings instead of a 2-dimensional search across bearings and distances.


\noindent\textbf{RSSI Filtering:} One assumption made in the PCAB algorithm is that the direct path is present in the measured channel in the first place. In cases where a large reflector blocks the direct path, no information can be obtained about the direct path's bearing. These non-line-of-sight (NLOS) scenarios are common and need to be handled adequately to avoid instability of the backend optimizer. We observe that in these situations, overall received signal power (RSSI) is typically very low, as the majority of the signal has been blocked. To avoid this, we reject all measurements with RSSI below $-65$dBm, which we empirically observe filters out the vast majority of these obstructed packets. Thus, \name provides real-time, unambiguous and accurate bearing measurements to be fed into the WiFi factor graph, described in ~\cref{sec:design-graph1}.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
    \vspace{-1em}
\end{figure}

% \subsection{Dual Graph Integration}\label{sec:design-camera}
% Thus we have seen on how the WiFi graph optimizes for accurate and real-time 3-DoF robot poses without requiring any loop-closures when provided with the odometry measurements.
% These Odometry can simply come from a wheel encoder and gyroscope of the wheeled robot but it will not have any visual context to be able to provide any human-readable maps.
% In contrast, in \name-SLAM's design, we utilize a dual graph approach, wherein we utilize existing VIO/LIO SLAM systems without their loop closure detection and corrections enabled.
% So, while these VIO/LIO systems can correct for local drifts in the wheel encoders or the IMUs, they cannot perform global corrections.
% These locally corrected robots 3-DoF poses are used to provide the Odometry measurements for the WiFi-graph that we have built in ~\cref{sec:design-graph1}.

% The advantage with turning off the loop closure detection and corrections though is that the rate of memory of consumption and compute required is minimized.
% Thus, the `VIO/LIO graph` can map the environment while providing locally corrected odometry measurements to the `WiFi-graph`.
% The WiFi-graph thus then performs global corrections without the need of loop-closure detection thus enabling \name-SLAM to be an accurate, real-time robot navigation system that can minimizing the rate of memory consumption and the amount of compute.

\subsection{Building and Optimizing the WiFi-Graph}\label{sec:design-graph1}

With these WiFi-bearing measurements, the first idea would be to integrate them within the factor graph of an available Visual Factor graph~\cite{rosinol2021kimera}. Unfortunately, discovery and addition of new AP's and global drift corrections made to the graph introduce brief periods of instability (order of few seconds) to the robot's trajectory estimations. These instabilities can introduce large computation overheads as it may demand corrections to the tracked visual landmarks as well. To isolate these periods of instability, we propose a dual graph approach, where the drift-corrected poses from the WiFi graph can be utilized for globally consistent mapping. But unlike prior work~\cite{arun2022p2slam, ferris2007wifi}, we do not use end-end optimization and instead opt to use the incremental smoothing and mapping (iSAM)~\cite{gtsam} to provide real-time pose estimates, which demands a more accurate and realtime bearing estimation as described in Sec.~\ref{sec:design-bearing}. 

At a high level, the state space at time $t$, $S_t$, is a set of robot poses and access point locations over $t$ time steps in our graph, $S_t = \{\Vec{p}_i \; \forall i \in [1, t]\} \cup \{\Vec{x}_j \; \forall j \in [1, N]\}$, with the robot pose, $\Vec{p}_i \in SE(3)$ and the $N$ access points positions observed till time $t$, $x_i \in \mathbb{R}^3$. 
We can the define odometry measurements (from VIO/LIO or wheel encoders, as shown in Fig~\ref{fig:wifi-factor}) between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps as:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion.
Similarly, the bearing factors AP $j$ at robot position $x_i$ is $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$:
\begin{align}\label{eq:ping-pred}
    &\hat{z}^{bearing}_{ij}(p_i, x_j) = \mathrm{Local}(\mathrm{TransformTo}(x_j, p_i), p_i) \\
                                &= \mathrm{Local}([\cos(\phi)\cos(\theta), \cos(\phi)\sin(\theta), \sin(\phi)]^T, p_i) \nonumber
\end{align}
where, \textit{TransformTo}$(\cdot)$ transforms the coordinates of the AP $x_j$ to the coordinate system provided by the robot at $p_i$, in which the AP subtends an elevation angle of $\phi$ and an azimuth angle of $\theta$. \textit{Local}$(\cdot)$ projects this bearing measurement to the tangent plane defined by the current pose of the robot, $p_i$. 


So, once we have defined the measurement models we can estimate the optimized robot poses $S^{opt}_t$ for time instance $t$ by minimizing the total error between our predictions and actual measurements,
\begin{align}\label{eq:graph-optim-head}
    S^{opt}_t = \argmin_{S_t} & \sum_{i \leq t} \sum_{j \leq N}  \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and bearing measurements respectively. Further note that the bearing measured in Sec.~\ref{sec:design-bearing} measured $\theta$, the azimuth angle in the robot's local frame and we assume that the elevation, $\phi$, of the incoming signal is $0$, hence $z_{ij} = [\cos(\theta) \sin(\theta)]$. We can assume the elevation angle is $0$ despite AP's placed at differing heights as it doesn't affect the azimuth bearing estimation~\cite{arun2022p2slam}. 


\subsection{Initialization of Factors}\label{sec:design-init}
Next, we initialize each of the $t$ robot positions and $N$ AP positions for the optimizer. 
Similar to prioir works~\cite{arun2022p2slam}, the robot positions are initialized using the relative odometry measurements. These poses have accumulated drift over time which we seek to correct.
A naive initialization for the AP's would be to place them at the origin and allow the optimizer to place them appropriately in the environment. Unfortunately, the iSAM optimizer, given the limited number of measurements it has seen up until time $t$, can fail to converge with this naive initialization. 
% Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
% While one could naively initialize all known APs in the environment at the origin, some APs may not be receiving any signals at all as they are actually very far from the robot's origin, thus might be too far away when the optimizer is started.

% Since these faraway APs have no measurements attached to them, the cost associated with them is ill-defined and the optimization problem is unsolvable.
% Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this in-determinancy due to poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been study extensively in the past for localization.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's pose $p_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maximum among all current robot's poses $p_i \forall i \in [1,t]$, with the intuition that this is where the robot passed closest to the AP.
We can then initialize the $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation. This random perturbation is added to avoid in-determinancy with the optimizer. Finally, with the real-time, compute-efficient WiFi-bearing in hand, along with a reliable way to integrate these measurements with local odometry measurements, we can proceed with the graph optimization iteratively with each time-step. In the following section we will provide specific implementation details and robustly test \name over a variety of environments. 


% Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
% Given good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.



==> ViWiD SLAM_arx/design/design7.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

% \todo{provide some more info on factor graphs here}
% \todo{add some background of p2slam and how this work differs}
\name seeks to deploy a SLAM system which can be compute and memory efficient. However, most current visual-based SLAM systems rely on resource-intensive loop closures to correct for inevitable drifts in robot's trajectory predictions and ensure consistency. Fortunately, a solution to circumvent these loop closure operations exists -- deploy \textit{identifiable} and \textit{mappable} landmarks in the environment to anchor the robot to it's environment and help it provide accurate trajectory estimates. But most of the current visual markers fail in dynamic environments or are tedious to deploy. To improve the robustness of these unique landmarks and hence guarantee a consistent trajectory, \name leverages WiFi access points in the environments as the much-needed landmarks. WiFi access points are uniquely identifiable from the hardware MAC address and can be mapped in the environment as shown by recent work~\cite{arun2022p2slam}, thus meeting the two criteria for a landmark. Moreover, unlike aforementioned visual landmarks, WiFi is ubiquitously deployed in indoor environments, and it is unaffected by visual occlusions or dynamic environments.

However, we are presented with three important challenges. \textit{First}, for the access point to be `mapped' into the environment, we require consistent and error-free WiFi measurements from the WiFi signals received at the robot from these access points (\cref{sec:design-bearing}). \textit{Second}, these WiFi measurements need to be appropriately optimized with visual and odometry sensors to provide a globally consistent trajectory (\cref{sec:design-graph1}). And \textit{third}, the optimizer needs to be well initialized to ensure timely convergence so that a real-time trajectory may be furnished (\cref{sec:design-init}). In the following sections we will seek to surmount these challenges to deliver \name, an accurate and resource efficient SLAM system. 

% A robot, mounted with WiFi and camera (or Lidar) sensors, navigates in the environment. Through local feature matching (or scan matching) and the inertial measurements from IMU (or wheel encoder), the SLAM algorithm provides accurate local pose measurements for the robot in real time. These pose updates from the local-odometry are fed into the WiFi-graph (described in ~\cref{sec:design-graph1}) which incorporates the bearing of the incoming WiFi signal (described in ~\cref{sec:design-bearing}) to track a deployed WiFi access point (AP) in an environment. In effect, the AP is treated as a stationary and unique landmark. Furthermore, since the incoming WiFi signal identifies the access point it originated from, this design removes the need for compute and memory heavy correlation (`loop-closure') operations. Finally, it is imperative to initialize our access points optimally to ensure stability of the convergence (described in~\cref{sec:design-init}). 

% We first formulate and describe this drift-free pose generation in ~\cref{sec:design-graph1} assuming we have the local-odometry from VIO/LIO.
% We first detail on how to get accurate WiFi measurements for the WiFi graph's real-time optimization in ~\cref{sec:design-bearing}. 

\subsection{Providing accurate and real-time WiFi measurements}\label{sec:design-bearing}

Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearings are a viable WiFi-based measurement for indoor localization and tracking.
Inspired from these works, we use the bearing measured from the incoming signals at the robot as our WiFi measurements (as shown by the solid line in Figure~\ref{fig:wifi-meas}) to help the robot `map' the access points in the environment. 
Specifically, these bearing measurements at the robot provide the direction of the WiFi AP's in the robot's local frame along the azimuth plane. In fact, this is similar pixel coordinates of a corner feature in an image frame which provide its bearing in both azimuth and elevation. 

These WiFi-bearings can be estimated using the Channel State Information, CSI, measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi}. However there are \textit{three} challenges which need to be surmounted for accurate bearing estimates, \textbf{(a)} multiple reflected copies of the same WiFi signal arrive at the robot and corrupt the bearing measurements; \textbf{(b)} concrete walls or metal reflectors can block the direct path signals and create inconsistent bearing estimates; \textbf{(c)} linear antenna array geometries commonly deployed in \cite{arun2022p2slam, spotfi} can reduce the diversity of bearings which can be measured definitively and in turn reduce the number of measurements which can be incorporated into the system. Let's tackle the first challenge by modelling the WiFi channel in the environment. 

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows WiFi bearings ($\theta$) measured using a linear antenna array with antenna separation $d$. The additional distance $d\sin(\theta)$ travelled by the signals can be exploited to estimate the bearing}
    \label{fig:wifi-meas}
    % \vspace{-0.1in}
\end{figure}

\noindent\textbf{Accurate and Real-time bearing measurements:} The primary reason for inaccuracies in the bearing measurements for indoors is multipath~\cite{spotfi,ayyalasomayajula2020deep,ma2019wifi}. 
A WiFi signal, with wavelength $\lambda$, is broadcast, and multiple reflections of the signal (\textit{multipath}) along with the direct path, impinge at the receiver as shown in Figure~\ref{fig:wifi-meas} (left). Clearly, the `direct-path' (solid-line) is the only path helpful in estimating the bearing ($\theta$) to the source and the rest of the `reflected-paths' (dotted lines) are the cause for erroneous bearing estimates. 

% \todo{Eq 1 is not needed?}
To understand these effects, we provide a simple mathematical model. The receiver measures, at time $t$, a complex-valued channel state information (CSI) describing the phase delay and attenuation across each of the $M$ receiver antennas and $N$ orthogonal frequencies~\cite{spotfi} as,
\begin{align}
    X^{m, n}_t &=  a_{m, n} e^{j \phi_m (\theta)} e^{-j (2\pi f_n \tau + \psi)}; \quad X_t \in \mathbb{C}^{M \times N} \nonumber \\ 
    \phi_m(\theta) &= -\frac{2\pi}{\lambda} m d \sin(\theta) \label{eq:angle-phases}
\end{align}
where, $a_{m, n}$ is the attenuation; $d$ is the antenna separation for the linear antenna array; $f_n$ is the orthogonal frequency; $\tau$ is the time-of-travel of the signal, which is often corrupted by the random $\psi$ phase offset due to lack of transmitter-receiver clock synchronization; and $\phi_m (\theta)$ is the additional phase accumulated at the $m^\mathrm{th}$ antenna (Figure~\ref{fig:wifi-meas}) due to the additional distance travelled by the signal. 
% Hence, we measure a CSI matrix at time $t$ as $X_t \in \mathbb{C}^{M \times N}$. 
The various reflected paths impinging on this linear array will add to each antenna and frequency component in a similar manner. 

To identify the direct signal's path among the multiple reflected paths, past Wi-Fi systems\cite{ma2019wifi} have used algorithms that `super-resolve' the measured signal. By using information across these $N$ different frequency bins, they measure the relative time offset between different signal paths. This allows identification of the direct path, as it must have traveled the least distance of all paths and thus arrives before the other reflections. However, the addition of this extra dimension of time-offset adds computation overhead, making them unsuitable for resource-efficient SLAM algorithms. 
%, as the space of signals to be searched over increases from $[0,2\pi)$ to $[0,2\pi)\times[-T,T]$, where $T$ is the space of possible time delays. 


% With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ receive antenna and $n^\mathrm{th}$, assuming $K$ multipath components as 
% \begin{align}\label{eq:sensor_model1}
%     H^{m, n} = \underbrace{\Big[H^{m}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
% \end{align}

So, in \name, we reduce the dimensionality of our problem and yet reliably segregate the direct path signals from the clutter of the reflected paths. Specifically, from the channel model described in Spotfi~\cite{spotfi}, the largest eigenvector ($U_t \in \mathbb{C}^{M}$) of $X_tX_t^H \in \mathbb{C}^{M \times M}$ provides the largest contribution to the channel measured across the $M$ receive antennas. However, this largest component could potentially be corrupted by multipath. To remove the effect of multipath, we make a simple observation -- reflected paths are susceptible to small changes in the robot's position as opposed to the direct path which will arrive at a consistent bearing. Hence we can effectively `average-out' the effects of multipath from our bearing estimation if we can combine our measurements across time (over multiple packets). We can effectively do this by finding the largest eigenvector over most recent $T$ measurements across the past $.5$ seconds:
$$
U_t = \boldsymbol{\lambda}(\sum_{i= t-T}^t X_{i}{X}_{i}^H),
$$
Where $\boldsymbol{\lambda}(\cdot)$ extracts the largest eigenvector, which is trivial to compute for our $M \times  M$ autocorrelation matrix. From here, our direct path signal $U_t$ can be mapped to a bearing by a coarse search over the space of possible bearings,  
\begin{align}
    \theta^* = \argmax_{\theta \in [-90^\circ, 90^\circ]} \sum_{i=1}^M \phi_m(\theta) U_t(m) \label{eq:bearing-search}
\end{align}
This method, dubbed Principle Component Analysis based Bearing (PCAB), allows us to achieve similar bearing estimation performance to the standard 2D-FFT algorithm~\cite{arun2022p2slam} and Spotfi~\cite{spotfi} at just a fraction of the compute. 

% \todo{cite that the rssi is not env dependent, but hardware dependent}
\noindent\textbf{RSSI Filtering:} But we have made an implicit assumption in PCAB that a direct path signal from an access point is present. However, in cases where a large reflector blocks the direct path, no information can be obtained about the direct path's bearing, and hence can lead to inconsistent bearing measurements. These non-line-of-sight (NLOS) scenarios are common and need to be handled adequately to avoid instability of the factor graph. We observe that in these situations, overall received signal power (RSSI) is typically very low, as the majority of the signal has been blocked. Hence, we reject all measurements with RSSI below $-65$dBm, which we empirically observe filters out the vast majority of these obstructed packets. Thus, \name provides real-time, unambiguous and accurate bearing measurements to be fed into the WiFi factor graph, described in ~\cref{sec:design-graph1}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/eval_ral/aoa-err-boxplot.pdf}
    \caption{Bearing errors are accumulated in steps of $10^\circ$ for the the square antenna array (\textit{Top}) and linear array (\textit{Bottom}).}
    \label{fig:aoa-array}
    % \vspace{-0.1in}
\end{figure}

\noindent\textbf{Unambiguous Measurements:} Finally, to enable reliable `mapping' of our WiFi landmarks, we would like to measure bearings from the largest range of angles. Unfortunately, the uniform linear arrays used by existing bearing estimation algorithms~\cite{spotfi, arun2022p2slam} are vulnerable to aliasing - they can only measure bearings in a $180^\circ$ range(i.e. the top half plane in Figure~\ref{fig:wifi-meas}) at a time, as there is no distinction between signals coming from opposite sides of the array. This is further seen in the search space of bearing angles as in Eq~\ref{eq:bearing-search}. Furthermore, as shown in Figure~\ref{fig:aoa-array}(bottom), these arrays have poorer accuracy when WiFi signals arrive nearly parallel to the array (near $\pm 90$). To maximize the range of measured angles, we resolve this ambiguity by adopting a square antenna array, which does not suffer from aliasing. 
This can be further seen from Figure~\ref{fig:aoa-array}(top) -- \name finds a good trade-off between resolution and aliasing, and is able to resolve angles from $-160^{\circ}$ to $160^{\circ}$. Note however we cannot extend the range to the entire $360^\circ$ due to ambiguity present for WiFi signals arriving from behind the robot. 
Transitioning to a square array however changes the differential phases measured (Eq~\ref{eq:angle-phases}) as, 
\begin{align}
    \phi_m(\theta) = -\frac{2\pi}{\lambda} (X_m \cos(\theta) + Y_m \sin(\theta)),
\end{align}
the relative position of antenna $m$ is $(X_m, Y_m)$ with respect to the first antenna.
% \begin{align}
%     H^{m}_i (\theta_i, l_i) = a_i \times & \exp\left({\textstyle -\iota 2 \pi \frac{f}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right)  \notag\\ &  \times \exp \left({\textstyle -\iota 2\pi  \frac{f}{c} l_i}\right)
% \end{align}
    
Finally note that these CSI measurements need to be sanitized beforehand the of random phase offsets ($\psi$) and a one-time calibration needs to be applied as further explained in Spotfi~\cite{spotfi}. Hence, by averaging-out multipath over multiple consecutive packets, rejecting NLOS measurements via RSSI filtering and incorporating a square antenna array at the robot, we have effectively furnished low-compute and accurate bearings over a $320^\circ$ range of angles to reliably `map' our WiFi landmarks. Next, we tackle how to incorporate these WiFi measurements into our optimizing backend to correct for trajectory drift.   


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
    % \vspace{-1ems}
\end{figure}

% \subsection{Dual Graph Integration}\label{sec:design-camera}
% Thus we have seen on how the WiFi graph optimizes for accurate and real-time 3-DoF robot poses without requiring any loop-closures when provided with the odometry measurements.
% These Odometry can simply come from a wheel encoder and gyroscope of the wheeled robot but it will not have any visual context to be able to provide any human-readable maps.
% In contrast, in \name-SLAM's design, we utilize a dual graph approach, wherein we utilize existing VIO/LIO SLAM systems without their loop closure detection and corrections enabled.
% So, while these VIO/LIO systems can correct for local drifts in the wheel encoders or the IMUs, they cannot perform global corrections.
% These locally corrected robots 3-DoF poses are used to provide the Odometry measurements for the WiFi-graph that we have built in ~\cref{sec:design-graph1}.

% The advantage with turning off the loop closure detection and corrections though is that the rate of memory of consumption and compute required is minimized.
% Thus, the `VIO/LIO graph` can map the environment while providing locally corrected odometry measurements to the `WiFi-graph`.
% The WiFi-graph thus then performs global corrections without the need of loop-closure detection thus enabling \name-SLAM to be an accurate, real-time robot navigation system that can minimizing the rate of memory consumption and the amount of compute.

\subsection{Building and Optimizing the WiFi-Graph}\label{sec:design-graph1}

% \todo{provide overview here and intuition}

% \todo{explain what poses are?}

Given these WiFi-bearing measurements, the first idea would be to integrate them within the factor graph of an available Visual Factor graph~\cite{rosinol2021kimera}. Unfortunately, discovery and addition of new AP's and global drift corrections introduce brief periods of instability (order of few seconds) to the robot's trajectory estimates. These instabilities can introduce large computation overheads as it may demand corrections to the tracked visual landmarks as well. To isolate these periods of instability, we propose a dual graph approach, where the drift-corrected poses from the WiFi graph can be utilized for globally consistent mapping. But unlike prior work~\cite{arun2022p2slam, ferris2007wifi}, we do not use end-end optimization and instead opt to use incremental smoothing and mapping (iSAM~\cite{gtsam}) to provide real-time pose estimates, which demands a more accurate and realtime bearing estimation as achieved in Sec.~\ref{sec:design-bearing}. 

To build the WiFi graph, consider the state space at time $t$, $S_t$. It is a set of robot poses and access point locations over $t$ time steps in our graph, $S_t = \{\Vec{p}_i \; \forall i \in [1, t]\} \cup \{\Vec{x}_j \; \forall j \in [1, N]\}$, with the robot pose, $\Vec{p}_i \in SE(3)$ and the $N$ access points positions observed till time $t$, $x_i \in \mathbb{R}^3$. 
We can the define odometry measurements (from VIO/LIO or wheel encoders, as shown in Fig~\ref{fig:wifi-factor}) between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps as:
\begin{align*}
    \hat{z}_i^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion.
Similarly, the bearing factors from  AP $j$ at robot position $x_i$ is $\hat{z}^{Bearing}_{ij}(p_i, x_j) \in \mathbb{R}^2$:
\begin{align}\label{eq:ping-pred}
    &\hat{z}^{Bearing}_{ij}(p_i, x_j) = \mathrm{Local}(\mathrm{TransformTo}(x_j, p_i), p_i) \\
                                &= \mathrm{Local}([\cos(\phi)\cos(\theta), \cos(\phi)\sin(\theta), \sin(\phi)]^T, p_i) \nonumber
\end{align}
where, \textit{TransformTo}$(\cdot)$ transforms the coordinates of the AP $x_j$ to the coordinate system provided by the robot at $p_i$, in which the AP subtends an elevation angle of $\phi$ and an azimuth angle of $\theta$. \textit{Local}$(\cdot)$ projects this bearing measurement to the tangent plane defined by the current pose of the robot, $p_i$. 


Having defined the measurement models, we can estimate the optimized robot poses $S^{opt}_t$ for time $t$ by minimizing the total error between our predictions and actual measurements,
\begin{align}\label{eq:graph-optim-head}
    S^{opt}_t = \argmin_{S_t} & \sum_{i \leq t} \sum_{j \leq N}  \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{Bearing}_{ij} - \hat{z}^{Bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$; $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error; $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and bearing measurements respectively. Further note that the bearing measured in Sec.~\ref{sec:design-bearing} measured $\theta$, the azimuth angle in the robot's local frame and we assume that the elevation, $\phi$, of the incoming signal is $0$, hence $z^{Bearing}_{ij} = [\cos(\theta) \sin(\theta)]$. We can assume the elevation angle is $0$ despite AP's placed at differing heights as it has little affect to the azimuth bearing estimation~\cite{arun2022p2slam}. 


\subsection{Initialization of Factors}\label{sec:design-init}
% \todo{this is difficult since we do not have complete observability of the AP's in one time step unlike usual fiducials}
Next, we initialize each of the $t$ robot positions and $N$ AP positions for the optimizer. 
Similar to prior works~\cite{arun2022p2slam}, the robot positions are initialized using the relative odometry measurements. These poses have accumulated drift over time which we seek to correct.
A naive initialization for the AP's would be to place them at the origin and allow the optimizer to place them appropriately in the environment~\cite{arun2022p2slam}. Unfortunately, the iSAM optimizer, given the limited number of measurements it has seen until time $t$, can fail to converge with this naive initialization. 
% Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
% While one could naively initialize all known APs in the environment at the origin, some APs may not be receiving any signals at all as they are actually very far from the robot's origin, thus might be too far away when the optimizer is started.

% Since these faraway APs have no measurements attached to them, the cost associated with them is ill-defined and the optimization problem is unsolvable.
% Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this in-determinancy due to poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been studied extensively in the past for localization.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's position $p^T_{ap-j} \in \mathbb{R}^3$ at which the $j^{th}$ AP's RSSI measurement has an maxima inflection point among all current robot's poses $p_i \forall i \in [1,t]$, with the intuition that this is where the robot passed closest to the AP.
We can then initialize the $j^{th}$ AP's pose $x_j$ as $x_j = p^T_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation. This random perturbation is added to avoid in-determinancy with the optimizer. Finally, with the real-time, compute-efficient WiFi-bearing in hand, along with a reliable way to integrate these measurements with local odometry measurements, we can proceed with the graph optimization iteratively with each time-step. In the following section we will provide specific implementation details.


% Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
% Given good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.




==> ViWiD SLAM_arx/discussion.tex <==
% !TEX root = root.tex
\section{Limitations and Future Work}\label{sec:conclusion}

% In this work, we have demonstrated a compute and memory efficient SLAM system using a dual-layered approach. We have ensured abstraction of the two layers is enforced and the smart buffer in between the two layers provide for a control mechanism, on how the data is transferred between each of these layer. With this we have shown low-memory and compute SLAM algorithm that also achieves state-of-the-art pose estimation and mapping accuracies and with \name-SLAM we have enabled a lot of new problems and future works that are enables:

% \todo{there are technically no limitations here}

In this work, we have demonstrated \name and its modular design can integrate into any existing VIO/LIO systems, to remove the need of compute and memory intensive loop-closures. Thus, \name provides a framework that can enable accurate, real-time, and resource-efficient SLAM compared to Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} for indoor robotics. However, there are still some limitations of \name's novel framework that opens new avenues for future work:

\noindent\textbf{(a)} While \name demonstrates loop-closure free SLAM through WiFi, any RF-sensor that can measure bearings to unique landmarks in the environment would work. In particular, UWB localization systems~\cite{zhao2021uloc} can be easily deployed in our framework to furnish 6 DoF poses.

\noindent\textbf{(b)} We have seen how different antenna array geometry on the robot provides varied results, extending the work to perform single-antenna based WiFi-SAR algorithms as demonstrated in WSR~\cite{jadhav2020wsr} would make the system more scalable.

\noindent\textbf{(c)} While \name demonstrates efficient SLAM for a single robot in the environment, extensions to collaborative SLAM for a fleet of robots presents additional challenges, making compute and memory efficiency even more important.


==> ViWiD SLAM_arx/evaluation/eval1.tex <==
% !TEX root = root.tex
\section{Results}\label{sec:eval}

Description of the environment. Ground truth data, how it is collected. How is it different from the cartogrpaher real-time and refer to DLoc as one of the examples that also show the same.

Then we show LiDAR and camera baselines with their real-time performances using Cartographer real-time and RTABMap real-time.

\subsection{Pose Estaimtion Accuracy}
We show CDF's of localization accuracy and orientaion accuracy for all of the baselines with \name.

We then show timeseries comparison with cartogrpaher, rtabmpa with \name alone for a couple of environments. highlighting how \name is close to camer and liddar alone.

\subsection{Compute, Latency and Memory}

Accuracy, compute required, latency required, memory required comparison table for all the three.

\subsection{Ablation}

\noindent\textbf{SVD-FFT vs FFT}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/svd_cdf_1.png}
    \caption{(a) Shows the various measurements that are made across various robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}
Individual CSI measurements are vulnerable to noise and transient multipath in the environment. As described above, we extract the underlying signal parameters from multiple CSI measurements across different transmitter antennas using Principle Component Analysis. We evaluate these new smoothed CSI measurement's performance with 2D-FFT.

\noindent\textbf{Square Vs ULA}

\section{Showcase: Autonomous Navigation}\label{sec:showcase}
Using fiduciary markers for labelling various locations in the map. These labels are then used to send commands for the robot to go around from point to point using \name's SLAM implementation.

==> ViWiD SLAM_arx/evaluation/eval2.tex <==
% !TEX root = root.tex
\section{Results}\label{sec:eval}

To evaluate \name implemented as mentioned in ~\cref{sec:implementation} we deployed \name's algorithms in one of the environments of the OpenSourced Datasest~\cite{arun2022p2slam} (which will be referred as Env-1). However $\mathrm{P^2}$SLAM dataset uses uniform linear arrays and assume the knowledge of the half-plane the AoA is measured.
Thus to overcome these limitations of their datasets, we collect one more Dataset in a $25m\times40m$ space (which we will be referred Env-2) with the square array we propose in \name's design that removes the half-plane ambiguities.
Additionally, the authors in $\mathrm{P^2}$SLAM use both AoA and AoD measurements of the robot, while in \name we only utilize only AoA and extract only those measurements from the dataset.

Additionally, we benchmark \name's results with two state-of-the-art SLAM systems: RTABMap~\cite{Labb2018RTABMapAA}, a RGB-D camera based SLAM algorithm and Cartographer~\cite{cartographer}, a LiDAR based SLAM algorithm. 
Here we would like to note that while a typical RGB-D and LIDAR sensors have a more denser feature map compared to a monocular camera we use in \name's implementation, the key-features/landmarks that are used for correlation matching are of the same order across monocular, RGB-D and LiDAR sensors.
We test \name's claims of compute and memory efficiency along with \name's SLAM performance.

\subsection{Evaluation Metrics}\label{sec:eval-metrics}

To measure the compute and memory usage we use the widely used open toolbox~\cite{toolbox} which reports \todo{whatever that is.}

\noindent\textbf{Memory Usage:} We use the memory (RAM in MB) usage of the SLAM algorithm as time progresses as the metric to compare \name against state of the art. Where we observe that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.

\noindent\textbf{Compute Usage:} We use the compute memory (MB) usage of the SLAM algorithm as time progresses as the metric to compare \name against state of the art. Where we observe that \name-SLAM reduces the average compute memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.

\noindent\textbf{Pose Estimation:} Since the system reports 4D pose ($(x,y,z,\theta)$) of the robot, which we compare with post-processing optimized cartographer poses as ground truth, as they have shown to have decent performance for indoor robots~\cite{diebel2006representing}. So, we use CDF of RMSE for $(x,y,z)$ and show a median tracking errors of \todo{xx}cm and L1 norm error for $(\theta)$, and a median robots orientation error of \todo{yy$^\circ$} on par with state of the art.

\noindent\textbf{Mapping Accuracy:} Finally, in the dataset we have collected we deploy \todo{xx} camera fiduciaries~\cite{fiducialtechused} across the environment, which are tracked and mapped in the environment by the camera graph.
Thus, the RMSE of the mapped locations of these fiduciaries help us to quantify the accuracy of \name's mapping capabilities.
Where we show that \name's is able to accurately map the environment with a median error of \todo{xx}cm.

\begin{figure*}[ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \caption{Robot Pose errors: (a) Shows the position estimation error of \name and RTABMap in Env-1 and Env-2. (b) Shows the orientation estimation error of \name and RTABMap in Env-1 and Env-2. (c,d) Show the time series tracking error of \name and cartographer and RTABMap in Env-1(c) and Env-2(d). (e,f) Show the time series orientation errors of \name and RTABMap in Env-1(e) and Env-2(f). and (g,h) Shows the top down view of the trajectory of \name compared with cartographer ground truth in Env-1(g) and Env-2(h).}
    \label{fig:tracking-errors}
\end{figure*}

\subsection{Compute and Memory Requirements}\label{sec:eval-compute}

\noindent\textbf{Memory \& Compute usage:}One of the most important contributions of \name's SLAM design is to achieve memory and compute efficient SLAM system without compromise the SLAM tasks. 
Thus we first evaluate the memory and compute usage of \name's overall system when deployed in both Env-1 and Env-2 and compare with two state-of-the-art SLAM systems RTABMap (that uses a RGB-D camera) and Cartographer (that uses a LiDAR).
We plot these memory usage in Figure~\ref{fig:memory-compute}{a} and compute usage in Figure~\ref{fig:memory-compute}{b} over time for each incoming sensor frame for all the three algorithms.
From these plots we can clearly see that \name's SLAM implementation on an average uses only \todo{$xx$} MB of compute memory which is \todo{$x\times$} (\todo{y$\times$}) lower than RTABMap (Cartographer). Additionally we can see that \name uses only \todo{$xx$} MB of memory (RAM) which is \todo{$x\times$} (\todo{y$\times$}) lower than RTABMap (Cartographer), thus demonstrating that \name is both memory and compute efficient by \todo{x$\times$} compared to the state-of-the-art camera and LiDAR based SLAM systems.

\noindent\textbf{Real-time performance of \name:} Additionally, we can also note from both Figure~\ref{fig:memory-compute}{a,b} that while \name's SLAM provides optimized poses and map in real-time and thus the plot ends at \todo{xx}secs when the data collection ends. On the other hand, RTABMap and Cartographer both take \todo{yyy}secs and \todo{zz}secs more to generate a better optimized paths and maps.
This further shows the deployability and scalability of \name due to its real-time performance compared to the existing SLAM systems that take additional time to perform end-to-end bundle adjustments~\cite{semenova2022quantitative} to get more accurate poses and maps.

\noindent\textbf{Ablation for \name's Memory \& Compute usage:} \\
\noindent We further analyze and look into the memory and compute usage of the individual components of \name, that is the individual WiFi and camera grapsh that are running in parallel.
We can see \todo{cool observation here}.

We also, note that for all the time-series plots shown in Figures~\ref{fig:memory-compute} have a series of vertical solid lines which show the AP initialization event happening for each of the individual AP's in the environment as per our smart initialization algorithm discussed in ~\cref{sec:design-graph1}.
We can see that the spikes in the WiFi graph for memory and compute occur at these instances noting that the measurements associated to the specific are laid down at this instant, but even these spikes are much lower than the overall compute and memory requirements of RTABMap and Cartogrpaher.

\begin{figure}[t]
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Map generated by \name for Env-1, (b) Map generated by \name for Env-2, also has the ground truh fiduciaries in blue circles and the predicted locations in red crosses}
    \label{fig:mapping}
\end{figure}

\subsection{Tracking Accuracy}\label{sec:eval-tracking}

\begin{figure*}[ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/svd_cdf_1.png}
        \subcaption{}
    \end{minipage}
    \caption{(a) Real-time tracking errors for \name, cartographer and RTABMap in Env-1, and (b) Real-time tracking errors for \name, cartographer and RTABMap in Env-2 .(c) Tracking errors for pose estimates provided from the WiFi-layer Poses Vs Visual layer for \name's implementation. (d) Shows the comparison of AoA accuracies for FFT Vs SVD-FFT}
    \label{fig:microbencmarks}
\end{figure*}

Now that we have demonstrated memory and compute efficiency of \name, we demonstrate that we achieve these low-compute and low-memory requirements while achieving state-of-the-art accuracies for robot pose estimation first, we will then demonstrate mapping accuracy of \name in ~\cref{sec:eval-mapping}. 

As stated earlier, we benchmark our results with end-to-edn cartographer processed poses as ground truth, against which we compare both \name and RTABMap to show tracking in Figure~\ref{fig:tracking-errors}{a} and orientation errors in Figure~\ref{fig:tracking-errors}{b} across both Env-1 and Env-2.
We can see that name achieves a median tracking error of $xx$cm and a median orientation error of $x^{\circ}$ which is on par with the median tracking error, $xx$cm and orientation error,$x^{\circ}$ of RTABMap. Thus showing that the pose estimation of \name is on par with the state-of-the-art Visual SLAM systems.

Additionally, we also provide the time-series plots of tracking errors across Env-1 and Env-2 in Figures~\ref{fig:tracking-errors}{c,d} and orientation errors in in Figures~\ref{fig:tracking-errors}{e,f} for both \name and RTABMap  showing that \todo{important thing you noticed here, showing that you are on par and providing with a reason why you might be falling short if you are.}

Finally, we also plot the \name's estimated path against the Cartographer's ground truth for both the environments in Figure~\ref{fig:tracking-errors}{g,h} to qualitatively show \name's accurate pose estimation across time.

\subsection{Mapping Accuracy}\label{sec:eval-mapping}

Finally, we evaluate \name's ability to amp features in the environment accurately. While, most of the works only give a qualitative map~\cite{Labb2018RTABMapAA,rosinol2021kimera,mur2015orb,qin2018vins} which also we present in Figure~\ref{fig:mapping}{a,b} for both Env-1 and ENv-2 respectively.
We additionally, place camera fiduciaries in Env-2 dataset that we have collected to measure if the locations of these fiduciaries are mapped accurately in the environment.
These camera fiduciary ground truth are highlighted in Figure~\ref{fig:mapping}{b} as blue circles and \name's mapped location in red crosses.
We compare these locations to provide the mapping errors, which we find has a mean mapping error of ~\todo{xx}cm.
% \todo{the median mapping error for all the fiduciaries is mentioned in text here for Env-2 as Env-2 does not fiduciaries.}



\subsection{Micro-benchmarks}

We have seen that \name demonstrates compute and memory efficient SLAM when deployed in real-world scenarios as seen in the results above. We now present few micro-benchmarks of \name's design to further demonstrate \name's robustness.

\noindent\textbf{Real-time Vs Bundle Adjustment Tracking errors:}\\
Firstly, as we have seen from ~\cref{sec:eval-compute} that while \name performs real-time optimizations, RTABMap and Cartographer post data collection bundle adjustments seen from the more time taken in Figures~\ref{fig:memory-compute}, so in order to perform a fair comparison with \name we look at the real-time poses that are reported when the robot is actually at that location without the pose correction optimizing the past locations and show the time series errors of these pose estimates in Figure~\ref{fig:microbencmarks}{a,b} for tracking and orientation errors respectively.
We can clearly observe from these time-series errors that compared to RTABMap and cartographer \name provide much better instantaneous pose estimates that are at least \todo{$x\times$} less erroneous.

\noindent\textbf{Time taken for each optimization stage on an average:}\\
Secondly, to understand the real-time performance of \name and the existing SLAM systems, we measure the total time taken for each algorithm and divide them by the total sensor frames.
This provides for the average latency for each pose estimation of the algorithms, and we find that while \name achieves real-time performance with a latency of \todo{xx}msec for a frame rate of $xx$fps, RTABMap and cartographer fall behind with \todo{xx}msec (for \todo{y}fps) and \todo{xx}msec (for \todo{y}fps) respectively.

\noindent\textbf{Justifying \name's Dual Layered Approach:}\\
Furthermore, while we have shown the pose estimation results of \name's WiFi graph, the camera graph also performs local pose corrections to these pose estimates while mapping the features in the environment.
So as to develop an insight towards the poses to use, we show the tracking errors for robot locations estimated using \name's WiFi graph and camera graph in Figure~\ref{fig:microbencmarks}{c} from where we can see that owing to its global perspective the WiFi graph provides with much more accurate location estimates than the Camera graph.
This further supports \name's dual graph idea where our intuition stems from the fact that WiFi-SLAM is best for pose estimation and camera-SLAM for mapping the environment.

\noindent\textbf{SVD-FFT vs FFT:}\\
Individual CSI measurements are vulnerable to noise and transient multipath in the environment. As described above, we extract the underlying signal parameters from multiple CSI measurements across different transmitter antennas using Singular Value Decomposition. We evaluate these new SVD CSI measurement's performance with 2D-FFT and show their AoA estimation accuracies as shown in Figure~\ref{fig:microbencmarks}{d}, where we can see that SVD-FFT based AoA estimates reduce the 90$^{th}$ percentile error from \todo{$xx^{\circ}$} to \todo{$yy^{\circ}$}.
We specifically note the 90$^{th}$ percentile errors as these are the corner cases where multipath and NLOS based errors are more prevalent. 
Thus demonstrating the performance improvement from \name's SVD-FFT implementation.
% \todo{table is optional}
% \begin{table}[ht]
%     \centering
%         \begin{tabular}{|l|l|l|l|}
%         \hline
%                      & Overall & Pose Estimation & Mapping   \\\hline \hline
%         ViWiD        &         &                 &           \\\hline
%         RTABMap      &         &                 &         \\\hline
%         Cartographer &         &                 &         \\ \hline
%         \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}



==> ViWiD SLAM_arx/evaluation/eval3.tex <==
% !TEX root = root.tex
\section{Results}

\begin{figure*}[ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-rtab-memory.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-rtab-cpu.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-abl-mem.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-abl-cpu.pdf}
        \subcaption{}
    \end{minipage}
    \caption{Memory and Compute: (a) Shows the memory usage (in MB) of \name compared with RTABMap (b) Shows the compute usage (in\% of a single core) of \name compared with RTABMap (c) Shows the memory usage of \name's WiFi and Camera graph, and (d) Shows the compute usage of \name's camera and WiFi graphs}
    \label{fig:memory-compute}
\end{figure*}

\begin{figure*}[ht]
    \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-all-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-all-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-28-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-4-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-28-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-4-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/rviz-3d-plot.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fiducials-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\name's SLAM performance: (a) Shows the position estimation error of \name and RTABMap in Env-1 and Env-2. (b) Shows the orientation estimation error of \name and RTABMap in Env-1 and Env-2. (c,d) Show the time series tracking error of \name and RTABMap in Env-1(c) and Env-2(d). (e,f) Show the time series orientation errors of \name and RTABMap in Env-1(e) and Env-2(f). and (g) Map generated by \name for Env-2 shown along with 3D features mapped in white, the path in red and the APs mapped in green. (h) Map generated by \name for Env-3, also has the ground truth fiducials in blue circles and the predicted locations in red crosses}
    \label{fig:tracking-errors}
\end{figure*}

To evaluate \name implemented as mentioned in ~\cref{sec:implementation} we deployed \name's algorithms over three datasets. We have scenarios covering two different paths driven in a $25 \times 30$ m and a third dataset in which mapping performace of \name is evaluated. Over the three datasets, the robot is driven a cumulative distance of over $1000$ m.
We also note that the authors in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} use AoA measurements at both the bot and the access points, while in \name we only utilize only AoA and extract only those measurements from the dataset.

Additionally, we benchmark \name's results with a state-of-the-art SLAM algorithm, RTABMap~\cite{Labb2018RTABMapAA}, a RGB-D camera based SLAM algorithm.
Additionally, we use the expensive and compute heavy LiDAR based SLAM algorithm, Cartographer~\cite{cartographer}, to compare against for ground truth pose and mapping estaimtes. 
Here we would like to note that while a typical RGB-D and LIDAR sensors have a more denser feature map compared to a monocular camera we use in \name's implementation, the key-features/landmarks that are used for correlation matching are of the same order across monocular, RGB-D and LiDAR sensors.
We test \name's claims of compute and memory efficiency along with \name's SLAM performance.

\subsection{Evaluation Metrics}\label{sec:eval-metrics}

To measure the compute and memory usage we use the widely used open toolbox\footnote{\url{https://github.com/alspitz/cpu_monitor}} which reports the memory used in MB by each individual node running and the compute in percentage of utilization per unit core, so for an 8-core machine, the compute usage can go from 0-800\%.

\noindent\textbf{Memory Usage:} We use the memory (RAM in MB) usage of the SLAM algorithm as time progresses as the metric to compare \name against state of the art. Where we observe that \name-SLAM reduces the average memory utilization to $300$MB which is $3\times$ the Visual SLAM.

\noindent\textbf{Compute Usage:} We use the percentage of a single core used by the SLAM algorithm as time progresses as the metric to compare \name against state of the art. 
That is for an 8-core machine, the compute usage can range from 0\%-800\%
Where we observe that \name-SLAM reduces the average compute memory utilization to $20$\% which is $5\times$ the Visual SLAM.

\noindent\textbf{Pose Estimation:} Since the system reports 4D pose ($(x,y,z,\theta)$) of the robot, which we compare with post-processing optimized cartographer poses as ground truth, as they have shown to have decent performance for indoor robots~\cite{diebel2006representing}. So, we use CDF of RMSE for $(x,y,z)$ and show a median tracking errors of 50cm and L1 norm error for $(\theta)$, and a median robots orientation error of 2$^\circ$ on par with state of the art.

\noindent\textbf{Mapping Accuracy:} Finally, to evaluate mapping performance, we wanted to deploy fiducial markers and get the accuracy by comparing their mapped poses to the ground truth poses. Thus
to evaluate the mapping performance we collect one more Dataset in a $25m\times40m$ space (which we will refer as Env-3). In this dataset we have collected  ArUCo camera fiducials~\cite{garrido2014automatic} across the environment, which are tracked using the OpenCV toolbox available~\cite{opencvaruco} and mapped in the environment by the camera graph.
Thus, the RMSE of the mapped locations of these fiducials help us to quantify the accuracy of \name's mapping capabilities.
Where we show that \name's is able to accurately map the environment with a median error of 105cm.

\subsection{Compute and Memory Requirements}\label{sec:eval-compute}

\noindent\textbf{Memory \& Compute usage:} One of the most important contributions of \name's SLAM design is to achieve memory and compute efficient SLAM system without compromise the SLAM tasks. 
Thus we first evaluate the memory and compute usage of \name's overall system when deployed in both Env-1 and Env-2 and compare with a state-of-the-art SLAM system, RTABMap (that uses a RGB-D camera).
We plot these memory usage in Figure~\ref{fig:memory-compute}{a} and compute usage in Figure~\ref{fig:memory-compute}{b} over time for each incoming sensor frame for bot the algorithms.
From these plots we can clearly see that \name's SLAM implementation on an average uses only $300$ MB of memory which is $3\times$ lower than RTABMap. Additionally we can see that \name uses only $20$\% of compute which is $5\times$ lower than RTABMap, thus demonstrating that \name is both memory and compute efficient by 4$\times$ compared to the state-of-the-art camera SLAM systems.

% \noindent\textbf{Real-time performance of \name:} Additionally, we can also note from both Figure~\ref{fig:memory-compute}{a,b} that while \name's SLAM provides optimized poses and map in real-time and thus the plot ends at \todo{xx}secs when the data collection ends. On the other hand, RTABMap and Cartographer both take \todo{yyy}secs and \todo{zz}secs more to generate a better optimized paths and maps.
% This further shows the deployability and scalability of \name due to its real-time performance compared to the existing SLAM systems that take additional time to perform end-to-end bundle adjustments~\cite{semenova2022quantitative} to get more accurate poses and maps.

\noindent\textbf{Ablation for \name's Memory \& Compute usage:} \\
\noindent We further analyze and look into the memory and compute usage of the individual components of \name, that is the individual WiFi and camera graph that are running in parallel.
We can see most of the  memory and compute usage for \name's algorithm are due to the camera features that are tracked and the \name WiFi layer needs very little compute.

We also, note that for all the time-series plots shown in Figures~\ref{fig:memory-compute} have a series of vertical solid lines which show the AP initialization event happening for each of the individual AP's in the environment as per our smart initialization algorithm discussed in ~\cref{sec:design-graph1}.
We can see that the spikes in the WiFi graph for memory and compute occur at these instances noting that the measurements associated to the specific are laid down at this instant, but even these spikes are much lower than the overall compute and memory requirements of RTABMap.

\begin{figure*}[t]
    \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-top-down-8-28-crop.pdf}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/rtab-top-down-8-28-crop.pdf}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-top-down-8-4-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Shows the top down view of the trajectory of \name compared with cartographer ground truth in Env-1, (b) Shows the top down view of the trajectory of RTABMap compared with cartographer ground truth in Env-1 and (c)hows the top down view of the trajectory of \name compared with cartographer ground truth in Env-2 }
    \label{fig:mapping}
\end{figure*}

\subsection{Tracking Accuracy}\label{sec:eval-tracking}

\begin{figure}[ht]
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-wifi-cam_trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/fft-pca-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Tracking errors for pose estimates provided from the WiFi-layer Poses Vs Visual layer for \name's implementation. (b) Shows the comparison of AoA accuracies for FFT Vs SVD-FFT}
    \label{fig:microbencmarks}
\end{figure}

Now that we have demonstrated memory and compute efficiency of \name, we demonstrate that we achieve these low-compute and low-memory requirements while achieving state-of-the-art accuracies for robot pose estimation first, we will then demonstrate mapping accuracy of \name in ~\cref{sec:eval-mapping}. 

As stated earlier, we benchmark our results with end-to-edn cartographer processed poses as ground truth, against which we compare both \name and RTABMap to show tracking in Figure~\ref{fig:tracking-errors}{a} and orientation errors in Figure~\ref{fig:tracking-errors}{b} across both Env-1 and Env-2.
We can see that name achieves a median tracking error of $50$cm for both Env-1 and Env-2 and a median orientation error of $1^{\circ}$ and $2.8^{\circ}$ for both env-1 and env-2. These are on par with the median tracking errors of $60$cm and $38$cm and median orientation errors, $5^{\circ}$ and $3^{\circ}$ across Env-1 and Env-2 for RTABMap. Thus showing that the pose estimation of \name is on par with the state-of-the-art Visual SLAM systems.

Additionally, we also provide the time-series plots of tracking errors across Env-1 and Env-2 in Figures~\ref{fig:tracking-errors}{c,d} and orientation errors in in Figures~\ref{fig:tracking-errors}{e,f} for both \name and RTABMap  showing that \name performs on par in terms of pose estimations with the RTABMap. We can also see that the high errors in \name are only in the initial stages where it is searching for the APs in the environment and it stabilizes for later stages, showing the robustness of our system. On the other hand, loop-closure dependant SLAM algorithms need a location to be revisted to avoid any drifts.

Finally, we also plot the \name's estimated path against the Cartographer's ground truth for both the environments in Figure~\ref{fig:tracking-errors}{g,h} to qualitatively show \name's accurate pose estimation across time.

\subsection{Mapping Accuracy}\label{sec:eval-mapping}

Finally, we evaluate \name's ability to amp features in the environment accurately. While, most of the works only give a qualitative map~\cite{Labb2018RTABMapAA,rosinol2021kimera,mur2015orb,qin2018vins} which also we present in Figure~\ref{fig:tracking-errors}{g,h} for both Env-1 and Env-3 respectively.
We additionally, place camera fiducials in Env-3 dataset that we have collected to measure if the locations of these fiducials are mapped accurately in the environment.
These camera fiducial ground truth are highlighted in Figure~\ref{fig:tracking-errors}{h} as blue circles and \name's mapped location in red crosses.
We compare these locations to provide the mapping errors, which we find has a mean mapping error of 103cm.


\subsection{Micro-benchmarks}

We have seen that \name demonstrates compute and memory efficient SLAM when deployed in real-world scenarios as seen in the results above. We now present few micro-benchmarks of \name's design to further demonstrate \name's robustness.

% \noindent\textbf{Real-time Vs Bundle Adjustment Tracking errors:}\\
% Firstly, as we have seen from ~\cref{sec:eval-compute} that while \name performs real-time optimizations, RTABMap and Cartographer post data collection bundle adjustments seen from the more time taken in Figures~\ref{fig:memory-compute}, so in order to perform a fair comparison with \name we look at the real-time poses that are reported when the robot is actually at that location without the pose correction optimizing the past locations and show the time series errors of these pose estimates in Figure~\ref{fig:microbencmarks}{a,b} for tracking and orientation errors respectively.
% We can clearly observe from these time-series errors that compared to RTABMap and cartographer \name provide much better instantaneous pose estimates that are at least \todo{$x\times$} less erroneous.

% \noindent\textbf{Time taken for each optimization stage on an average:}\\
% Firstly, to understand the real-time performance of \name and the existing SLAM systems, we measure the total time taken for each algorithm and divide them by the total sensor frames.
% This provides for the average latency for each pose estimation of the algorithms, and we find that while \name achieves real-time performance with a latency of \todo{xx}msec for a frame rate of $xx$fps, RTABMap and cartographer fall behind with \todo{xx}msec (for \todo{y}fps) and \todo{xx}msec (for \todo{y}fps) respectively.

\noindent\textbf{Justifying \name's Dual Layered Approach:}\\
Firstly, while we have shown the pose estimation results of \name's WiFi graph, the camera graph also performs local pose corrections to these pose estimates while mapping the features in the environment.
So as to develop an insight towards the poses to use, we show the tracking errors for robot locations estimated using \name's WiFi graph and camera graph in Figure~\ref{fig:microbencmarks}{c} from where we can see that owing to its global perspective the WiFi graph provides with much more accurate location estimates than the Camera graph.
This further supports \name's dual graph idea where our intuition stems from the fact that WiFi-SLAM is best for pose estimation and camera-SLAM for mapping the environment.

\noindent\textbf{PC-FFT vs FFT:}\\
Additionally, the individual CSI measurements are vulnerable to noise and transient multipath in the environment. As described above, we extract the underlying signal parameters from multiple CSI measurements across different transmitter antennas using Singular Value Decomposition, to identify the principle component of CSI. We evaluate these new SVD CSI measurement's performance with 2D-FFT and show their AoA estimation accuracies as shown in Figure~\ref{fig:microbencmarks}{d}, where we can see that SVD-FFT based AoA estimates reduce the 90$^{th}$ percentile error from $40^{\circ}$ to $25^{\circ}$.
We specifically note the 90$^{th}$ percentile errors as these are the corner cases where multipath based errors are more prevalent. 
Thus demonstrating the performance improvement from \name's PC-FFT implementation.


==> ViWiD SLAM_arx/evaluation/eval4.tex <==
% !TEX root = root.tex
\section{Microbenchmarks}~\label{sec:eval-micro}

\subsection{VIO memory vs accuracy}
In this section we describe the details of Kimera~\cite{rosinol2021kimera}, a VIO SLAM system that we utilize as a benchmark comparison.
We also use Kimera as the first-graph 
-- William as of 7/26

\begin{itemize}
    \item Median translation error vs memory and median orientation error vs memory -- \textbf{with and without LCD}
    \item Loop Closure detection frequency vs memory rate 
    \item set a tolerable limit and use that memory requirement and accuracy requirement as a baseline
\end{itemize}

\subsection{Wheel Odom vs VIO without LCD Odom}

Comparison of just the wheel odometery and VIO without LCD odometry to ensure that we are using comparable systems

\subsection{FFT, PC-FFT, MUSIC}
\begin{itemize}
    \item accuracy
    \item compute
\end{itemize}

\begin{figure*}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem-interframetime.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation_no_lc.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/aoa_err.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\textbf{Microbenchmarks}: \textbf{(a) Kimera:} Shows the trade-off between memory consumption(red) and the accuracy(blue) for various interframe rates. \textbf{(b) Cartographer:} Shows the trade-off between compute required(red) and the accuracy(blue) for various scan-matching thresholds. \textbf{(c) Odometry-Graph:} Shows the comparison on how various odometry inputs to the WiFi graph look before optimization.\textbf{(d) Bearing Measurement Algorithms:} Comparison between 2D-FFT from $\mathrm{P^2}$SLAM, MUSIC and our proposed PC-FFT}
    \label{fig:micro}
    \vspace{-0.1in}
\end{figure*}

\section{Results}\label{sec:eval}

\begin{figure*}
    \begin{minipage}{0.20\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/top-down-kimera.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.20\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/top-down-viofi.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_translation.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_orientation.pdf}    
        \subcaption{}
    \end{minipage}
    
    \caption{\textbf{End-to-end evaluation}: \textbf{(a)} Trajectory estimated by Kimera with loop closures (Orange) and ground truth (dashed-Blue). \textbf{(b)} Trajectory estimated by \name using odometry predictions from Kimera without loop closures (Orange, \textit{WiFi + Kimera w/o LC}) and ground truth (dashed-Blue). \textbf{(c, d)} Time series of translation and orientation error comparing Kimera with loop closure (dashed-Orange) against \name's predictions. \name uses odomtery from Kimera without loop closures (Blue) and just wheel odometry (dashed-Yellow).}
    \label{fig:end-end1}
    \vspace{-0.1in}
\end{figure*}

\begin{figure}[t]
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_orientation.pdf}
    \end{minipage}
    \caption{\textbf{Error analysis:} }
    \label{fig:end-end2}
\end{figure}


\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.42\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem_cpu_w_aoa_ts.pdf}
    \end{minipage}
    \caption{Notes: memory avg slope, Kimera -- 0.56, \name -- 0.2 MB/s}
    \label{fig:mem-cpu}
\end{figure}

To evaluate \name implemented as mentioned in ~\cref{sec:implementation} we deployed \name's algorithms over four datasets. The one presented in the following section was collected in a $25 \times 20$ m environment, with a total distance of $403$ m traversed over a duration of $23$ minutes. The subsequent 3 datasets are the P2SLAM datasets~\cite{arun2022p2slam}. Through these datasets, we have robustly tested \name across 3 distinct environments, 4 different access point placements, and traversed a cumulative distance of $1625$ m with a total travel time of 108 minutes. We also note that the authors in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} use AoA measurements at both the robot and the access points, while in \name we only utilize the AoA at the robot and extract the channels for only those measurements from the dataset.

Additionally, we benchmark \name's results with a state-of-the-art SLAM algorithm, Kimera~\cite{kim2019control}, a stereo-camera based SLAM algorithm. We run Kimera on our dataset with and without loop closures, labelled in the legends as `w/ LC' and `w/o LC' respectively. Additionally, for all the 4 datasets, we run cartographer in real time, with the `global SLAM' and LiDAR scan matching turned off to remove turn off loop closure. This is referred to as `Cartographer w/o LC'. Next, we carefully tune the loop closure parameters to obtain the best quality of loop closures (referred as `Cartographer w/ LC') in real time and benchmark \name against it. To obtain ground truth, we observe that due to compute constraints Cartographer in unable to incorporate all the LiDAR scans in real time, but allowing it to run past the time of data collection allows it to optimize over all the LiDAR scans to provide a near-groundtruth trajectory. The performance of this trajectory was further characterized in DLoc~\cite{ayyalasomayajula2020deep}. 

In the following sections, using the Cartographer ground truth generated, we benchmark \name against Kimera and Cartographer (when run in real-time) and provide results for the translation and orientation errors. We further measure the CPU and memory usage across these SLAM frameworks\footnote{\url{https://github.com/alspitz/cpu_monitor}} and compare the total memory used, the rate of memory increase and the CPU resources used over the entire run of the datasets. 


\subsection{End-to-end evaluation:}

\begin{itemize}
    \item CDFs of translation and orientation errors for \name, Kimera with LCD, WiFi with wheel Odom (real-time)
    \item time-series for of translation and orientation errors for \name, Kimera with LCD, WiFi with wheel Odom (real-time)
    \item overall memory requirements for \name, Kimera, WiFi with wheel Odom
    \item time-series of memory requirement increase for \name, Kimera, WiFi with wheel Odom \todo{extrapolate the time series till 8GB}
\end{itemize}

\subsection{Memory and Accuracy with Various VIO inputs}

understanding how existing VIOs will effect our algorithm

\begin{table*}[ht]
    \centering
    \footnotesize
    \caption{}
    \begin{tabular}{|l|ccc|ccc|ccc|}
    \hline
    \multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{Cart. w/ LC}} & \multicolumn{3}{c|}{\textbf{\name + Cart. w/o LC}} & \multicolumn{3}{c|}{\textbf{\name + Odom}} \\ \cline{2-10} 
     & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \multicolumn{1}{l|}{\textbf{DS 3}} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}Translation \\ Error (cm)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0 \\ (224)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}134.1 \\ (1097)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}23.3\\ (37.4)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}65.9\\ (92.2)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}67.3\\ (182.6)\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}48.6 \\ (114.4)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0\\ (100.2)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}75.5\\ (204.9)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}66.44\\ (234.7)\end{tabular} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}Orientation \\ Error (deg)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{0.8}\\ (4.66)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}5.3\\ (12.6)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.6\\ (1.4)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2.4\\ (4.66)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{2.8}\\ (12)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}1.4\\ (3.3)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1.7\\ (\textbf{2.7})\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.0\\ (\textbf{6.2})\end{tabular}} & \begin{tabular}[c]{@{}c@{}}2.0 \\ (10.3)\end{tabular} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}Total \\ Memory (MB)\end{tabular}} & \multicolumn{1}{c|}{702} & \multicolumn{1}{c|}{658} & 423 & \multicolumn{1}{c|}{613} & \multicolumn{1}{c|}{706} & 356 & \multicolumn{1}{c|}{288} & \multicolumn{1}{c|}{\textbf{252}} & \textbf{163} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}Rate of \\ memory (MB/s)\end{tabular}} & \multicolumn{1}{c|}{0.29} & \multicolumn{1}{c|}{0.33} & 0.38 & \multicolumn{1}{c|}{0.22} & \multicolumn{1}{c|}{0.33} & 0.26 & \multicolumn{1}{c|}{\textbf{0.10}} & \multicolumn{1}{c|}{\textbf{0.11}} & \textbf{0.14} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}CPU (fraction \\ of cores)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.2\\ (4.2)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.8\\ (4.2)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}1.85\\ (4.4)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.62\\ (2.1)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.85\\ (2.8)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.77\\ (1.1)\end{tabular} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.2\\ (1.6)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.28 \\ (1.7)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.22 \\ (0.5)\end{tabular}} \\ \hline
    \end{tabular}
\end{table*}


\if 0
\begin{figure*}[ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-rtab-memory.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-rtab-cpu.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-abl-mem.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-abl-cpu.pdf}
        \subcaption{}
    \end{minipage}
    \caption{Memory and Compute: (a) Shows the memory usage (in MB) of \name compared with RTABMap (b) Shows the compute usage (in\% of a single core) of \name compared with RTABMap (c) Shows the memory usage of \name's WiFi and Camera graph, and (d) Shows the compute usage of \name's camera and WiFi graphs}
    \label{fig:memory-compute}
\end{figure*}

\begin{figure*}[ht]
    \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-all-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-all-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-28-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-4-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-28-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-4-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/rviz-3d-plot.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fiducials-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\name's SLAM performance: (a) Shows the position estimation error of \name and RTABMap in Env-1 and Env-2. (b) Shows the orientation estimation error of \name and RTABMap in Env-1 and Env-2. (c,d) Show the time series tracking error of \name and RTABMap in Env-1(c) and Env-2(d). (e,f) Show the time series orientation errors of \name and RTABMap in Env-1(e) and Env-2(f). and (g) Map generated by \name for Env-2 shown along with 3D features mapped in white, the path in red and the APs mapped in green. (h) Map generated by \name for Env-3, also has the ground truth fiducials in blue circles and the predicted locations in red crosses}
    \label{fig:tracking-errors}
\end{figure*}

\subsection{Evaluation Metrics}\label{sec:eval-metrics}

To measure the compute and memory usage we use the widely used open toolbox\footnote{\url{https://github.com/alspitz/cpu_monitor}} which reports the memory used in MB by each individual node running and the compute in percentage of utilization per unit core, so for an 8-core machine, the compute usage can go from 0-800\%.

\noindent\textbf{Memory Usage:} We use the memory (RAM in MB) usage of the SLAM algorithm as time progresses as the metric to compare \name against state of the art. Where we observe that \name-SLAM reduces the average memory utilization to $300$MB which is $3\times$ the Visual SLAM.

\noindent\textbf{Compute Usage:} We use the percentage of a single core used by the SLAM algorithm as time progresses as the metric to compare \name against state of the art. 
That is for an 8-core machine, the compute usage can range from 0\%-800\%
Where we observe that \name-SLAM reduces the average compute memory utilization to $20$\% which is $5\times$ the Visual SLAM.

\noindent\textbf{Pose Estimation:} Since the system reports 4D pose ($(x,y,z,\theta)$) of the robot, which we compare with post-processing optimized cartographer poses as ground truth, as they have shown to have decent performance for indoor robots~\cite{diebel2006representing}. So, we use CDF of RMSE for $(x,y,z)$ and show a median tracking errors of 50cm and L1 norm error for $(\theta)$, and a median robots orientation error of 2$^\circ$ on par with state of the art.

\noindent\textbf{Mapping Accuracy:} Finally, to evaluate mapping performance, we wanted to deploy fiducial markers and get the accuracy by comparing their mapped poses to the ground truth poses. Thus
to evaluate the mapping performance we collect one more Dataset in a $25m\times40m$ space (which we will refer as Env-3). In this dataset we have collected  ArUCo camera fiducials~\cite{garrido2014automatic} across the environment, which are tracked using the OpenCV toolbox available~\cite{opencvaruco} and mapped in the environment by the camera graph.
Thus, the RMSE of the mapped locations of these fiducials help us to quantify the accuracy of \name's mapping capabilities.
Where we show that \name's is able to accurately map the environment with a median error of 105cm.

\subsection{Compute and Memory Requirements}\label{sec:eval-compute}

\noindent\textbf{Memory \& Compute usage:} One of the most important contributions of \name's SLAM design is to achieve memory and compute efficient SLAM system without compromise the SLAM tasks. 
Thus we first evaluate the memory and compute usage of \name's overall system when deployed in both Env-1 and Env-2 and compare with a state-of-the-art SLAM system, RTABMap (that uses a RGB-D camera).
We plot these memory usage in Figure~\ref{fig:memory-compute}{a} and compute usage in Figure~\ref{fig:memory-compute}{b} over time for each incoming sensor frame for bot the algorithms.
From these plots we can clearly see that \name's SLAM implementation on an average uses only $300$ MB of memory which is $3\times$ lower than RTABMap. Additionally we can see that \name uses only $20$\% of compute which is $5\times$ lower than RTABMap, thus demonstrating that \name is both memory and compute efficient by 4$\times$ compared to the state-of-the-art camera SLAM systems.

% \noindent\textbf{Real-time performance of \name:} Additionally, we can also note from both Figure~\ref{fig:memory-compute}{a,b} that while \name's SLAM provides optimized poses and map in real-time and thus the plot ends at \todo{xx}secs when the data collection ends. On the other hand, RTABMap and Cartographer both take \todo{yyy}secs and \todo{zz}secs more to generate a better optimized paths and maps.
% This further shows the deployability and scalability of \name due to its real-time performance compared to the existing SLAM systems that take additional time to perform end-to-end bundle adjustments~\cite{semenova2022quantitative} to get more accurate poses and maps.

\noindent\textbf{Ablation for \name's Memory \& Compute usage:} \\
\noindent We further analyze and look into the memory and compute usage of the individual components of \name, that is the individual WiFi and camera graph that are running in parallel.
We can see most of the  memory and compute usage for \name's algorithm are due to the camera features that are tracked and the \name WiFi layer needs very little compute.

We also, note that for all the time-series plots shown in Figures~\ref{fig:memory-compute} have a series of vertical solid lines which show the AP initialization event happening for each of the individual AP's in the environment as per our smart initialization algorithm discussed in ~\cref{sec:design-graph1}.
We can see that the spikes in the WiFi graph for memory and compute occur at these instances noting that the measurements associated to the specific are laid down at this instant, but even these spikes are much lower than the overall compute and memory requirements of RTABMap.

\begin{figure*}[t]
    \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-top-down-8-28-crop.pdf}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/rtab-top-down-8-28-crop.pdf}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-top-down-8-4-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Shows the top down view of the trajectory of \name compared with cartographer ground truth in Env-1, (b) Shows the top down view of the trajectory of RTABMap compared with cartographer ground truth in Env-1 and (c)hows the top down view of the trajectory of \name compared with cartographer ground truth in Env-2 }
    \label{fig:mapping}
\end{figure*}

\subsection{Tracking Accuracy}\label{sec:eval-tracking}

\begin{figure}[ht]
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-wifi-cam_trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/fft-pca-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Tracking errors for pose estimates provided from the WiFi-layer Poses Vs Visual layer for \name's implementation. (b) Shows the comparison of AoA accuracies for FFT Vs SVD-FFT}
    \label{fig:microbencmarks}
\end{figure}

Now that we have demonstrated memory and compute efficiency of \name, we demonstrate that we achieve these low-compute and low-memory requirements while achieving state-of-the-art accuracies for robot pose estimation first, we will then demonstrate mapping accuracy of \name in ~\cref{sec:eval-mapping}. 

As stated earlier, we benchmark our results with end-to-edn cartographer processed poses as ground truth, against which we compare both \name and RTABMap to show tracking in Figure~\ref{fig:tracking-errors}{a} and orientation errors in Figure~\ref{fig:tracking-errors}{b} across both Env-1 and Env-2.
We can see that name achieves a median tracking error of $50$cm for both Env-1 and Env-2 and a median orientation error of $1^{\circ}$ and $2.8^{\circ}$ for both env-1 and env-2. These are on par with the median tracking errors of $60$cm and $38$cm and median orientation errors, $5^{\circ}$ and $3^{\circ}$ across Env-1 and Env-2 for RTABMap. Thus showing that the pose estimation of \name is on par with the state-of-the-art Visual SLAM systems.

Additionally, we also provide the time-series plots of tracking errors across Env-1 and Env-2 in Figures~\ref{fig:tracking-errors}{c,d} and orientation errors in in Figures~\ref{fig:tracking-errors}{e,f} for both \name and RTABMap  showing that \name performs on par in terms of pose estimations with the RTABMap. We can also see that the high errors in \name are only in the initial stages where it is searching for the APs in the environment and it stabilizes for later stages, showing the robustness of our system. On the other hand, loop-closure dependant SLAM algorithms need a location to be revisted to avoid any drifts.

Finally, we also plot the \name's estimated path against the Cartographer's ground truth for both the environments in Figure~\ref{fig:tracking-errors}{g,h} to qualitatively show \name's accurate pose estimation across time.

\subsection{Mapping Accuracy}\label{sec:eval-mapping}

Finally, we evaluate \name's ability to amp features in the environment accurately. While, most of the works only give a qualitative map~\cite{Labb2018RTABMapAA,rosinol2021kimera,mur2015orb,qin2018vins} which also we present in Figure~\ref{fig:tracking-errors}{g,h} for both Env-1 and Env-3 respectively.
We additionally, place camera fiducials in Env-3 dataset that we have collected to measure if the locations of these fiducials are mapped accurately in the environment.
These camera fiducial ground truth are highlighted in Figure~\ref{fig:tracking-errors}{h} as blue circles and \name's mapped location in red crosses.
We compare these locations to provide the mapping errors, which we find has a mean mapping error of 103cm.


\subsection{Micro-benchmarks}

We have seen that \name demonstrates compute and memory efficient SLAM when deployed in real-world scenarios as seen in the results above. We now present few micro-benchmarks of \name's design to further demonstrate \name's robustness.

\noindent\textbf{Justifying \name's Dual Layered Approach:}\\
Firstly, while we have shown the pose estimation results of \name's WiFi graph, the camera graph also performs local pose corrections to these pose estimates while mapping the features in the environment.
So as to develop an insight towards the poses to use, we show the tracking errors for robot locations estimated using \name's WiFi graph and camera graph in Figure~\ref{fig:microbencmarks}{c} from where we can see that owing to its global perspective the WiFi graph provides with much more accurate location estimates than the Camera graph.
This further supports \name's dual graph idea where our intuition stems from the fact that WiFi-SLAM is best for pose estimation and camera-SLAM for mapping the environment.

\noindent\textbf{PC-FFT vs FFT:}\\
Additionally, the individual CSI measurements are vulnerable to noise and transient multipath in the environment. As described above, we extract the underlying signal parameters from multiple CSI measurements across different transmitter antennas using Singular Value Decomposition, to identify the principle component of CSI. We evaluate these new SVD CSI measurement's performance with 2D-FFT and show their AoA estimation accuracies as shown in Figure~\ref{fig:microbencmarks}{d}, where we can see that SVD-FFT based AoA estimates reduce the 90$^{th}$ percentile error from $40^{\circ}$ to $25^{\circ}$.
We specifically note the 90$^{th}$ percentile errors as these are the corner cases where multipath based errors are more prevalent. 
Thus demonstrating the performance improvement from \name's PC-FFT implementation.

\fi


==> ViWiD SLAM_arx/evaluation/eval5.tex <==
% !TEX root = root.tex
\section{Microbenchmarks}\label{sec:eval-micro}

\begin{figure*}[t]
    \begin{minipage}{0.20\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/top-down-kimera.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.20\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/top-down-viofi.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_translation.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_orientation.pdf}    
        \subcaption{}
    \end{minipage}
    
    \caption{\textbf{End-to-end evaluation}: \textbf{(a)} Trajectory estimated by Kimera with loop closures (Orange) and ground truth (dashed-Blue). \textbf{(b)} Trajectory estimated by \name using odometry predictions from Kimera without loop closures (Orange, \textit{WiFi + Kimera w/o LC}) and ground truth (dashed-Blue). \textbf{(c, d)} Time series of translation and orientation error comparing Kimera with loop closure (dashed-Orange) against \name's predictions. \name uses odomtery from Kimera without loop closures (Blue) and just wheel odometry (dashed-Yellow).}
    \label{fig:end-end1}
    \vspace{-0.1in}
\end{figure*}


\name-SLAM uses Kimera (for VIO) and cartographer (for LIO) as both benchmarks and also the Odometry inputs for the WiFi-graph defined in ~\cref{sec:design-graph1}. We first analyze how the key parameters in Kimera and Cartographer in ~\cref{sec:micro-vio} and ~\cref{sec:micro-lio} respectively.

\subsection{VIO memory vs accuracy}\label{sec:micro-vio}
To first understand Kimera's performance with various parameters, we have found that the most memory demanding is the interframe time that determines how frequently does Kimera search for a keyframe for loop-closure. That is, lesser the interframe time is the better the loop-closure accuracy and the higher the memory consumption rate. To further understand this trade-off between memory consumption and navigation accuracy, we plotted the average translation error and the total memory consumed for one of the datasets we have collected in Figure~\ref{fig:micro}(a). From this plot, we can clearly see that the best median translation error with reasonably low memory consumption occurs at an interframe time of $1$~sec. Thus in our experiments we utilize the Kimera system with the inteframe rate set to $1$sec as the baseline which we call Kimera with LC (loop-closure). We also utilize the same interframe time for the Odometry given from Kimera without the loop closure detector which we call Kimera w/o LC.

\subsection{LIO compute vs accuracy}\label{sec:micro-lio}
To next understand the performance of Cartographer we first note that single-plane based LIO systems have sparser LiDAR scans. This sparse representation demands extensive scan-matching algorithms~\cite{cartographer} that consume more compute while the scans themselves have lesser memory requirements. Thus to understand and utilize the best tuned cartogrpaher model, we again run the cartogrpaher model with various compute limits enforced onto the system. That is limiting the compute provided to the system, limits the accuracy of scan matching and thus the navigation performance of the system. So, as shown in Figure~\ref{fig:micro}(b) where we plot the median translation accuracy vs the compute consumed for various thresholds, from which we can see \todo{text to come here that will describe the observation and the numbers}.
Thus taking this into account, for all the results we use cartographer both with loop-closure detection (cart w/ LC) and without loop closure detection (cart w/o LC) enabled to run at ~\todo{cxx}compute resources.

\subsection{Wheel Odom vs VIO without LCD Odom}\label{sec:micro-odom}
We showed fine-tuned Kimera and Cartographer systems that perform the best with the practical memory and compute limits. 
Now, let us compare how accurate are their Odometry measurements to the standard odometry provided by a wheeled robots wheel-encoder and see how accurate their navigations are in terms of their translation errors.
The Figure~\ref{fig:micro}(c) shows the comparison from which we can see that the odometry measurements from the Kimera and Cartographer without LC perform better than the odometry from wheel-encoders.
This supports the dual-graph design inuition of \name-SLAM wherein the odometry from VIO/LIO-graph is locally corrected and so is better in local odometry and mapping.

\subsection{2D-FFT, PCA-2DFFT vs PCA-FFT}\label{sec:micro-fft}
Finally, now that we have ensured the accuracy of the odometry measurements from VIO/LIO graph, we also need to understand the accuracy of WiFi bearing measurements that complete the WiFi-graph.
To understand the accuracy and timeliness of the bearings and the need for the design of PCA-FFT described in ~\cref{sec:design-bearing} we compare it with the 2D-FFT defined in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, a 2D-FFT version of the PCA algorithm, and the PCA-FFT algorithm we propose. As shown in Figure~\ref{fig:micro}(d), we can see that the PCA version of the algorithms far outperform in accurate bearing measurements the 2D-FFT from $\mathrm{P^2}$SLAM. On the other hand, while bearing errors for PCA-2D FFT are marginally lower than PCA-FFT, we not that the compute required for PCA-2D FFT is of the orders of \todo{xx} cores, while PCA-FFT only required \todo{xx} cores. Thus we can see that for the sake of both timeliness and accuracy PCA-FFT is a better trade-off.

\section{Results}\label{sec:eval}

\begin{figure}[t]
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_orientation.pdf}
    \end{minipage}
    \caption{\textbf{Error analysis:} }
    \label{fig:end-end2}
\end{figure}

To evaluate \name implemented as mentioned in ~\cref{sec:implementation} we deployed \name's algorithms over four datasets. The one presented in ~\cref{sec:eval-kimera} (\name DS) was collected in a $25 \times 20$ m environment, with a total distance of $403$ m traversed over a duration of $23$ minutes. The subsequent 3 datasets (DS 1/2/3) are the P2SLAM datasets~\cite{arun2022p2slam}. Through these datasets, we have robustly tested \name across 3 distinct environments, 4 different access point placements, and traversed a cumulative distance of $1625$ m with a total travel time of $108$ minutes. We note the datasets in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} use AoA measurements at both the robot and the access points, while in \name we only utilize the AoA at the robot and extract the channels for only those measurements from the dataset. Finally, it is important to note that while in DS1/2/3 linear antenna arrays are used, we use square antenna array on the robot in \name DS.

As stated in ~\cref{sec:eval-micro}, we benchmark \name's results with a state-of-the-art SLAM algorithm, Kimera~\cite{rosinol2021kimera}, a stereo-camera based SLAM algorithm. We run Kimera on only \name DS with and without loop closures, labelled in the legends as `w/ LC' and `w/o LC' respectively, since DS1/2/3 lack required IMU measurements. Additionally, for all the 4 datasets, we run Cartographer in real time, with and without the `global SLAM' and LiDAR scan matching, which turn on/off loop closures. These are referred to as `Cart w/LC' and `Cart w/o LC' respectively. As discussed in ~\cref{sec:eval-micro} we have carefully finetuned both Kimera and Cartographer to their best performance as benchmarks. To obtain ground truth, we observe that allowing Cartographer to run past the time of data collection without any compute constraints allows it to provide a near-groundtruth trajectory as characterized in DLoc~\cite{ayyalasomayajula2020deep}. 

In the following sections, using the Cartographer ground truth generated, we benchmark \name against Kimera, Cartographer(when run in real-time), and WiFi graph run with the wheel-encoder odometry (WiFi+Odom) and provide results for the translation and orientation errors. We further measure the CPU and memory usage across these SLAM frameworks\footnote{\url{https://github.com/alspitz/cpu_monitor}} and compare the total memory used, the rate of memory increase and the CPU resources used over the entire run of the datasets.

\subsection{End-to-end evaluation (\name with Kimera):}\label{sec:eval-kimera}

% \begin{table*}[ht]
%     \centering
%     \footnotesize
%     \caption{}
%     \begin{tabular}{|l|cccc|cccc|cccc|}
%     \hline
%     \multirow{2}{*}{} & \multicolumn{4}{c|}{\textbf{Cart. w/ LC}} & \multicolumn{4}{c|}{\textbf{\name + Cart. w/o LC}} & \multicolumn{4}{c|}{\textbf{\name + Odom}} \\ \cline{2-13} 
%      & \multicolumn{1}{l|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3} & \multicolumn{1}{l|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3} & \multicolumn{1}{l|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \multicolumn{1}{l|}{\textbf{DS 3}} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}Translation \\ Error (cm)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}88.0\\ (169.4)\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0 \\ (224)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}134.1 \\ (1097)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}23.3\\ (37.4)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}98.5\\ (252.5)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}65.9\\ (92.2)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}67.3\\ (182.6)\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}48.6 \\ (114.4)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}88.1\\ (193)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0\\ (100.2)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}75.5\\ (204.9)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}66.44\\ (234.7)\end{tabular} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}Orientation \\ Error (deg)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4.8\\ (7.9)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{0.8}\\ (4.66)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}5.3\\ (12.6)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.6\\ (1.4)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.5\\ (6.9)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2.4\\ (4.66)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{2.8}\\ (12)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}1.4\\ (3.3)\end{tabular} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}1.0\\ (3.7)\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1.7\\ (\textbf{2.7})\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.0\\ (\textbf{6.2})\end{tabular}} & \begin{tabular}[c]{@{}c@{}}2.0 \\ (10.3)\end{tabular} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}Total \\ Memory (MB)\end{tabular}} & \multicolumn{1}{c|}{520} & \multicolumn{1}{c|}{702} & \multicolumn{1}{c|}{658} & 423 & \multicolumn{1}{c|}{486} & \multicolumn{1}{c|}{613} & \multicolumn{1}{c|}{706} & 356 & \multicolumn{1}{c|}{\textbf{270}} & \multicolumn{1}{c|}{\textbf{288}} & \multicolumn{1}{c|}{\textbf{252}} & \textbf{163} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}Rate of \\ memory (MB/s)\end{tabular}} & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{0.29} & \multicolumn{1}{c|}{0.33} & 0.38 & \multicolumn{1}{c|}{0.32} & \multicolumn{1}{c|}{0.22} & \multicolumn{1}{c|}{0.33} & 0.26 & \multicolumn{1}{c|}{\textbf{0.16}} & \multicolumn{1}{c|}{\textbf{0.10}} & \multicolumn{1}{c|}{\textbf{0.11}} & \textbf{0.14} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}CPU (fraction \\ of cores)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.8\\ (4.4)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.2\\ (4.2)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.8\\ (4.2)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}1.85\\ (4.4)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.73\\ (1.90)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.62\\ (2.1)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.85\\ (2.8)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.77\\ (1.1)\end{tabular} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.19\\ (1.4)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.2\\ (1.6)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.28 \\ (1.7)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.22 \\ (0.5)\end{tabular}} \\ \hline
%     \end{tabular}
% \end{table*}


\begin{table*}[t]
    \centering
    \footnotesize
    \caption{}
    \label{tab:cart}
    \begin{tabular}{|l||cccc||cccc|}
    \hline
    \multirow{2}{*}{}                   & \multicolumn{4}{c||}{\textbf{Cart. w/ LC}}                                                                                                                    & \multicolumn{4}{c|}{\textbf{\name + Cart. w/o LC}}                                                                                                   \\ \cline{2-9} 
                                        & \multicolumn{1}{c|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}}       & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3}        & \multicolumn{1}{c|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}}        & \multicolumn{1}{c|}{\textbf{DS 2}}         & \textbf{DS 3}      \\ \hline
    \textbf{Translation Error (cm)}     & \multicolumn{1}{c|}{\textbf{88.0 (169.4)}}            & \multicolumn{1}{c|}{74.0 (224)}          & \multicolumn{1}{c|}{134.1 (1097)}  & \textbf{23.3 (37.4)} & \multicolumn{1}{c|}{98.5 (252.5)}                     & \multicolumn{1}{c|}{\textbf{65.9 (92.2)}} & \multicolumn{1}{c|}{\textbf{67.3 (182.6)}} & 48.6 (114.4)       \\ \hline
    \textbf{Orientaion Error ($^\circ$)} & \multicolumn{1}{c|}{4.8 (7.9)}                        & \multicolumn{1}{c|}{\textbf{0.8 (4.66)}} & \multicolumn{1}{c|}{5.3 (12.6)}    & \textbf{0.6 (1.4)}   & \multicolumn{1}{c|}{\textbf{3.5 (6.9)}}               & \multicolumn{1}{c|}{2.4 (4.66)}           & \multicolumn{1}{c|}{\textbf{2.8 (12)}}     & 1.4 (3.3)          \\ \hline
    \textbf{Total Memory (MB)}          & \multicolumn{1}{c|}{520}                              & \multicolumn{1}{c|}{702}                 & \multicolumn{1}{c|}{\textbf{658}}  & 423                  & \multicolumn{1}{c|}{\textbf{486}}                     & \multicolumn{1}{c|}{\textbf{613}}         & \multicolumn{1}{c|}{706}                   & \textbf{356}       \\ \hline
    \textbf{Rate of Memory (MBps)}      & \multicolumn{1}{c|}{\textbf{0.30}}                    & \multicolumn{1}{c|}{0.29}                & \multicolumn{1}{c|}{0.33}          & 0.38                 & \multicolumn{1}{c|}{0.32}                             & \multicolumn{1}{c|}{\textbf{0.22}}        & \multicolumn{1}{c|}{\textbf{0.33}}         & \textbf{0.26}      \\ \hline
    \textbf{CPU (fraction of cores)}    & \multicolumn{1}{c|}{3.8 (4.4)}                        & \multicolumn{1}{c|}{3.2 (4.2)}           & \multicolumn{1}{c|}{3.8 (4.2)}     & 1.85 (4.4)           & \multicolumn{1}{c|}{\textbf{0.73 (1.90)}}             & \multicolumn{1}{c|}{\textbf{0.62 (2.1)}}  & \multicolumn{1}{c|}{\textbf{0.85 (2.8)}}   & \textbf{0.7 (1.1)} \\ \hline
    \end{tabular}
\vspace{-0.1in}
\end{table*}



In this section we demonstrate in depth on how \name-SLAM compares to the state of the art Kimera VIO SLAM on our \name DS.

\noindent\textbf{Navigation Accuracy:} Firstly, we look at the translation and orientation errors of \name-SLAM + Kimera w/o LC and compare it with \name-SLAM+Odom and Kimera w/ LC across Figures~\ref{fig:end-end2},~\ref{fig:end-end1}. Firstly from Figure~\ref{fig:end-end2} we can see that \name-SLAM + Kimera w/o LC has a median ($90^{th}$\%) translation error of $85$cm ($185$cm) and median ($90^{th}$\%) orientation errors of $3^{\circ}$ ($8^{\circ}$). 
We can also see that WiFi+Odom very closely at a median ($90^{th}$\%) translation errors of $90$cm ($205$cm) and median ($90^{th}$\%) orientation errors of $1^{\circ}$ ($4^{\circ}$). While we see that Kimera w/ LC has a median ($90^{th}$\%) translation errors of $105$cm ($300$cm) and median ($90^{th}$\%) orientation errors of $5^{\circ}$ ($20^{\circ}$)showing that  \name-SLAM's WiFi graph implementation out-performs the state-of-the-art Kimera w/ LC, without needing loop-closure detection. Additionally, we can also see that the translation errors and orientation errors for WiFi+Kimera w/o LC are smaller than and on par that for WiFi+Odom respectively, showing how the locally-corrected Odom measurements from Kimera w/o LC aid in better global optimizations.

The understand this further we can see from Figure~\ref{fig:end-end1}(a) where we plot the predicted trajectory for Kimera w/ LC against ground truth where we can see that it looses tracking around the region of $[-5 5] and [-20 -15]$ along $X and Y$ axes, which can be further demonstrated at the $1100$ sec mark in the time series plots shown for the red-dotted line in Figures~\ref{fig:end-end1}(c,d). We can see that after $1100$secs Kimera w/ LC performs incorrect Loop Closure leading to the translation errors shooting up to $~450$cm and orientation errors up to $~25^{\circ}$. In contrast we can see from the blue-solid (green-dotted) line in Figures~\ref{fig:end-end1}(c,d) that \name's WiFi+Kimera w/o LC (WiFi+Odom) closely track the ground truth where it caps at about $~200$cm translation error and $~10^{\circ}$ orientation error.
So we have seen that \name's SLAM navigation is on-par or even more accurate due to its robustness to global corrections than the state-of-the-art VIO, Kimera.

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.42\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem_cpu_w_aoa_ts.pdf}
    \end{minipage}
    \caption{Notes: memory avg slope, Kimera -- 0.56, \name -- 0.2 MB/s}
    \label{fig:mem-cpu}
\end{figure}

\noindent\textbf{Memory and Compute:} Next, we run \name-SLAM and Kimera under various settings on \name DS and evaluate the memory and compute consumption of each components of \name SLAM that uses Kimera w/o LC and Kimera w/ LC and plot the time-series as shown in Figure~\ref{fig:mem-cpu}. From the Figure~\ref{fig:mem-cpu}(left) we can see taht Kimera w/ LC has a huge start-up cost of about $2$GB after which we see that it has a memory consumption rate of about $0.56$MBps, in contrast we can see that the memory consumption for \name+Kimera w/o LC has a startup of $0.5$GB, with a consumption rate of only $0.2$MBps. That is given a standard RPi of 8GB RAM, while Kimera w/ LC can only run upto $3$hrs before the robot crashes due to lack of space, \name+Kimera w/o LC can run up to $10$hrs, that is in general \name + Kimera w/o LC has a $3.3\times$ lesser memory consumption rate than the state-of-the-art Kimera system.
To further understand the individual components that lead to this memory consumption we have also plotted the timeseries memory consumption of Kimera w/o LC and WiFi only systems in Figure~\ref{fig:mem-cpu}(left). From which we can see that due to a fix lag local drift correction algorithm that Kimera w/o LC employs it has a constant memory consumption of $0.3$GB. On the other hand, WiFi only has a increasing memory rate of $0.2$MBps because we do not employ a fix-lag filter~\cite{xxxx}, but accumulate all the nodes over all the time. This is not exactly required for the global corrections to occur as these WiFi anchors act as unique self-identifiable landmarks in the environment.

Finally, we can also see from Figure~\ref{fig:mem-cpu}(right) that the compute requirements for \name's WiFi+Kimera w/o LC is upto a $1$ core, while Kimera w/ LC takes up to $1.5$ cores owing to its compute heavy loop closure detection and correction algorithms. Thus \name's design requires about $3.3\times$ less memory and $1.5\times$ less compute than state-of-the-art Kimera system, while achieving about $30\%$ better navigation performance.

\subsection{End-to-end evaluation (\name with Cartographer):}\label{sec:eval-cart}

We further also demonstrate that \name-SLAM can also improve the performance of the state-of-the-art LIO SLAM, Cartographer. So, we compare \name's WiFi+Cart w/o LC against the Cartographer w/ LC when run in real-time. Additionally, since we have the cartographer LiDAR data from the open-sourced $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} datasets, DS 1/2/3 we provide the translation, orientation errors, memory consumption and compte requirements for \name and cartographer in Table~\ref{tab:cart}. From this table we can see that mostly \name's WiFi+Cart w/o LC performs on-par with Cart w/ LC in terms of translation and orientation accuracies. There are two notably different navigation accuracy performances: (a) in DS 2 \name's median ($90^{th}$) translation and orientation errors are $2\times$ ($5\times$) lower for \name's Cart W/o LC than Cart W/ LC. (b) in DS 3 cart. w/ LC has $2\times$ lesser translation and orientation errors than WiFi+cart w/o LC. But we can see that the maximum errors in translation (orientation )are only $114.4$cm (3.3$^\circ$) which are tolerable.

In contrast looking at the memory consumption, both the systems perform almost the same with minor differences. This occurs because unlike Kimera's VIO system where each camera frame consists of dense features, Cartographer's LIO system's each scan has fewer number of features. This limited features in each scan greatly reduces the load on the memory consumption. Instead, having sparser features, LIO systems like Cartographer tend to execute complex scan-matching algorithms for loop closures, which in turn increase the compute requirements of the VIO-SLAM systems. In constrast, since in \name's implementaiton of WiFi+Cart. w/o LC does not require these complex scan matching for loop closures, demands much lesser compute resources. This can be clearly observed in the last row of Table~\ref{tab:cart} which shows the average number of cores used over the entire run of the robot navigation with the maximum number of cores used in parentheses.
Where we can see that \name's WiFi+cart w/o LC requires $4\times$ lesser peak compute than real-time Cartographer implementation across all the 4 datasets.

==> ViWiD SLAM_arx/evaluation/eval6.tex <==
% !TEX root = root.tex

\begin{figure*}[t]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_cdf_translation.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_cdf_orientation.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_translation.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_orientation.pdf}    
        \subcaption{}
    \end{minipage}
    
    \caption{\textbf{End-to-end evaluation}:  \textbf{(a, b)} Translation and orientation errors comparing Kimera with loop closure against \name's predictions. \name uses odometry from Kimera without loop closures and just wheel odometry . \textbf{(c, d)} Time series of translation and orientation error comparing Kimera with loop closure against \name's predictions. \name uses odometry from Kimera without loop closures.}
    \label{fig:end-end1}
    % \vspace{-0.2in}
\end{figure*}

\section{Results}\label{sec:eval}

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.18\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/top-down-kimera.pdf}
    \end{minipage}
    \; \;
    \begin{minipage}[t]{0.18\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/top-down-viofi.pdf}
    \end{minipage}
    \caption{\textbf{Trajectories:} A top-down view showing the Trajectories estimated by \textbf{(a)} Kimera with loop closures and ground truth. \textbf{(b)} \name using odometry predictions from Kimera without loop closures (\textit{WiFi + VIO}) and ground truth. }
    \label{fig:end-end2}
    % \vspace{-0.1in}
\end{figure}

Next, we demonstrate \name's performance in 4 datasets and compare it with state-of-the-art SLAM systems Kimera~\cite{rosinol2021kimera} (VIO) and Cartographer~\cite{cartographer} (LIO). Across these datasets, we compare three aspects of each algorithm's performance: 

\noindent\textbf{(a)} \textbf{3-DoF Navigation Accuracy}: XY euclidean translation error and absolute orientation error, 

\noindent\textbf{(b)} \textbf{Memory Consumption:}\footnote{\url{https://github.com/alspitz/cpu_monitor}} The total memory consumed for a run of the dataset, and also the rate of memory consumption, to understand scalability to larger indoor spaces, and 

\noindent\textbf{(c)} \textbf{Compute Cost:} As the max and average number of cores required by the algorithm to perform online SLAM.

\noindent\textbf{Datasets:} To demonstrate our system against Kimera (which requires a stereo-camera), we deploy a robot in a $20 \times 25$ m environment with 3 WiFi APs, with the robot traversing a total distance of $403$ m over a duration of $23$ minutes (called \name DS). We also use the open-sourced datasets~\cite{arun2022p2slam} that we call DS 1/2/3. But these 3 datasets do not have stereo-camera data, and use a linear antenna array on the robot, for which the aliasing is resolved using ground truth information. Through these 4 datasets, we have robustly tested \name across 3 distinct environments, 4 different and realistic access point placements, and traversed a cumulative distance of $1625$ m with a total travel time of $108$ minutes. To obtain ground truth labels, we allow Cartographer to run offline with very extensive search parameters, which converges to a near ground truth trajectory as characterized in DLoc~\cite{ayyalasomayajula2020deep}. Finally we intend to open source this dataset for the benefit of the larger research community up on the paper's acceptance. 

\noindent\textbf{Baselines:} We compare \name's performance with (a) Kimera in the \name DS, (b) Cartographer in all the datasets. Kimera and Cartographer have their loop-closures fine-tuned to provide the best realtime performance. 

% \todo{explain what vio means, it's only using camera + imu; no wheel odometry}

\name's modular dual-graph design enables the WiFi-graph to receive odometry measurements from different SLAM systems. Thus, we give \name the following sources of odometry:
\textbf{(a)} \textbf{WiFi+VIO}: Online Kimera without the Loop Closure detection node,
\textbf{(b)} \textbf{WiFi+LIO}: Online Cartographer without global scan matching, and
\textbf{(c)} \textbf{WiFi+Odom}: The built-in wheel encoder on the TurtleBot.
% \todo{this is not fully clear} 
Further note that we disabled visualization on Kimera and Cartographer to only account for the memory and computation by the optimization backend and keyframe storage.

We compare Kimera with WiFi+VIO and Cartographer with WiFi+LIO and provide an in-depth analysis of results and plots for Kimera~\cref{sec:eval-kimera} and summarize the results for Cartographer in a table in ~\cref{sec:eval-cart} due to space constraints.
Finally, in ~\cref{sec:eval-micro} we demonstrate the fine-tuning and trade-offs for both Kimera and Cartographer.

\subsection{End-to-end evaluation (\name with Kimera):}\label{sec:eval-kimera}

First, we show how \name provides a resource-efficient alternative to Kimera's loop closure detection module with on-par or better navigation accuracy.

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.42\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem_cpu_w_aoa_ts.pdf}
    \end{minipage}
    \caption{Timeseries of memory (\textit{left}) and CPU consumption (\textit{right}) of VIO, Kimera and \name + VIO. The resource consumption of the \name's WiFi graph is also analysed (\textit{Wifi only})}
    \label{fig:mem-cpu}
    % \vspace{-0.1in}
\end{figure}

% \todo{explain why 4b has wifi+vio is worse than wifi+odom}

\noindent\textbf{Navigation Accuracy:} We compare the CDF and time-series translation errors in Figure~\ref{fig:end-end1}(a)(c) respectively for \name's WiFi+VIO, WiFi+Odom, and Kimera. 
From these plots we can see that the median ($90^{th}\%$) translation errors for \name's WiFi+VIO is $85$cm ($185$cm), and WiFi+Odom is $90$cm ($205$cm), which are $60\%$ lower compared to Kimera with median ($90^{th}\%$) translation errors of $105$cm ($300$cm).
Similarly Figure~\ref{fig:end-end1}(b)(d) compares the cumulative and time-series orientation error respectively for \name's WiFi+VIO, WiFi+Odom, and Kimera. 
From these plots we can see that the median ($90^{th}\%$) orientation errors for \name's WiFi+VIO is $3^{\circ}$ ($8^{\circ}$), and WiFi+Odom is $1^{\circ}$ ($4^{\circ}$), i.e. $60\%$ lower compared to Kimera with median ($90^{th}\%$) orientation errors of $5^{\circ}$ ($20^{\circ}$).

\begin{table*}[ht]
    \centering
    \footnotesize
    \caption{Translation, Orientation, and resource analysis of Cartographer and \name + LIO, median ($99^\mathrm{th} percentile$ error)}
    \label{tab:cart}
    \begin{tabular}{|l||cccc||cccc|}
    \hline
    \multirow{2}{*}{}                   & \multicolumn{4}{c||}{\textbf{Cartographer~\cite{cartographer}}}                                                                                                                    & \multicolumn{4}{c|}{\textbf{\name + LIO}}                                                                                                   \\ \cline{2-9} 
                                        & \multicolumn{1}{c|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}}       & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3}        & \multicolumn{1}{c|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}}        & \multicolumn{1}{c|}{\textbf{DS 2}}         & \textbf{DS 3}      \\ \hline
    \textbf{Translation Error (cm)}     & \multicolumn{1}{c|}{\textbf{47.0 (98.9)}}            & \multicolumn{1}{c|}{74.0 (224)}          & \multicolumn{1}{c|}{134.1 (1097)}  & \textbf{23.3 (37.4)} & \multicolumn{1}{c|}{50.34 (152.4)}                     & \multicolumn{1}{c|}{\textbf{65.9 (92.2)}} & \multicolumn{1}{c|}{\textbf{67.3 (182.6)}} & 48.6 (114.4)       \\ \hline
    \textbf{Orientaion Error ($^\circ$)} & \multicolumn{1}{c|}{4.8 (7.9)}                        & \multicolumn{1}{c|}{\textbf{0.8 (4.66)}} & \multicolumn{1}{c|}{5.3 (12.6)}    & \textbf{0.6 (1.4)}   & \multicolumn{1}{c|}{\textbf{3.5 (6.9)}}               & \multicolumn{1}{c|}{2.4 (4.66)}           & \multicolumn{1}{c|}{\textbf{2.8 (12)}}     & 1.4 (3.3)          \\ \hline
    \textbf{Total Memory (MB)}          & \multicolumn{1}{c|}{520}                              & \multicolumn{1}{c|}{702}                 & \multicolumn{1}{c|}{\textbf{658}}  & 423                  & \multicolumn{1}{c|}{\textbf{486}}                     & \multicolumn{1}{c|}{\textbf{613}}         & \multicolumn{1}{c|}{706}                   & \textbf{356}       \\ \hline
    \textbf{Rate of Memory (MBps)}      & \multicolumn{1}{c|}{\textbf{0.30}}                    & \multicolumn{1}{c|}{0.29}                & \multicolumn{1}{c|}{0.33}          & 0.38                 & \multicolumn{1}{c|}{0.32}                             & \multicolumn{1}{c|}{\textbf{0.22}}        & \multicolumn{1}{c|}{\textbf{0.33}}         & \textbf{0.26}      \\ \hline
    \textbf{CPU (fraction of cores)}    & \multicolumn{1}{c|}{3.8 (4.4)}                        & \multicolumn{1}{c|}{3.2 (4.2)}           & \multicolumn{1}{c|}{3.8 (4.2)}     & 1.85 (4.4)           & \multicolumn{1}{c|}{\textbf{0.73 (1.90)}}             & \multicolumn{1}{c|}{\textbf{0.62 (2.1)}}  & \multicolumn{1}{c|}{\textbf{0.85 (2.8)}}   & \textbf{0.7 (1.1)} \\ \hline
    \end{tabular}
\vspace{-0.2in}
\end{table*}

While the median translation and orientation errors for Kimera are comparable to \name running on Kimera's odometry, the reason for high errors in the $90^{th}\%$ are due to an incorrect loop-closure that occurs in Kimera at around $1100$~sec time-mark as can be clearly seen from the sudden spike in errors in both Figures~\ref{fig:end-end1}(c,d). This can be seen in the two top-down views of the estimated trajectories shown in Figure~\ref{fig:end-end2}.
This further demonstrates the strength of WiFi-measurements for global corrections.

\noindent\textbf{Memory Consumption:} We have seen that WiFi provides more accurate and real-time global drift corrections than Kimera's loop closures. Now, we evaluate the memory consumption of the individual components of Kimera and \name and observe the trends shown in Figure~\ref{fig:mem-cpu} (left), from which we can see that while Kimera needs a start up memory of $2$ GB and from then on accumulates memory at a rate of $0.56$ MBps. In contrast, WiFi + VIO only has a start-up memory of $0.4$ GB and memory accumulation rate of $0.2$ MBps, which will on an average enable \name to run $3.3\times$ longer than Kimera on a typical RAM of $8$ GB before crashing.
We can further verify that Kimera's memory consumption is dominated by loop closures -- the black line in Figure~\ref{fig:mem-cpu} (left) for the VIO, which is Kimera without loop-closures, indicates the memory remains constant at $0.2$ GB. It is important to note here that since Kimera's VIO has near-constant memory consumption, the accruing memory consumption of \name's stack is purely due to the WiFi-graph as shown by the purple dashed line in Figure~\ref{fig:mem-cpu} (left).
We note that this could be avoided if the WiFi-graph employs a fixed-lag smoothing optimization strategy similar to the VIO system, which will be left for future work.

\noindent\textbf{Compute Requirements:} Finally, we can also see from Figure~\ref{fig:mem-cpu} (right) that \name requires only one core to run on our system, while Kimera takes up to $1.5$ cores owing to its loop closure detection and correction algorithms. Thus \name's WiFi+VIO design requires about $3.3\times$ less memory and $1.5\times$ less compute than a state-of-the-art Kimera system while achieving about $60\%$ better navigation performance.

\begin{figure*}[pt]
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem-interframetime.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/cart_err_vs_cores.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation_no_lc.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/aoa_err.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\textbf{Microbenchmarks}: \textbf{(a) Kimera:} Trade-off between memory consumption and the accuracy for various interframe rates. \textbf{(b) Cartographer:} Trade-off between compute required and the accuracy for various scan-matching thresholds. \textbf{(c) Odometry-Graph:} Comparison on how various odometry inputs to the WiFi graph look before optimization. \textbf{(d) Bearing Measurement Algorithms:} Comparison between 2D-FFT from $\mathrm{P^2}$SLAM, Spotfi and our proposed PCAB.}
    \label{fig:micro}
    \vspace{-0.1in}
\end{figure*}

\subsection{End-to-end evaluation (\name with Cartographer):}\label{sec:eval-cart}

We also test \name running on Cartographer's LIO and compare it online with full-stack Cartographer across all the 4 datasets, DS 1/2/3 and \name DS and present a summary of the results in Table~\ref{tab:cart} due to space constraints.

\noindent\textbf{Navigation Accuracy:} From this table, we can see that \name's trajectory estimation performs on-par with Cartographer's loop closure detector across most datasets in terms of translation and orientation accuracy. There are two notable differences in navigation accuracy performance: 

\textbf{(a)} in \textit{DS 2} \name's median ($90^{th}$) translation and orientation errors are $2\times$ ($5\times$) lower for \name + LIO than Cartographer. In this scenario, Cartographer makes an incorrect loop closure leading to a very inconsistent trajectory prediction, as can be common with visual-based loop closures. 

\textbf{(b)} in  \textit{DS 3}, Cartographer has $2\times$ lesser translation and orientation errors than WiFi+LIO. We notice this performance degradation from the use of linear array on the robot. As discussed in \cref{sec:design-bearing}, bearing measurements closer to $\pm 90^\circ$ suffer from higher errors, and due to a non-optimal orientation of linear array, we observe a larger number of bearing measurements at these higher angles, reducing the SLAM performance. Utilizing a square array resolves these issues. 

\noindent\textbf{Memory Consumption:} The memory consumption of \name and Cartographer are similar. This occurs because, unlike Kimera's VIO system where each camera frame consists of dense features, Cartographer's LIO system's LiDAR scans are much smaller, reducing Cartographer's memory consumption.

\noindent\textbf{Compute Requirements:} Due to the sparsity of LiDAR features, Cartographer needs to run scan-matching algorithms for loop closures, which in turn increases Cartographer's compute requirements. In contrast, since \name running on Cartographer's local odometry does not require scan matching to correct the global trajectory, it demands much lesser compute resources. This can be observed in the last row of Table~\ref{tab:cart} which shows the average number of cores used over the entire run of the robot navigation with the maximum number of cores used in parentheses. We can see that \name needs $4\times$ lesser peak compute than the full-stack Cartographer implementation across all 4 datasets.

\subsection{Microbenchmarks}\label{sec:eval-micro}


\noindent{\textbf{VIO Memory vs Accuracy:}}
To characterize Kimera's memory usage, we alter the rate at which it records keyframes for loop closure detection. A lower time between keyframes will lead to more loop closure detections at the cost of increased memory consumption. To understand how Kimera's loop closure detection accuracy is limited by memory, we plot the median translation error and the total memory consumed in \name DS (Figure~\ref{fig:micro}(a)). From this plot, we can see that the best median translation error with reasonably low memory consumption occurs at a keyframe period of $1$~second and we use this keyframe rate for our baseline.

\noindent{\textbf{LIO Compute vs Accuracy:}}
To next understand the performance of Cartographer we first note that single-plane-based LIO systems have sparse features in LiDAR scans, as opposed to denser stereo data. This sparser representation demands extensive scan-matching algorithms~\cite{cartographer} with higher compute. Thus to understand Cartographer's compute requirements, we run Cartographer on \name DS and limit the number of CPU cores it can access. We plot the median translation accuracy vs number of CPU cores accessible in Figure~\ref{fig:micro}(b). We can see that median translation error improves with a larger number of cores, verifying that compute power is a bottleneck for accurate scan matching, and thus navigation performance.
Keeping in mind that many low-compute platforms are limited to 4 cores, we restrict Cartographer to use 4 compute cores only in the end-to-end comparison.

\noindent{\textbf{Wheel-based Odometry vs Kimera without LCD (VIO) and Cartographer without LCD (LIO):}}
Now, let us compare how accurate the odometry measurements from Kimera and Cartographer without loop closures are to wheel odometry provided by the Turtlebot.
Figure~\ref{fig:micro}(c) shows the comparison of their translation errors, from which we can see that the odometry measurements from Kimera and Cartographer without loop closure have lesser errors at both the median and $90^{th}\%$ than odometry from wheel-encoders.
This supports the dual-graph design intuition of \name wherein the odometry from the VIO/LIO-graph is locally corrected and so is better at local odometry and mapping than simple wheel-encoder systems.

\noindent{\textbf{Bearing Accuracy and Compute:}}
Finally, to understand the accuracy and compute-requirements of bearing-estimation algorithms and the need PCAB (\cref{sec:design-bearing}), we compare it with \textit{2D-FFT} defined in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} and \textit{Spotfi}~\cite{spotfi}. As shown in Figure~\ref{fig:micro}(d), PCAB outperforms 2D-FFT in bearing estimation by $1.43\times$ ($2 \times$) at the median and $80^\mathrm{th}\%$. Additionally, we note that the average CPU utilization of PCAB on our robot is $11\%$, whereas 2D-FFT required $565\%$ core usage (an improvement of approx. $50\times$). Moreover, we compute the AoA predictions with Spotfi~\cite{spotfi} and find PCAB performs $1.8\times$ ($2.2\times$) at the median and $80^\mathrm{th}\%$. Moreover, Spotfi consumes $1200$ percentage of cores (all cores of our machine). Clearly, both the 2D-FFT and Spotfi estimations are unsuitable for low-compute SLAM applications.

==> ViWiD SLAM_arx/implementation/implementation.tex <==
% !TEX root = root.tex
\section{Implementation}\label{sec:implementation}

\noindent{\textbf{Hardware: }}\label{sec:implement-soft} We implement \name on the Turtlebot 2 platform. For WiFi CSI data collection, we attach an off-the-shelf WiFi radio~\cite{nexmon:project} to the Turtlebot. Then we place a few of the similar APs near the ceiling at a density of roughly one every ten meters. We transmit on channel 42 of 5GHz WiFi. We then use an open-sourced toolbox~\cite{nexmon:project} to collect channel state information (CSI) data from all the APs at the WiFi radio on the robot.
Our robot is also equipped with a Hokuyo UTM-30LX LiDAR and a Intel D455 RGBD camera with an IMU.

\noindent\textbf{Software:}
Given this setup, we compare our system against the realtime performance of two systems (a) Kimera~\cite{rosinol2021kimera}, a state-of-the-art VIO that uses the Intel D455 + IMU for its SLAM, and (b) Cartographer~\cite{cartographer}, a state-of-the-art LIO that uses the wheel encoders and the Hokuyo LiDAR for its SLAM.
The Turtlebot is controlled with a laptop running Robot Operating System (ROS-Kinetic), which manages all sensor input. WiFi CSI measurements are also integrated into ROS, and \name is implemented as a C++ application to ensure realtime operation and integrated within ROS as a ROS-node, allowing for easy integration with other robotics systems.
The Wi-Fi factor graph is implemented in GTSAM~\cite{gtsam}, and we utilize the open-sourced library to implement Kimera and Cartographer. \name's codebase will be open-sourced upon the paper's acceptance. 
 
% \subsection{Datasets}\label{sec:datasets}
% To evaluate and compare \name, we demonstrate \name-SLAM's performance in 4 datasets. Open-sourced datasets from $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} that we call DS 1/2/3. But these 3 datasets do not have any IMU data, use linear antenna array on the robot to collect the data, and collect the channel (CSI) data at both the robot and the APs of which we only need the robot sided measurements. Thus to demonstrate our system against Kimera, we deployed the robot in a $25 \times 20$ m environment with 3 WiFi APs, with the robot traversing a total distance of $403$ m over a duration of $23$ minutes (called \name DS). Through these 4 datasets, we have robustly tested \name across 3 distinct environments, 4 different access point placements, and traversed a cumulative distance of $1625$ m with a total travel time of $108$ minutes. All these datasets have been stored as `ROSbags', which can be played to emulate real-time runs for multiple tests. Thus, we were able to evaluate the realtime performance of \name-SLAM and the Kimera and Cartographer baselines using these datasets.

% Since, only \name DS has camera and IMU data, we demonstrate \name's and Kimera's realtime performance only on \name DS. On the other hand we compare against the realtime cartographer across all the 4 datasets (DS 1/2/3 and \name DS). Since, owing to the modular design idea of \name-SLAM, the graph/node providing real-time Odometry measurements to the WiFi-graph as described in ~\cref{sec:design-graph1} can be either the VIO (Kimera without the Loop Closure), LIO (Cartographer without the Loop Closure), or the wheel-encoders on the robot.
% We evaluate \name-SLAM using all the three odometry nodes and for brevity we use the following terminology \name-SLAM and the baselines:
% \begin{itemize}
%     \item \textbf{WiFi+Kimera w/o LC:} \name-SLAM run with the odometry measurements coming from the realtime Kimera running without the Loop Closure detection.
%     \item \textbf{WiFi+Cart. w/o LC:} \name-SLAM run with the odometry measurements coming from the realtime Cartographer running without the Loop Closure detection.
%     \item \textbf{WiFi+Odom:} \name-SLAM run with the odometry measurements coming from the wheel encoders and gyroscope of the robot.
%     \item \textbf{Kimera w/ LC:} Kimera running realtime with the Loop Closure detection.
%     \item \textbf{Cart. w/ LC:} Cartographer running realtime with the Loop Closure detection.
% \end{itemize}
% \noindent\textbf{WiFi+Kimera w/o LC:} \name-SLAM run with the odometry measurements coming from the realtime Kimera running without the Loop Closure detection.

% \noindent\textbf{WiFi+Cart. w/o LC:} \name-SLAM run with the odometry measurements coming from the realtime Cartographer running without the Loop Closure detection.

% \noindent\textbf{WiFi+Odom:} \name-SLAM run with the odometry measurements coming from the wheel encoders and gyroscope of the robot.

% \noindent\textbf{Kimera w/ LC:} Kimera running realtime with the Loop Closure detection.

% \noindent\textbf{Cart. w/ LC:} Cartographer running realtime with the Loop Closure detection.

% Finally, to obtain ground truth, we observe that allowing Cartographer to run past the time of data collection without any compute constraints allows it to provide a near-groundtruth trajectory as characterized in DLoc~\cite{ayyalasomayajula2020deep}. 

==> ViWiD SLAM_arx/intro/intro-1.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.


Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Since these Visual and LiDAR SLAM systems perform sensor fusion to provide a human-readable map and to reduce the local and global drifts introduced by the odometry sensors.
This mapping and corrections are possible by performing feature identification and feature correlation across current and past frames to re-detect the previously visited location (typically termed as `loop-closure detection'), which leads to two distinct problems: 
(a) The robot needs to have an active memory of all the past features of all the time, making the system limited by the active memory (typically the RAM size). 
(b) Also as time progresses, the search time to find a matching features frame across all the past frames continues to rise.
These issues in the best could lead to the robot just taking longer in state transition, and accidents in the worst owing to inconsistency in the current state and the predicted state, leading to incorrect state-transition decisions.

In this work, so we ask and answer the question what if we can remove these memory intensive and time consuming loop-closures? For which we can see that $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} which performs end-to-end robot navigation optimization without requiring any loop closure detection. Inspired from this observation in this paper, we will present how WiFi can be integrated with visual sensors for real-time autonomous navigation.

\subsection{Literature Review}

Most of the existing Visual and LiDAR SLAM algorithms try to resolve the memory and search-time issues in loop-closure detection and identification by: (a) optimizing on the algorithms for key-frame and key-point detection~\cite{mur2015orb,rosinol2021kimera} to reduce the number of key-frames stored, and (b) using smart representation, like bag-of-words~\cite{rosinol2021kimera} to reduce the search time. While these solutions might extend the run-time of a robot temporarily, it would quickly run into the same issues once it is used for larger or more involved spaces like warehouses.

In a past work~\cite{arun2022p2slam} we demonstrated Radio Frequency(RF) technologies, especially WiFi as a navigation sensor for SLAM robots owing to the ubiquitous deployment of WiFi.
Although $\mathrm{P^{2}}$SLAM performs only end-to-end optimization and cannot translate to real-time navigation of the robot.
There have been other works like WSR~\cite{jadhav2020wsr} that only demonstrates robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi,hashemifar2019augmenting, liu2019collaborative} depend only on WiFi readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

The other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation, like UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi and thus are limited in scalability.
% \footnote{We also want to note that, while we have used WiFi as a sensor in \name, \name's design is modular enough to easily scale to other RF-technologies.}.

Finally, there also exist a few other series of works called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel} that try to reduce the memory usage and processing time by running two different optimizations for mapping and pose-estimation in parallel which tend to drift in real-time while they are corrected post-facto. There are also a few works that perform Decentralized SLAM that off-loads the memory and time intensive loop closure detection and map updates to the cloud~\cite{nandikolla2021navigation,kiss2019gps}. We later demonstrate that even such works can benefit from \name's design and implementation.

\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered SLAM system which overcomes the need of loop-closure detection making it memory efficient and timely.
To build a SLAM system that consumes minimal-memory and performs real-time robot navigation without any delays using the the existing visual and WiFi sensor technologies and architectures have the following limitations:

\noindent\textbf{Noisy WiFi Measurements:} WiFi measurements are not always reliable and are quite noisy for real-time and accurate navigation. While, existing $\mathrm{P^2}$SLAM demonstrates WiFi as a sensor for navigation, it performs retrospective end-to-end optimization and not real-time navigation and optimization. That is while WiFi as a sensor can provide accurate global corrections, for real-time navigation of the robot, WiFi measurements are too noisy, ambiguous and sparse.
    
\noindent \textbf{Naive Sensor Fusion:} One can solve this problem of noisy WiFi measurements by integrating more reliable existing Visual or LiDAR sensors. A naive way to integrate the WiFi and Camera systems are to integrate the WiFi measurements, like the two-way bearing measurements of $\mathrm{P^2}$SLAM into the existing Visual SLAMs as new measurements. This naive integration of bearings into VIO would make the system complex, as the WiFi sensors being more noisier than camera for local pose corrections, that the system might completely neglect WiFi measurements or worse, make incorrect local-corrections.

\subsection{\name SLAM's Solution}

To overcome these the core idea for \name SLAM's design relies on two important aspects (a) Visual sensors are accurate, does not require a lot of memory and are real-time for local drift corrections and feature mapping, and (b) WiFi sensors while sparse and noisy in smaller areas, have accurate global perspective to correct for the global drifts of the robot. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Dual Graph:} The first idea that we propose in \name SLAM is to construct a novel Visual WiFi Dual graph system, where utilizing the the VIO systems like Kimera, ORB-SLAM, or RTABMap that can provide the odometer measurements without performing any global loop closure detection. These local drift corrected odometer measurements are then sent to our WiFi graph, which utilizes these Visual Inertial Odometer (VIO) measurements in tandem with the WiFi measurements made from multiple access points in the environment, whose locations are also not known. These measurements are then combined together in a real-time navigation GraphSLAM optimization backend, for which we use the open-sourced iSAM~\cite{gtsam} toolbox. While, there are visual fiducial markers ~\cite{opencvaruco} that can also act as global constant markers that can help in global corrections with minimal memory overhead. Though, unlike WiFi sensors, visual markers can be easily blocked in a dynamic environment making them less reliable.

\noindent\textbf{(b) Accurate WiFi Measurements:} We have seen from existing works like $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} and WSR~\cite{jadhav2020wsr} that bearing measurements are robust and accurate for WiFi based SLAM algorithms. Unfortunately, the bearing measurement approach detailed in $\mathrm{P^2}$SLAM are not sufficiently accurate and the bearing measurement algorithms of WSR rely on measurements across time limiting the real-time robot navigation performance. 
While some existing bearing measurement algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide real-time AoA measurements at the rate needed for pose estimation.
Thus in \name SLAM we employ a low-compute algorithm, which reduces erroneous measurements by attenuating noisy components in the signal, by combining the WiFi channel measurements across time and finding its principle component which we call PC-CSI. 
The PC-CSI can then be fed to the 2D FFT transform we proposed in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, for more reliable and real-time bearing measurements.

\noindent\textbf{(c) Real-Time Navigation:} Finally, utilizing the locally corrected VIO's `odometer' measurements, and the sparse and more reliable PC-CSI based `bearing' measurements together to construct a factor graph, where the WiFi access point sin the environment are not known as well. So the robot's global drift corrections and the WiFi access points locations are simultaneously using an open-sourced real-time implementation of factor graph optimization backend called iSAM, where we use the VIO's odometer outputs as the measurements for the in-between factors and the robot to WiFi bearings as the WiFi measurements factors as shown in Figure~\ref{fig:wifi-factor}. Thus using these contributions \name SLAM is able to perform real-time and accurate indoor robot navigation with minimal memory requirements.

Finally, with these contributions, we have deployed our \name SLAM robot system on a Turtlebot2 that is equipped with a Hokuyo LiDAR, and Intel 455 RGB-D camera with an inbuilt IMU for deploying cartographer~\cite{cartographer}, RTABMap~\cite{Labb2018RTABMapAA}, and Kimera~\cite{rosinol2021kimera}. We also deploy a 4 antenna WiFi sensor, where the antennas are deployed as a square antennas array to avoid ambiguities, on top of the robot for measuring the bearing to the access points in the environment. We have deployed this robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs along with two of our open-sourced datasets that we use to demonstrate \name's deployability with RTABMap and Cartographer as well. Across these deployments the robot traverses for an overall time of ~\todo{xx}mins covering a distance of ~\todo{xxx} kms across a space of ~\todo{xx} sq. m. where in we show that \name achieves a median translation error of \todo{xx} m and a median orientation error of \todo{$x^{\circ}$}, on par with the state-of-the-art Kimera system with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of ~\todo{xx} MB for a ~\todo{xx} min run, wherein Kimera needs ~\todo{yy} MB. Thus \name SLAM demonstrates accurate, real-time and low-memory SLAM.

==> ViWiD SLAM_arx/intro/intro-2.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.


Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Since these Visual and LiDAR SLAM systems perform sensor fusion to provide a human-readable map and to reduce the local and global drifts introduced by the odometry sensors.
This mapping and corrections are possible by performing feature identification and feature correlation across current and past frames to re-detect the previously visited location (typically termed as `loop-closure detection').
Unfortunately, this loop-closure detection needs the SLAM system running on a robot to store all the important features (called `key-frames`) up to the current state.
This implies that the as the robot navigates in increasingly large spaces, the SLAM system running on the robot consumes increasingly more memory.
This increasing memory for SLAM would eventually leaving little for the other applications and processes, which would lead the robot to start malfunctioning or becoming extremely slow.


% the (a) The robot needs to have an active memory of all the past features of all the time, making the system limited by the active memory (typically the RAM size). 
% (b) Also as time progresses, the search time to find a matching features frame across all the past frames continues to rise.
% These issues in the best could lead to the robot just taking longer in state transition, and accidents in the worst owing to inconsistency in the current state and the predicted state, leading to incorrect state-transition decisions.

In this work, so we ask and answer the question what if we can remove these memory intensive loop-closures? 
The first key-insight we make is that the need for loop-closure detection occurs because the individual landmarks or the key-frames identified in the environment are not unique. That is each key-frame does not have a unique ID. If that were possible, it would remove the need for storing each key-frame but only its unique ID.
Whereby we note that through $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, we have demonstrated on how the WiFi routers placed in the environment can act as these unique key-frames that can perform self loop-closure detection.
Inspired from this observation in this paper, we will present our solution that integrates WiFi with visual sensors for real-time autonomous navigation that does not need memory expensive loop-closure detection.

\subsection{Literature Review}

Most of the existing Visual and LiDAR SLAM algorithms try to resolve the memory issues in loop-closure detection and identification by: (a) optimizing on the algorithms for key-frame and key-point detection~\cite{mur2015orb,rosinol2021kimera} to reduce the number of key-frames stored, or by (b) using smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions might lessen the amount of memory required per frame. But the underlying issue of every increasing memory consumption would lead to the same issues once it is used for larger or more involved spaces like warehouses.

As noted earlier, in a past work~\cite{arun2022p2slam} we demonstrated Radio Frequency(RF) technologies, especially WiFi as a navigation sensor for SLAM robots owing to the ubiquitous deployment of WiFi.
In $\mathrm{P^{2}}$SLAM, while we demonstrated accurate WiFi based SLAM, it performs only end-to-end optimization and cannot translate to real-time navigation of the robot.
There have been other works like WSR~\cite{jadhav2020wsr} that only demonstrates robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi,hashemifar2019augmenting, liu2019collaborative} depend only on WiFi readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

The other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation, like UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi and thus are limited in scalability to large spaces or ubiquitous deployment.
% \footnote{We also want to note that, while we have used WiFi as a sensor in \name, \name's design is modular enough to easily scale to other RF-technologies.}.

\todo{Aditya-- can you check the accuracy in technicalities in the following:}
Finally, there also exist a few other series of works called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel} that try to reduce the memory usage and processing time by running two different optimizations for mapping and pose-estimation in parallel which tend to drift in real-time while they are corrected post-facto. There are also a few works that perform Decentralized SLAM that off-loads the memory and time intensive loop closure detection and map updates to the cloud~\cite{nandikolla2021navigation,kiss2019gps}. We later detail on how even such works can benefit from \name's design and implementation.

\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory efficient.
To build a SLAM system that consumes minimal-memory and performs real-time robot navigation without any delays using the the existing visual and WiFi sensor technologies and architectures have the following limitations:

\noindent\textbf{(a) Noisy and sparse WiFi Measurements:} As demonstrated in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} WiFi as a SLAM sensor can provide accurate global corrections without the need of loop closure detection for end-to-end optimization. Although for real-time navigation of the robot, WiFi bearings measured from 2D-FFT are too noisy, ambiguous and sparse.

\noindent\textbf{(b) Unknown WiFi anchors:} Secondly, we do not assume any apriori knowledge of the WiFi access points(APs) in the environments, including their locations. Thus, we need to map the APs accurately, one can initialize the APs at the origin but all the APs do not have measurements with the WiFi radio on the robot leading to ill-defined optimization. Thus, optimal initialization and mapping of the WiFi APs becomes challenging.
    
\noindent \textbf{(c) Naive Sensor Fusion:} One can solve the problem of noisy WiFi measurements by integrating more reliable existing Visual or LiDAR sensors. A naive integration of bearings into existing VIO would make the system complex, as the WiFi sensors are more noisier than camera for local pose corrections, leading to the system to completely neglect WiFi measurements or worse, make incorrect local-corrections.

\subsection{\name SLAM's Solution}

To overcome these the core idea for \name SLAM's design relies on two important aspects (a) Visual sensors are accurate, does not require a lot of memory and are real-time for local drift corrections and feature mapping, and (b) WiFi sensors while sparse and noisy in smaller areas, have accurate global perspective to correct for the global drifts of the robot. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Accurate WiFi Measurements:} We have seen from existing works like $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} and WSR~\cite{jadhav2020wsr} that bearing measurements are robust and accurate for WiFi based SLAM algorithms. Unfortunately, these algorithms have more noisier bearings than are tolerable for real-time robot navigation. 
While some existing bearing measurement algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide real-time AoA measurements at the rate needed for pose estimation.
Thus in \name SLAM we employ a low-compute algorithm, which reduces erroneous measurements by attenuating noisy components in the signal, by combining the WiFi channel measurements across time and finding its principle component which we call PC-CSI. 
The PC-CSI can then be fed to the 2D FFT transform we proposed in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, for more reliable and real-time bearing measurements.

\noindent\textbf{(b) Accurate mapping of WiFi anchors:} For accurate navigation of the robot, the WiFi APs also need to be mapped accurately in the environment. Since, \name-SLAM's accurate navigation without loop closure detection relies on these unique key-frames/landmarks in the WiFi domain, as each AP is uniquely identifiable. The robot while moving around, cannot see all the APs all the time, the number of WiFi APs it can get reasonable data from is limited and thus we have to smartly initialize each AP's location, as the robot connects to one for the first time. Thus, to enable smart mapping of the WiFi APs, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an infection point in the signal strength measured for that AP. Thus, in \name we perform accurate smart AP initialization to map them accurately.

\noindent\textbf{(c) Dual Graph:} The first idea that we propose in \name SLAM is to construct a novel Visual WiFi Dual graph system, where utilizing the the VIO systems like Kimera, ORB-SLAM, or RTABMap that can provide the odometer measurements without performing any global loop closure detection. These local drift corrected odometer measurements are then sent to our WiFi graph, which utilizes these Visual Inertial Odometer (VIO) measurements in tandem with the WiFi measurements made from multiple access points in the environment, whose locations are also not known. These measurements are then combined together in a real-time navigation GraphSLAM optimization backend, for which we use the open-sourced iSAM~\cite{gtsam} toolbox. While, there are visual fiducial markers ~\cite{opencvaruco} that can also act as global constant markers that can help in global corrections with minimal memory overhead. Though, unlike WiFi sensors, visual markers can be easily blocked in a dynamic environment making them less reliable.

% \noindent\textbf{(c) Real-Time Navigation:} Finally, utilizing the locally corrected VIO's `odometer' measurements, and the sparse and more reliable PC-CSI based `bearing' measurements together to construct a factor graph, where the WiFi access point sin the environment are not known as well. So the robot's global drift corrections and the WiFi access points locations are simultaneously using an open-sourced real-time implementation of factor graph optimization backend called iSAM, where we use the VIO's odometer outputs as the measurements for the in-between factors and the robot to WiFi bearings as the WiFi measurements factors as shown in Figure~\ref{fig:wifi-factor}. Thus using these contributions \name SLAM is able to perform real-time and accurate indoor robot navigation with minimal memory requirements.

Finally, with these contributions, we have deployed our \name SLAM robot system on a Turtlebot2 that is equipped with a Hokuyo LiDAR, and Intel d455 RGB-D camera with an in-built IMU for deploying cartographer~\cite{cartographer}, \todo{RTABMap}~\cite{Labb2018RTABMapAA}, and Kimera~\cite{rosinol2021kimera}. We also deploy a 4 antenna WiFi sensor, where the antennas are deployed as a square antennas array to avoid ambiguities, on top of the robot for measuring the bearing to the access points in the environment. We have deployed this robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs along with two of our open-sourced datasets that we use to demonstrate \name's deployability with RTABMap and Cartographer as well. Across these deployments the robot traverses for an overall time of ~\todo{xx}mins covering a distance of ~\todo{xxx} kms across a space of ~\todo{xx} sq. m. where in we show that \name achieves a median translation error of \todo{xx} m and a median orientation error of \todo{$x^{\circ}$}, on par with the state-of-the-art Kimera system with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of ~\todo{xx} MB for a ~\todo{xx} min run, wherein Kimera needs ~\todo{yy} MB. Thus \name SLAM demonstrates accurate, real-time and low-memory SLAM.

==> ViWiD SLAM_arx/intro/intro-3.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Diverse indoor applications like inventory management in warehouses, last-mile delivery, and disaster relief~\cite{melenbrink2020site,lastmile} are increasingly interested in deploying autonomous robot systems.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, most current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Since these Visual (VIO) and LiDAR (LIO) SLAM systems utilize the camera frames  or LiDAR scans for sensor fusion to provide a human-readable map and to reduce the local and global drifts that are typically accrued by the odometry sensors.
To perform this, these Visual (LiDAR) sensors identify key-features/landmarks in each camera frame (Lidar scan) and track them across different robot locations.
This landmark mapping and tracking is possible by performing feature correlation across current and past frames (scans) to re-detect the previously visited location (typically termed as `loop-closure detection').

Unfortunately, this loop-closure detection needs the SLAM system running on a robot to store all the important features (called `key-frames`) up to the current state.
This implies to a trade-off as the robot navigates in increasingly large spaces: (a) On one side, the rate of memory consumption of the SLAM system running on the robot would be alarmingly high for systems with dense features (typical VIOs). (b) On the other hand, systems with sparse features, the compute starts to get occupied to enable complex feature matching algorithms (typical single plane LIOs). Additionally, since these features are not uniquely identifiable in bad lighting conditions or monotonous environments~\cite{deng2018feature,zhang2020comparison}, loop-closure detection failure can further detrimentally impact the quality of the SLAM output.

% This trade-off arising from the need of loop-closure detection limits the available memory and/or compute for the other applications and processes, which would lead the robot to start malfunctioning or becoming extremely slow.

In this work, we ask and answer the question what if we can remove these memory and/or compute intensive loop-closures? 
The first key-insight we make is that the need for loop-closure detection occurs because the individual landmarks identified in the environment are not unique. \todo{update the upcoming sentence or this paragraph, it doesn't nor does it deliver punchline...}If that were possible, it would remove the need for storing each key-frame but only its unique ID and circumvent key-frame searches.
Whereby we note that through $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, we have demonstrated on how the WiFi routers placed in the environment can act as these unique landmarks. 
Inspired from these observations, we present our solution that integrates WiFi with visual sensors for real-time autonomous navigation which removes the need for loop-closure detection.

\subsection{Literature Review}
Most of the existing Visual and LiDAR SLAM algorithms try to resolve the memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or by (b) using smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions might lessen the amount of memory required per frame, the underlying issue of ever increasing memory consumption would lead to the same issues once it is used for larger or more involved spaces like warehouses.

As noted earlier, in a past work~\cite{arun2022p2slam} while we demonstrated accurate WiFi based SLAM, it performs only end-to-end optimization and cannot translate to real-time navigation of the robot.
There have been other works like WSR~\cite{jadhav2020wsr} that only demonstrates robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

The other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation, like UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi and thus are limited in scalability to large spaces or ubiquitous deployment.
% \footnote{We also want to note that, while we have used WiFi as a sensor in \name, \name's design is modular enough to easily scale to other RF-technologies.}.

% \todo{Aditya-- can you check the accuracy in technicalities in the following:}
Finally, there also exist a few other series of works called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel} that try to reduce the memory usage and processing time by running two different optimizations for mapping and pose-estimation in parallel which tend to drift in real-time while they are corrected post-facto. There are also a few works that perform Decentralized SLAM that off-loads the memory and time intensive loop closure detection and map updates to the cloud~\cite{nandikolla2021navigation,kiss2019gps}. We later detail on how even such works can benefit from \name's design and implementation.

\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient.

To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Noisy and sparse WiFi Measurements:} As demonstrated in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, WiFi as a SLAM sensor can provide accurate global corrections without the need of loop closure detection for end-to-end optimization. Although for real-time navigation of the robot, WiFi bearings measured from 2D-FFT are too noisy, ambiguous and compute-intensive.

\noindent\textbf{(b) Unknown WiFi anchors:} Secondly, we do not assume any apriori knowledge of the WiFi access points(APs) in the environments, including their locations, and we need to map the APs accurately. One can initialize the APs at the origin but all the APs do not have measurements with the WiFi radio on the robot leading to ill-defined optimization. Thus, optimal initialization of WiFi AP's in imperative for the stability of the SLAM optimization.
    
\noindent \textbf{(c) Naive Sensor Fusion:} One can solve the problem of noisy WiFi measurements by integrating more reliable existing Visual or LiDAR sensors. A naive integration of bearings into existing VIO would make the system complex, as the WiFi sensors are more noisier than camera for local pose corrections, leading to the system to completely neglect WiFi measurements or worse, make incorrect local-corrections.

\subsection{\name SLAM's Solution}
\todo{should we call this statement of contributions?}
To overcome these challenges, the core idea for \name SLAM's design relies on two important aspects (a) Visual sensors are accurate, does not require a lot of memory and are real-time for local drift corrections and feature mapping, and (b) WiFi sensors while sparse and noisy in smaller areas, have accurate global perspective to correct for the global drifts of the robot. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots. \todo{careful to not just call A+B... }

\noindent\textbf{(a) Accurate WiFi Measurements:} We have seen from existing works like $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} and WSR~\cite{jadhav2020wsr} that bearing measurements are robust and accurate for WiFi based SLAM algorithms. Unfortunately, these algorithms have more noisier bearings than are tolerable for real-time robot navigation. 
While some existing bearing measurement algorithms like MUSIC and SpotFi~\cite{spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide real-time AoA measurements at the rate needed for pose estimation.
Thus in \name SLAM we employ a low-compute algorithm, which reduces erroneous measurements by attenuating noisy components in the signal, by combining the WiFi channel measurements across time and finding its principle component which we call PC-CSI. 
The PC-CSI can then be fed to a FFT transform~\cite{arun2022p2slam}, for more reliable and real-time bearing measurements.

\noindent\textbf{(b) Accurate mapping of WiFi anchors:} For accurate navigation of the robot, the WiFi APs also need to be mapped accurately in the environment. As discussed, a naive initialization can lead to an unstable optimization and higher compute. 
Thus, to enable dynamically map of the WiFi APs as they are seen for the first time, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an inflection point in the change of signal strength measured for that AP. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

\noindent\textbf{(c) Dual Graph:} Finally, to make best use of the WiFi and visual sensors, \name proposes to construct a Visual WiFi Dual graph system. We utilize  VIO (or LIO) systems like Kimera~\cite{rosinol2021kimera} (Cartographer~\cite{cartographer}) to provide local odometer measurements without performing any global loop closure detection. These odometer measurements are fused with WiFi measurements from multiple access points in the environment by our WiFi graph, built on open-sourced iSAM~\cite{gtsam} backend. Alternatively, visual fiducial markers ~\cite{opencvaruco} that can also act as global constant markers that can help in global corrections with minimal memory overhead. Though, unlike WiFi sensors, visual markers can be easily blocked in a dynamic environment making them less reliable. \todo{add layering}

Finally, we have deployed our \name SLAM robot system on a Turtlebot2~\cite{turtlebot2} that is equipped with a Hokuyo LiDAR,~\cite{hoku} and Intel d455 RGB-D camera with an in-built IMU for deploying cartographer~\cite{cartographer}, and Kimera~\cite{rosinol2021kimera}. We also deploy a 4 antenna WiFi sensor~\cite{blanco2021accurate}. We have deployed this robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs along with three of our open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of 108 minutes covering a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera system with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of 0.72 GB for a 25 min run, wherein Kimera needs 2.82 GB. Thus \name SLAM demonstrates accurate, real-time and low-memory SLAM. Further note that we disabled visualization on Kimera to only account for the memory consumption by the optimization backend and keyframe storage. 

==> ViWiD SLAM_arx/intro/intro-4.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Diverse indoor applications~\cite{melenbrink2020site,lastmile} are increasingly interested in deploying autonomous robot systems.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. Current state-of-the-art SLAM systems\todo{may be connect with robot or SLAM from previous sentence} like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Over time, however, fusing these measurements accrues drift in the robot poses predicted due to sensors errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{xxx} which correlate the current observation with a stored dictionary of past observation.

\todo{may be a sentence claiming loop-closures requires high computational resources and memory resources then the two sentence below explaining that point.}
But as we look towards deploying SLAM systems to larger spaces, performing adequate loop closures demands the storage of a larger dictionary of unique observation made in the environment. Furthermore, the feature matching needed to detect loop closures and performing the adequate corrections over the entire trajectory in real time demands higher computational resources. \todo{may be a connecting sentence communication} Thus, to allow for accurate, scalable and real-time SLAM systems, it is imperative to reduce memory and computational requirements of SLAM systems. Additionally, in monotonous or visually dynamic environment, incorrect feature matching can be detrimental to robot pose prediction. Hence, we ask and answer the question what if we can remove these memory and compute intensive loop-closures? 


% But performing loop closures comes at a trade-off of higher memory and compute consumption. 
% Specifically, the rate of memory consumption of the SLAM system running on the robot would be alarmingly high for systems with dense features (typical VIOs). (b) On the other hand, systems with sparse features, the compute starts to get occupied to enable complex feature matching algorithms (typical single plane LIOs). Additionally, since these features are not uniquely identifiable in bad lighting conditions or monotonous environments~\cite{deng2018feature,zhang2020comparison}, loop-closure detection failure can further detrimentally impact the quality of the SLAM output.

% This trade-off arising from the need of loop-closure detection limits the available memory and/or compute for the other applications and processes, which would lead the robot to start malfunctioning or becoming extremely slow.


\todo{this paragraph is a bit weak and slow... make it more punchy, it is long and un-clear}As the first step, we observe that loop-closures aid in re-identifying previously visited spaces and re-aligns the robot to be consistent with past pose predictions. Alternatively, if the environment could instead inform the robot of it's inconsistency, we could circumvent loop-closures entirely. To allow this, we can incorporate static landmarks in the environment with unique ID's and provide the robot definitive anchors in the environment. Interestingly, these visual landmarks exist~\cite{opencvaruco} and are commonly deployed in environments where loop-closures are insufficient to correct for drifts. Unfortunately, these visual landmarks fail in dynamic conditions, in situations of blockage and can be inconvenient to deploy in some environments. To circumvent these challenges and provide robust unqiue landmarks, we find an alternative in the form of WiFi access points~\cite{arun2022p2slam} and develop \name which integrates WiFi measurements with visual sensors for real-time SLAM. 

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem is that, since the robot must always have memories of everything it has seen on hand, memory consumption is linear in the length of the robot's trajectory, meaning that the even most efficient representations will eventually run out of space given a large or complex enough environment.

As noted earlier, in a past work~\cite{arun2022p2slam} we demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and thus was not suitable for real-time operation on a robot.
There have also been other works like WSR~\cite{jadhav2020wsr} that demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi, meaning they are limited in applicability to deployments without pre-existing localization infrastructure.
% \footnote{We also want to note that, while we have used WiFi as a sensor in \name, \name's design is modular enough to easily scale to other RF-technologies.}.

% \todo{Aditya-- can you check the accuracy in technicalities in the following:}
% Finally, there also exist a few other series of works called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel} that try to reduce the memory usage and processing time by running two different optimizations for mapping and pose-estimation in parallel which tend to drift in real-time while they are corrected post-facto. There are also a few works that perform Decentralized SLAM that off-loads the memory and time intensive loop closure detection and map updates to the cloud~\cite{nandikolla2021navigation,kiss2019gps}. We later detail on how even such works can benefit from \name's design and implementation.

\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient. To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Time-consuming, noisy and sparse WiFi Measurements:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use super-resolution algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain the low-noise bearing measurements needed for online operation. However, because these algorithms require high compute in order to differentiate signal paths, they are not suitable for deployment on devices with low compute capabilities or at large scales.

\todo{justify this instability}
\noindent \textbf{(b) Naive Sensor Fusion:} WiFi-bearings can provide robust corrections to account for global drift. But a naive integration of these WiFi-bearings into existing VIO would make the system difficult to optimize, as the WiFi sensors measurements are more noisier than cameras for local pose corrections.

\noindent\textbf{(c) Unknown WiFi anchors:} Finally, the locations of the AP's are unknown in the environment and need to be dynamically added and mapped during the operation of the robot. A poor initialization of the AP's position estimate can lead to it falling into a local minimum or the estimate becoming numerically unstable or indeterminate.

\subsection{\name's Contributions}
To overcome these challenges, the \name's core design relies on two important aspects: (a) Visual sensors can provide accurate and real-time odometry measurements at a local scale, and (b) WiFi sensors can correct global drifts in odometry, as each measurement comes pre-labeled with a MAC address, meaning no cross-correlation of measurements needs to be done. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots. \todo{careful to not just call A+B... }

\noindent\textbf{(a) Accurate WiFi Measurements:} 
We design a low-compute PCA-based WiFi-bearing estimation algorithm which can estimate the true path a WiFi signal traveled without having to search across all paths or do any super-resolution. 

\noindent\textbf{(b) Dual Graph:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual WiFi Dual graph system. We utilize  VIO~\cite{rosinol2021kimera} or LIO~\cite{cartographer} to provide local odometer measurements (without global loop closure detection). These local odometer measurements are fused with WiFi measurements from access points in the environment by our WiFi graph, built on open-sourced iSAM~\cite{gtsam} backend. We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Accurate mapping of WiFi anchors:} To dynamically map the WiFi APs as they are seen for the first time, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an inflection point in the change of signal strength measured for that AP. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

To verify our claims, we have deployed \name on a Turtlebot2~\cite{turtlebot2} that is equipped with a Hokuyo LiDAR~\cite{hoku} and Intel d455 RGB-D camera~\cite{realsense} with an in-built IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also deploy a 4 antenna WiFi sensor~\cite{blanco2021accurate}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs in addition with three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes covering a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} systems with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB. Additionally, \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name SLAM demonstrates accurate, low-compute and low-memory SLAM. Further note that we disabled visualization on Kimera and Cartographer to only account for the memory and computation by the optimization backend and keyframe storage. 

==> ViWiD SLAM_arx/intro/intro-5.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications~\cite{melenbrink2020site,lastmile} are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks for the basis to enable real-time navigation and generate a human-readable map of the robot's environment. \todo{may be connect with robot or SLAM from previous sentence}
And most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Over time, however, fusing these measurements accrues drift in the robot poses predicted due to sensors errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{xxx} which correlate the current observation with a stored dictionary of past observation.

\todo{may be a sentence claiming loop-closures requires high computational resources and memory resources then the two sentence below explaining that point.}

But as we look towards deploying SLAM systems to larger spaces, performing adequate loop closures demands the storage of a larger dictionary of unique observation made in the environment. Furthermore, the feature matching needed to detect loop closures and performing the adequate corrections over the entire trajectory in real time demands higher computational resources.  Thus, to allow for accurate, scalable and real-time SLAM systems, it is imperative to reduce memory and computational requirements of SLAM systems and move away from compute and memory intensive loop closure algorithms~\cite{arshad2021role}. Additionally, in monotonous or visually dynamic environment, incorrect feature matching can be detrimental to robot pose prediction. Hence, we ask and answer the question what if we can remove these memory and compute intensive loop-closures? 


\todo{this paragraph is a bit weak and slow... make it more punchy, it is long and un-clear}

As the first step, we observe that loop-closures aid in re-identifying previously visited spaces and re-aligns the robot to be consistent with past pose predictions. Alternatively, if the environment could instead inform the robot of it's inconsistency, we could circumvent loop-closures entirely. \todo{this statement comes too early:}To allow this, we can incorporate static landmarks in the environment with unique ID's and provide the robot definitive anchors in the environment. Interestingly, these visual landmarks exist~\cite{opencvaruco} and are commonly deployed in environments where loop-closures are insufficient to correct for drifts. Unfortunately, these visual landmarks fail in dynamic conditions, in situations of blockage and can be inconvenient to deploy in some environments. To circumvent these challenges and provide robust unqiue landmarks, we find an alternative in the form of WiFi access points~\cite{arun2022p2slam} and develop \name which integrates WiFi measurements with visual sensors for real-time SLAM. 

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem is that, since the robot must always have memories of everything it has seen on hand, memory consumption is linear in the length of the robot's trajectory, meaning that the even most efficient representations will eventually run out of space given a large or complex enough environment.

As noted earlier, in a past work~\cite{arun2022p2slam} we demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and thus was not suitable for real-time operation on a robot.
There have also been other works like WSR~\cite{jadhav2020wsr} that demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi, meaning they are limited in applicability to deployments without pre-existing localization infrastructure.


\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient. To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Time-consuming, noisy and sparse WiFi Measurements:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use super-resolution algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain the low-noise bearing measurements needed for online operation. However, because these algorithms require high compute in order to differentiate signal paths, they are not suitable for deployment on devices with low compute capabilities or at large scales.

\noindent \textbf{(b) Naive Sensor Fusion:} WiFi-bearings can provide robust corrections to account for global drift. But a naive integration of these WiFi-bearings into existing VIO would make the system difficult to optimize, as the WiFi sensors measurements are more noisier than cameras for local pose corrections. This leads to indeterminancy of the factor graph and higher compute times. 

\noindent\textbf{(c) Unknown WiFi anchors:} Finally, the locations of the AP's are unknown in the environment and need to be dynamically added and mapped during the operation of the robot. A poor initialization of the AP's position estimate can lead to it falling into a local minimum or the estimate becoming numerically unstable or indeterminate.

\subsection{\name's Contributions}
To overcome these challenges, the \name's core design relies on two important aspects: (a) Visual sensors can provide accurate and real-time odometry measurements at a local scale, and (b) WiFi sensors can correct global drifts in odometry, as each measurement comes pre-labeled with a MAC address, meaning no cross-correlation of measurements needs to be done. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots. \todo{careful to not just call A+B... }

\noindent\textbf{(a) Accurate WiFi Measurements:} 
We design a low-compute PCA-based WiFi-bearing estimation algorithm which can estimate the true path a WiFi signal traveled without having to search across all paths or do any super-resolution. 

\noindent\textbf{(b) Dual Graph:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual WiFi Dual graph system. We utilize  VIO~\cite{rosinol2021kimera} or LIO~\cite{cartographer} to provide local odometer measurements (without global loop closure detection). These local odometer measurements are fused with WiFi measurements from access points in the environment by our WiFi graph, built on open-sourced iSAM~\cite{gtsam} backend. We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Accurate mapping of WiFi anchors:} To dynamically map the WiFi APs as they are seen for the first time, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an inflection point in the change of signal strength measured for that AP. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

To verify our claims, we have deployed \name on a Turtlebot2~\cite{turtlebot2} that is equipped with a Hokuyo LiDAR~\cite{hoku} and Intel d455 RGB-D camera~\cite{realsense} with an in-built IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also deploy a 4 antenna WiFi sensor~\cite{blanco2021accurate}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs in addition with three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes covering a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} systems with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB. Additionally, \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name SLAM demonstrates accurate, low-compute and low-memory SLAM. Further note that we disabled visualization on Kimera and Cartographer to only account for the memory and computation by the optimization backend and keyframe storage. 

==> ViWiD SLAM_arx/intro/intro-6.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications~\cite{melenbrink2020site} are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks to enable real-time navigation and generate a human-readable map of the robot's environment.
And most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Over time, however, fusing these measurements accrues drift in the robot poses predicted due to sensors errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{arshad2021role} which correlate the current observation with a stored dictionary of past observation.

Unfortunately, these much-needed loop-closures are also the components of SLAM system that increase the memory and compute requirements for these robots.
That is, as we look towards deploying SLAM systems to larger spaces, performing adequate loop closures demands the storage of a larger dictionary of unique observations made during past traversal of the environment (memory usage). Furthermore, the feature matching needed to detect loop closures to perform adequate corrections over the entire trajectory in real time, demands running matching algorithm over a large database of past key points leading to high computational resources (cpu intensive). Thus, to allow for accurate, and easy to  scale real-time SLAM systems, it is imperative to reduce the memory and computational requirements of SLAM systems and possibly move away from compute and memory-intensive loop closure algorithms~\cite{arshad2021role}. Additionally, in a monotonous or visually dynamic environment, incorrect feature matching can be detrimental to robot pose prediction. Hence, we ask and answer the question what if we can remove these memory and compute intensive loop-closures? 
A key observation is that the only purpose of the memory and compute intense loop-closures is to aid in re-identifying previously visited spaces and re-align the robot to be consistent with past pose predictions. So, we tackle this issue in \name by developing a system that can smartly overcome the need for these loop-closures and mitigate the mo.
One way to do this is to incorporate static landmarks in the environment with unique ID's and provide the robot definitive anchors in the environment. Interestingly, these visual landmarks exist~\cite{opencvaruco} and are commonly deployed in environments where loop-closures are insufficient to correct for drifts. Unfortunately, these visual landmarks fail in dynamic conditions, in situations of blockage and can be inconvenient to deploy in some environments. To circumvent these challenges and provide robust unique landmarks, we find an alternative in WiFi-sensors measurements and develop \name which integrates them with visual sensors for accurate and real-time SLAM. 

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem is that, since the robot must always have memories of everything it has seen on hand, memory consumption is linear in the length of the robot's trajectory, meaning that the even most efficient representations will eventually run out of space given a large or complex enough environment.

As noted earlier, in a past work~\cite{arun2022p2slam} we demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and thus was not suitable for real-time operation on a robot.
There have also been other works like WSR~\cite{jadhav2020wsr} that demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi, meaning they are limited in applicability to deployments without pre-existing localization infrastructure.


\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient. To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Time-consuming, noisy and sparse WiFi Measurements:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use super-resolution algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain the low-noise bearing measurements needed for online operation. However, because these algorithms require high compute in order to differentiate signal paths, they are not suitable for deployment on devices with low compute capabilities or at large scales.

\noindent \textbf{(b) Naive Sensor Fusion:} WiFi-bearings provide robust corrections to account for global drift. But a naive fusion of these bearings into existing VIO~\cite{rosinol2021kimera} would make the system difficult to optimize, as the WiFi sensors measurements are more noisier than cameras', for local pose corrections. This may lead to higher compute or an indeterminant factor graph. 

\noindent\textbf{(c) Unknown WiFi anchors:} Finally, the locations of the AP's are unknown in the environment and need to be dynamically added and mapped during the operation of the robot. A poor initialization of the AP's position estimate can lead to it falling into a local minimum or the estimate becoming numerically unstable or indeterminate.

\subsection{\name's Contributions}
To overcome these challenges, the \name's core design relies on two modules to function appropriately: (a) a Visual sensor module that can provide accurate and real-time odometry measurements at a local scale, and (b) and a WiFi sensor module that can in real-time correct global drifts in odometry. While $\mathrm{P^2}$SLAM shows that as each WiFi measurement comes pre-labeled with a MAC address, no cross-correlation of measurements needs to be done but it cannot perform real-time navigation~\cite{arun2022p2slam} and so cannot be deployed. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Accurate WiFi Measurements:} 
We design a low-compute PCA-based WiFi-bearing estimation algorithm which can estimate the true path a WiFi signal traveled without having to search across all paths or do any super-resolution. 

\noindent\textbf{(b) Dual Graph:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual-WiFi Dual graph system. We utilize  VIO~\cite{rosinol2021kimera} or LIO~\cite{cartographer} to provide local odometer measurements (without global loop closure detection). These local odometer measurements are fused with WiFi measurements from access points in the environment by our WiFi graph, built on open-sourced iSAM~\cite{gtsam} backend. We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Accurate mapping of WiFi anchors:} To dynamically map the WiFi APs as they are seen for the first time, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an inflection point in the change of signal strength measured for that AP. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

To verify our claims, we have deployed \name on a ground robot Turtlebot2 platform that is equipped with a Hokuyo LiDAR and Intel d455 RGB-D camera with a built-in IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also deploy a 4 antenna WiFi channel sensor~\cite{nexmon:project}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs (with loop-closures turned off) in addition with three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes and a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} systems with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB. Additionally, \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average, showing \name can perform accurate, low-compute and low-memory SLAM. Further note that we disabled visualization tools on Kimera and Cartographer to only account for the memory and computate used by the optimization backend and keyframe storage.

==> ViWiD SLAM_arx/intro/intro7.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks to enable real-time navigation and generate a human-readable map of the robot's environment.
To enable these applications, most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Over time, however, fusing these measurements accrues drift in the robot poses predicted due to sensors errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{arshad2021role} which correlate the current observation with a stored dictionary of past observations to ensure consistency of the robot's trajectory over long periods of time.

Unfortunately, these much-needed loop-closures are also weakest links in SLAM systems and increase the memory requirements and are compute intensive as they are not robust.
In a monotonous or visually dynamic environment, many false-positive loop closures can be detrimental to robot pose predictions. Furthermore, as we look towards deploying SLAM systems to larger spaces, performing loop closures demands the storage of an ever-larger dictionary of unique observations made during past traversal of the environment, demanding higher memory usage. Additionally, the feature matching needed to discover loop closures in real time demands running a cross-correlation algorithm over a large database of past key points leading to high compute requirements. Thus, to allow for accurate and scalable real-time SLAM systems, it is imperative to reduce their memory and compute requirements, and ideally move away from compute and memory-intensive loop closure algorithms~\cite{arshad2021role}.  Hence, we explore if these loop closures can be entirely removed while maintaining SLAM accuracy. 
% \todo{maybe saying "how to remove loop-closures while maintaining accuracies" might sound better?}
% \todo{should we make these two purpose eliminate loop closure and help monotonous envrionments?}

% \todo{From the how question above, maybe you can relate to saying that, "to be able to remove we first understand that loop-closures are only used for...". Then the WiFi part becomes more of a key observation in terms of robustly removing loop-closures.}
To develop a SLAM system without loop closures, we need to find an alternative method to re-identify previously visited spaces and make the current pose estimate consistent with past estimates in that space.
Incorporating static and \textit{uniquely identifiable} landmarks in the environment aids in re-identifying previously visited spaces. Furthermore, \textit{accurately mapping} their positions allows the robot to leverage these landmarks to anchor itself to the environment and hence circumvent loop closures. Various static landmarks which are identifiable by cameras~\cite{olson2011apriltag} or LiDARs~\cite{huang2021lidartag} have been deployed where loop closures are insufficient to correct for drifts.  
Unfortunately, these visual landmarks can fail in dynamic conditions, in situations of blockage, or in dynamic lighting conditions and are inconvenient or impossible to deploy in some environments. 

\todo{reword the following as Problem statement:}
\noindent\textbf{Problem Statement:} To circumvent these challenges in providing unique landmarks, in this work, we demonstrate that WiFi access points are a robust replacement to these visual landmarks and can aid in removing `loop-closures'. 
% To circumvent these challenges in providing unique landmarks, we find a better alternative in WiFi access points as these landmarks by making a key observation -- WiFi measurements are robust to the environmental changes which detrimentally affect these specialized landmarks. 
Hence, to capitalize on these WiFi sensors, we develop \name which integrates them with visual sensors for accurate and resource-efficient SLAM without relying on loop closures.

% \todo{tie it back to loop closures?}. 

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem is that, since the robot must always have memories of everything it has seen on hand, memory consumption is linear in the length of the robot's trajectory, meaning that the even most efficient representations will eventually run out of space given a large or complex enough environment.

In a past work~\cite{arun2022p2slam},   demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and thus was not suitable for real-time operation on a robot.
There have also been other works like WSR~\cite{jadhav2020wsr} that demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi, meaning they are limited in applicability to deployments without pre-existing localization infrastructure.


\subsection{Challenges}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient. To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Tradeoff between WiFi Measurement accuracy and compute:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use super-resolution algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain the low-noise bearing measurements needed for online operation. However, because these algorithms require high compute in order to differentiate signal paths, they are not suitable for deployment on devices with low compute capabilities or at large scales.

\todo{call it scalability? Compatibility? Bring out how we are actually not only solving loop-closures but also aiding the existing VIO/LIO systems to remove their `loop-closures' making existing works accurate with low-compute and memory.}
\noindent \textbf{(b) Naive Sensor Fusion:} Utilizing WiFi access points as landmarks provide robust corrections to account for global drift. But a naive fusion of these WiFi measurements into existing VIO~\cite{rosinol2021kimera} would make the system difficult to optimize, as they are more noisier than cameras' feature tracking for local pose corrections. This may lead to higher compute or an indeterminant factor graph. 

\todo{Strengthen the following: The AP location are not known, and adding them without a good prior would make the system instable needing heavy compute and worse making the system indeterminate.}
\noindent\textbf{(c) Unknown WiFi anchors:} Finally, the locations of the AP's are unknown in the environment and need to be dynamically added and mapped during the operation of the robot. A poor initialization of the AP's position estimate can lead to it falling into a local minimum or the estimate becoming numerically unstable or indeterminate.

\subsection{\name's Contributions}
To overcome these challenges, \name's core design relies on two modules to function appropriately: (a) a Visual sensor module that can provide accurate and real-time odometry measurements at a local scale, and (b) and a WiFi sensor module that can in real-time correct global drifts in odometry. 
Using these insights, we make the following contributions to enable accurate, real-time indoor navigation for robots.

% While $\mathrm{P^2}$SLAM shows that as each WiFi measurement comes pre-labeled with a MAC address, no cross-correlation of measurements needs to be done but it cannot perform real-time navigation~\cite{arun2022p2slam} and so cannot be deployed. 


\noindent\textbf{(a) Accurate WiFi Measurements:} 
We design a low-compute PCA-based WiFi-bearing estimation algorithm which can estimate the true path a WiFi signal traveled without having to search across all paths or do any super-resolution. 

\noindent\textbf{(b) Dual Graph:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual-WiFi Dual graph system. We utilize local odometry measurements (without global loop closure detection) extracted via inertial sensors and visual feature tracking. These local odometer measurements are then fused with WiFi measurements to tracking the WiFi landmarks in the environment by our WiFi graph. We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Accurate initialization of WiFi landmarks:} Finally, to dynamically map these WiFi landmarks as they are seen for the first time, we track the signal strength of WiFi measurement to that AP. Next, we initialize the APs location to the robot's current location when we see an inflection point in the change of signal strength measured. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

To verify our claims, we have deployed \name on a ground robot Turtlebot2 platform that is equipped with a Hokuyo LiDAR and Intel d455 RGB-D camera with an in-built IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also deploy a 4 antenna WiFi sensor~\cite{nexmon:project}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs (with loop-closures turned off) in addition with three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes and a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} systems with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB. Additionally, \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name SLAM demonstrates accurate, low-compute and low-memory SLAM. Further note that we disabled visualization on Kimera and Cartographer to only account for the memory and computation by the optimization backend and keyframe storage. 

==> ViWiD SLAM_arx/intro/intro8.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

% \todo{summarize loop closures quickly, talk about real-timeliness and working with existing works; combine 1st and 3rd para; talk abut making more systems work of smaller computers }
Diverse indoor applications are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks to enable real-time navigation and to generate a human-readable map of the robot's environment.
To enable these applications, most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Despite this fusion, error in the predicted trajectory increases over time due to accumulation of sensor errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{arshad2021role} which correlate the current observation with a dictionary of past observations, ensuring self-consistency of the robot's estimated trajectory on a global scale.

Unfortunately, these much-needed loop-closures are also the weakest links in SLAM systems, as they increase the memory requirements, are compute intensive, and are not robust~\cite{arshad2021role}.
In particular, false-positive loop closures, common in monotonous or visually dynamic environments, are highly detrimental to robot pose predictions. Furthermore, as we scale to larger spaces, performing loop closures demands the storage of an ever-larger dictionary of unique observations, demanding higher memory usage. Consequently, the feature matching needed to discover loop closures in large spaces requires extensive search, leading to high compute requirements. Thus, for real-time SLAM systems to be both accurate and scalable, it is imperative they are resource-efficient. Hence, we explore if these resource consuming loop closures can be entirely removed while maintaining SLAM accuracy.

% \todo{we don't technically do re-identification}
To develop a SLAM system without loop closures, we need to find an alternative method to re-identify previously visited spaces and make the current pose estimate consistent with past estimates in that space.
Incorporating static and \textit{uniquely identifiable} landmarks in the environment aids in re-identifying previously visited spaces. Furthermore, \textit{accurately mapping} their poses allows the robot to leverage these landmarks to anchor its estimate to the environment and circumvent loop closures. Accordingly, various static landmarks which are identifiable by cameras~\cite{olson2011apriltag} or LiDARs~\cite{huang2021lidartag} have been deployed where loop closures are insufficient to correct for drifts.  
Unfortunately, these visual landmarks can fail in situations of blockage or dynamic lighting conditions. Their deployment further scales poorly to large environments. 

\noindent\textbf{Goal:} Clearly, to deliver a resource-efficient and real-time SLAM system, we need to incorporate `uniquely identifiable' and `mappable' landmarks in our environments. These landmarks need to be robust in dynamic environments and easily scalable to large spaces.  

To achieve this goal, we demonstrate that WiFi access points are a robust replacement to these visual landmarks and can aid in removing `loop-closures'. We develop \name which integrates them with visual sensors for accurate and resource-efficient SLAM without relying on loop closures. \name is also readily scalable, as WiFi access points are already ubiquitously deployed in indoor environments making them a natural choice for a landmark.

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem of the memory consumption being linear in the length of the robot's trajectory remains. This implies that even the most efficient representations will eventually run out of memory given a large or complex enough environment.

% \todo{this takes away novelty here, don't force loop closure as much, but the timeliness}
Past work~\cite{arun2022p2slam} demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and cannot perform online robot operation.
There are also works like WSR~\cite{jadhav2020wsr}, which demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are unreliable in dynamic indoor scenarios~\cite{ma2019wifi} and require a-priori fingerprinting data for navigation.

% \todo{this is deviating, maybe move it above after the goal para?} 
Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF-sensors are \textbf{(a)} not as ubiquitously deployed limiting wider adoption or \textbf{(b)} have shorter ranges compared to WiFi limiting their scalability to large spaces. 

\subsection{Challenges}
% \todo{convert to problem/solution format }
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it resource efficient. To build \name, we surmount the following challenges:

\noindent\textbf{(a) Tradeoff between WiFi measurement accuracy and compute:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use \textit{super-resolution} algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain low-noise bearing measurements needed for online operation. However, this accuracy comes at the cost of computation, and are not suitable for realt-time deployment on devices with low compute capabilities.

% \todo{call it scalability? Compatibility? Bring out how we are actually not only solving loop-closures but also aiding the existing VIO/LIO systems to remove their `loop-closures' making existing works accurate with low-compute and memory.}
% \todo{single factor graph does not make sense, why is multiple bad?}
\noindent \textbf{(b) Infeasible sensor fusion via a single factor graph:} Most sensor-fusion techniques rely on incorporating measurements within factor graphs~\cite{gtsam} to optimally solve for the SLAM problem. Unfortunately, WiFi is subject to outlier measurements due to transient reflections, so immediate incorporation of every measurement can hurt the local state estimate. Hence, a simple integration of WiFi landmarks into the same framework as a Visual/LiDAR sensor~\cite{rosinol2021kimera} can lead to a poor estimate of the recent robot poses due to local inconsistency in WiFi measurements.
% Utilizing WiFi access points as landmarks provide robust corrections to account for global drift. But a naive fusion of these WiFi measurements into existing VIO~\cite{rosinol2021kimera} would make the system difficult to optimize, as they are more noisier than cameras' feature tracking for local pose corrections. This may lead to higher compute or an indeterminant factor graph. 

% \todo{Strengthen the following: The AP location are not known, and adding them without a good prior would make the system instable needing heavy compute and worse making the system indeterminate.}
\noindent\textbf{(c) Initialization of Unknown WiFi anchors:} As new landmarks, visual or WiFi-based, are discovered, they need to be accurately placed in the map to ensure stable convergence of the factor graph. 
This task is easy in the case of visual markers'~\cite{olson2011apriltag, huang2021lidartag} owing to the pixel-scale accuracy of cameras and LiDARs. Unfortunately, the poorer resolution offered by WiFi measurements makes initialization of the AP's position estimate in the environment nontrivial. A poor initialization can lead to the non-optimal state estimate or worse, an indeterminacy in the solution. 

\subsection{\name's Contributions}
% \todo{mention what VIO contains, the sensors it utilizes}
To overcome these challenges, \name deploys a bifurcated design: (a) a third-party visual-inertial odometry (VIO) module that can provide accurate and real-time odometry measurements at a local scale, and (b) and a WiFi sensor module that can plugs into an existing VIO system and performs online correction of global drifts.
Using these insights, we make the following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Accurate and compute-efficient WiFi Measurements:} 
\name breaks away from the accuracy-compute tradeoff by designing a PCA-based WiFi Bearing (PCAB) estimation algorithm. By adequately combining WiFi measurements over time to suppress noise, PCAB circumvents compute intensive super resolution algorithms whilst delivering accurate and real-time bearing estimates.

\noindent\textbf{(b) Extensible dual graph optimization:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual-WiFi Dual graph system. We utilize local odometry measurements (without global loop closure detection) extracted via inertial sensors and visual feature tracking. These local odometry measurements are then fused with WiFi measurements to track the WiFi landmarks in the environment by our WiFi graph. This dual-graph approach further allows robots to plug-and-play \name into the existing Visual/LiDAR SLAM systems whilst reducing their compute and memory consumption. 
% We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Smart initialization of WiFi landmarks:} Finally, to dynamically map these WiFi landmarks when they are first observed, the robot tracks the strength of the WiFi signal from the access point (AP). Next, we initialize the APs location close to the robot's current location when we see an inflection point in the change of signal strength measured. This allows us to initialize the AP close to its true location, which improves the convergence of the factor graph. 

% \todo{too many details and no takeaway, bring in abstract}
% \todo{add some system level contributions; like cartographer could not be run on rpi; increases the run time of kimera on rpi due to memory savings etc.}
To verify our claims, we have deployed \name on a ground robot TurtleBot2 platform that is equipped with a Hokuyo LiDAR and Intel Realsense D455 RGB-D camera with a built-in IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also equip it with a 4 antenna WiFi radio~\cite{nexmon:project}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs (with loop-closures turned off), \textit{in addition} to three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with LiDAR-inertial odometry (LIO) from Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes and a distance of $1625$ m. 
% \todo{show that this works on COTS devices, does not come out}
We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer}. While achieving a similar navigation accuracy: (a) \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB, (b) \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name demonstrates accurate, low-compute and low-memory SLAM.  


==> ViWiD SLAM_arx/intro/intro9.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

\todo{summarize loop closures quickly, talk about real-timeliness and working with existing works; combine 1st and 3rd para; talk abut making more systems work of smaller computers }
Diverse indoor applications are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks to enable real-time navigation and to generate a human-readable map of the robot's environment.
To enable these applications, most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Despite this fusion, error in the predicted trajectory increases over time due to accumulation of sensor errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{arshad2021role} which correlate the current observation with a dictionary of past observations, ensuring self-consistency of the robot's estimated trajectory on a global scale.

Unfortunately, these much-needed loop-closures are also the weakest links in SLAM systems, as they increase the memory requirements, are compute intensive, and are not robust~\cite{arshad2021role}.
In particular, false-positive loop closures, common in monotonous or visually dynamic environments, are highly detrimental to robot pose predictions. Furthermore, as we scale to larger spaces, performing loop closures demands the storage of an ever-larger dictionary of unique observations, demanding higher memory usage. Consequently, the feature matching needed to discover loop closures in large spaces requires extensive search, leading to high compute requirements. Thus, for real-time SLAM systems to be both accurate and scalable, it is imperative they are resource-efficient. Hence, we explore if these resource consuming loop closures can be entirely removed while maintaining SLAM accuracy.

\todo{we don't technically do re-identification}
To develop a SLAM system without loop closures, we need to find an alternative method to re-identify previously visited spaces and make the current pose estimate consistent with past estimates in that space.
Incorporating static and \textit{uniquely identifiable} landmarks in the environment aids in re-identifying previously visited spaces. Furthermore, \textit{accurately mapping} their poses allows the robot to leverage these landmarks to anchor its estimate to the environment and circumvent loop closures. Accordingly, various static landmarks which are identifiable by cameras~\cite{olson2011apriltag} or LiDARs~\cite{huang2021lidartag} have been deployed where loop closures are insufficient to correct for drifts.  
Unfortunately, these visual landmarks can fail in situations of blockage or dynamic lighting conditions. Their deployment further scales poorly to large environments. 

\noindent\textbf{Goal:} Clearly, to deliver a resource-efficient and real-time SLAM system, we need to incorporate `uniquely identifiable' and `mappable' landmarks in our environments. These landmarks need to be robust in dynamic environments and easily scalable to large spaces.  

To achieve this goal, we demonstrate that WiFi access points are a robust replacement to these visual landmarks and can aid in removing `loop-closures'. We develop \name which integrates them with visual sensors for accurate and resource-efficient SLAM without relying on loop closures. \name is also readily scalable, as WiFi access points are already ubiquitously deployed in indoor environments making them a natural choice for a landmark.

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem of the memory consumption being linear in the length of the robot's trajectory remains. This implies that even the most efficient representations will eventually run out of memory given a large or complex enough environment.

\todo{this takes away novelty here, don't force loop closure as much, but the timeliness}
Past work~\cite{arun2022p2slam} demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and cannot perform online robot operation.
There are also works like WSR~\cite{jadhav2020wsr}, which demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are unreliable in dynamic indoor scenarios~\cite{ma2019wifi} and require a-priori fingerprinting data for navigation.

\todo{this is deviating, maybe move it above after the goal para?} Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF-sensors are \textbf{(a)} not as ubiquitously deployed limiting wider adoption or \textbf{(b)} have shorter ranges compared to WiFi limiting their scalability to large spaces. 

\subsection{Challenges}
\todo{convert to problem/solution format }
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it resource efficient. To build \name, we surmount the following challenges:

\noindent\textbf{(a) Tradeoff between WiFi measurement accuracy and compute:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use \textit{super-resolution} algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain low-noise bearing measurements needed for online operation. However, this accuracy comes at the cost of computation, and are not suitable for realt-time deployment on devices with low compute capabilities.

% \todo{call it scalability? Compatibility? Bring out how we are actually not only solving loop-closures but also aiding the existing VIO/LIO systems to remove their `loop-closures' making existing works accurate with low-compute and memory.}
\todo{single factor graph does not make sense, why is multiple bad?}
\noindent \textbf{(b) Infeasible sensor fusion via a single factor graph:} Most sensor-fusion techniques rely on incorporating measurements within factor graphs~\cite{gtsam} to optimally solve for the SLAM problem. Unfortunately, WiFi is subject to outlier measurements due to transient reflections, so immediate incorporation of every measurement can hurt the local state estimate. Hence, a simple integration of WiFi landmarks into the same framework as a Visual/LiDAR sensor~\cite{rosinol2021kimera} can lead to a poor estimate of the recent robot poses due to local inconsistency in WiFi measurements.
% Utilizing WiFi access points as landmarks provide robust corrections to account for global drift. But a naive fusion of these WiFi measurements into existing VIO~\cite{rosinol2021kimera} would make the system difficult to optimize, as they are more noisier than cameras' feature tracking for local pose corrections. This may lead to higher compute or an indeterminant factor graph. 

% \todo{Strengthen the following: The AP location are not known, and adding them without a good prior would make the system instable needing heavy compute and worse making the system indeterminate.}
\noindent\textbf{(c) Initialization of Unknown WiFi anchors:} As new landmarks, visual or WiFi-based, are discovered, they need to be accurately placed in the map to ensure stable convergence of the factor graph. 
This task is easy in the case of visual markers'~\cite{olson2011apriltag, huang2021lidartag} owing to the pixel-scale accuracy of cameras and LiDARs. Unfortunately, the poorer resolution offered by WiFi measurements makes initialization of the AP's position estimate in the environment nontrivial. A poor initialization can lead to the non-optimal state estimate or worse, an indeterminacy in the solution. 

\subsection{\name's Contributions}
\todo{mention what VIO contains, the sensors it utilizes}
To overcome these challenges, \name deploys a bifurcated design: (a) a third-party visual-inertial odometry (VIO) module that can provide accurate and real-time odometry measurements at a local scale, and (b) and a WiFi sensor module that can plugs into an existing VIO system and performs online correction of global drifts.
Using these insights, we make the following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Accurate and compute-efficient WiFi Measurements:} 
\name breaks away from the accuracy-compute tradeoff by designing a PCA-based WiFi Bearing (PCAB) estimation algorithm. By adequately combining WiFi measurements over time to suppress noise, PCAB circumvents compute intensive super resolution algorithms whilst delivering accurate and real-time bearing estimates.

\noindent\textbf{(b) Extensible dual graph optimization:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual-WiFi Dual graph system. We utilize local odometry measurements (without global loop closure detection) extracted via inertial sensors and visual feature tracking. These local odometry measurements are then fused with WiFi measurements to track the WiFi landmarks in the environment by our WiFi graph. This dual-graph approach further allows robots to plug-and-play \name into the existing Visual/LiDAR SLAM systems whilst reducing their compute and memory consumption. 
% We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Smart initialization of WiFi landmarks:} Finally, to dynamically map these WiFi landmarks when they are first observed, the robot tracks the strength of the WiFi signal from the access point (AP). Next, we initialize the APs location close to the robot's current location when we see an inflection point in the change of signal strength measured. This allows us to initialize the AP close to its true location, which improves the convergence of the factor graph. 

\todo{too many details and no takeaway, bring in abstract}
\todo{add some system level contributions; like cartographer could not be run on rpi; increases the run time of kimera on rpi due to memory savings etc.}
To verify our claims, we have deployed \name on a ground robot TurtleBot2 platform that is equipped with a Hokuyo LiDAR and Intel Realsense D455 RGB-D camera with a built-in IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also equip it with a 4 antenna WiFi radio~\cite{nexmon:project}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs (with loop-closures turned off), \textit{in addition} to three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with LiDAR-inertial odometry (LIO) from Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes and a distance of $1625$ m. 
\todo{show that this works on COTS devices, does not come out}
We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer}. While achieving a similar navigation accuracy: (a) \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB, (b) \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name demonstrates accurate, low-compute and low-memory SLAM.  


==> ViWiD SLAM_arx/intro/intros_old/intro1.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

A strong need for automation in various industries spanning hospitality to security has led to an increased adoption of robots capable of autonomous, reliable and safe indoor navigation. The trend kick-started by the early adoption of automated vacuum cleaners has grown many-fold to use these robots for monitoring security in office spaces, serving patrons at restaurants and moving large equipment in hospitals. The autonomy, reliability and safety these robots boast is owed to the suite of sensors they use. Most autonomous robots can be commonly spotted sporting 
1. a LiDAR at the top to provide a 360-degree view, 
2. a stereo/RGBD camera facing forward to provide a detailed 3D-map, 
3. bumper sensors to avoid catastrophic collisions,
4. odometry sensors (wheel encoder and IMU) to provide high-resolution odometry data, and
5. GPS/GNSS to aid in locating the robot (outdoor only) in a global frame. 
The data from these sensors are expertly fused taking into consideration each sensors reliability within a back-end optimization framework to generate an accurate estimate of the robot's location and its relation to the environment around it. The fusion of these different sensing modalities provides a very robust solution for autonomous navigation for robots.

% let's see how good sensor fusion works; explain landmarks, features, loop closure in few sentences...
To achieve autonomous navigation, the first key step is for the robot to build a map of it's environment and localize itself within this map in real time. 
Furthermore, this map should consist of rich contextual data -- labels of room numbers, descriptions of spaces, markings for various exits and entrances of buildings. 
This problem is commonly called Simultaneous Localization and Mapping (SLAM). 
In a two-step process, which involves first extracting and tracking the characteristic features from visual sensors, and second, combining the data from these sensors with odometry, the robot can build an accurate map and localize itself within this map. The characteristic features (\textit{landmarks}) extracted generally include corners or edges in Camera images or LiDAR scans. Tracking these features provides corrections to errors accumulated by odometry sensors, and saving some of the salient features helps the robot recognize and create additional constraints (\textit{loop-closures}) with previously visited places. Through this two-step process, robots can effectively navigate the strengths and weaknesses of individual sensors to solve the SLAM problem.

% but this fails in monotonous envs ...\todo{because of the same reasons we have mentioned in P2SLAM}
Unfortunately, in indoor environments we observe gaps left behind this common suite of sensors generally employed on robots. LiDAR's, although great in providing an accurate point cloud of an environment, fail in environments with little structural features, like long corridors or spaces larger than the field of view of the LiDAR. Furthermore, they are expensive, bulky and power hungry. Stereo or RGBD cameras offer an advantage over LiDAR's in that they allow for finer feature detection. For example, a long corridor adorned with posters and paintings provide robust and recognizable features to track against. Unfortunately, motion blur, dynamic lighting conditions and monotonous visual environments can all lead to feature tracking failure and even false positive loop closure hypothesis.
Furthermore, viable distances to obtain accurate depth from RGBD/Stereo sensor range from \todo{xx} m - \todo{xx} m, making them unusable in large spaces. 
Discounting the LiDAR's and cameras in these challenging environments leaves us with two remaining sensors -- odometry sensors and GPS. A combination of wheel encoders and IMU's provide accurate change in position over \todo{a local region and time}
% a period of few minutes. 
Unfortunately, lacking the \todo{global} correction provided by visual sensors, these odometry sensors can accrue large drifts, in the order of many tens of meters, when traversing large distances of hundreds of meters. In outdoor environments, we have the advantage of falling back on GPS location information, accurate to a few meters, to correct for these large drifts in odometry \todo{at a global scale}. Unfortunately, this is not the case in indoor environments, where GPS information is scantly available. This leaves an open problem for autonomous navigation for indoor robotics -- what is the best sensor we could incorporate to fill in the gaps left by these multitude of sensors? 

% bring up and kill other sensors, distill to wifi, rebuff it after a better lit review ...
To answer this pressing question, we can in fact take inspiration from GPS. Using a network of satellites, GPS can position a GPS-capable device to within a few meters with a global frame of reference. This can help to correct for drifts accumulated due to odometry and incorrect measurements from visual sensors \todo{within the local frames}. In this vein, we observe that an alternative signal is abundant indoors -- RF-signals like Bluetooth, Ultrawide-band (UWB) or WiFi. RF-based sensing can provide, in a loose sense, replace GPS and many recent works have proposed the use RF-based sensing to fill the gaps left by visual sensors. VIRAL SLAM~\cite{nguyen2021viral} uses UWB based ranging in conjunction with LiDAR's, cameras and IMU's to develop a tightly coupled and robust 3D drone based localization and mapping. \todo{not strong enough: Unfortunately, the deployment of various UWB anchors in the environment limits the adoption of this solution}. \todo{kill radar: Why?} The systems proposed in \cite{sato2019rapid, jadidi2018radio} use range information extracted from BLE's received signal strength to correct for drifts accrued by the onboard IMU. Unfortunately, RSSI-based systems have been proven to be inadequate to changing environment conditions and hence act as a poor proxy to range. RFly~\cite{ma2017drone} takes advantage of  RFID tags attached in the environment as robust landmarks, and in conjunction with RFID readers deployed in the environment, jointly estimates the location of a drone and these RFID tags. In a similar vein, Rover~\cite{zhang2020robot} uses WiFi backscatter tags placed in the environment to jointly estimate the location of the robot and tags. Unfortunately, these tags have small range and these systems would require a dense deployment of tags to work, scaling poorly to large environments and requiring a high cost of deployment. The final RF based sensing briefly touched upon before is WiFi. It provides inherent advantages due to its long range and ubiquitous deployment both in the environment and on most robots. 

% WiFi alone cannot give us the map of the environment or a physical representation of a map or context
Keeping these advantages in mind, many systems have been proposed incorporating WiFi sensors within SLAM, ranging from aiding loop closure~\cite{hashemifar2019augmenting, liu2019collaborative} or incorporating them as range~\cite{huang2011efficient,ferris2007wifi} and bearing sensor~\cite{xxx}. Unfortunately, the systems in \cite{hashemifar2019augmenting, liu2019collaborative} and \cite{ huang2011efficient,ferris2007wifi} utilize RSSI for fingerprinting or as a proxy for range respectively and hence lack robustness in dynamic environments. While, P2SLAM~\cite{xxx}, incorporating bearings extracted from CSI~\cite{ayyalasomayajula2018bloc}, is more robust to dynamic environments, it does not tightly fuse with visual sensors, and hence its locations lack contextual information with respect to a map. \name seeks to solve this problem by showcasing a system which tightly couples visual landmarks from a monocular camera and readily deploys in any unknown environment. The key deliverable for \name is to provide an end-to-end sensing solution (WiFi + monocular camera, in conjunction with odometry sensors), which furnishes context-rich location information in real-time without requiring any prior information about the environment. \name achieves this by incorporating WiFi as a bearing sensor~\cite{xxx}, employing the feature tracker from VINS-MONO~\cite{qin2018vins} and fusing odometry from a combination of a wheel encoder and IMU with an open-sourced GraphSLAM framework~\cite{gtsam}. Furthermore, we showcase our system with a simple application which builds a map labelled with room numbers and autonomously navigates to a given room number to deliver a package. 

% but there are problems to implementing this...
But there are three key problems which \name seeks to solve to enable dense \underline{V}isual \underline{I}nertial \underline{O}dometry with Wi\underline{Fi} possible. 
\begin{itemize}
    \item \textbf{Accurate AoA measurements:} Movement of the robot and limited knowledge of antenna placements on the access points (AP) deployed in the environment reduces the accuracy of the angle of arrival measured at the robot. \name observes that for each frequency and packet, extracting the strongest principal component helps to reduce non-idealities introduced by the robots velocity and vibration and accurate average across multiple transmit antenna. In this vein, \name uses an SVD-FFT algorithm to accurate estimate the angle of arrival on the robot (Sec.~\ref{sec:xxx}).
    \item \textbf{2.5D:} AP's are generally deployed higher than the robot's WiFi receiver. This implies we need to estimate both the azimuth and polar angle of arrival (3D-AoA). Unfortunately, with four or fewer antennas~\footnote{Most commercially available WiFi receivers come with only four or fewer antennas~\cite{quantenna, halperin2011tool, gringoli2019free}}, measuring 3D-AoA is very difficult due to reduced resolution. \name overcomes this by observing that the measured angle of arrival of a signal impinging from a higher elevation lies on the inclined plane connecting the AP and the robot, oriented according the heading of the robot. This observation allows \name to extract a single inclined-AoA from a linear antenna array and incorporate these measurements within GraphSLAM~\cite{gtsam} by defining a new measurement factor (Sec.~\cite{xxx}).
    \item \textbf{Half-plane Ambiguity:} Using a linear antenna array creates an ambiguity in the incline-AoA measured in the $360^\circ$ search-space. Using MH-iSAM2\cite{hsiao2019mh}, \name elegantly resolves this ambiguity by incorporating the multiple hypothesis within GraphSLAM and prunes the incorrect hypothesis in the future when more measurements are available (Sec.~\cite{xxx}).
\end{itemize}

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publically available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry. 

% we make this solution possible by ... efficiently fusing WiFi and camera for their strong suits, where our system relies on WiFi majorly for it's localization and tracking purposes and camera for it's map building and optimal and safe navigation purposes


% with \name, we implement and observe the following ...solutions which make realizing low-cost, robust indoor navigation robots a reality



% \subsection{Storyline}
% WiFi+camera with simplistic sensors, and plug them for the robot
% Monocular cameras are not sufficient within themselves
% So people have moved to stereo-vision and LiDAR
% Under 50\$ we can give you context based mapping with robust localization.

==> ViWiD SLAM_arx/intro/intros_old/intro10.tex <==


% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholder.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features
%Thus, existing Visual SLAM systems are not light-weight and require extensive compute and memory resources to operate in real time, 
hindering their deployment in the real world~\cite{semenova2022quantitative}. 
However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous `Localization' and `Mapping' that is compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm which is memory and compute efficient and scalable. \name SLAM's  key insight is to eliminate memory intensive storage and computationally expensive correlation operations over the past measurement. \name system/robot consists of a WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. These pose estimates are then fed to \name's visual layer as shown in Figure~\ref{fig:intro-fig}, used by \name visual layer to label visual data with a pose.  
Since Wi-Fi pose measurements do not accrue drift over time, unlike standard visual SLAM algorithms, \name visual SLAM does not need to cross-correlate measurements across time to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.
While \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method generalizes to other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or next gen 5G femto-cell implementations~\cite{5g}. 
% call out real-time


Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with a clear interface of sharing of pose estimation from WiFi layer, to enable visual layers for the environment mapping. Such layering would bring the advantages of networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled, it would enable researchers in wireless sensing and visual SLAM domain to improve the individual algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm. 
%each layer can improved by themselves and such improvement would improve overall performance    
%above paragraph: emphasize no AP priors

% This abstraction of the complementary pose estimation WiFi SLAM, and the environment mapping Visual SLAM layers has advantages as in networking layer abstractions~\cite{session1994it5}.
% That is both the pose estimation layer and the mapping layer can be optimized within themselves without effecting the other layer's performance.
% For example, while we use WiFi-sensor for \name's implementation due to its widespread deployment in indoors, other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative sensors depending on the use case.

% figure: robot, rf layer -> visual layer
%Design ideas behind dual-graph (bring up performance), can use more than just Wi-Fi.

However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi localization solutions and feeding them into existing Visual SLAM algorithms.
We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free pose estimates from the Wi-Fi layer to be robust and real-time. To get these pose estimates from the Wi-Fi-layer, we employ Angle of Arrival (AoA) based localization~\cite{spotfi,jadhav2020wsr,arun2022p2slam,ayyalasomayajula2018bloc}, due to its widespread use.
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these systems use compute intensive super-resolution algorithms, which cannot provide AoA measurements at the rate needed for real time pose estimation.
%I would be cautious about bragging too much about svdfft, it is not a new algorithm.
To solve this, in \name we employ a [] algorithm, borrowing intuition from MUSIC~\cite{schmidtmusic,spotfi}, which both smooths erroneous measurements and attenuates multipath components in the signal. This smoothed CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. We use this method to measure AoA between the robot and Wi-Fi access points in the environment. However, this alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we cannot assume access point locations are known a priori.

\noindent\textbf{Unknown Wi-Fi Access Point Locations:} GraphSLAM~\cite{gtsam} is well known to jointly solve for multi-variate optimization as long as these variable are connected by some measurements.
So we define the Wi-Fi graph with the Odometry measurements connecting two continuous robot poses, and the Wi-Fi AoA measurements connecting the robot's current pose with each AP's position the AoA corresponds to. 
Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, we need to provide initial values to variables in question. 
While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. 
To overcome this issue, a naive solution can be to initialize all the AP locations at the origin. 
This is not an issue when the AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. 
However, when few measurements constrain the AP's pose, as is the case when the robot first traverses the environment for the real time, the optimizer is poorly conditioned. 
To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) proximity sensing~\cite{ez,zee}.
That is we initialize the location of the Wi-Fi AP at the time instance when the RSSI measured for a given access point is a local maxima along the path taken.

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Finally, the optimized robot poses generated by the Wi-Fi graph need to update the robot poses in the camera graph in real-time.
Unfortunately, if the already traversed robot poses are getting large corrections very frequently, it would result in large and frequent feature map corrections in the camera graph as well, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made.
These accumulated corrections are only pushed to the Camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.


These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We extract widely used Shi-Tomasi features~\cite{shi1994good} for the camera sensor using the opensourced VINS-MONO feature tracker~\cite{qin2018vins}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> ViWiD SLAM_arx/intro/intros_old/intro11.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholder.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment, it would construct a 'loop closure'.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features.
%Thus, existing Visual SLAM systems are not light-weight and require extensive compute and memory resources to operate in real time, 
hindering their deployment in the real world~\cite{semenova2022quantitative}. However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous `Localization' and `Mapping' that is compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm which is memory and compute efficient and scalable. \name's SLAM key insight is to eliminate  memory intensive storage and computationally expensive correlation over the past measurement, essentialy develop a loop-closure free SLAM. \name system/robot consists of has WiFi radio, which is fed to a Wi-Fi sensing layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. These pose estimates are then fed to \name's visual layer as shown in Figure~\ref{fig:intro-fig}, used by visual layer to label visual data with a pose.  
Since Wi-Fi pose measurements do not accrue drift over time, unlike standard visual SLAM algorithms, \name visual SLAM does not need to cross-correlate measurements across time to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.
While \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method generalizes to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance}. 

Additionally, \name presents a layered abstraction for both WiFi layaer and Visual SLAM layer, with a clear interface of sharing of pose estimation from WiFi layer, to enable visual layers for the environment mapping. Such layering would bring the advantages of networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled, it would enable researchers in wireless sensing and visual SLAM domain to improve the individual algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm. %each layer can improved by themselves and such improvement would improve overall performance    
%above paragraph: emphasize no AP priors

% This abstraction of the complementary pose estimation WiFi SLAM, and the environment mapping Visual SLAM layers has advantages as in networking layer abstractions~\cite{session1994it5}.
% That is both the pose estimation layer and the mapping layer can be optimized within themselves without effecting the other layer's performance.
% For example, while we use WiFi-sensor for \name's implementation due to its widespread deployment in indoors, other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative sensors depending on the use case.

% figure: robot, rf layer -> visual layer
%Design ideas behind dual-graph (bring up performance), can use more than just Wi-Fi.

However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi sensing solutions and feeding them into existing Visual SLAM algorithms.
We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free robot pose estimates from the Wi-Fi layer to be robust and real-time. To get these pose estimates from the Wi-Fi-layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve WiFi-layer pose. %Extracting angle-of-arrival has been studied extensively in literature, due to use of those in WiFi localization~\cite{spotfi,jadhav2020wsr,arun2022p2slam,ayyalasomayajula2018bloc}. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use compute intensive super-resolution algorithms, which cannot provide compute efficient AoA measurements at the rate needed for real time pose estimation.
%I would be cautious about bragging too much about svdfft, it is not a new algorithm.
To solve this, in \name we employ a low-compute algorithm, which both smooths erroneous measurements and attenuates multipath components in the signal, by combining the CSI across time. The smoothed CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points. 

\noindent\textbf{Unknown Wi-Fi Access Point Locations:}
An obvious idea would be to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization, which includes WiFi-AP locations. Specifically, we define the Wi-Fi graph with the robot side AoA measurements from different APs and concurrent odometry measurements, with robot pose and AP's location as variables. %connecting two continuous robot poses, and the Wi-Fi AoA measurements connecting the robot's current pose with each AP's position the AoA corresponds to. 
Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, initial values to variables are extreme importance to lead the optimizer in a trajectory to solve the problem. 
While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. Furthermore, arbitrary initializing AP's locations would work only when AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. 
However, to be compute efficient with a few measurements and constrain the AP's pose, as is the case when the robot in real-time maps the environment, the optimizer is poorly conditioned for AP's location. 
To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) as proximity sensing~\cite{ez,zee} to initialize the location of WiFi AP. The location of the Wi-Fi AP is initialized with robot pose at the time instance when the RSSI measured for a given access point is a local maxima along the path taken. 

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Finally, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As robot moves, the WiFi graph continues to optimize its previous robot poses. A continuous updates of already traversed robot poses to the camera graph, would trigger large corrections and those too very frequently, and result in large and frequent feature map corrections, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made. The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.


These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We extract widely used Shi-Tomasi features~\cite{shi1994good} for the camera sensor using the opensourced VINS-MONO feature tracker~\cite{qin2018vins}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> ViWiD SLAM_arx/intro/intros_old/intro12.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholder.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features, hindering their deployment in the real world~\cite{semenova2022quantitative}. 
However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous `Localization' and `Mapping' that is compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm which is memory and compute efficient and scalable. \name SLAM's  key insight is to eliminate memory intensive storage and computationally expensive correlation operations over the past measurement. \name system/robot consists of a WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. These pose estimates are then fed to \name's visual layer as shown in Figure~\ref{fig:intro-fig}, used by \name visual layer to label visual data with a pose.  
Since Wi-Fi pose measurements do not accrue drift over time, unlike standard visual SLAM algorithms, \name visual SLAM does not need to cross-correlate measurements across time to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with a clear interface of sharing of pose estimation from WiFi layer, to enable visual layers for the environment mapping. Such layering would bring the advantages of networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled.
It would enable researchers in wireless sensing and visual SLAM domain to improve the independent algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm.
For example, while \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 

However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi sensing solutions and feeding them into existing Visual SLAM algorithms.
We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free,robust and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduce erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 

\noindent\textbf{Unknown Wi-Fi Access Point Locations:}
An obvious idea would be to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization, which includes WiFi-AP locations. Specifically, we define the Wi-Fi graph with the robot side AoA measurements from different APs and concurrent odometry measurements, with robot pose and AP's location as variables. 
Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, initial values to variables are extreme importance to lead the optimizer in a trajectory to solve the problem. 
While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. Furthermore, arbitrary initializing AP's locations would work only when AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. 
However, to be compute efficient with few AoA measurements that constrain the AP's pose, as is the case when the robot in real-time maps the environment, the optimizer is poorly conditioned for AP's location. 
To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) based proximity sensing~\cite{ez,zee} to initialize the location of WiFi AP. The location of the Wi-Fi AP is initialized to the robot pose at the time instance when the RSSI measured for a given access point is a local maxima along a path taken. 

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Finally, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As robot moves, the WiFi graph continues to optimize its previous robot poses. A continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.


These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> ViWiD SLAM_arx/intro/intros_old/intro13.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/viwid_intro-crop.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement units) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements requires the SLAM system to be both memory and compute intensive.~\cite{semenova2022quantitative}.
The way these Visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory through its environment, because when the robot returns to a previous location, it will observe the same features.
The drawback of this method is that as new features are observed, they must constantly be correlated with past observed features, to check if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observes more new features. This hinders their deployment in the real world~\cite{semenova2022quantitative}. 
However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous Localization and Mapping system that is compute and memory efficient, to make autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm which is memory and compute efficient, and scalable. \name SLAM's  key insight is a method to eliminate memory intensive storage and computationally expensive correlation operations over past measurements. \name system/robot consists of a WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. These pose estimates are then fed to \name's visual layer as shown in Figure~\ref{fig:intro-fig}, used by \name visual layer to label visual data with a pose.  
\name's key observation is that Wi-Fi pose measurements do not accrue drift over time, as they are derived from fixed WiFi anchors in the environment. Therefore, unlike standard visual SLAM algorithms, \name visual SLAM can leverage drift free robot pose as input, and thus, do not require the SLAM algorithms to cross-correlate measurements across time to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with a interface of sharing of robot poses from WiFi layer, to enable the visual layer to map the environment without any correlation. Such layering would bring the advantages similar to networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled.
It would enable researchers in wireless sensing and visual SLAM domain to improve the independent algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm.
For example, while \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 


% WiFi graph

\noindent\textbf{WiFi Graph:}
A natural question is can we use large work on WiFi sensing to develop the WiFi layer/graph which can construct the robot poses (location and orientation). Without the location knowledge of the access points in the environment eliminates ability to leverage large body of research in WiFi Localization. Furthermore, recent works~\cite{ayyalasomayajula2020locap,xxx} leverages an autonomous visual SLAM robot to map the WiFi access, which requires the visual SLAM to have converged, leading to similar compute and memory challenges. In \name, we design a computational efficient WiFi-graph, which in real-time enables the robot to provide poses (location and orientation), without knowledge of WiFi APs location. \name key insight is to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization to solve for both the robot pose and AP's location as variables. Specifically, \name deploys multi-antenna radio at the robot to achieve robot side AoA measurements from different APs in the environment and simultaneous odometry measurements forms an input to graphSLAM. Furthermore, \name develops many optimizations for WiFi graph to make it compute efficient, to output robot poses over time. Intutively, graphSLAM combines the inputs from odometry and AoA's over time to backpropogate and refine the robot pose estimate and WiFi AP position over time. 

% Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, initial values to variables are extreme importance to lead the optimizer in a trajectory to solve the problem. While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. Furthermore, arbitrary initializing AP's locations would work only when AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. However, to be compute efficient with few AoA measurements that constrain the AP's pose, as is the case when the robot in real-time maps the environment, the optimizer is poorly conditioned for AP's location. To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) based proximity sensing~\cite{ez,zee} to initialize the location of WiFi AP. The location of the Wi-Fi AP is initialized to the robot pose at the time instance when the RSSI measured for a given access point is a local maxima along a path taken. 

% 
% However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi sensing solutions and feeding them into existing Visual SLAM algorithms.
% We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Next, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As robot moves, the WiFi graph continues to optimize its previous robot poses via back-propagation. A continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free,robust and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduce erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 

These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiducial markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> ViWiD SLAM_arx/intro/intros_old/intro13_ag.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and generating human readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/viwid_intro-crop.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features, hindering their deployment in the real world~\cite{semenova2022quantitative}. 
% However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous `Localization' and `Mapping' that is compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM system which is low-cost\footnote{requires only Camera as a visual sensor, doesn't require LiDAR}, memory, compute efficient and scalable. \name SLAM's  key insight is to eliminate memory intensive storing of past measurements and computationally expensive correlation operations over the past measurement. 
\name system/robot consists of a multi-antenna WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. 
These pose estimates are then fed to \name's visual layer to label visual data with a prior pose (as shown in Figure~\ref{fig:intro-fig}). 
\name's key observation is that WiFi layers robot pose measurements do not accrue drift over time, as they are derived from fixed WiFi anchors in the environment. 
Therefore, unlike standard visual SLAM algorithms, \name visual SLAM can leverage drift free robot pose as input, and thus, does not require the SLAM algorithms to cross-correlate across past measurement to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Visual layer (needs only camera).

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with a interface of sharing of robot poses from WiFi layer, to enable the visual layer to map the environment without any correlation. Such layering would bring the advantages similar to networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled.
It would enable researchers in wireless sensing and visual SLAM domain to improve the independent algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm.
For example, while \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 


% WiFi graph

\noindent\textbf{WiFi Graph:}
A natural question is can we simply use the work on WiFi sensing to develop the WiFi layer which can construct the robot poses (location and orientation). Turns out, most state of the art in WiFi sensing assume knowledge of access point to localize \cite{}. However, ideally no prior knowledge of environment is desirable as it leads to ease of deployment~\cite{ayyalasomayajula2020locap}. Thus, not assuming the WiFi AP location hinders the ability to simply piggyback on using existing prior works in WiFi sensing to deploy the WiFi layer. 
% Furthermore, recent work~\cite{ayyalasomayajula2020locap} pose an inverse problem with WiFi sensing, where they leverage an autonomous visual SLAM robot to map the WiFi access points to make the WiFi sensing deploy-able.
% This however, requires the visual SLAM to have converged, leading to similar compute and memory challenges to map the WiFi access points themselves. 
Bypassing these issues entirely, in \name, we design a computational efficient WiFi-graph, which in real-time enables the robot to provide poses (location and orientation), without knowledge of WiFi APs location. \name key insight is to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization; for example, solve for both the robot pose and AP's location variables. 
The idea here is to do a coarse initialization of WiFi access points, based on their RSSI measurements, and the GraphSLAM framework would use the WiFi measurements and Odometry measurement to optimize for access point locations implicitly, and robot poses explicitly. Intuitively, it combines measurements of wifi-sensor, odometry across a trajectory (time-series of multiple location) to obtain accurate robot poses.  

% Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, initial values to variables are extreme importance to lead the optimizer in a trajectory to solve the problem. While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. Furthermore, arbitrary initializing AP's locations would work only when AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. However, to be compute efficient with few AoA measurements that constrain the AP's pose, as is the case when the robot in real-time maps the environment, the optimizer is poorly conditioned for AP's location. To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) based proximity sensing~\cite{ez,zee} to initialize the location of WiFi AP. The location of the Wi-Fi AP is initialized to the robot pose at the time instance when the RSSI measured for a given access point is a local maxima along a path taken. 

% 
% However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi sensing solutions and feeding them into existing Visual SLAM algorithms.
% We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:


\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:}
Naturally, the graphSLAM would require high-quality, real-time input to achieve robust robot poses as well implicit locations of the AP, which do not accrue drift. 
% Specifically, \name deploys multi-antenna radio at the robot to achieve robot side AoA measurements from different APs in the environment and simultaneous odometry measurements forms an input to graphSLAM. 
% Furthermore, \name develops many optimizations for WiFi graph to make it compute efficient, to output robot poses over time. 
% Intutively, graphSLAM combines the inputs from odometry and AoA's over time to backpropogate and refine the robot pose estimate and WiFi AP position over time. 
In order to accurately estimate the map, the visual layer requires drift-free, robust and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose from the fixed APs located at implict positions optimized by the SLAM framework. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduce erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 


\noindent\textbf{Efficient Pose Updates to Camera Graph:} Next, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As robot moves, the WiFi graph continues to optimize its previous robot poses via back-propagation. A continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.



These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We benchmark our results against the state-of-the-art Visual SLAM system, RTABMap~\cite{Labb2018RTABMapAA}, and we use the high compute and expensive LiDAR sensor readings reported in the Datasets~\cite{arun2022p2slam} to estimate thee ground truth for our measurements.
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} the Visual SLAM.
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$}the Visual (LiDAR).
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> ViWiD SLAM_arx/intro/intros_old/intro14.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and generating a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/viwid_intro-crop.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}


Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute-intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observes more new features, hindering their deployment in the real world~\cite{semenova2022quantitative}. 


In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM system which is low-cost\footnote{requires only Camera as a visual sensor, doesn't require LiDAR}, memory, compute efficient and scalable. \name SLAM's key insight is to eliminate memory-intensive storing of past measurements and computationally expensive correlation operations over the past measurement. 
\name system/robot consists of a multi-antenna WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of the robot, without assuming the knowledge of Wi-Fi access point locations in a map. 
These pose estimates are then fed to \name's visual layer to label visual data with a prior pose (as shown in Figure~\ref{fig:intro-fig}). 
\name's key observation is that WiFi layers robot pose measurements do not accrue drift over time, as they are derived from fixed WiFi anchors in the environment. 
Therefore, unlike standard visual SLAM algorithms, \name visual SLAM can leverage drift-free robot pose as input, and thus, does not require the SLAM algorithms to cross-correlate across past measurement to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory-efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Visual layer (needs only camera).

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with an interface of sharing of the robot poses from WiFi layer, to enable the visual layer to map the environment without any correlation. Such layering would bring advantages similar to networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in the WiFi layer and Visual layer are completely decoupled.
It would enable researchers in wireless sensing and visual SLAM domain to improve the independent algorithms, \name's architecture could leverage that improvement to build a more accurate SLAM algorithm.
For example, while \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 


\noindent\textbf{WiFi Graph:}
A natural question is can we simply use the work on WiFi sensing to develop the WiFi layer which can construct the robot poses (location and orientation). Turns out, most state-of-the-art in WiFi sensing assume knowledge of access points to localize \cite{arraytrack,spotfi}. However, ideally, no prior knowledge of the environment is desirable as it leads to ease of deployment~\cite{ayyalasomayajula2020locap}. Thus, not assuming the WiFi AP location hinders the ability to simply piggyback on using existing prior works in WiFi sensing to deploy the WiFi layer. 
Bypassing these issues entirely, in \name, we design a computational efficient WiFi-graph, which in real-time enables the robot to provide poses (location and orientation), without knowledge of WiFi APs location. \name key insight is to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization; for example, solve for both the robot pose and AP's location variables. 
The idea here is to do a coarse initialization of WiFi access points, based on their RSSI measurements, and the GraphSLAM framework would use the WiFi measurements and Odometry measurement to optimize for access point locations implicitly, and robot poses explicitly. Intuitively, it combines measurements of wifi-sensor, odometry across a trajectory (time-series of multiple locations) to obtain accurate robot poses.  


\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:}
Naturally, the graphSLAM would require high-quality, real-time input to achieve robust robot poses as well implicit locations of the AP, which do not accrue drift. 
To accurately estimate the map, the visual layer requires drift-free, robust, and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose from the fixed APs located at implicit positions optimized by the SLAM framework. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real-time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduces erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 


\noindent\textbf{Efficient Pose Updates to Camera Graph:} Next, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As the robot moves, the WiFi graph continues to optimize its previous robot poses via back-propagation. Continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute-intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made to the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates make the camera graph optimization efficient by avoiding any possible memory or compute-intensive stages.



These effective solutions surmount the key challenges to integrating Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We evaluate \name over two different where  we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this, we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot-driven cumulative distance of over $1000$ m across these two environments. 
We benchmark our results against the state-of-the-art Visual SLAM system, RTABMap~\cite{Labb2018RTABMapAA}, and we use the high compute and expensive LiDAR sensor readings to estimate the ground truth for our measurements.
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to $20\%$ of cores which is $5\times$ better than current Visual SLAM.
    \item We also show that \name-SLAM reduces the average memory utilization to $300$MB which is $3\times$ the Visual (LiDAR).
    \item We show a pose estimation performance with 50cm median location estimation error and $2^{\circ}$ median orientation estimation error on par with the state-of-the-art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiducial markers placed in the environment to within 105cm of error.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in the layered SLAM domain for sensor fusion approaches.



==> ViWiD SLAM_arx/intro/intros_old/intro15.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/viwid_intro-crop.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}


Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory intensive, as the robot must keep all features it has seen in memory. 
Furthermore, they spend increasing compute time looking them up and comparing them as it observes more new features, hindering their deployment in the real world~\cite{semenova2022quantitative}. 


In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM system which is a memory+compute efficient, scalable and low-cost\footnote{requires only a monocular camera as a visual sensor, does not require LiDAR}. 
\name SLAM's key insight is to eliminate memory-intensive storing of past measurements and computationally expensive correlation operations while maintaining drift free robot trajectory to ensure accurate SLAM. 
\name system/robot consists of a multi-antenna WiFi radio, which is fed to \name's Wi-Fi layer to provide 3D-pose (position and orientation) estimates of the robot, without assuming the knowledge of Wi-Fi access point locations in a map. 
These pose estimates are then fed to \name's visual layer to label visual data with a prior pose (as shown in Figure~\ref{fig:intro-fig}). 
\todo{Causes confusion for Reviewer 3: does this mean you're replacing standard odometry?}
\name's key observation is that WiFi layers robot pose measurements do not accrue drift over time, as they are derived from fixed WiFi anchors in the environment. 
Therefore, unlike standard visual SLAM algorithms, \name's visual SLAM can leverage drift-free robot pose as input, effectively circumventing the memory+compute intensive cross-correlation across past measurements.
Thus, \name enables compute and memory-efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Visual layer (needs only camera).

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with an interface of sharing of the robot poses from WiFi layer, to enable the visual layer to map the environment without any correlation operations. 
Such layering would bring advantages similar to networking layer abstractions~\cite{session1994it5} to the SLAM research. 
Specifically, a powerful implication of our layered architecture is that innovations in the WiFi layer and Visual layer are completely decoupled.
This decoupling would enable researchers in wireless sensing and visual SLAM domain to independently improve algorithms, and allow \name's architecture to easily leverage these improvement to build a more accurate SLAM algorithm.
For example, while \name's Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 


\noindent\textbf{WiFi Graph:}
A natural question is can we simply use the work on WiFi sensing to develop the WiFi layer which can construct the robot poses (location and orientation). Turns out, most state-of-the-art in WiFi sensing assume knowledge of access points to localize \cite{arraytrack,spotfi}. However, ideally, for ease of deployment, no prior knowledge of the environment is desirable~\cite{ayyalasomayajula2020locap}. Thus, not assuming the WiFi AP location hinders the ability to simply piggyback on using existing prior works in WiFi sensing to deploy the WiFi layer. 
Bypassing these issues entirely, in \name, we design a computational efficient WiFi-graph, which in real-time enables the robot to provide poses (location and orientation), without knowledge of WiFi APs location. 
\name's key insight is to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization; specifically in the case of the WiFi-graph, solve for both the robot's pose and AP's location variables. 
The idea here is to first coarsely initialize the WiFi access points as new access points are discovered prior to optimization. 
Next, the GraphSLAM framework would use the WiFi measurements and Odometry measurements to optimize for access point locations implicitly, and robot poses explicitly. 
Intuitively, it combines measurements of wifi-sensor, odometry across a trajectory (time-series of multiple locations) to obtain accurate robot poses.  


\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:}
% Naturally, the graphSLAM would require high-quality, real-time input to achieve robust robot poses as well as implicit locations of the AP, which do not accrue drift. 
To accurately estimate the map, the visual layer requires drift-free, robust, and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name's Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose from the fixed APs located at implicit positions optimized by the SLAM framework. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real-time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduces erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. 
However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. 
This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 


\noindent\textbf{Efficient Pose Updates to Camera Graph:} Next, the optimized robot poses generated by the Wi-Fi graph are fed to update the robot poses in the camera graph in real-time. 
As the robot moves, the WiFi graph continues to optimize its previous robot poses via \todo{back-propagation (not the best term)}. 
Continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute-intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made to the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates make the camera graph optimization efficient by avoiding any possible memory or compute-intensive stages.

These effective solutions surmount the key challenges to integrating Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM2~\cite{gtsam}.
We evaluate \name over two different paths driven in a $25 \times 30$ m. 
In addition to this, we also collect one more dataset in the $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot-driven cumulative distance of over $1000$ m across these three datasets. 
We benchmark our results against the state-of-the-art Visual SLAM system, RTABMap~\cite{Labb2018RTABMapAA}, and we use the high compute and expensive LiDAR sensor readings to estimate the ground truth for our measurements.
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to $20\%$ of cores which is $5\times$ better than current Visual SLAM.
    \item We also show that \name-SLAM reduces the average memory utilization to $300$MB which is $3\times$ less than Visual-SLAM.
    \item We show a pose estimation performance with $50$ cm median location estimation error and $2^{\circ}$ median orientation estimation error, performing on par with the state-of-the-art systems.
    \item We also show the \name's real-time mapping accuracy by mapping the camera fiducial markers placed in the environment to within $105$ cm of error using a monocular camera.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the datasets we have collected, to enable further research and development in the layered SLAM domain for sensor fusion approaches.



==> ViWiD SLAM_arx/intro/intros_old/intro2.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

A strong need for automation in various industries spanning hospitality to security has led to an increased adoption of robots capable of autonomous, reliable and safe indoor navigation. The trend kick-started by the early adoption of automated vacuum cleaners has grown many-fold to use these robots for monitoring security in office spaces, serving patrons at restaurants and moving large equipment in hospitals. The autonomy, reliability and safety these robots boast is owed to the suite of sensors they use. Most autonomous robots can be commonly spotted sporting 
1. a LiDAR at the top to provide a 360-degree view, 
2. a camera facing forward to provide a feature-rich map, 
3. bumper sensors to avoid catastrophic collisions, and
4. odometry sensors (wheel encoder and IMU) to provide high-resolution odometry data.
The data from these sensors are expertly fused taking into consideration each sensors reliability within a back-end optimization framework to generate an accurate estimate of the robot's location and its relation to the environment around it. The fusion of these different sensing modalities provides a very robust solution for autonomous navigation of robots.

% let's see how good sensor fusion works; explain landmarks, features, loop closure in few sentences...
To achieve autonomous navigation, the first key step is for the robot to build a map of its environment and localize itself within this map in real time. 
Furthermore, this map should consist of rich contextual data -- labels of room numbers, descriptions of spaces, markings for various exits and entrances of buildings. 
This problem is commonly called Simultaneous Localization and Mapping (SLAM). 
In a two-step process, which involves first extracting and tracking the characteristic features from visual sensors, and second, combining the data from these sensors with odometry, the robot can build an accurate map and localize itself within this map. The characteristic features (\textit{landmarks}) extracted generally include corners or edges in Camera images or LiDAR scans. Tracking these features provides corrections to errors accumulated by odometry sensors, and saving some of the salient features helps the robot recognize and create additional constraints (\textit{loop-closures}) with previously visited places. Through this two-step process, robots can effectively navigate the strengths and weaknesses of individual sensors to solve the SLAM problem.

% but this fails in monotonous envs ...\todo{because of the same reasons we have mentioned in P2SLAM}
Unfortunately, in indoor environments, we observe gaps left behind this common suite of sensors generally employed on robots. LiDAR's, although great in providing an accurate point cloud of an environment, fail in environments with little structural features, like long corridors or spaces larger than the field of view of the LiDAR. Furthermore, they are expensive, bulky and power hungry. To combat these weaknesses of LiDARs or to develop robots at lower cost-points, cameras (monocular, stereo or RGBD) are employed. Cameras offer an advantage over LiDAR's in that they allow for finer feature detection. For example, a long corridor adorned with posters and paintings provide robust and recognizable features to track against. Unfortunately, motion blur, dynamic lighting conditions and monotonous visual environments can all lead to feature tracking failure and even false positive loop closure hypothesis.
% Furthermore, viable distances to obtain accurate depth from RGBD/Stereo sensor range from \todo{xx} m - \todo{xx} m, making them unusable in large spaces. 
Discounting LiDAR's or cameras in these challenging environments leaves us with odometry sensors. A combination of wheel encoders and IMU's provide accurate change in position over a local region and a period of few minutes. 
Unfortunately, lacking the global correction provided by visual sensors via loop-closures, these odometry sensors can accrue large drifts, in the order of many tens of meters, when traversing large distances of hundreds of meters. This leaves an open problem for autonomous navigation for indoor robotics -- what is the best sensor we could incorporate to fill in the gaps left by these multitude of sensors? 

% bring up and kill other sensors, distill to wifi, rebuff it after a better lit review ...
To answer this pressing question, we can in fact take inspiration from GPS. Using a network of satellites, GPS can position a GPS-capable device to within a few meters with a global frame of reference. This can help to correct for large drifts accumulated due to odometry and incorrect tracking from visual sensors. But, GPS signals are scantly available in indoor scenarios to provide the necessary corrections. Fortunately, we observe that an alternative, RF-signals, like Bluetooth, Ultrawide-band (UWB) or WiFi, are abundant indoors. RF-based sensing can, in a loose sense, replace GPS and many recent works have proposed the use RF-based sensing to fill the gaps left by visual sensors. As expanded in Section~\ref{sec:related}, implementations based on UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot} exist. Unfortunately, these systems are limitedly employed due to high deployment cost or poor scalability. Fortunately, as compared to UWB and BLE, WiFi is more ubiquitously deployed (reducing deployment cost) and provides a larger range than RFID or other backscatter devices (making it scalable). Keeping these advantages in mind, many systems have been proposed incorporating WiFi sensors within SLAM, for aiding loop closures~\cite{hashemifar2019augmenting, liu2019collaborative} or incorporating them as range~\cite{huang2011efficient,ferris2007wifi} or bearing sensors~\cite{xxx}. Unfortunately, the systems in \cite{hashemifar2019augmenting, liu2019collaborative} and \cite{ huang2011efficient,ferris2007wifi} utilize RSSI for fingerprinting or as a proxy for range respectively and hence lack robustness in dynamic environments. While, P2SLAM~\cite{xxx}, incorporating bearings extracted from CSI~\cite{ayyalasomayajula2018bloc}, is more robust to dynamic environments, it does not tightly fuse with visual sensors, and hence its locations lack contextual information with respect to a map. 

\name seeks to solve this problem by showcasing a system which tightly couples visual landmarks from a monocular camera and readily deploys in any unknown environment. The key deliverable for \name is to provide an end-to-end sensing solution (WiFi + monocular camera, in conjunction with odometry sensors), which furnishes context-rich location information in real-time without requiring any prior information about the environment. \name achieves this by incorporating WiFi as a bearing sensor~\cite{xxx}, employing the feature tracker from VINS-MONO~\cite{qin2018vins} and fusing odometry from a combination of a wheel encoder and IMU with an open-sourced GraphSLAM framework~\cite{gtsam}. Furthermore, we showcase our system with a simple application which builds a map labelled with room numbers and autonomously navigates to a given room number to deliver a package. 

% but there are problems to implementing this...
But there are three key problems which \name seeks to solve to enable dense \underline{V}isual \underline{I}nertial \underline{O}dometry with Wi\underline{Fi} possible. 
\begin{itemize}
    \item \textbf{Accurate AoA measurements:} Movement of the robot and limited knowledge of antenna placements on the access points (AP) deployed in the environment reduces the accuracy of the angle of arrival measured at the robot. \name observes that for each frequency and packet, extracting the strongest principal component helps to reduce non-idealities introduced by the robots velocity and vibration and accurate average across multiple transmit antenna. In this vein, \name uses an SVD-FFT algorithm to accurate estimate the angle of arrival on the robot (Sec.~\ref{sec:xxx}).
    \item \textbf{2.5D:} AP's are generally deployed higher than the robot's WiFi receiver. This implies we need to estimate both the azimuth and polar angle of arrival (3D-AoA). Unfortunately, with four or fewer antennas~\footnote{Most commercially available WiFi receivers come with only four or fewer antennas~\cite{quantenna, halperin2011tool, gringoli2019free}}, measuring 3D-AoA is very difficult due to reduced resolution. \name overcomes this by observing that the measured angle of arrival of a signal impinging from a higher elevation lies on the inclined plane connecting the AP and the robot, oriented according the heading of the robot. This observation allows \name to extract a single inclined-AoA from a linear antenna array and incorporate these measurements within GraphSLAM~\cite{gtsam} by defining a new measurement factor (Sec.~\cite{xxx}).
    \item \textbf{Half-plane Ambiguity:} Using a linear antenna array creates an ambiguity in the incline-AoA measured in the $360^\circ$ search-space. Using MH-iSAM2\cite{hsiao2019mh}, \name elegantly resolves this ambiguity by incorporating the multiple hypothesis within GraphSLAM and prunes the incorrect hypothesis in the future when more measurements are available (Sec.~\cite{xxx}).
\end{itemize}

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publically available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry. 

% we make this solution possible by ... efficiently fusing WiFi and camera for their strong suits, where our system relies on WiFi majorly for it's localization and tracking purposes and camera for it's map building and optimal and safe navigation purposes


% with \name, we implement and observe the following ...solutions which make realizing low-cost, robust indoor navigation robots a reality



% \subsection{Storyline}
% WiFi+camera with simplistic sensors, and plug them for the robot
% Monocular cameras are not sufficient within themselves
% So people have moved to stereo-vision and LiDAR
% Under 50\$ we can give you context based mapping with robust localization.

==> ViWiD SLAM_arx/intro/intros_old/intro3.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Increasing research into autonomous robots for indoors, have spun a myriad of applications and use cases like in equipment and inventory management ranging from hospitals~\cite{hospital,tracking,robots} to warehouses~\cite{warehouse,management,robots} in addition to the usual indoor navigation~\cite{indoor,navigation,robots} and exploration robots~\cite{distaster,zone,exploration,robots}. 
Most of these applications like inventory management and delivery in the critical cases like hospitals demands a fleet of robust, secure and autonomous robots.
While, there has been an effort in deploying a fleet of robots for last-mile delivery in the recent past~\cite{last,mile,delivery,papers}, the technology has not scaled up due to high cost to return value in deploying these robots.
The expensive costs, both in terms of price and compute come from the usage of suite of sensors on these robots~\cite{last,mile,ecomically,inefficient}.
Most algorithms~\cite{visual,slam,algorithms} on these autonomous robots can be commonly spotted utilizing the sensor data from a LiDAR, RGBD or monocular camera in tandem with odometry sensors (wheel encoder and IMU) to provide high-resolution simultaneous mapping and localization.
These pool of sensors, especially LiDAR and RGBD sensors, become expensive in terms of compute and price as the robustness requirement for the autonomous deployment increases.
Unfortunately, this cost ultimately limits these autonomous systems from scaling to deployment. 
Thus, to be able to realize these applications, the Simultaneous Localization and Mapping (SLAM) algorithms to be deployed on these fleet of autonomous robots need to be (a) low-cost, (b) low-compute, and (c) capable of understanding its surroundings.


A majority of current SLAM algorithms on these robots utilize visual (monocular/RGBD cameras)~\cite{camera,slam,algorithms} and LiDAR~\cite{lidar,slam,algorithms} sensors.
While these LiDAR and visual sensors provide the context of the surroundings to the robot, they have extensive compute and memory requirements, and are very expensive, which limit them to scale towards these low-cost, context aware autonomous robots.
So, in this paper, we first ask the question on how we can reduce the cost/expense of these autonomous robots?
In the recent past, there has been a lot of research towards Radio Frequency (RF) sensors as the low-cost, low-compute sensors for robust SLAM algorithms~\cite{wifi,uwb,ble,p2slam,papers}.
While the RF-sensors enable low-power and low-compute SLAM algorithms, these SLAM algorithms fall short in two categories, firstly most of these algorithms~\cite{rf,fingerprinting,slam,algos} utilize these RF-measurements as landmarks, which require labour intensive fingerprinting. 
Secondly, the other algorithms~\cite{p2slam,other,similar,papers} that utilize only RF-sensors and integrate them completely into the SLAM algorithms lack the understanding of their surroundings, which becomes important when deployed in real-world.
Thus, there is a lack of a SLAM algorithm that uses low-cost, low-compute sensor and still be able to get an understanding or context of the environment around the robot.
% inexpensive semantic mapping

In this paper, we thus present \name, a low-cost, low-compute SLAM algorithm that has an awareness of the surrounding environment. 
To achieve this \name implements first of its kind integration of low-cost, low-compute RF sensor with a simple monocular camera
\todo{ temporary copy paste from the previous iteration of the intro:}
in real-time without requiring any prior information about the environment. \name achieves this by incorporating WiFi as a bearing sensor~\cite{xxx}, employing the feature tracker from VINS-MONO~\cite{qin2018vins} and fusing odometry from a combination of a wheel encoder and a gyroscope with an open-sourced GraphSLAM framework~\cite{gtsam}. 
While, \name's implementation is demonstrated using WiFi owing to its widescale deployment one of the major advantages \name is that it abstracts bearing as the RF-sensor measurement.
Thus any RF-sensor that can report their bearings like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as altnerative RF-sensors.
Furthermore, we showcase our system with a simple application which builds a map labelled with room numbers and autonomously navigates to a given room number to deliver a package. 

% but there are problems to implementing this...
But there are three key problems which \name seeks to solve to enable dense \underline{V}isual \underline{I}nertial \underline{O}dometry with Wi\underline{Fi} possible. 
\begin{itemize}
    \item \textbf{Accurate AoA measurements:} Movement of the robot and limited knowledge of antenna placements on the access points (AP) deployed in the environment reduces the accuracy of the angle of arrival measured at the robot. \name observes that for each frequency and packet, extracting the strongest principal component helps to reduce non-idealities introduced by the robots velocity and vibration and accurate average across multiple transmit antenna. In this vein, \name uses an SVD-FFT algorithm to accurate estimate the angle of arrival on the robot (Sec.~\ref{sec:xxx}).
    \item \textbf{2.5D:} AP's are generally deployed higher than the robot's WiFi receiver. This implies we need to estimate both the azimuth and polar angle of arrival (3D-AoA). Unfortunately, with four or fewer antennas~\footnote{Most commercially available WiFi receivers come with only four or fewer antennas~\cite{quantenna, halperin2011tool, gringoli2019free}}, measuring 3D-AoA is very difficult due to reduced resolution. \name overcomes this by observing that the measured angle of arrival of a signal impinging from a higher elevation lies on the inclined plane connecting the AP and the robot, oriented according the heading of the robot. This observation allows \name to extract a single inclined-AoA from a linear antenna array and incorporate these measurements within GraphSLAM~\cite{gtsam} by defining a new measurement factor (Sec.~\cite{xxx}).
    \item \textbf{Half-plane Ambiguity:} Using a linear antenna array creates an ambiguity in the incline-AoA measured in the $360^\circ$ search-space. Using MH-iSAM2\cite{hsiao2019mh}, \name elegantly resolves this ambiguity by incorporating the multiple hypothesis within GraphSLAM and prunes the incorrect hypothesis in the future when more measurements are available (Sec.~\cite{xxx}).
\end{itemize}

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publically available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.

==> ViWiD SLAM_arx/intro/intros_old/intro4.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Recent time has seen a rise in demand for autonomous robots and drones for various applications ranging from inventory management in warehouses, hospitals, construction sites~\cite{hosptials,warehoueses,construction,sites} in addition to the navigation~\cite{navigation,robots} and exploration robots~\cite{exploration,robots} for last-mile delivery~\cite{last,mile,delivery}, mapping~\cite{Labb2018RTABMapAA}, and disaster relief~\cite{disaster,relief,jadhav2020wsr}. 
This increasing demand has led the researchers towards deploying fleets of robots to increase the efficiency for these applications, in for example last-mile delivery~\cite{last,mile,delivery} or collaborative robots for indoor explorations~\cite{collab,bots}.
These applications brings forth some important requirements for the current SLAM algorithms to be scalable and deployable:
(a) they should be `low-compute', as they need to run most of the times on a compute-limited platforms, (b) they should be `low-cost', so as to be able to deploy them widely, and (c) they should be `adaptable' to different environmental changes, like dynamic-visibility conditions and/or obstacles in the path.


There exist a lot of powerful tools for autonomous robot systems~\cite{Labb2018RTABMapAA,cartographer,orbslam}, these are far from being scalable to a fleet of robots.
Most of these existing works in SLAM use either IMU/odometry to get the poses of the robot. 
These pose measurements in tandem with camera/LiDAR visual sensors are used to jointly optimize for absolute poses by correcting for the drifts of the IMU/odometry measurements and also to map the environment. 
Firstly, these LiDAR sensors are very expensive, making the LiDAR based SLAM algorithms hard to deploy.
Secondly, while the camera sensors are cheap the joint optimization for optimal Visual SLAM has three distinct operations: (1) feature extraction and tracking, (2) local feature matching and mapping, and (3) global loop-closures. 
While the first two components are not compute intensive, the global loop-closure algorithms are very compute hungry and increase the latency of the system in a compute-restrained scenario~\cite{semenova2022quantitative}.
% 

In contrast, there is a couple of decades of research in RF-based localization and tracking that uses existing RF deployment architectures in the environment, like WiFi, to locate and track various devices in the environment.
As most of the current robots are connected to these internet, they have access to WiFi connectivity which has led the researchers to delve into using WiFi for SLAM implementations~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
These algorithms have been shown to not need global loop-closures making them `low-cost' and 'low-compute' systems~\cite{arun2022p2slam,zhang2020robot}.
Although, unfortunately due to the low-wavelength of RF-signals, these algorithms suffer from lack of context or a map of their surroundings. 
Thus making them non-adaptable to various environmental changes that require awareness of the surroundings/map.

% Current research in Visual SLAM and RF-sensing have thus completely bifurcated from each other. 
% Although as stated above, it is apparent that if we can appropriately integrate the `low-cost', `low-compute' RF sensor with a simple monocular camera that can provide context/map(`adaptable') we can achieve a deployable and scalable SLAM algorithm.
% One might assume

To solve these issues, in this paper we present \name (\underline{V}isual \underline{I}nertial \underline{O}dometry with Wi-\underline{Fi}), that amalgamates the best of both RF and camera worlds. 
While there exist few current works that try to incorporate RF-signals into existing Visual SLAM algorithms~\cite{hashemifar2019augmenting, liu2019collaborative,nguyen2021viral,jadhav2020wsr}, but these systems only try to use the RF signals to aid in the `global loop closures' ~\cite{hashemifar2019augmenting, liu2019collaborative} or depend on the Visual SLAM system to provide the pose of the RF sensor on board~\cite{nguyen2021viral,jadhav2020wsr} making them compute hungry.
In contrast, \name is a first of its kind integration that maintains the `low-cost' and `low-compute' of RF sensor, and simultaneously utilizes a simple monocular camera that can provide context/map(`adaptable') making it a scalable and deployable SLAM system.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/placeholder.pdf}
    \caption{\name's layered approach: WiFi bearings and IMU/Odomtry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time.}
    \label{fig:intro_fig}
\end{figure}


To perform this optimal integration in \name's design, we make a simple yet key observation that both the RF-sensors and the camera-sensors have two independent tasks that can be easily layered to make the system truly scalable.
To be more precise, a camera sensor is the best possible solution to provide real-time current context to the robot regarding its surrounding environment, but it cannot directly help towards estimating the robots absolute pose.
% This has led the researchers in the past to develop complex and compute hungry global loop-closures based optimization for accurate SLAM.
If only these robots could have access to an `Oracle' that could provide these absolute pose measurements they could obtain an optimized map by just performing low-compute feature extraction and local feature matching.
On the other hand, if the existing RF based SLAM approaches could somehow get context awareness and adaptability while maintaining low-cost and low-compute demand. 
We solve both of these problems in \name using the inspiration from network layering/abstraction principals, where in each layer has distinct functionalities and clear boundaries as shown in Figure~\ref{fig:intro_fig}. 
Wherein we firstly use RF measurements and fusing odometry from a combination of a wheel encoder and IMU with an open-sourced GraphSLAM framework~\cite{gtsam} to obtain the optimized poses of the robot.
These global poses are then fed into the the camera feature tracker of one of the widely used VINS-MONO~\cite{qin2018vins} as the `Oracle' camera locations to perform just the low-compute optimization stages of: (1) feature extraction and tracking, and (2) local feature matching and mapping. 
Thus achieving the best of both worlds and making \name's implementation low-cost, low-power and adaptable.

To achieve robust and stable performance with this key insight, we firstly identify that amongst the existing RF sensors, WiFi is the most ubiquitously deployed in the related application scenarios. 
While few of the past works have tried to integrate RSSI measurements~\cite{bruno2011wislam,ferris2007wifi} it is well known that these RSSI measurements are very fickle for indoor scenarios. 
Further, in recent past, researchers have shown reliable performance with bearing/angle of arrival(AoA) to or from the WiFi sensor on the robot~\cite{arun2022p2slam,jadhav2020wsr} to the Access Points in the environment as the WiFi feature measurement.
So, \name utilizes the WiFi sensor on the robot to measure the bearing/AoA to the Access Point.
% \footnote{Thus any RF-sensor that can report their bearings like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative RF-sensors.}.
% Additionally one can also use the bearing measurement from the Access Point to the WiFi sensor on-board~\cite{jadhav2020wsr,arun2022p2slam}, which would require the Access Points' infrastructure to collaborate with the robot.
We only use the bearing measurements from the Access Point to the robot's WiFi sensor, since the toherway around would require the Access Points to report their measurements to the robot which is not always feasible.
% This collaboration is not always possible and so to ease \name's deployment we just use an on-board WiFi sensor that can report the AoA from the Access Point to the robot's WiFi sensor.

These bearing measurements need to be optimized over multiple poses of the bot in real-time and have to backpropogate any errors in these two-way bearing measurements to optimize for the overall bot and AP poses in real-time. 
To this extent, \name utilizes open-sourced GraphSLAM library's real-time implementation of iSAM~\cite{gtsam} by laying down these additional bearing measurements incrementally as and when they come in along with the relative-pose measurement within a factor graph.
At a high level, the presence of bearings measured at the robot allows for accurate mapping of the WiFi access points in the environment and also simultaneously locate itself with respect to these global landmarks.
Thus, \name does not also need to assume the location of the WiFi access points in the environment, making it independent from the WiFi infrastructure.

Since, \name is not performing end-to-end optimization, the bearing measurements being added to the iSAM factor graph cannot be sparse, noisy or ambiguous to avoid ill-defined factor graph optimization. Unfortunately WiFi signals go though heavy multipath and Non Line of Sight(NLoS) Scenarios in the indoor environment making these bearing measurements more noisier than tolerable. 
To overcome this issue, 
% previous works use packet averaging based techniques in tandem with complex MUSIC algorithms that are time consuming, increasing the latency of the bearing measurement fed into the factor graph for optimization. This in turn would delay the updates in the camera feature tracker, which could lead to disastrous performance in mapping and environment awareness. 
in \name we use novel SVD-FFT based averaging algorithm that performs temporal averaging and measure the accurate bearing measurements in real-time.
Additionally most of the solutions for WiFi bearing measurements assume uniform linear arrays~\cite{ayyalasomayajula2020deep,spotfi,arraytrack,soltanaghaei2018multipath} which can only solve half space, providing an ambiguous aliased peak in the other half plane. To avoid this, in \name we utilize a 4-antenna square array with a side length of $3\lambda/8$, where $\lambda$ is the wavelength of the WiFi signal received. This removes the half-plane ambiguities in our system, thus providing reliable, continuous and unambiguous WiFi bearing measurements in real-time to the iSAM factor graph for real-time pose estimation.

Finally, once the optimized robot poses are generated, these are then sent to the camera factor graph that is using the camera features to track and map the environment. To perform this environment mapping, \name uses the camera feature tracker of one of the widely used VINS-MONO~\cite{qin2018vins} implementations, which uses the WiFi factor graph provided robot poses as the camera's pose initialization with a strong confidence. 
The camera factor graph is also implemented as an iSAM factor graph, using the open-sourced real time GraphSLAM framework~\cite{gtsam}. 
This camera factor graph takes the camera features in tandem with robot poses to them track the features and map the environment without the need for any compute heavy global loop closures. 
Thus \name designs first of its kind layered (dual-graph) approach by bringing the best of both (camera and WiFi) sensors together to solve for a low-cost, low-compute and adaptable SLAM system.

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publically available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.
Furthermore, we showcase our system with a simple application which builds a map labelled with room numbers and autonomously navigates to a given room number to deliver a package. 

==> ViWiD SLAM_arx/intro/intros_old/intro5.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Recent time has seen a rise in demand for autonomous robots and drones for various applications ranging from inventory management in warehouses, hospitals, construction sites~\cite{hosptials,warehoueses,construction,sites} in addition to the navigation~\cite{navigation,robots} and exploration robots~\cite{exploration,robots} for last-mile delivery~\cite{last,mile,delivery}, mapping~\cite{Labb2018RTABMapAA}, and disaster relief~\cite{disaster,relief,jadhav2020wsr}. 
This increasing demand has led the researchers towards deploying fleets of robots to increase the efficiency for these applications, for example in last-mile delivery~\cite{last,mile,delivery} or collaborative robots for indoor explorations~\cite{collab,bots}.
These applications brings forth some important requirements for the current SLAM algorithms to be real-time, scalable and deployable:
(a) they should be `low-compute', as they need to run in real-time and sometimes in a memory and compute-limited scenario, (b) they should be `low-cost', so as to be able to deploy them widely, and (c) they should be `adaptable' to different environmental changes, like dynamic-visibility conditions and/or obstacles in the path.


There exist a lot of powerful tools for autonomous robot systems~\cite{Labb2018RTABMapAA,cartographer,orbslam} but these are far from being scalable.
Most of these existing works in SLAM use either IMU/odometry to get the poses of the robot. 
These pose measurements in tandem with camera/LiDAR visual sensors are used to jointly optimize for absolute poses by correcting for the drifts of the IMU/odometry measurements and also to map the environment. 
Firstly, the LiDAR sensors are very expensive, making the LiDAR based SLAM algorithms too costly to deploy.
Secondly, while the camera sensors are low-cost they are compute intensive. 
The joint optimization for optimal Visual SLAM has three distinct operations: (1) feature extraction and tracking, (2) local feature matching and mapping, and (3) global loop-closures. 
While the first two components are not compute intensive but only useful for local pose estimation and mapping, and the global loop-closure algorithms are very compute intensive, memory consuming, time consuming~\cite{semenova2022quantitative} but are required for global corrections, robot poses and map generation.


In contrast, there is a couple of decades of research in RF-based localization and tracking that uses existing RF deployment architectures in the environment, like WiFi, to locate and track various devices in the environment.
As most of the current robots are connected to WiFi and owing to wide-spread deployment of WiFi, researchers have explored towards using WiFi for SLAM implementations~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
These algorithms have been shown to not need global loop-closures making them `low-cost' and 'low-compute' systems~\cite{arun2022p2slam,zhang2020robot}.
\todo{kill p2slam with real-time and zhang et al with range and }
Although, due to the low-wavelength of the WiFi-signals, these algorithms suffer from lack of context or a map of their surroundings. 
Thus making them non-adaptable to various environmental changes that require awareness of the surroundings/map.


To solve these issues, in this paper we present \name-SLAM (\underline{Vi}sual \underline{Wi}Fi \underline{D}ual graph SLAM), that amalgamates the best of both WiFi and camera worlds. 
While there exist few current works that try to incorporate WiFi-signals into existing Visual SLAM algorithms~\cite{hashemifar2019augmenting, liu2019collaborative,nguyen2021viral,jadhav2020wsr}, but these systems only try to use the WiFi signals to aid in the `global loop closures' ~\cite{hashemifar2019augmenting, liu2019collaborative} or depend on the Visual SLAM system to provide the pose of the WiFi sensor on board~\cite{nguyen2021viral,jadhav2020wsr} making them compute and memory hungry, and time consuming.
In contrast, \name is a first of its kind integration that maintains the `low-cost' and `low-compute' of RF sensor, and simultaneously utilizes a simple monocular camera that can provide context/map(`adaptable') making it a scalable and deployable SLAM system.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/placeholder.pdf}
    \caption{\name's layered approach: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time.}
    \label{fig:intro_fig}
\end{figure}


To perform this optimal integration in \name's design, we make two key observations with respect to the existing camera and Visual SLAM systems.
Firstly, while a camera sensor is the best possible solution to provide real-time and low-compute local robot pose and local map, it needs heavy memory and compute resources to perform global robot pose estimation and optimization.
So, if these camera SLAM systems could have access to an `Oracle' that could provide these global robot pose estimates they can just perform the low-compute feature extraction and local feature matching to obtain a final optimized map with global optimized robot poses.
On the other hand, we observe that while the existing WiFi based SLAM approaches provide optimized global robot poses with low-memory and compute demands. So, all these WiFi SLAM systems need are local context/map which could provided by the visual SLAM approaches.
From these observations, \name is designed using the inspiration from network layering/abstraction principals, where in each layer has distinct functionalities and clear boundaries as shown in Figure~\ref{fig:intro_fig}. 
Wherein we firstly use WiFi measurements along with odometry from a combination of a wheel encoder and IMU with an open-sourced GraphSLAM framework~\cite{gtsam} to obtain the optimized global pose estimates of the robot in real-time.
These global pose estimates are then fed as the `Oracle' camera locations into the the camera feature tracker in real-time.
We use one of the widely used VINS-MONO~\cite{qin2018vins} to perform just the low-compute optimization stages of: (1) feature extraction and tracking, and (2) local feature matching and mapping. 
Thus using the best of both sensors and making \name a real-time, scalable and deployable SLAM.

To start with the WiFi factor graph, while a few of the past works have tried to integrate RSSI measurements~\cite{bruno2011wislam,ferris2007wifi} it is well known that these RSSI measurements are very fickle for indoor scenarios. 
Further, in recent past, researchers have shown reliable performance with bearing/angle of arrival(AoA) to or from the WiFi sensor on the robot~\cite{arun2022p2slam,jadhav2020wsr} to the Access Points in the environment as the WiFi feature measurement.
So, \name utilizes the WiFi sensor on the robot to measure the bearing/AoA to the Access Point.
We only use the bearing measurements from the Access Point to the robot's WiFi sensor, since the other way around would require the Access Points to report their measurements to the robot which is not always feasible.
These WiFi bearing measurements are fed to the graph in tandem with IMU/Odometer over multiple poses of the bot in real-time for optimization. This optimization is done over all the robot poses till date in the graph by backpropogating any errors to optimize for the overall bot and AP poses in real-time. 
To this extent, \name utilizes open-sourced GraphSLAM library's real-time implementation of iSAM~\cite{gtsam} by laying down these additional bearing measurements and relative-IMU/Odometer measurements incrementally as and when they come within a factor graph.
At a high level, the presence of bearings measured at the robot allows for accurate mapping of the WiFi access points in the environment and also simultaneously locate itself with respect to these global landmarks.
Thus, \name's WiFi factor graph does not also need to assume the location of the WiFi access points in the environment, making it independent from the WiFi infrastructure.

Additionally, \name's WiFi graph needs to be optimized in real-time as these optimized global pose estimates are fed into the camera graph for real-time local estimates. This real-time WiFi graph optimization poses many challenges to WiFi bearing estimation:

\noindent \textbf{(i) Real-Time Bearing measurements:} Real-time WiFi factor graph optimization in turn demands that the bearing measurements have to be done with minimum latency. While there exist  simple FFT based approaches~\cite{ayyalasomayajula2018bloc} are too inaccurate and provide noisy bearing measurements.

\noindent \textbf{(ii) Accurate Bearing measurements:} Additionally moving WiFi sensors, especially in indoor settings lead to dynamic multipath and Non Line of Sight(NLoS) scenarios making the bearing measurements erroneous and sparse. While, accurate bearing measurement algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} that utilize packet averaging across time, they involve high-latency computations.

\noindent \textbf{(iii) Ambiguous Half-Plane measurements:} Finally most of the solutions for WiFi bearing measurements assume uniform linear arrays~\cite{ayyalasomayajula2020deep,spotfi,arraytrack,soltanaghaei2018multipath} that only solve half space, providing an ambiguous aliased peak in the other half space. 

\name uses a novel SVD-FFT based averaging algorithm that performs real-time temporal averaging by actually identifying the strongest direction component across all the packets.
This leads to reduced noise in the WiFi measurements enabling measurement of accurate bearings in real-time, solving for the first two issues together.
Finally, to avoid the ambiguous peaks problem, in \name we deploy a 4-antenna square array with a side length of $3\lambda/8$ on the robot, where $\lambda$ is the wavelength of the WiFi signal received. 
This removes the half-plane ambiguities in our system, thus providing reliable, continuous and unambiguous WiFi bearing measurements in real-time to the iSAM factor graph for real-time pose estimation.


Secondly for the camera factor graph, the optimized robot poses generated from the WiFi graph are fed to the camera factor graph in real-time.
The camera's local feature tracker and mapping operations are then initialized with these global robot pose estimates with a strong confidence and are optimized using using the open-sourced real time GraphSLAM framework~\cite{gtsam}, iSAM.
For these local pose corrections and mapping, \name uses the camera feature tracker of one of the widely used VINS-MONO~\cite{qin2018vins} implementations.
Since, the camera factor graph utilizes the pre-optimized global pose estimates, it does not need the compute and memory heavy global loop-closure operation.
Thus \name designs first of its kind layered (dual-graph) approach by bringing the best of both (camera and WiFi) sensors together to solve for a low-cost, low-compute and adaptable SLAM system.

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publicly available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.
Furthermore, we showcase \name with a simple application that maps with labelled room numbers and autonomously navigates to a given room number to deliver a package. 

==> ViWiD SLAM_arx/intro/intros_old/intro6.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Recent times have seen a rise in demand for autonomous robots and drones for various applications ranging from inventory management in warehouses, hospitals and construction sites~\cite{hosptials,warehoueses,construction,sites} to the navigation~\cite{navigation,robots} and exploration robots~\cite{exploration,robots} for last-mile delivery~\cite{last,mile,delivery}, mapping~\cite{Labb2018RTABMapAA}, and disaster relief~\cite{disaster,relief,jadhav2020wsr}. 
Furthermore, many of these applications demand a fleet of coordinated robots to perform tasks efficiently. 
To deliver on these applications, Simultaneous Localization and Mapping (SLAM) algorithms need to be (a) `low-compute', to ensure real-time operation on memory and compute constrained machines, (b) `low-cost', to ensure wide deployment, and (c) `context-aware' of environmental changes, which requires a map/context of the environment the robot is exploring.

There exist many powerful tools for autonomous robot systems,~\cite{Labb2018RTABMapAA,cartographer,orbslam} but these are far from being scalable.
Most of these existing works in SLAM use either an IMU or wheel-encoder to get the relative poses of the robot over time. 
These relative pose measurements in tandem with camera/LiDAR visual sensors are used to jointly optimize for absolute robot poses and simultaneously map the environment by correcting for the drifts in the IMU/odometry measurements. Unfortunately, introducing these camera/LiDAR sensors make the SLAM problem very compute and memory intensive.

Joint optimization for optimal Visual SLAM has three distinct operations: (1) feature extraction and tracking, (2) local feature matching and mapping, and (3) global loop-closures. 
The first two components aid in local pose estimation of the robot and mapping of the environment and are generally computationally light. Unfortunately, over time, these pose estimates accrue drifts and when robots revisit previously mapped areas, their current pose estimate disagrees with the map. The third component, performing global loop-closures, corrects for these erroneous drifts and builds coherent maps. Unfortunately, this is very compute and memory intensive and time consuming. 
% While the first two components are not compute intensive but only useful for local pose estimation and mapping, global loop-closure algorithms are very compute intensive, memory consuming, time consuming~\cite{semenova2022quantitative} but are required for global corrections, robot poses and map generation.
Furthermore, LiDAR-sensor based SLAM systems~\cite{cartographer} also utilize a similar three component structure, and the component performing global loop-closures is the most compute and memory intensive. 
% There are also LiDAR sensor based SLAM systems~\cite{cartographer} which also uses global loop closures, and are additionally very expensive, making LiDAR based SLAM algorithms too expensive and high-compute to deploy. 
%will: I moved the lidar sentence to the end of this paragraph since it was stuck in the middle of explaining why camera SLAM is bad

In contrast, there are a couple of decades of research in RF-based localization and tracking~\cite{ayyalasomayajula2018bloc,spotfi,uwb,bacscatter,rfid} that uses existing RF deployment architectures in the environment, like WiFi, to locate and track various devices in the environment.
As most of the current robots are connected to WiFi and owing to wide-spread deployment of WiFi, researchers have explored developing WiFi radios as sensor for SLAM implementations~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
These algorithms have been shown to not need global loop-closures making them `low-cost' and 'low-compute' systems~\cite{arun2022p2slam,zhang2020robot}.
However, \cite{zhang2020robot} uses WiFi backscatter that has very limited range and needs very extensive deployment of backscatter tags making them an expensive deployment.
On the other hand, in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, the authors employ an end-to-end optimization, sidestepping the challenges which arise when real-time pose estimates are needed.
Additionally, WiFi cannot map the space leading to lack of `context-awareness' for both the systems~\cite{arun2022p2slam,zhang2020robot}.


To solve these issues, in this paper we present \name, that amalgamates the best of both WiFi and camera worlds. 
While there exist few current works that try to incorporate WiFi-signals into existing Visual SLAM algorithms~\cite{hashemifar2019augmenting, liu2019collaborative,nguyen2021viral,jadhav2020wsr}, these systems only try to use the WiFi signals to aid in `global loop closures' ~\cite{hashemifar2019augmenting, liu2019collaborative} or depend on the Visual SLAM system to provide the pose of the WiFi sensor on board~\cite{nguyen2021viral,jadhav2020wsr} making them compute and memory hungry, and time consuming.
In contrast, \name is a first of its kind integration that maintains the `low-cost' and `low-compute' of RF sensor, and simultaneously utilizes a simple monocular camera that can provide `context-awareness' through mapping making it a scalable and deployable SLAM system.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/placeholder.pdf}
    \caption{\name's layered approach: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time.}
    \label{fig:intro_fig}
\end{figure}


Two key observations that inspires this scalable \name's design are that firstly, the existing camera based SLAM systems are the best possible solutions to provide a real-time and low-compute local map.
But these camera systems need heavy memory and compute resources to perform global robot pose estimations and optimization. 
So, if these camera SLAM systems could have access to an `Oracle' that could provide these global robot pose estimates, absent of any drifts, they can avoid compute heavy global loop-closures. 
Secondly, the existing WiFi based SLAM approaches provide optimized global robot poses with low-memory and compute demands but do not have context of the map or local surroundings.
Thus, these WiFi SLAM systems can provide for the global optimized poses to the camera SLAM systems which can then be fed as `Oracle' measurements to avoid global loop-closures.
With this intuition and the well established concepts of network layering/abstraction principals, we design a Dual-graph solution for WiFi and Visual SLAM nodes.
Wherein the first WiFi SLAM layer is defined with iSAM, an open-sourced GraphSLAM framework~\cite{gtsam} to obtain the optimized global pose estimates of the robot in real-time.
These global pose estimates are then fed in real-time as the `Oracle' camera locations (or odometry measurements) to the Visual SLAM layer that performs just the low-compute optimization stages of: 
(i) feature extraction and tracking using VINS-MONO~\cite{qin2018vins} algorithm, and 
(ii) local feature mapping and robot pose optimization  using a second `Camera graph' defined in iSAM.
This layered approach make the best use of the individual strengths of each sensing modality allowing \name-SLAM to be a real-time, scalable and deployable SLAM solution.


This \underline{Vi}sual \underline{Wi}Fi \underline{D}ual graph SLAM solution of \name-SLAM leads to the following set of challenges,

\noindent\textbf{Robust WiFi Measurements:} To define the measurements to be used in the WiFi factor graph, few of the past works have tried to integrate RSSI measurements~\cite{bruno2011wislam,ferris2007wifi}. Unfortunately, it is well known that these RSSI measurements are very fickle for indoor scenarios. 
So in recent past, researchers have shown reliable performance with using angle-of-arrivals measured to or from the WiFi sensor on the robot~\cite{arun2022p2slam,jadhav2020wsr} to the Access Points in the environment as the WiFi feature measurement.
Thus, in \name we utilize these robust bearing measurements in tandem with IMU/Odometer over multiple poses of the robot in real-time for optimization.

\noindent\textbf{Real-time and accurate WiFi pose estimates:} Real-time WiFi factor graph optimization in turn demands that the bearing measurements have to be furnished with minimum latency. 
While there exist simple FFT based approaches~\cite{ayyalasomayajula2018bloc} which are low-latency, they can be very inaccurate in estimating the bearing due to dynamic multipath and non-line of sight (NLoS) scenarios. 
While this is currently solved by temporal averaging in MUSIC and SpotFi~\cite{arraytrack,spotfi}, these algorithms are very time-consuming.
But, these algorithms demonstrate that since direct path is the only consistent path over time, temporal averaging would increase the signal strength recieved for direct path over all the reflected paths.
Thus, \name uses SVD-FFT that takes the advantage of packet averaging ideas from the MUSIC and SpotFi~\cite{arraytrack,spotfi} while maintaining the latency of the order of FFT based approaches~\cite{ayyalasomayajula2018bloc}.
These real-time accurate WiFi bearing measurements are then fed to the WiFi graph in tandem with IMU/Odometer measurements over multiple poses of the robot for optimization defined by the iSAM's factor graph~\cite{gtsam}. 

\noindent\textbf{Access Point Initialization:} \name's WiFi real-time iSAM GraphSLAM implementation does not assume the location of the WiFi access points in the environment as most of the existing WiFi SLAM algorithms~\cite{ferris2007wifi,arun2022p2slam}. 
Although unlike the existing works~\cite{arun2022p2slam} that perform end-to-end optimization, \name does real-time pose estimates using incremental pose-graph optimization using iSAM.
This leads to the optimization becoming indeterminate or ill-conditioned in the WiFi graph optimization if the APs are all initialized at the origin.
Thus to overcome this ill-defined optimization issues, in \name we smartly initialize the location of the WiFi AP at the time instance when the signal strength measured for the access point is a local maxima along the path taken.
This further implies that all the bearing factors measured to that AP are also fed into the factor graph at the instance the AP is placed, thus avoiding any ill-conditioned factor graph optimizations.
% This optimization is done over all the robot poses to date in the graph by backpropagating any errors to optimize for the overall bot and AP poses in real-time. \todo{this is not right?} 
% At a high level, the presence of bearings measured at the robot allows for accurate mapping of the WiFi access points in the environment and also simultaneously locate itself with respect to these global landmarks.
% Thus, \name's WiFi factor graph does not also need to assume the location of the WiFi access points in the environment, making it independent from the WiFi infrastructure.

\noindent\textbf{Judicious Pose updates to Camera Graph:} Finally, these optimized robot poses generated from the WiFi graph need to be updated to the camera factor graph defined with iSAM in real-time.
Unfortunately, this is not as straightforward as obtaining real-time pose updates to all the existing odometry pose factors of the camera graph.
As too frequent pose updates that are significantly large for the past Odometer readings would trigger frequent end-to-end graph optimization and updates in the camera graph which becomes memory intensive as the number of robot poses keep increasing.
To avoid this, \name's WiFi graph's pose updates are maintained in a buffer that is continuously updated when there are frequent large updates.
This buffer of pose-updates are pushed as odometer updates to the camera graph only when these global pose updates are lesser than a threshold, which is empirically determined.
This buffer-based updates avoids frequent global camera graph optimization avoiding high compute and memory demanding operations.
% While this buffered-updates creates lag in the camera graph's updates with respect to the WiFi graph.
% Fortunately though, the WiFi Graph optimization is triggered at 100s of Hz that this delay due to buffer-based camera pose updates are not observable for practical robot's real-time mapping and pose-estimation that is performed at 1-10Hz.

With these solutions \name overcomes the challenges of designing first of its kind layered (dual-graph) approach to solve for a low-cost, low-compute and context-aware SLAM system.
% Thus \name designs first of its kind layered (dual-graph) approach by bringing the best out of both the camera and the WiFi sensors to solve for a low-cost, low-compute and adaptable SLAM system.


These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publicly available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.
% Furthermore, we showcase \name with a simple application that maps with labelled room numbers and autonomously navigates to a given room number to deliver a package. 

==> ViWiD SLAM_arx/intro/intros_old/intro7.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/placeholder.pdf}
    \caption{\name Deployed in a real world environment with the WiFi SLAM providing accurate global pose estimates and the camera graph providing accurate map of the environment}
    \label{fig:intro_fig}
\end{figure}

Recent times have seen a rise in demand for autonomous robots and drones for various applications ranging from inventory management in warehouses, hospitals and construction sites~\cite{hosptials,warehoueses,construction,sites} to the navigation~\cite{navigation,robots} and exploration robots~\cite{exploration,robots} for last-mile delivery~\cite{last,mile,delivery}, mapping~\cite{Labb2018RTABMapAA}, and disaster relief~\cite{disaster,relief,jadhav2020wsr}. 
Furthermore, many of these applications demand a fleet of coordinated robots to perform tasks efficiently. 
To deliver on these applications, Simultaneous Localization and Mapping (SLAM) algorithms need to be (a) `low-compute', to ensure real-time operation on memory and compute constrained machines, (b) `low-cost', to ensure wide deployment, and (c) `context-aware' to be able to react to environmental changes, which requires a map of the environment the robot is exploring.

There exist many powerful tools for autonomous robot systems,~\cite{Labb2018RTABMapAA,cartographer,orbslam} but these are far from being scalable.
Most of these existing works in SLAM use either an IMU or wheel-encoder to get the relative poses of the robot over time. 
These relative pose measurements in tandem with Visual/LiDAR sensors are used to jointly optimize for absolute robot poses and simultaneously map the environment by correcting for the drifts in the IMU/odometry measurements. 
Unfortunately, introducing these Visual/LiDAR sensors make the SLAM problem very compute and memory intensive.

Joint optimization for optimal Visual SLAM has three distinct operations: (1) feature extraction and tracking, (2) local feature matching and mapping, and (3) global loop closures. 
The first two components aid in local pose estimation of the robot and mapping of the environment and are generally computationally light. Unfortunately, over time, these pose estimates accrue drifts and when robots revisit previously mapped areas, their current pose estimate disagrees with the map. The third component, performing global loop closures, corrects for these erroneous drifts and builds coherent maps. Unfortunately, this is very compute and memory intensive and time consuming. 
Furthermore, LiDAR-sensor based SLAM systems~\cite{cartographer} also utilize a similar three component structure, and the component performing global loop closures is the most compute and memory intensive. 

In contrast, there are a couple of decades of research in RF-based localization and tracking~\cite{ayyalasomayajula2018bloc,spotfi,uwb,bacscatter,rfid,ma2019wifi} that uses existing RF deployment architectures in the environment, like WiFi, to locate and track various devices in the environment.
As most of the current robots are connected to WiFi and owing to wide-spread deployment of WiFi, researchers have explored developing WiFi radios as sensor for SLAM implementations~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
These algorithms have been shown to not need global loop closures making them `low-cost' and 'low-compute' systems~\cite{arun2022p2slam,zhang2020robot}.
However, \cite{zhang2020robot} uses WiFi backscatter that has very limited range and needs very extensive deployment of backscatter tags making them an expensive deployment.
On the other hand, in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, the authors employ an end-to-end optimization, sidestepping the challenges which arise when real-time pose estimates are needed.
Additionally, WiFi cannot map the space leading to lack of `context-awareness' for both the systems~\cite{arun2022p2slam,zhang2020robot}.


To solve these issues, in this paper we present \name, that amalgamates the best of both WiFi and camera worlds and provides for accurate pose estimations and low-compute, low-power mapping as demonstrated in Figure~\ref{fig:intro_fig}.
While there exist few current works that try to incorporate WiFi-signals into existing Visual SLAM algorithms~\cite{hashemifar2019augmenting, liu2019collaborative,jadhav2020wsr}, these systems only try to use the WiFi signals to aid in `global loop closures' ~\cite{hashemifar2019augmenting, liu2019collaborative} or depend on the Visual SLAM system to provide the pose of the WiFi sensor on board~\cite{jadhav2020wsr} making them compute and memory hungry, and time consuming.
In contrast, \name is a first of its kind integration that maintains the `low-cost' and `low-compute' of RF sensor, and simultaneously utilizes a simple monocular camera that can provide `context-awareness' through mapping making it a scalable and deployable SLAM system.


Two key observations that inspires this scalable \name's design are that firstly, the existing camera based SLAM systems are the best possible solutions to provide a real-time and low-compute local map.
But these camera systems need heavy memory and compute resources to perform global robot pose estimations and optimization~\cite{semenova2022quantitative}. 
So, if these camera SLAM systems could have access to an `Oracle' that could provide these global robot pose estimates, absent of any drifts, they can avoid compute heavy global loop closures. 
Secondly, the existing WiFi based SLAM approaches provide optimized global robot poses with low-memory and compute demands~\cite{arun2022p2slam,jadhav2020wsr} but do not have context of the map or local surroundings.
Thus, these WiFi SLAM systems can provide for the global optimized poses to the camera SLAM systems which can then be fed as `Oracle' measurements to avoid global loop closures.
With this intuition and the well established concepts of network layering/abstraction principals~\cite{session1994it5}, we design a Dual-graph solution for WiFi and Visual SLAM nodes.
Wherein the first WiFi SLAM layer obtains the optimized global pose estimates of the robot in real-time.
These global pose estimates are then fed in real-time as the `Oracle' camera locations (or odometry measurements) to the Visual SLAM layer.
This Visual SLAM system not needing global loop-closures only performs just the low-compute optimization stages (1 and 2 from above) providing local pose corrections and environment mapping. Thus making \name's design scalable.


This \underline{Vi}sual \underline{Wi}Fi \underline{D}ual graph SLAM solution of \name-SLAM leads to the following set of challenges:

\noindent\textbf{(a) Robust WiFi Measurements:} To define the measurements to be used in the WiFi factor graph, few of the past works have tried to integrate RSSI measurements~\cite{bruno2011wislam,ferris2007wifi}. 
Unfortunately, it is well known that these RSSI measurements are very fickle for indoor scenarios. 
So in recent past, researchers have shown reliable performance with using angle-of-arrivals measured to or from the WiFi sensor on the robot~\cite{arun2022p2slam,jadhav2020wsr} to the Access Points in the environment as the WiFi feature measurement.
Thus in \name, we utilize these robust bearing measurements in tandem with IMU/Odometer over multiple poses of the robot in real-time for optimization.

While most of these bearing measurements are done taking the advantage of Uniform Linear arrays~\cite{arraytrack, spotfi}, but these linear arrays can only solve for half-planes thus providing for ambiguity whether the robot is in front or at the back of the AP. Thus in \name we avoid this issue by adapting to a square antenna array with appropriate antenna spacing to avoid any ambiguities.

\noindent\textbf{(b) Real-time \& accurate WiFi Bearing estimates:} Real-time WiFi factor graph optimization in turn demands that the bearing measurements have to be furnished with minimum latency. 
While there exist simple FFT based approaches~\cite{ayyalasomayajula2018bloc} which are low-latency, they can be very inaccurate in estimating the bearing due to dynamic multipath and non-line of sight (NLoS) scenarios. 
While this is currently solved by temporal averaging in MUSIC and SpotFi~\cite{arraytrack,spotfi}, these algorithms are very time-consuming.
But, these algorithms demonstrate that since direct path is the only consistent path over time, temporal averaging would strengthen the signal received for direct path over all the reflected paths.

\name uses novel SVD-FFT algorithm that takes the advantage of packet averaging ideas from the MUSIC and SpotFi~\cite{arraytrack,spotfi} while maintaining the latency of the order of FFT based approaches~\cite{ayyalasomayajula2018bloc}.
These real-time accurate WiFi bearing measurements are then fed to the WiFi graph in tandem with IMU/Odometer measurements over multiple poses of the robot for optimization defined in iSAM~\cite{gtsam}. 

\noindent\textbf{(c) Access Point Initialization:} \name's WiFi real-time iSAM GraphSLAM implementation does not assume the location of the WiFi access points in the environment as most of the existing WiFi SLAM algorithms~\cite{ferris2007wifi,arun2022p2slam}. 
Although unlike the existing works~\cite{arun2022p2slam} that perform end-to-end optimization, \name does real-time pose estimates using incremental pose-graph optimization using iSAM.
This leads to the optimization to be ill-conditioned in the WiFi graph optimization if the APs are all initialized at the origin.

To overcome this ill-defined optimization issues, in \name we initialize the location of the WiFi AP at the time instance when the signal strength measured for the access point is a local maxima along the path taken.
This further implies that all the bearing factors measured to that AP are also fed into the factor graph at the instance the AP is placed, thus avoiding any ill-conditioned factor graph optimizations.


\noindent\textbf{(d) Judicious Pose updates to Camera Graph:} Finally, the optimized robot poses generated by the WiFi graph update the robot poses in the camera factor graph in real-time.
A straightforward way to update these robot poses would be for the WiFi graph to push all the updates and trigger an end-to-end optimization of the camera graph to fix all pose drifts accumulated. 
Unfortunately, frequent, numerous and large pose updates which trigger end-to-end graph optimization in the camera graph becomes memory intensive. 

To keep the memory usage low and provide accurate pose updates to camera graph, \name's WiFi graph's updates are buffered when frequent and large corrections are made. 
Finally, once the large corrections to the WiFi graph are completed, which spans a period of few seconds, this buffer of pose corrections is pushed as `Oracle' updates to the camera graph. This buffer-based updates avoids frequent global camera graph optimization avoiding high compute and memory demanding operations.

% \noindent\textbf{Easy Integration of All Sensing Modalities:}  \todo{Add final system level contribution of enabling easy integration of any sensing modality with wifi graph.}

With these solutions \name overcomes the challenges of designing first of its kind layered (dual-graph) approach to solve for a low-cost, low-compute and context-aware SLAM system. 
Additionally, this layered approach of \name enables the same advantages as it did for communication layers, in that each layer could be independently used as a plug and play model.
That is, although we have demonstrated \name using WiFi owing to its wide-scale deployment one of the major advantages \name is that it abstracts bearing as the sensor measurement input, and global pose updates as the output.
Thus any RF-sensor that can report their bearings like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative RF-sensors.
These sensors like WiFi sensors would also provide the global pose estimates that can be plugged into the camera graph. Similarly, the camera graph is not limited to either the VINS-MONO feature extractor or on camera itself, we can easily replace it with LiDAR and its corresponding sensor to get the similar mapping results from the global pose estimates received from the RF-Graph.

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publicly available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.

==> ViWiD SLAM_arx/intro/intros_old/intro8.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/visual_drawbacks-crop.pdf}
    \caption{Drawbacks of Visual SLAM systems: (a) Local loop-closures are scalable (b) Global loop-closures and corrections make these systems memory and compute intensive.}
    \label{fig:visual-bad}
\end{figure}
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
The advantage of these robots, apart from being autonomous, is that they can be deployed without any prior knowledge of the environment and the robots can explore and navigate within the environment.
This is because these robots utilize a Simultaneous Localization and Mapping (SLAM) framework, where they can simultaneously locate themselves and map the environment around them.
Despite these advantages, the current SLAM based robot systems are not yet widely deployed for these indoor applications.


The majority of current SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometer measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment.
These visual and LiDAR sensors that grant the system mapping and localization capabilities also make the system both memory and compute intensive~\cite{semenova2022quantitative}.
This is mainly because of the `loop-closures' happening as shown in Figure~\ref{fig:visual-bad}b.

Conceptually these Visual sensors are identifying key features (f1-f10k) in the environment called `landmarks'.
These landmarks are mapped and in turn the robot locating itself with respect to how these landmarks are changing from one instance to the other, thus performing SLAM.
However, as seen the robot can quickly accrue drift due to Odometer readings and needs correction which happens by matching current landmarks with old ones.
While this is not memory or compute intensive for local corrections as shown in Figure~\ref{fig:visual-bad}a which requires smaller search space of `landmarks' and fewer pose corrections.
But global `loop-closure' as shown in Figure~\ref{fig:visual-bad}b would need active memory of all the 10k landmarks and corrections backpropagated over many poses, making the system memory and compute intensive.
In order to make these SLAM robotic systems scalable we need a SLAM system design that achieves compute and memory efficiency without compromising on the robot pose estimation and environment mapping.
Consequently, identifying a sensor to use in the SLAM systems that can alleviate these limitations of Visual and LiDAR sensors is required.
WiFi based SLAM systems are an attractive sensor modality which have shown to be memory and compute efficient~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
So the idea of the dual-layered SLAM is that the first WiFi SLAM layer obtains the optimized global pose estimates of the robot in real-time, which are then sent over to the camera SLAM.
Unfortunately though, since they utilize WiFi as the only sensor neglecting the already widely deployed cameras on the robots which in turn disable them from getting the map of the environment compromising the intent of SLAM.

To that end, we propose \name's key idea of a Dual-layered solution for WiFi and Visual (camera) SLAM nodes, or rather ViWiD-SLAM (\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered SLAM) that is inspired from the network layering/abstraction principals~\cite{session1994it5}. 
A key intuition that motivates this dual-layered design of \name, is that for the camera SLAM can be made compute and power efficient if the robot had accurate pose estimates from an `Oracle'.
Since, this knowledge of accurate pose estimates, would not lead to the accrued drift on a global scale as shown in Figure~\ref{fig:visual-bad}b.
This avoids the need for compute and memory intensive global loop closures, while still being able to map the environment using local mapping.
Thus, the Visual SLAM system can utilize the global poses from WiFi layer as `Oracle' measurements and can track the landmarks from the monocular camera and optimize for local pose corrections and provide a map of the environment.
Thus, this Dual-layered WiFi and Visual SLAM systems enable compute and memory efficient SLAM system that can provide accurate global pose estimations and map.

This abstraction of the complementary pose estimation WiFi SLAM, and the environment mapping Visual SLAM layers has advantages as in networking layer abstractions~\cite{session1994it5}.
That is both the pose estimation layer and the mapping layer can be optimized within themselves without effecting the other layer's performance.
For example, while we use WiFi-sensor for \name's implementation due to its widespread deployment in indoors, other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative sensors depending on the use case.

To implement \name, we have deployed both the WiFi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
This GraphSLAM framework utilizes the measurements from the sensors as factors to tie the mapped environment to the robot poses and optimize for both robot poses and the map simultaneously.
So, we need to first identify the measurements for both WiFi and the Visual camera sensors that can be used to define the graph for the GraphSLAM optimization framework.
To this extent, we use the widely used Shi-Tomasi features~\cite{shi1994good} for the camera sensor and extract them using the opensourced VINS-MONO feature tracker~\cite{qin2018vins}.
For the WiFi sensor features, it has been extensively shown that the angle of arrival(AoA) measurements  based localization~\cite{spotfi,arraytrack} and SLAM~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} are more robust.
Thus in \name, we utilize these AoA measurements in tandem with IMU/Odometer over multiple poses of the robot in real-time for optimization of the WiFi SLAM layer.


In the WiFi SLAM layer, to provide the `Oracle' global pose estimates to the Camera graph, we need to be able to perform real-time WiFi graph optimization. 
This in turn demands real-time and robust AoA measurements from the WiFi readings.
While the  existing AoA prediction algorithm like MUSIC and SpotFi~\cite{arraytrack,spotfi} provide robust measurements using temporal averaging and super-resolution, they are very time-consuming.
But, these algorithms demonstrate that since direct path is the only consistent path over time, temporal averaging would strengthen the signal received for direct path over all the reflected paths.
With this intuition, in \name we create a novel real-time and robust AoA estimation algorithm we call \textit{SVD-FFT}.
This algorithm takes the advantage of packet averaging ideas from the MUSIC and SpotFi~\cite{arraytrack,spotfi} while maintaining the latency of the order of 2D-FFT based approaches~\cite{ayyalasomayajula2018bloc,xie2019md}.
These real-time accurate WiFi bearing measurements are then fed to the WiFi graph in tandem with IMU/Odometer measurements over multiple poses of the robot for optimization defined in iSAM~\cite{gtsam}. 


Additionally, as with any SLAM system \name's WiFi SLAM layer does not assume apriori information about the environment which includes the location of the WiFi access points to which robot measures its AoA. 
This lack of knowledge of WiFi access points do not lead to any inconsistencies when the WiFi graph is optimized end-to-end in post-factum to data collection as demonstrated in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}.
Unlike $\mathrm{P^2}$SLAM, \name does real-time pose estimates using incremental pose-graph optimization using iSAM that lays down the WiFi AoA measurements incrementally.
This would lead to many of the APs have which not yet been discovered in the environment or are not effected by the current incoming bearing measurements, thus making the optimization problem ill-defined.
To overcome this ill-defined optimization issues, in \name we take advantage of the WiFi received signal strength (RSSI) proximity sensing~\cite{ez,zee}.
That is we initialize the location of the WiFi AP at the time instance when the RSSI measured for a given access point is a local maxima along the path taken.
This further implies that all the AoA measurements to that AP are also fed into the graph optimization at the instance the AP is placed, thus avoiding any ill-conditioned optimization definitions.


Finally, the optimized robot poses generated by the WiFi graph update the robot poses in the camera graph in real-time.
Unfortunately, frequent, numerous and large pose updates which trigger end-to-end graph optimization in the camera graph becomes memory and compute intensive. 
While, we can naively add simple timed buffer to lag the camera graph behind the WiFi graph this would be inefficient as these numerous and large pose updates do not always occur.
Instead, in \name's design we buffer the WiFi graph's updates only when frequent and large corrections to the past poses are made. 
Once the large corrections to the WiFi graph are completed, this buffer of pose corrections is pushed as `Oracle' updates to the camera graph. 
This smart buffer-based updates avoids frequent global camera graph optimization avoiding high compute and memory demanding camera optimization operations.

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over a publicly available dataset~\cite{arun2022p2slam} and also a more complete dataset we have collected. Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} cpu cores which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item Finally, we show that this low-compute and low-memory does not compromise \name's SLAM performance. Where we show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error which are on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Additionally, we would also open-source the dataset that we have collected to enable further research and development in this layered SLAM domain for sensor fusion approaches.



==> ViWiD SLAM_arx/intro/intros_old/intro9.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot.
However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholder.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, as when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM systems are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features.
Thus, existing Visual SLAM systems are not light-weight and require extensive compute and memory resources to operate in real time, hindering their deployment in the real world~\cite{semenova2022quantitative}. However, visual sensors are still necessary for building a contextual map of the robot's environment. So, there is a need for a robust Simultaneous `Localization' and `Mapping' solution that is also compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
We present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm, which uses a Wi-Fi sensing based layer to provide pose (position and orientation) estimations, without assuming the Wi-Fi access point locations, to \name's visual layer as shown in Figure~\ref{fig:intro-fig}.
Since Wi-Fi pose measurements do not accrue drift over time, unlike standard visual SLAM algorithms, \name does not need to cross-correlate measurements across time to correct for these drifts.
Thus, using the \name Wi-Fi layer's pose estimations the map can be estimated by the \name visual layer in a compute and memory efficient manner.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.
While \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method generalizes to other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or next gen 5G femto-cell implementations~\cite{5g}. 
Additionally, this abstraction of the complementary pose estimation WiFi layer, and the environment mapping \name Visual layers will bring the advantages of networking layer abstractions~\cite{session1994it5} to the research in SLAM.
%above paragraph: emphasize no AP priors

% figure: robot, rf layer -> visual layer
%Design ideas behind dual-graph (bring up performance), can use more than just Wi-Fi.

However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi localization solutions and feeding them into existing Visual SLAM algorithms.
We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free pose estimates from the Wi-Fi layer to be robust and real-time. To get these pose estimates from the Wi-Fi-layer, we employ Angle of Arrival (AoA) based localization~\cite{spotfi,jadhav2020wsr,arun2022p2slam,ayyalasomayajula2018bloc}, due to its widespread use.
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these systems use compute intensive super-resolution algorithms, which cannot provide AoA measurements at the rate needed for real time pose estimation.
%I would be cautious about bragging too much about svdfft, it is not a new algorithm.
To solve this, in \name we employ a CSI de-noising algorithm, borrowing intuition from MUSIC~\cite{schmidtmusic,spotfi}, which both smooths erroneous measurements and attenuates multipath components in the signal. This smoothed CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. We use this method to measure AoA between the robot and Wi-Fi access points in the environment. However, this alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we cannot assume access point locations are known a priori.

\noindent\textbf{Unknown Wi-Fi Access Point Locations:} GraphSLAM~\cite{gtsam} is well known to jointly solve for multi-variate optimization as long as these variable are connected by some measurements.
So we define the Wi-Fi graph with the Odometry measurements connecting two continuous robot poses, and the Wi-Fi AoA measurements connecting the robot's current pose with each AP's position the AoA corresponds to. 
Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, we need to provide initial values to variables in question. 
While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. 
To overcome this issue, a naive solution can be to initialize all the AP locations at the origin. 
This is not an issue when the AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. 
However, when few measurements constrain the AP's pose, as is the case when the robot first traverses the environment for the real time, the optimizer is poorly conditioned. 
To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) proximity sensing~\cite{ez,zee}.
That is we initialize the location of the Wi-Fi AP at the time instance when the RSSI measured for a given access point is a local maxima along the path taken.

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Finally, the optimized robot poses generated by the Wi-Fi graph need to update the robot poses in the camera graph in real-time.
Unfortunately, if the already traversed robot poses are getting large corrections very frequently, it would result in large and frequent feature map corrections in the camera graph as well, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made.
These accumulated corrections are only pushed to the Camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.


These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We extract widely used Shi-Tomasi features~\cite{shi1994good} for the camera sensor using the opensourced VINS-MONO feature tracker~\cite{qin2018vins}.
We evaluate \name over a publicly available dataset~\cite{arun2022p2slam} and also a more complete dataset we have collected.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.

==> ViWiD SLAM_arx/related_work/related.tex <==
% !TEX root = root.tex
\section{Related Work}\label{sec:related}

\name's design motivation is to develop a context enabled SLAM algorithm that is low-cost, low-compute and solves for the problems plaguing many existing works. 
These existing works span the fields of visual sensor based SLAM, RF-sensors in SLAM and RF-sensor based localization, mapping, and tracking algorithms.

\noindent\textbf{Visual SLAM:} SLAM for Indoor navigation has been actively pursued by the robotics community for the past decade that led to a myriad of SLAM algorithms~\cite{Labb2018RTABMapAA,mur2015orb,qin2018vins,cartographer}. Most of these algorithms extensively rely on LiDAR~\cite{cartographer} and/or cameras (both monocular or RGBD)~\cite{Labb2018RTABMapAA, mur2015orb}. While these algorithms achieve cm-accurate localization and feature-rich mapping of the environment, they tend to fail under poor-lighting conditions, feature-degenerate conditions. These algorithms also rely on `loop closures' and `re-localization' for larger spaces that require heavy compute on edge making them difficult to scale. In contrast, \name is designed to rely on WiFi for localization and camera for context/mapping thus removing the need for loop closures for the compute intensive camera features. This design ensures that it does not rely on loop closures as the WiFi APs are a constant landmarks known to the robot making it low-compute  and still providing the context of the map.

\noindent\textbf{Dual Layered SLAM:} There are other dual layered SLAM body of works that just use Visual sensors for both the pose estimation and the mapping, called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel}. 
While, these works try to minimize the calls but still use loop-closures loop-closures and bundle adjustments making them less memory and compute efficient compared to \name's design.
On the other hand, there are some Decentralized SLAM works that off-load the memory intensive loop-closure and map updates~\cite{cieslewski2018data,ahmad2020carmap} to the cloud to minimize the memory and compute on the device deployed on the robot. Even these works can benefit from \name's implementation to make systems more efficient even at the cloud.
Finally, there are some outdoor navigation works that utilize GPS as an additional sensor for outdoor autonomous driving assistance systems~\cite{nandikolla2021navigation,kiss2019gps} but are still limited to using loop-closures to correct for the car's pose in the long run owing to GPS's poor resolution.

\noindent\textbf{RF-sensors for SLAM:} Many RF-technology based SLAM implementations based on UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot} exist. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi. 
We note that, extension of \name's WiFi implementation to other RF-sensors is trivial, as we abstract bearing as the measurement feature of the WiFi sensor's measurement. 
Thus, as long as they are able to measure bearings~\cite{uloc} to and/or from the robot to fixed access points in the environment any RF system can make use of \name's implementation.


\noindent\textbf{WiFi-SLAM:} There are a few existing works~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi,hashemifar2019augmenting, liu2019collaborative} that try to utilize WiFi sensor readings to improve SLAM algorithms. Unfortunately, most of these works utilize RSSI as the features metric which needs intense mapping of the space and are known to vary drastically in dynamic indoor scenarios~\cite{ma2019wifi}, making them unsuitable metrics for WiFi signals.
While there are recent works~\cite{jadhav2020wsr,arun2022p2slam} that utilize bearing measurements for their SLAM implementations, WSR~\cite{jadhav2020wsr} does not perform localization but just robot reconnaissance. On the other hand, $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} does not provide any context of the surroundings and performs an end-to-end optimization which does not help in making real-time context aware decisions for the robots. In contrast, \name uses camera features for providing real-time context to in-tandem WiFi bearing measurements that are enabling accurate localization of the robot.

\noindent\textbf{RF Localization:} Past two decades of research in RF-based localization, does not SLAM but only localization and tracking~\cite{spotfi,arraytrack,soltanaghaei2018multipath,ayyalasomayajula2020deep, ma2019wifi} of either the source or the receiving sensor. In contrast, \name integrates WiFi with camera to Simultaneously Locate the bot and Map the environment, without assuming any prior information about locations in the environment.


\iffalse
\name's concept and design overlap with a myriad of fields ranging from SLAM for robotics to RF-sensors based localization, tracking and navigation systems
% Visual sensors -- Camera/Lidar based

\noindent\textbf{Visual Sensors:} Indoor navigation has been actively pursued by the robotics community in the past decades. There is extensive work relying on LIDAR's~\cite{} and cameras~\cite{} which allow for cm-accurate navigation estimates in feature-rich and well-lit environments. Unfortunately, as discussed above, these assumptions may not be valid in a large number of environments. 

Radar Based 

Audio/Ultrasonic

RFID based

UWB/Bluetooth based

WiFi Based sensing
1. Cover existing localization work -- spotfi, arraytrack, ubilocate etc.
  Work poorly in Low density scenario

k poorly in Low density scenario
  Show only stationary device results
  Do not demonstrate real-time localization requirements
  Do not identify poor packets and provide confidence metrics
2. RSSI-based SLAM
3. Loop closure assistance using RSSI
4. CSI-AoA methods

VIRAL SLAM~\cite{nguyen2021viral} uses UWB based ranging in conjunction with LiDAR's, cameras and IMU's to develop a tightly coupled and robust 3D drone based localization and mapping. \todo{not strong enough: Unfortunately, the deployment of various UWB anchors in the environment limits the adoption of this solution}. \todo{kill radar: Why?} The systems proposed in \cite{sato2019rapid, jadidi2018radio} use range information extracted from BLE's received signal strength to correct for drifts accrued by the onboard IMU. Unfortunately, RSSI-based systems have been proven to be inadequate to changing environment conditions and hence act as a poor proxy to range. RFly~\cite{ma2017drone} takes advantage of  RFID tags attached in the environment as robust landmarks, and in conjunction with RFID readers deployed in the environment, jointly estimates the location of a drone and these RFID tags. In a similar vein, Rover~\cite{zhang2020robot} uses WiFi backscatter tags placed in the environment to jointly estimate the location of the robot and tags. Unfortunately, these tags have small range and these systems would require a dense deployment of tags to work, scaling poorly to large environments and requiring a high cost of deployment. The final RF based sensing briefly touched upon before is WiFi. It provides inherent advantages due to its long range and ubiquitous deployment both in the environment and on most robots. 
\fi

==> ViWiD SLAM_arx/related_work/related2.tex <==
% !TEX root = root.tex
\section{Related Work}\label{sec:related}

\name's design motivation is to develop a context enabled SLAM algorithm that is low-cost, low-compute and solves for the problems plaguing many existing works. 
These existing works span the fields of visual sensor based SLAM, RF-sensors in SLAM and RF-sensor based localization, mapping, and tracking algorithms.

\noindent\textbf{Visual SLAM:} SLAM for Indoor navigation has been actively pursued by the robotics community for the past decade that led to a myriad of SLAM algorithms~\cite{Labb2018RTABMapAA,mur2015orb,qin2018vins,cartographer}. Most of these algorithms extensively rely on LiDAR~\cite{cartographer} and/or cameras (both monocular or RGBD)~\cite{Labb2018RTABMapAA, mur2015orb}. While these algorithms achieve cm-accurate localization and feature-rich mapping of the environment, they tend to fail under poor-lighting conditions, feature-degenerate conditions. These algorithms also rely on `loop closures' and `bundle-adjustments' for larger spaces that require heavy compute on edge making them difficult to scale. In contrast, \name does not need loop closures or `bundle adjustments'  to provide accurate pose estimations and human readable maps.

\noindent\textbf{Dual Layered SLAM:} There are other dual layered SLAM body of works that just use Visual sensors for both the pose estimation and the mapping, called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel}. 
While, these works try to minimize the calls but still use loop-closures loop-closures and bundle adjustments making them less memory and compute efficient compared to \name's design.
On the other hand, there are some Decentralized SLAM works that off-load the memory intensive loop-closure and map updates~\cite{cieslewski2018data,ahmad2020carmap} to the cloud to minimize the memory and compute on the device deployed on the robot. Even these works can benefit from \name's implementation to make systems compute and memory efficient even at the cloud, owing to \name's light-weight design.
Finally, there are some outdoor navigation works that utilize GPS as an additional sensor for outdoor autonomous driving assistance systems~\cite{nandikolla2021navigation,kiss2019gps} but are still limited to using compute and memory intensive loop-closures to correct for the car's pose in the long run owing to GPS's poor resolution.

\noindent\textbf{RF-sensors for SLAM:} Many RF-technology based SLAM implementations based on UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot} exist. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi. 
We note that, extension of \name's WiFi implementation to other RF-sensors is trivial, as we abstract bearing as the measurement feature of the WiFi sensor's measurement. 
Thus, as long as they are able to measure AoAs~\cite{zhao2021uloc} to and/or from the robot to fixed access points in the environment any RF system can make use of \name's implementation.


\noindent\textbf{WiFi-SLAM:} There are a few existing works~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi,hashemifar2019augmenting, liu2019collaborative} that try to utilize WiFi sensor readings to improve SLAM algorithms. Unfortunately, most of these works utilize RSSI as the features metric which needs intense mapping of the space and are known to vary drastically in dynamic indoor scenarios~\cite{ma2019wifi}, making them unsuitable metrics for WiFi signals.
While there are recent works~\cite{jadhav2020wsr,arun2022p2slam} that utilize bearing measurements for their SLAM implementations, WSR~\cite{jadhav2020wsr} does not perform localization but just robot reconnaissance. On the other hand, $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} does not provide any maps of the surroundings and performs an end-to-end optimization which does not help in making real-time awareness to the robots for example to avoid crashes into other robots or humans. In contrast, \name uses camera features for providing real-time context to in-tandem WiFi bearing measurements that are enabling accurate localization of the robot.

% \noindent\textbf{RF Localization:} Past two decades of research in RF-based localization, does not SLAM but only localization and tracking~\cite{spotfi,arraytrack,soltanaghaei2018multipath,ayyalasomayajula2020deep, ma2019wifi} of either the source or the receiving sensor. In contrast, \name integrates WiFi with camera to Simultaneously Locate the bot and Map the environment, without assuming any prior information about locations in the environment.

==> abstract/abstract1.tex <==
% !TEX root = root.tex

\begin{abstract}
% A recent spur of interest in indoor robotics has increased the importance of robust simultaneous localization and mapping algorithms in indoor scenarios. This robustness is typically provided by the use of multiple sensors which can correct each others' deficiencies. In this vein, exteroceptive sensors, like cameras and LiDARs, employed for fusion are capable of correcting the drifts accumulated by wheel odometry or inertial measurement units (IMU's). However, these exteroceptive sensors suffer their own deficiencies in highly structured environments and dynamic lighting conditions. This paper will present WiFi as a robust and straightforward sensing modality capable of circumventing these issues. Specifically, we make three contributions. First, we will understand the necessary features to be extracted from WiFi signals. Second, we characterize the quality of these measurements. Third, we integrate these features with odometry into a state-of-art GraphSLAM backend. We present our results in a $25 \times 30$ m and $50 \times 40$ environment and robustly test the system by driving the robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $6 \times$ with respect to odometry-only estimation and perform on par with one of the state-of-the-art Visual-based SLAM. 

WiFi infrastructure is ubiquitous in most indoor settings and thus can be leveraged as a sensor for indoor mapping and navigation. In this paper, we present \name, which incorporates WiFi as a bearing sensor and densely fuses it with visual features from a monocular camera and odometry sensors. The sensor fusion proposed in \name provides accurate and accessible localization and mapping capabilities scalable to large indoor environments. To showcase these claims, \name is deployed in two real-world environments, spanning $25 \times 30$ m and $50 \times 40$ m, and robustly tested by driving the robot a cumulative distance of over $1225$ m. In these evaluations, \name shows an improvement of $xx \times$ and $xx \times$ over solely using odometry and visual-inertial odometry respectively. \name is further showcased by deploying an application which autonomously navigates an office space to deliver packages to specific rooms. 
\end{abstract}

==> background/background1.tex <==
\section{Background and Motivation}

To robustly solve the SLAM problem requires two parts -- the sensing front-end and the optimization back-end. Consider a simple monocular camera sensor, the sensing front end would consist of two parts -- identifying robust feature keypoints in the images, and matching them across different camera image frames based on their unique descriptions. These keypoints are generally comprised of corners or edges in an image and are matched across frames by using their unique feature descriptions. A similar ideology is applied for LiDAR's or RGBD/Stereo cameras. Once a set unique keypoints, or landmarks, have been identified and matched, they are passed on to the optimization backend. In parallel, relative changes in orientation and translations are fed back to the optimization backend by the odometry sensors and GPS.

% next, the backend optimization does ...
The main purpose of the backend optimization is to take these incoming measurements from the sensing front end, collate them and provide a location estimate and create a map of the environment. To collate the information from different sensors, we need to formally define the behavior of these sensors. Each of the visual or odometry sensors are governed by observation functions, which given the current state of the robot (its position, orientation, velocity, noise and other bias parameters) and the map, can predict the potential measurement coming from the respective sensor. By design if the observation function is given an accurate state of the robot and map, it would perfectly predict the measurement from a sensor. And inversely, if we poorly predict an incoming measurement, it means an incorrect estimate of the state. In fact, this inconsistency between the predicted measurement and the true measurement can serve as an error function upon which to estimate our current state. Given multiple measurements over time and across different sensors, the backend optimizer can use this error function to converge towards an accurate state for the system. 

% NOTE: Push erroneous sensor measurements to later, maybe background and motivation ... 
To correct the former is the job of the backend optimizer; whereas the latter is a failure on part of the sensor which would hurt our state's estimation. Unfortunately, it is not easy to discern between an erroneous state estimation or a sensor's failure and depending on the environment, different sensors better serve as an accurate predictor of our state. For instance in a well lit and static environment, the landmarks extracted from a camera front-end is stable and consistent, and serve as a strong predictor of the state of our system. Hence, it falls upon the backend optimizer to keep track of ...

==> background/background2.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system that overcomes the current SLAM systems, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of both the Visual Inertial Odometry (VIO) SLAM systems and existing Graph SLAM approaches that utilize WiFi bearing measurements. 

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}

Firstly, we describe the operations of the VIO based SLAM algorithms. 
In The existing VIO-SLAM algorithms, we take VINS-MONO~\cite{qin2018vins} as characteristic example but the understanding could be easily extended to any other systems like ORB-SLAM, RTABMap, or cartographer~\cite{orbslam,Labb2018RTABMapAA,cartographer}.

A typical VIO-SLAM that uses a monocular camera in tandem with an inertial odometry measurement has three major components that contribute towards their global pose estimation and the environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since, it is very memory intensive to store all the images for each frame, the VIO-SLAM first identifies appropriate features for each frame~\cite{swift}. 
These features are then tracked across frames to assign a fixed landmark label to consistent features, thus updating the local map of features and their identifiers, which are dubbed as `landmarks'.

\noindent(2) \textbf{Local Feature Mapping:} The multiple frames that have these landmarks are tracked across, are dubbed as `keyframes'.
These landmarks tracked across the keyframes in tandem with the inertial odometry measurements provide for a joint estimate of where these landmarks are in the 3D space and also the robot poses that have enabled this mapping. 
Thus both local robot pose and the local map are simultaneously optimized using these landmarks and odometry measurements.

Both of these above measurements do not require either large memory or heavy compute. 
This is because both of these operations need to have an active memory of last few seconds of keyframes and their landmarks that are tracked and searched within. 
Thus, they are low-compute and low-latency operations.
So, the robot continues to perform local loop-closures for every few frames to generate and incrementally build the map and estimating the robot's pose.

\noindent(3) \textbf{Global Loop Closures:}  However in the long run the robot poses and the map that has been built accrues errors. 
A few of the reasons this happens due to the drift accrued in the inertial odometer measurement and camera's turn estimated incorrectly. 
This can be avoided if let us say the camera can see very old keyframe features and correct for the accumulated drift and back-propagate this error through all the existing poses and the map.
This global drift correction is what is called global loop closure. 

However, to perform these global loop closures the SLAM algorithm needs to maintain a memory consuming dictionary of the past key frames amongst which it has to continuously search for global loop-closures, which in itself is memory and compute intensive process. Additionally, a global loop-closure detected has to optimize for the entire graph which is again a time and compute consuming operation.

We can see that cameras as a sensor are very capable to provide accurate and detailed information of local robot poses and maps. 
However, they cannot perform accurate global pose estimation and map generation in memory and compute efficient fashion. 
We observe that the global loop-closure requirements arise due to accumulated drifts and errors in the inertial odometer measurements reported to the VINS-MONO optimizer.
So if there is a sensor that can give optimized global poses for the robot without any accumulated drifts or errors.
This can be used in tandem with camera, that can handle local pose estimation and mapping and avoid the global loop-closures.

\subsection{WiFi GraphSLAM}\label{sec:back-wifi}

Now that we have established a requirement of a low-cost `Oracle' system that can provide global poses to the camera local feature tracker we can achieve low-compute and adaptable SLAM for indoor robotics. To this extend, we make few interesting observations. (i) all robots are equipped with a WiFi transceiver (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is a relatively cheap sensor modality, and (iv) there has been a couple of decades of research in WiFi based localization and tracking. Owing to these reasons we utilize WiFi as the low-cost `Oracle' sensor that can report global robot poses to the camera graph optimizer.

To that extent, we have observed that bearing measurements have been widely used as the WiFi measurements used for WiFi based SLAM algorithms in the recent past~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot}. Inspired from these system, in \name we utilize WiFi as a bearing measurement sensor.
In contrast to the existing works that either depend on the APs reporting their measurements~\cite{arun2022p2slam} or end-to-end optimization~\cite{arun2022p2slam,zhang2020robot}. 
In \name we only use the bearings measured at the robot's end and enable real-time graph optimization using  the factor graph optimization technique, incremental SAM implementation (iSAM)~\cite{gtsam} as further detailed in ~\cref{sec:design}.

A key thing to observe here is that these WiFi sensors provide low-compute global poses because they do not need time-taking, and memory and compute consuming global loop closure searches for landmark matching. The main reason for this is because each WiFi AP acts as a unique landmark that also has a consistent unique identifier called the hardware MAC address. This removes the need for landmark search making the global pose estimations of WiFi graph low-compute, low-power and accurate.

% To robustly solve the SLAM problem requires two parts -- the sensing front-end and the optimization back-end. Consider a simple monocular camera sensor, the sensing front end would consist of two parts -- identifying robust feature keypoints in the images, and matching them across different camera image frames based on their unique descriptions. These keypoints are generally comprised of corners or edges in an image and are matched across frames by using their unique feature descriptions. A similar ideology is applied for LiDAR's or RGBD/Stereo cameras. Once a set unique keypoints, or landmarks, have been identified and matched, they are passed on to the optimization backend. In parallel, relative changes in orientation and translations are fed back to the optimization backend by the odometry sensors and GPS.

% % next, the backend optimization does ...
% The main purpose of the backend optimization is to take these incoming measurements from the sensing front end, collate them and provide a location estimate and create a map of the environment. To collate the information from different sensors, we need to formally define the behavior of these sensors. Each of the visual or odometry sensors are governed by observation functions, which given the current state of the robot (its position, orientation, velocity, noise and other bias parameters) and the map, can predict the potential measurement coming from the respective sensor. By design if the observation function is given an accurate state of the robot and map, it would perfectly predict the measurement from a sensor. And inversely, if we poorly predict an incoming measurement, it means an incorrect estimate of the state. In fact, this inconsistency between the predicted measurement and the true measurement can serve as an error function upon which to estimate our current state. Given multiple measurements over time and across different sensors, the backend optimizer can use this error function to converge towards an accurate state for the system. 

% % NOTE: Push erroneous sensor measurements to later, maybe background and motivation ... 
% To correct the former is the job of the backend optimizer; whereas the latter is a failure on part of the sensor which would hurt our state's estimation. Unfortunately, it is not easy to discern between an erroneous state estimation or a sensor's failure and depending on the environment, different sensors better serve as an accurate predictor of our state. For instance in a well lit and static environment, the landmarks extracted from a camera front-end is stable and consistent, and serve as a strong predictor of the state of our system. Hence, it falls upon the backend optimizer to keep track of ...

==> background/background3.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system that overcomes the current SLAM systems, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of both the Visual Inertial Odometry (VIO) SLAM systems and existing Graph SLAM approaches that utilize WiFi bearing measurements. 

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}

Firstly, to describe the operations of the existing VIO based SLAM algorithms, we take VINS-MONO~\cite{qin2018vins} as characteristic example but the similar understanding could be easily extended to any other systems like ORB-SLAM, RTABMap, or cartographer~\cite{orbslam,Labb2018RTABMapAA,cartographer}.
Wherein, a typical VIO-SLAM that uses a monocular camera in tandem with an inertial odometry measurement has three major components that contribute towards their global pose estimation and the environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since, it is very memory intensive to store all the images for each frame, the VIO-SLAM first identifies appropriate features for each frame~\cite{swift}. 
These features are then tracked across frames to assign a fixed landmark label to consistent features, thus updating the local map of features and their identifiers, which are dubbed as `landmarks'.

\noindent(2) \textbf{Local Feature Mapping:} The multiple frames that have these landmarks are tracked across, are dubbed as `keyframes'.
These landmarks tracked across the keyframes in tandem with the inertial odometry measurements provide for a joint estimate of where these landmarks are in the 3D space and also the robot poses that have enabled this mapping. 
Thus both local robot pose and the local map are simultaneously optimized using these landmarks and odometry measurements.

Both of these above measurements do not require either large memory or heavy compute. 
This is because both of these operations need to have an active memory of last few seconds of keyframes and their landmarks that are tracked and searched within. 
Thus, they are low-compute and low-latency operations.
So, the robot continues to perform local loop-closures for every few frames to generate and incrementally build the map and estimating the robot's pose.

\noindent(3) \textbf{Global Loop Closures:}  However in the long run the robot poses and the map that has been built accrues errors. 
A few of the reasons this happens due to the drift accrued in the inertial odometer measurement and camera's turn estimated incorrectly. 
This can be avoided if let us say the camera can see very old keyframe features and correct for the accumulated drift and back-propagate this error through all the existing poses and the map.
This global drift correction is what is called global loop closure. 

However, to perform these global loop closures the SLAM algorithm needs to maintain a memory consuming dictionary of the past key frames amongst which it has to continuously search for global loop-closures, which in itself is memory and compute intensive process. Additionally, a global loop-closure detected has to optimize for the entire graph which is again a time and compute consuming operation.

We can see that cameras as a sensor are very capable to provide accurate and detailed information of local robot poses and maps. 
However, they cannot perform accurate global pose estimation and map generation in memory and compute efficient fashion. 
We observe that the global loop-closure requirements arise due to accumulated drifts and errors in the inertial odometer measurements reported to the VINS-MONO optimizer.
So if there is a sensor that can give optimized global poses for the robot without any accumulated drifts or errors.
This can be used in tandem with camera, that can handle local pose estimation and mapping and avoid the global loop-closures.

\subsection{WiFi GraphSLAM}\label{sec:back-wifi}

Now that we have established a requirement of a low-cost `Oracle' system that can provide global poses to the camera local feature tracker we can achieve low-compute and adaptable SLAM for indoor robotics. To that extent, we have observed that in the recent past~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} that bearing based WiFi sensor measurements have been widely used for global pose estimation without the need for global loop-closures. 
Most of these bearing based SLAM algorithms utilize factor graph optimization techniques like GTSAM, an open-sourced GraphSLAM framework~\cite{gtsam}, to obtain the robot poses in 2D~\cite{arun2022p2slam,zhang2020robot}.
%  Inspired from these system, in \name we utilize WiFi as a bearing measurement sensor.
% In contrast to the existing works that either depend on the APs reporting their measurements~\cite{arun2022p2slam} or end-to-end optimization~\cite{arun2022p2slam,zhang2020robot}. 
% In \name we only use the bearings measured at the robot's end and enable real-time graph optimization using the factor graph optimization technique, incremental SAM implementation (iSAM)~\cite{gtsam}.

To formally define and understand how the how the GraphSLAM approach is used for WiFi based global 2D pose estimation, we first assume that we have the readings from the wheel odometry of the robot like any other SLAM system. 
Typically, it is the wheel odometry and gyroscope sensors that provide relative pose measurements of the robots across time steps. 
Now, let us say that these relative pose measurement provided is $z_i$ with a diagonal covariance matrix $\Sigma_i \in \mathbb{R}^3$. 
This covariance is usually estimated by empirically modeling the noise in the odometer and gyroscope beforehand~\cite{lesson1966simple} which are reported by the manufacturer.
We can then define a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \;|\; \Vec{p}_i = (p^x_i, p^y_i, p^\theta_i) \in SE(2), \; \forall i \in [1, N]\}$, where each $p_i$ belongs to the Special Euclidean group ($SE(2)$). 
Next we need to define the measurement model for the odometer factors or the in-between factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$. The measurement model can be shown to be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(-p^\theta_i) [p^x_{i+1} - p^x_{i},\; p^y_{i+1} - p^y_{i}]^T\\
                    (p^\theta_{i+1} - p^\theta_i)
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(2)$ is the rotation matrix. This prediction function now allows us to constrain two consecutive robot poses via a between factor within GraphSLAM \cite{gtsam} and defines an error function between the measurement and prediction as $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$. 
Similarly, one can define the factor graph for the bearing measurements $\hat{z}^{AP}_{ij}(p_i, x_j)$ as well:
\begin{align}\label{eq:ping-pred}
    \hat{z}^{AP}_{ij}(p_i, x_j) = R(-p_i^\theta)\mathrm{atan}2(x^x_i - p^x_i, x^y_i - p^y_i)
\end{align}
where, $\{p_i \; \forall i \in [1, N]\}\ \bigcup\ \{x_j \; \forall j \in [1, N_{ap}]\}$, for $N$ number of robot poses and $N_{ap}$ WiFi AP poses as we do not want to usually assume the pose of the APs in the environment. 
$\mathrm{atan}2(\cdot)$ is the ``2-argument'' inverse tangent function. 
The rotation $R(-p_i^\theta)$ brings the bearing of the access point into the local coordinate frame of the robot. 
This bearing measurement is made on the robot's WiFi sensor from the WiFi access points in the environment.
While, the authors in $\mathrm{P^2}$SLAM assume the WiFi access points coordination in reporting the bearing measured at the access point from the robot we neglect those measurements as this coordination is not practical.

With the factor graph thus constructed, we can then define optimization function to find a set of values $S_{opt}$ such that the total error between our predictions and actual measurements is minimized
\todo{update the $S_{opt}$ equation}
\begin{align}\label{eq:graph-optim-head}
    & S_{opt} =  \argmin_{S} \sum_{i=1}^N \sum_{j=1}^{N_{ap}}  \rho\left(\frac{\big(e^{bearing}_{ij}\big)^2}{\sigma^{bearing}};c\right) \\
         & + \sum_{i=1}^N  \big(e^{odom}_i\big)^T \Sigma_i^{-1} e^{odom}_i.\nonumber 
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$. Thus providing for optimized global robot poses $\{p_i \; \forall i \in [1, N]\}$ without needing any memory and compute demanding global loop-closures. These global robot poses can now be sent over to the 

A key thing to observe here is that these WiFi sensors based factor graph optimization provide low-compute global poses because they do not need time-taking, and memory and compute consuming global loop closure searches for landmark matching. 
The main reason for this is because each WiFi AP acts as a unique landmark that also has a consistent unique identifier called the hardware MAC address. 
This removes the need for landmark search making the global pose estimations of WiFi graph low-compute, low-power and accurate, unlike the VIO-SLAM systems.
On the flip-side, while these WiFi graph SLAM frameworks provide optimized global pose estimations, there is not context of what the environment is and how the robot can navigate through this environment.
We can thus see that both these systems have their respective shortcomings, but have their own strengths.
That is we can use the optimized global pose estimates can be used as `Oracle' Odometer measurements for the camera graph which can provide the map of the environment, adding context to the environment the robot is exploring.
This is where we provide \name, which utilizes these advantages and creates a `Dual-graph' layered solution to provide a deployable and scalable SLAM system.





% Similarly, to incorporate for the WiFi bearing measurements into the factor graph, we first note that in \name we do not assume the initial position of the WiFi APs, and thus need to optimize for their poses as well as the robot's poses. To thus incorporate that, we append the poses of $Q$ WiFi APs ($x$) to our state space. The complete state space would then become $\{p_i \; \forall i \in [1, P]\}\ \bigcup\ \{x_j \; \forall j \in [1, Q]\}$.
% We thus define our prediction function to obtain the angle subtended by access point $x_j$ at robot pose $p_i$ as
% \begin{align}\label{eq:ping-pred}
%     \hat{z}^{AP}_{ij}(p_i, x_j) = R(-p_i^\theta)\mathrm{atan}2(x^x_i - p^x_i, x^y_i - p^y_i)
% \end{align}
% where $\mathrm{atan}2(\cdot)$ is the ``2-argument'' inverse tangent function. The rotation $R(-p_i^\theta)$ brings the bearing of the access point into the local coordinate frame of the robot. This bearing measurement is made when the WiFi radio receives the `pong' acknowledgement from the WiFi access points. 
% Finally, to anchor the robot to a fixed global frame of reference and align it with the ground truth trajectory and map generated by Cartographer~\cite{cartographer}, we further provide an initial prior, $p_0$, to the first pose. 

% With the factor graph constructed, we can then define optimization function to find a set of values $S_{opt}$ such that the total error between our predictions and actual measurements is minimized
% \todo{update the $S_{opt}$ equation}
% \begin{align}\label{eq:graph-optim-head}
%     & S_{opt} =  \argmin_{S} \sum_{i=1}^P \sum_{j=1}^Q  \rho\left(\frac{\big(e^{bearing}_{ij}\big)^2}{\sigma^{bearing}};c\right) \\
%          & + \sum_{i=1}^P  \big(e^{odom}_i\big)^T \Sigma_i^{-1} e^{odom}_i.\nonumber 
% \end{align}
% where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$. To further strengthen the optimization to outliers, we use a Huber cost function, $\rho(\cdot, c)$~\cite{zhang1997parameter}, for which
% we find through our experiments the threshold $c = 1.345$ provides the best estimate. This function is easily minimized in linear time proportional to the number of nodes initialized, i.e. $N+M$, via Levenberg-Marquadt \cite{gtsam}.

==> background/background4.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of existing visual-inertial odometry (VIO) SLAM systems, and graph SLAM approaches that utilize WiFi bearing measurements. 

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}
Let us first understand the operations of existing Visual Inertial Odometry (VIO) based SLAM algorithms like ORB-SLAM, RTABMap, or Kimera~\cite{orbslam,Labb2018RTABMapAA,rosinol2021kimera}.
A typical VIO-SLAM system that uses a monocular camera in tandem with an inertial odometry measurement unit has three major components that contribute towards global pose estimation and environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since it is very memory intensive to store the entire camera image for each frame, the VIO-SLAM system first identifies appropriate features for each frame~\cite{shi1994good}. 
These features are then tracked across frames by assigning a fixed identity label to consistent features, and updating a local map of features and their identifiers, which are dubbed as `landmarks'. Additionally, camera frames which have a large number of new landmarks are stored in memory and are dubbed `keyframes'. These keyframes will be later used for global drift corrections to the robot's trajectory.  

\noindent(2) \textbf{Local Feature Mapping:} Out of the landmarks tracked, some are judged stable and consistent, and are integrated into the map. 
These landmarks are localized in 3D space by jointly optimizing over the distinct robot positions at which the landmarks were observed. 
Thus, both local robot pose and the local map can be simultaneously optimized using these landmarks and odometry measurements.

It is important to note that both feature tracking and local mapping operations are low in memory and compute because these operations need to have an active memory of only the last few seconds of camera frames, observed landmarks and odometry measurements. 
So, the robot continues to perform local drift corrections for every few frames to incrementally build the map and estimate the robot's pose.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/WiViD_overview.pdf}
    \caption{\name's layered approach: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time.}
    \label{fig:layered-arch}
\end{figure*}

\noindent(3) \textbf{Global Loop Closures:}  However, in the long run the robot poses and the map that has been built accrue errors as drifts in inertial odometry measurements cannot be accurately cancelled via local corrections only.
These long-term drifts can are corrected by employing global loop closures. Specifically, if the robot revisits a space and the camera can find previously seen keyframe features, it can constrain the current robot's pose to the previously estimated pose at this keyframe and re-optimize the robot's trajectory considering this additional constraint. These large drift corrections, which affect a large number of nodes in the robot's pose, are called global loop closures. 

In order to perform these global loop closures, the SLAM algorithm needs to maintain a dictionary of all the past key frames, amongst which it has to continuously search for global loop closures. This buffer of keyframes and continuous search is a very memory and compute intensive process.  Additionally, a global loop closure detection triggers a re-optimization of the entire robot trajectory which is again a time and compute intensive operation. Furthermore, the required memory and search-time scales linearly with the size of the environment, reducing the scalability of the system as well.

In short, cameras as a sensor are capable of providing accurate and detailed information of local robot poses and maps. 
However, they cannot perform accurate global pose estimation and map generation in a memory and compute efficient fashion. 
We observe that requirements for global loop closures arise due to accumulated drifts and errors in the inertial odometry measurements reported to the optimizer.
Hence, there is a requirement for a sensor to provide these global `Oracle' poses for the robot, free of accumulated drifts and errors in a compute and memory-light fashion, so that the camera can coherently map and understand the environment.  
% So if a sensor that can give optimized global poses for the robot without any accumulated drifts or errors.
% This can be used in tandem with camera, that can handle local pose estimation and mapping and avoid the global loop closures.

\subsection{\name's design Motivation}\label{sec:back-wifi}

Now that we have established a requirement of a low-cost `Oracle' system that can provide global poses to the local feature tracker, we have a path to low-compute and adaptable SLAM for indoor robotics. 

We have observed that in the recent past~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot}, bearing based WiFi sensor measurements have been widely used for global pose estimation without the need for global loop closures. 
Most of these bearing based SLAM algorithms utilize factor graph optimization techniques like GTSAM, an open-sourced GraphSLAM framework~\cite{gtsam}, to obtain the robot and AP poses~\cite{arun2022p2slam,zhang2020robot}.

A key observation is these WiFi-sensor based GraphSLAM approaches provide low-compute global pose estimates, as they do not rely on memory and compute consuming global loop closure searches for landmark matching. 
While in camera SLAM, an increasing number of `landmarks' are needed to be kept in active memory to identify and perform loop closures, WiFi has fixed a number of `landmarks' in the form of WiFi Access Points deployed in the environment.
Furthermore, while camera-landmarks are unique features in a frame, they are vulnerable to ambiguities, resulting in false-positive loop closures in homogeneous spaces.
On the other hand, in WiFi SLAM each WiFi AP acts as a unique landmark that also has a consistent discernible identifier (hardware MAC address) removing any room for instability in the system. 
These consistently identifiable landmarks allow for global pose corrections sans global loop closures providing low-compute, low-power and accurate `Oracle' pose updates.
On the flip-side, while these WiFi graph SLAM frameworks provide optimized global pose estimations, they lack context of the environment, essential for autonomous robot navigation in any environment.

Thus both sensors have their advantages and disadvantages, and we present \name that amalgamates both the sensors to bring out the best of both camera and WiFi sensor capabilities. 
\if 0
We first present \name's dual-graph design  as shown in Figure~\ref{fig:layered-arch} in ~\cref{sec:design}, that demonstrates the scalability of \name's design. We then describe the challenges in estimating accurate measurements for camera and WiFi sensors in ~\cref{sec:design-measure}. We go on to detail implementation and deployment of \name in ~\cref{sec:implementation} and demonstrate \name's performance and a detailed analysis in ~\cref{sec:eval}. 
% Additionally, we showcase simple application where the robot autonomously navigates to a given room number to deliver a package in ~\cref{sec:showcase}.
Finally in ~\cref{sec:conclusion}, we present the limitations that hinder our current implementation of \name and future directions that our research in \name opens.
\fi

==> background/background5.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of existing visual-inertial odometry (VIO) SLAM systems, and graph SLAM approaches that utilize WiFi bearing measurements. 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/viwid_overview-crop.pdf}
    \caption{\name's Dual layered Design: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time. \todo{Fix numbers}}
    \label{fig:layered-arch}
\end{figure*}

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}
Let us first understand the operations of existing Visual Inertial Odometry (VIO) based SLAM algorithms like ORB-SLAM, RTABMap, or Kimera~\cite{mur2015orb,Labb2018RTABMapAA,rosinol2021kimera}.
A typical VIO-SLAM system that uses a monocular camera in tandem with an inertial odometry measurement unit has three major components that contribute towards global pose estimation and environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since it is very memory intensive to store the entire camera image for each frame, the VIO-SLAM system first identifies appropriate features for each frame~\cite{shi1994good}. 
These features are then tracked across frames by assigning a fixed identity label to consistent features, and updating a local map of features and their identifiers, which are dubbed as `landmarks'. Additionally, camera frames that have a large number of new landmarks are stored in memory and are dubbed `keyframes'. These keyframes will be later used for global drift corrections to the robot's trajectory.  

\noindent(2) \textbf{Local Feature Mapping:} Out of the landmarks tracked, some are judged stable and consistent, and are integrated into the map. 
These landmarks are localized in 3D space by jointly optimizing over the distinct robot positions at which the landmarks were observed. 
Thus, both the local robot pose and the local map can be simultaneously optimized using these landmarks and odometry measurements.

\noindent(3) \textbf{Global Loop Closures:}  However, in the long run, the robot poses and the map built accrue errors as drifts in inertial odometry measurements cannot be accurately canceled via local corrections alone.
These long-term drifts can are corrected by employing global loop closures. Specifically, if the robot revisits a space and the camera can find previously seen keyframe features, it can constrain the current robot's pose to the previously estimated pose at this keyframe and re-optimize the robot's trajectory considering this additional constraint. These large drift corrections, which affect a large number of robot poses, are called global loop closures. 

To perform these global loop closures, the SLAM algorithm needs to maintain a dictionary of all the past keyframes, amongst which it has to continuously search for global loop closures. This buffer of keyframes and continuous search is very memory and compute-intensive process~\cite{semenova2022quantitative}.  Additionally, a global loop closure detection triggers a re-optimization of the entire robot trajectory which is again a time and compute-intensive operation. Furthermore, the required memory and search times scale linearly with the size of the environment, reducing the scalability of the system.

\subsection{\name's design Motivation}\label{sec:back-wifi}

In short, cameras as a sensor are capable of providing accurate and detailed information of local robot poses and maps with low compute and memory resources. 
However, they cannot perform accurate global pose estimation and map generation in memory and compute efficient fashion. 
We observe that requirements for global loop closures arise due to accumulated drifts and errors in the inertial odometry measurements reported to the optimizer.
Hence, if the camera has access to global poses of the robot, free of accumulated drifts and errors in a compute and memory-light fashion, the camera SLAM can coherently map and understand the environment.
Now, this approach of abstraction of tasks similar to network layer abstraction~\cite{session1994it5} has pioneered the research and development of current data networks. This motivates the Dual-layer design of \name.

Inspired by this intuition, we observe recent SLAM development into WiFi sensor-based global pose estimation without the need for global loop closures~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot}.
So these WiFi-sensor-based SLAM approaches provide low-compute global pose estimates, as they do not rely on memory and compute consuming global loop closure searches for landmark matching. 
Thus, we use the WiFi-sensor-based SLAM systems as our drift-free pose estimation system that can provide poses of the robot to the camera SLAM can coherently map and understand the environment.
This leads to the Visual-WiFi Dual-layered SLAM design of \name that is described in ~\cref{sec:design}.

==> background/background6.tex <==
\section{Background and Motivation}\label{sec:background}

To understand that \name is a scalable system, it is important to look at the shortcomings of the current SLAM systems. So, we give a brief overview of existing visual-inertial odometry (VIO) SLAM systems, and graph SLAM approaches that utilize WiFi bearing measurements. 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/viwid_overview-crop.pdf}
    \caption{\name's Dual layered Design: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time. \todo{Fix numbers}}
    \label{fig:layered-arch}
\end{figure*}

\subsection{Visual Inertial Odometry SLAM}\label{sec:back-vio}
Let us first understand the operations of existing Visual Inertial Odometry (VIO) based SLAM algorithms like ORB-SLAM, RTABMap, or Kimera~\cite{mur2015orb,Labb2018RTABMapAA,rosinol2021kimera}.
A typical VIO-SLAM system that uses a monocular camera in tandem with an inertial odometry measurement unit has three major components that contribute towards global pose estimation and environment mapping: 

\noindent(1) \textbf{Feature Extraction and Tracking:} Since it is very memory intensive to store the entire camera image for each frame, the VIO-SLAM system first identifies appropriate features for each frame~\cite{shi1994good}. 
These features are then tracked across frames by assigning a fixed identity label to consistent features, and updating a local map of features and their identifiers, which are dubbed as `landmarks'. Additionally, camera frames that have a large number of new landmarks are stored in memory and are dubbed `keyframes'. These keyframes will be later used for global drift corrections to the robot's trajectory.  

\noindent(2) \textbf{Local Feature Mapping:} Out of the landmarks tracked, some are judged stable and consistent, and are integrated into the map. 
These landmarks are localized in 3D space by jointly optimizing over the distinct robot positions at which the landmarks were observed. 
Thus, both the local robot pose and the local map can be simultaneously optimized using these landmarks and odometry measurements.

\noindent(3) \textbf{Global Loop Closures:}  However, in the long run, the robot poses and the map built accrue errors as drifts in inertial odometry measurements cannot be accurately canceled via local corrections alone.
These long-term drifts are corrected by employing global loop closures. Specifically, if the robot revisits a space and the camera can find previously seen keyframe features, it can constrain the current robot's pose to the previously estimated pose at this keyframe and re-optimize the robot's trajectory considering this additional constraint. These large drift corrections, which affect a large number of robot poses, are called global loop closures. 

To perform these global loop closures, the SLAM algorithm needs to maintain a dictionary of all the past keyframes, amongst which it has to continuously search for global loop closures. This buffer of keyframes and continuous search is very memory and compute-intensive process~\cite{semenova2022quantitative}.  Additionally, a global loop closure detection triggers a re-optimization of the entire robot trajectory which is again a time and compute-intensive operation. Furthermore, the required memory and search times scale linearly with the size of the environment, reducing the scalability of the system.

\subsection{\name's Design Motivation}\label{sec:back-wifi}

In short, cameras as a sensor are capable of providing accurate and detailed information of local robot poses and maps with low compute and memory resources. 
However, they cannot perform accurate global pose estimation and map generation in memory and compute efficient fashion. 
We observe that requirements for global loop closures arise due to accumulated drifts and errors in the inertial odometry measurements reported to the optimizer.
Hence, if the camera has access to global poses of the robot, free of accumulated drifts and errors in a compute and memory-light fashion, the camera SLAM can coherently map and understand the environment.
Now, this approach of abstraction of tasks similar to network layer abstraction~\cite{session1994it5} has pioneered the research and development of current data networks. This motivates the Dual-layer design of \name.

Inspired by this intuition, we observe recent SLAM development into WiFi sensor-based global pose estimation without the need for global loop closures~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot}.
So these WiFi-sensor-based SLAM approaches provide low-compute global pose estimates, as they do not rely on memory and compute consuming global loop closure searches for landmark matching. 
Thus, we use the WiFi-sensor-based SLAM systems as our drift-free pose estimation system that can provide poses of the robot to the camera SLAM can coherently map and understand the environment.
This leads to the Visual-WiFi Dual-layered SLAM design of \name that is described in ~\cref{sec:design}.

==> design/design1.tex <==
% !TEX root = root.tex
\section{Design}\label{sec:design}

Assuming we have robust and accurate bearing measurements, we first detail \name's Dual-graph solution for a scalable SLAM system using the WiFi and camera sensors, describing each individual layer first and how they are connected with each other.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

To this extent, we make few interesting observations. (i) all robots are equipped with a WiFi transceiver (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is a relatively cheap sensor modality, and (iv) there has been a couple of decades of research in WiFi based localization and tracking. Owing to these reasons we utilize WiFi as the low-cost `Oracle' sensor that can report global robot poses to the camera graph optimizer.

To formally define and understand how the how the GraphSLAM approach is used for WiFi based global 2D pose estimation, we first assume that we have the readings from the wheel odometry of the robot like any other SLAM system. 
Typically, it is the wheel odometry and gyroscope sensors that provide relative pose measurements of the robots across time steps. 
Now, let us say that these relative pose measurement provided is $z_i$ with a diagonal covariance matrix $\Sigma_i \in \mathbb{R}^3$. 
This covariance is usually estimated by empirically modeling the noise in the odometer and gyroscope beforehand~\cite{lesson1966simple} which are reported by the manufacturer.
We can then define a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \;|\; \Vec{p}_i = (p^x_i, p^y_i, p^\theta_i) \in SE(2), \; \forall i \in [1, N]\}$, where each $p_i$ belongs to the Special Euclidean group ($SE(2)$). 
Next we need to define the measurement model for the odometer factors or the in-between factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$. The measurement model can be shown to be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(-p^\theta_i) [p^x_{i+1} - p^x_{i},\; p^y_{i+1} - p^y_{i}]^T\\
                    (p^\theta_{i+1} - p^\theta_i)
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(2)$ is the rotation matrix. This prediction function now allows us to constrain two consecutive robot poses via a between factor within GraphSLAM \cite{gtsam} and defines an error function between the measurement and prediction as $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$. 
Similarly, one can define the factor graph for the bearing measurements $\hat{z}^{AP}_{ij}(p_i, x_j)$ as well:
\begin{align}\label{eq:ping-pred}
    \hat{z}^{AP}_{ij}(p_i, x_j) = R(-p_i^\theta)\mathrm{atan}2(x^x_i - p^x_i, x^y_i - p^y_i)
\end{align}
where, $\{p_i \; \forall i \in [1, N]\}\ \bigcup\ \{x_j \; \forall j \in [1, N_{ap}]\}$, for $N$ number of robot poses and $N_{ap}$ WiFi AP poses as we do not want to usually assume the pose of the APs in the environment. 
$\mathrm{atan}2(\cdot)$ is the ``2-argument'' inverse tangent function. 
The rotation $R(-p_i^\theta)$ brings the bearing of the access point into the local coordinate frame of the robot. 
This bearing measurement is made on the robot's WiFi sensor from the WiFi access points in the environment.
While, the authors in $\mathrm{P^2}$SLAM assume the WiFi access points coordination in reporting the bearing measured at the access point from the robot we neglect those measurements as this coordination is not practical.

With the factor graph thus constructed, we can then define optimization function to find a set of values $S_{opt}$ such that the total error between our predictions and actual measurements is minimized
\todo{update the $S_{opt}$ equation}
\begin{align}\label{eq:graph-optim-head}
    & S_{opt} =  \argmin_{S} \sum_{i=1}^N \sum_{j=1}^{N_{ap}}  \rho\left(\frac{\big(e^{bearing}_{ij}\big)^2}{\sigma^{bearing}};c\right) \\
         & + \sum_{i=1}^N  \big(e^{odom}_i\big)^T \Sigma_i^{-1} e^{odom}_i.\nonumber 
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$. Thus providing for optimized global robot poses $\{p_i \; \forall i \in [1, N]\}$ without needing any memory and compute demanding global loop-closures.



Highlight that we use only measurements at the robot, making it in dependant of the environment and can be deployed even in the cases of distaster relief where the WiFi AP Locations are not known apriori.

The rest would be a description of p2slam's graphslam framework and optimization with intuitions.

then talk about how iSAM works and is different from end-to-end slam, and how it is more difficult and much more important for real-world deployments.

A key thing to observe here is that these WiFi sensors provide low-compute global poses because they do not need time-taking, and memory and compute consuming global loop closure searches for landmark matching. The main reason for this is because each WiFi AP acts as a unique landmark that also has a consistent unique identifier called the hardware MAC address. This removes the need for landmark search making the global pose estimations of WiFi graph low-compute, low-power and accurate.

\subsection{Camera Factor Graph}\label{sec:design-graph2}

The camera graph now utilizes the global optimized pose estimates outputted from the WiFi factor graph in real-time and uses them as the odometer factors for its graph optimization.

What are the exact outputs from the WiFi factor graph to the camera factor graph. Is it just locations? If so, how delayed are they and what happens when they are updated?

We make smart choices as to when to update them and how frequently to avoid the camera graph from breaking.

It then performs local mapping and pose corrections, providing with global optimized pose and map for the frames of data collected so far without the requirement of compute heavy graphslam.

\subsection{Accurate Bearing Measurements}\label{sec:design-bearing}

While existing works use end-to-end optimization, we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for real-time local updates. This demands that the bearing measurements made are accurate, more dense and do not have any ambiguities.

Thus to solve these problems in \name we make few innovations on the bearing estimation end.

Firstly to remove the ambiguities of the half-plane in the typically deployed ULAs in the literature, we use square antenna array with $3\lambda/8$ side length of the square, which has unique solution for theta in the full-space.

Next to increase the accuracy and density of bearing measurements to the WiFi access points in the environment while maintaining real time estimates we get inspired from the Spoti/MUSIC though are high compute and latency. 
We cannot simple averaging across FFT profiles, as each measurement has unique random phase offset that changes across time due to timing mismatches between the transmitting AP and the receiving WiFi sensor on the robot
In contrast, in \name the averaging is done by performing eigen or singular decomposition over a collated measurements both across time and if there multiple antennas on the transmitting AP, then across these antennas as well.

We then identify the component with strongest singular value, which corresponds to the direct path in most of the cases and perform a simple 2D FFT on it as mentioned/detailed in ~\cite{ayyalasomayajula2018bloc}. And from this we pick the global maxima to obtain cleaned, more accurate and denser bearing measurements if and when we perform a moving window averaging on these WiFi measurements.

Thus, \name solves for getting accurate and dense bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

Thus we have seen how the layered approach in bifurcating the tasks between the WiFi and camera sensors to utilize them for what they are best at brings the best of both the sensors. This WiFi and Visual Dual factor graph SLAM solution thus makes \name-SLAM, low-cost, low-compute, accurate and adaptable SLAM system. Thus enabling scalable and deployable robotics using \name-SLAM's design.

==> design/design2.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

% \begin{figure*}[ht]
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/placeholder.pdf}
%         \subcaption{}
%     \end{minipage}
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/placeholder.pdf}
%         \subcaption{}
%     \end{minipage}
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/placeholder.pdf}
%         \subcaption{}
%     \end{minipage}
%     \caption{\name's design: (a) Shows the layered design where the inputs to and outputs from each layer are detailed. (b) Shows the details of the implementation of the WiFi graph (c) Details on how the camera graph uses the WiFi Odometry measurements for Mapping.}
%     \label{fig:design-overview}
% \end{figure*}

The existing VIO SLAM and WiFi SLAM systems have their respective shortcomings and strengths as described in ~\cref{sec:background}.
To overcome the limitations of these existing systems, and make use of the best use of these two individual sensors, we propose \name a `Dual-graph' layered solution to provide a deployable and scalable SLAM system.
We detail \name's `Dual-graph' design in this section where we first assume that we have accurate real-time bearings available for robots poses and define the WiFi graph optimization in ~\cref{sec:design-graph1} that provides optimized robot poses. 
These WiFi-optimized robot poses are then smartly fed to the camera graph which is described in ~\cref{sec:design-graph2}, to jointly optimize for the robot positions and the various visual landmarks observed in the environment.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

Firstly, to identify the sensor modality to use within the first graph that provides for the optimized global pose estimates to the second graph, we make few interesting observations:
(i) all robots are equipped with a WiFi transceiver (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is an inexpensive sensing modality, and (iv) WiFi based localization and tracking~\cite{ma2019wifi} is well studied which can be exploited for the global pose estimation. Owing to these four reasons, we utilize WiFi as the low-cost `Oracle' sensor that can be used to build the first SLAM module to provide global robot poses to the second Camera-based graph optimizer.

\noindent\textbf{Bearings as Robust WiFi Measurements:} To enable this `dual-graph' idea, the WiFi SLAM module should take the WiFi measurements at multiple robot poses from access points deployed in the environment as shown in Figure~\ref{fig:wifi-factor}a and optimize for global pose estimates.
To demonstrate that in \name, these WiFi measurements are integrated with the widely deployed GraphSLAM~\cite{gtsam} approach.
This GraphSLAM approach lays down these WiFi measurements, $z_{ij}^\mathrm{bot}$, as factors in a factor graph, connecting the access points' pose estimates, $ \Vec{x}_j$ to the robot pose, $ \Vec{p}_i$, across frames. 
These robot pose estimates are further connected with the wheel-encoder and gyroscope measurements which provide relative odometry measurements, $z_i^\mathrm{odom}$ between two consecutive pose estimates.
Once we lay down these WiFi measurements and relative odometry measurements as shown in Figure~\ref{fig:wifi-factor}b, it can be optimized to estimate accurate global poses.

With the high-level factor graph laid out, we have to choose the appropriate WiFi-based measurements which provide the necessary global pose corrections.
Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} have shown that bearing measurements are one of the most robust estimates that can be used for Indoor localization and tracking.
Inspired from these works we utilize bearings as the WiFi measurements to be integrated into our WiFi factor graph's definition.
These bearing measurements can be estimated either at the robot's WiFi device or at the WiFi access points in the environment using the channel state information (CSI) measured while receiving WiFi signal~\cite{arun2022p2slam,spotfi,arraytrack}.

Unfortunately, these implementations either assume the apriori pose of the WiFi access points in the environment~\cite{spotfi} or assume the CSI measurements at the WiFi APs are reported back to the robot~\cite{arun2022p2slam}. These assumptions reduce the deployability of the WiFi-SLAM system, requiring fine-grained measurements of AP's locations or cooperation from infrastructure. 
In  \name's WiFi factor graph, we break away from these assumptions, and do not require any knowledge of the environment including the AP poses or collaboration between the AP's and the robot.
Thus in \name, we utilize the bearing estimates, $z_{ij}^{bot}$ made only at the robot's end with respect to the AP's in the environment as can also be seen in the factor graph shown in Figure~\ref{fig:wifi-factor}.
The final requirement for real-time wide-deployability is to provide timely global pose updates to the Camera-graph and ensure accurate mapping of the environment.
These timely global pose estimates demands that the bearing measurements be real-time and accurate, which poses its unique challenges that we solve as discussed later in ~\cref{sec:design-bearing}. For the sake of brevity we first assume that we have these accurate real-time bearing measurements and describe \name's WiFi factor graph implementation.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across various robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}

\noindent\textbf{Building and Optimizing the WiFi-Graph:}
To formally define and understand how the GraphSLAM approach is used for WiFi based global 4DoF pose estimation, we first assume that we have the readings from the wheel odometry and gyroscope measurements from the robot like any other SLAM system. 
Typically, these sensors provide relative pose measurements of the robots across time steps. 
Now, let us say that these relative pose measurement provided is $z_i$ with a diagonal covariance matrix $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$. 
This covariance is usually estimated by empirically modeling the noise in the odometer and gyroscope beforehand~\cite{lesson1966simple} which are reported by the manufacturer.
We can then define a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \;|\; \Vec{p}_i = (p^x_i, p^y_i, p^z_i, q^x_i, q^y_i, q^z_i) \in SE(3), \; \forall i \in [1, N]\}$, where each $p_i$ belongs to the Special Euclidean group ($SE(3)$). Specifically, each $\Vec{p}_i$ has two components, the translation in space, $p^t_i = (p^x_i, p^y_i, p^z_i)$, and the quaternion representing its rotation, $p^q_i(q^x_i, q^y_i, q^z_i, 1 - ||(q^x_i, q^y_i, q^z_i)||^2)$.
Next we need to define the measurement model for the odometer factors or the in-between factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$. The measurement model can be shown to be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion~\cite{diebel2006representing}. This prediction function now allows us to constrain two consecutive robot poses via a between factor within GraphSLAM \cite{gtsam} and defines an error function between the measurement and prediction as $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$. 
Similarly, one can define the factor graph for the bearing measurements of AP $j$ at robot position $x_i$ as $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$:
\begin{align}\label{eq:ping-pred}
    &\hat{z}^{bot}_{ij}(p_i, x_j) = \mathrm{Local}(\mathrm{TransformTo}(x_j, p_i), p_i) \\
                                &= \mathrm{Local}([\cos(\phi)\cos(\theta), \cos(\phi)\sin(\theta), \sin(\phi)]^T, p_i) \nonumber
\end{align}
where, $\{p_i \; \forall i \in [1, N]\}\ \bigcup\ \{x_j \; \forall j \in [1, N_{ap}]\}$, for $N$ number of robot poses and $N_{ap}$ WiFi AP poses. Furthermore, \textit{TransformTo}$(\cdot)$ transforms the coordinates of the AP $x_j$ to the coordinate system provided by the robot at $p_i$, in which the AP subtends an elevation angle of $\phi$ and an azimuth angle of $\theta$. \textit{Local}$(\cdot)$ projects this bearing measurement to the tangent plane defined by the current pose of the robot, $p_i$. 

At this point, we are faced with an interesting choice. As mentioned previously, the angle of arrival of signal from an access point is the measurement of choice. We can consider extracting both the elevation and azimuth angle given a 2D antenna array as opposed to just the azimuth angle. Unfortunately this comes with two challenges, (1) it doubles the state-space of the optimization, (2) most WiFi clients have four or fewer antennas~\cite{quantenna}, resulting in poor resolution and incorrect estimation of elevation angles. Hence, we set $\phi = 0$, regardless of the height of the access point, and only extract the azimuth angle, $\theta$. \todo{bringing out elevation sucks, only azimuth, confirm here}. Finally, we also define the covariance of these bearing measurements, $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$. 

With the factor graph thus constructed, we can define optimization function to find a set of values $S_{opt}$ such that the total error between our predictions, $\hat{z}$'s, and actual measurements, $z$'s, is minimized. 
Unlike the existing WiFi SLAM architectures~\cite{arun2022p2slam,ferris2007wifi} we do not perform end-to-end optimization, we instead use the incremental smoothing and mapping (iSAM) implementation of the GraphSLAM approach~\cite{gtsam}.
At a high level, GTSAM framework optimizes for all the variables, $\{p_i \; \forall i \in [1, N]\}\ \bigcup\ \{x_j \; \forall j \in [1, N_{ap}]\}$, end-to-end considering all the measurements, $\{z_i^{odom},\hat{z}^{AP}_{ij}(p_i, x_j)\} \forall i \in [1, N]$ and $\forall j \in [1, N_{ap}]\}$ together and optimizing for them as a post processing step.
On the other hand, in iSAM, the graph is optimized every time a new measurement is added to the factor graph. 
This might lead to incredibly high compute and memory requirements as the factor graph gets bigger with each new measurement coming in.
In order to avoid this, in iSAM~\cite{gtsam}, the authors determine which of the past poses are effected by the new incoming measurement and only those subset of pose estimates are optimized.
Specifically, given $I={p_i,x_j: i<n, \forall j \in [1, N_{ap}]}$, where $n$ is the current time instance when a new measurement is added to the factor graph, only a subset of the factors $I_{sub} \subseteq I$ are optimized.
We can estimate the optimized robot poses $S_{opt}^n$ for time instance $n$ by minimizing the total error between our predictions and actual measurements for the subset $I_{sub}$, i.e.
\begin{align}\label{eq:graph-optim-head}
    S_{opt}^n = \argmin_{S} \sum_{i\in I_{sub}} \sum_{j\in I_{sub}}  & \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. Thus providing for optimized global robot poses $\{p_i \; \forall i \in I_{sub}\}$ without needing any memory and compute demanding global loop closures.

\noindent\textbf{Initialization of Factors:} Finally, we also need to initialize each of the $N$ robot positions and $N_{ap}$ AP positions for the optimizer. 
Like any other SLAM system, we initialize the robot positions using the relative odometry measurements. But it is important to note that these priors will be affected by drift accumulated by the odometer. 
We also do not assume apriori location of the AP's in the environment, but unlike for the end-to-end optimization scenario, real-time incremental optimizations we cannot initialize all the AP poses at the origin at the beginning of the optimization.
This is because many of these APs have not yet been discovered or are not effected by the current incoming bearing measurements, thus making the optimization problem ill-defined. Furthermore, AP's which have been discovered may not have enough bearing measurements to strongly constrain the system. This makes the optimization unstable and converge to poor estimates. Thus, we need to initialize the APs in a smart fashion considering the most probable bearing measurement factors when getting added that effect the AP and robot poses.

To solve for the indeterminate solution due to incorrect WiFi AP initialization, we draw from the intuition of WiFi signal propagation characteristics.
More specifically WiFi received signal signal strength (RSSI) statistics, which have been studied in the past for localization.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's translation $p^t_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maxima among all the robots poses $p_i \forall i \in [1,n]$ measured at $n^{th}$ time instance.
We can then initialize $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation.
Once all the APs in the environment are detected and initialized in this fashion the factor graph optimization system is no more indeterminate or ill-defined.
Thus solving all the challenges for the \name's WiFi graph optimization, which can now provide accurate and real-time global pose estimates for the camera graph to consume.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/camera_factor.pdf}
    \caption{Shows the details of the implementation of the Camera Factor graph}
    \label{fig:cam-factor}
\end{figure}

\subsection{Camera Factor Graph}\label{sec:design-graph2}

As we described in ~\cref{sec:back-vio}, a typical Visual Inertial Odometer based SLAM system needs camera features and Odometer measurements. 
To extract, track and map the camera features we utilize the Shi-Tomasi features~\cite{shi1994good} from the VINS-MONO implementation~\cite{qin2018vins}.
These camera features are undistorted and then mapped onto a unit sphere to get an approximate estimate of the 3D point cloud projections.
These projections are then laid down as the map projections or `landmarks' in the factor graph for a fixed set of local frames. 
These `landmarks' now in tandem with the Odometer measurements could jointly optimize to perform local pose corrections. 
These local corrections ensure accurate 3D mapping of the `landmark' point clouds in the environment as shown in Figure~\ref{fig:cam-factor}

% We detail on how we extract robust camera measurements in ~\cref{sec:design-camera}, where we go into further details on how we use the feature extraction provided by the VINS-MONO feature extractor and tracker~\cite{qin2018vins}.
In addition to this, these VIO-SLAM systems trigger global loop closures for two distinct reasons (i) because of the drift accrued in the robot pose estimates provided by the Inertial Odometry sensors for long runs, and (ii) the homogeneity of the visual features based landmarks that demands constant trigger for feature matching and thus large memory cache of all the landmarks.
In \name, we overcome both of these issues using the global pose estimates provided by the WiFi graph as the `Oracle' robot pose measurements for the camera graph.
Since, these WiFi global pose estimates can be made with low-compute and in real-time with high-accuracy we can eliminate the need for global loop closure in the camera features based VIO-SLAM systems.

\begin{algorithm}[t]
\caption{Implementation of the buffered WiFi Pose updates to the Camera Odometry factors.\todo{The algo is not correct, correct it!!!!!!!}}
\label{algo:pose-buffer}
    \SetAlgoLined
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    % \SetKwData{Circular}{circularCache_w}
    \Input{Pose threshold $t$, stability threshold size $st$, moving window size $w$}
    initialization Circular Cache $C_0 \leftarrow \{\}$, Buffer $V \leftarrow \{\} $, Pose Updates $S_{opt}^0\leftarrow \{\} $, Cache size $Vs \gets 0$ \\
    
    \For{$n \gets 1$ \KwTo $N$}{
        Estimate $S_{opt}^n$ from Eq~\ref{eq:graph-optim-head}\\
        $N_n \gets |S_{opt}^n|$ \\
        \eIf{$C_{n-1} > st$ }{
            $C_n \gets \mathrm{circularCache}_w\{C_{n-1}, N_n\}$ \\
            }{}
        
        \eIf{$RMSE(C_n - C_{n-1}) \leq t$}{
            $V \gets S_{opt}^n$ \\
            Push $V$ as pose updates
          }{
          $V \gets V+S_{opt}^n$ \\
          $Vs \gets Vs + N_n$ \\
              \If{$Vs \geq ct$}{
                  Push $V$ as pose updates
              }
          }
    }
\end{algorithm}

So these WiFi global pose estimates could be sent to the camera graph as camera's Odometer measurements for every frame of the WiFi measurement.

\textbf{Smart Pose Update Buffering:}
However, numerous and large updates to the odometry measurements in the camera graph would trigger frequent graph optimization for large number of camera factors.
These camera factors will keep increasing as the number of robot poses keep increasing, leading to updates in the camera graph which becomes memory intensive.
Thus we cannot naively send each and every WiFi graph's pose updates to the camera graph and observe that these WiFi frames usually are updated at a rate of ~100Hz while camera frames are only fed at ~2-10Hz.
With this observation, \name's WiFi graph's pose updates are maintained in a buffer that is continuously updated when there are frequent large updates.
This buffer of pose-updates are pushed as odometer updates to the camera graph only when these global pose updates are lesser than a threshold as described in Algorithm~\ref{algo:pose-buffer}.
This buffer-based updates avoids frequent global camera graph optimization avoiding high compute and memory demanding operations. \todo{this needs to be corrected}

From the Algorithm~\ref{algo:pose-buffer} we can see that the Pose updates buffer $V$, can create significant delay between the WiFi graph and camera graph. To avoid such significant delays we limit the size of the number of pose updates that can be held in the buffer $V$, thus avoiding any observable delays in the camera graph optimization.

Finally, once the camera factor graph receives the pose updates from the WiFi graph, they are used as `Oracle' pose measurements.
These measurements are used to constrain the camera locations where certain camera frames features have been detected and mapped.
We utilize VINS-MONO~\cite{qin2018vins} features extractor for feature extraction and feature matching across various frames. Once the feature matching across local frames has been performed they are then mapped into the 3D space as point clouds which are then optimized for in tandem with the WiFi global pose updates for optimized mapping and local pose corrections of the robot. \todo{add more information about SmartProjectionPoseFactors from GTSAM}
Thus \name solves for low-cost, low-compute, and context-aware SLAM system using a `Dual-graph' layered approach.

\section{Measurements For factor Graphs}\label{sec:design-measure}
To further demonstrate and deploy \name on COTS devices, we need to estimate accurate measurements for each factor graph.
So in this section, we present our solution for estimating accurate and robust WiFi bearing and camera measurements for the WiFi graph in ~\cref{sec:design-bearing} and camera graph in ~\cref{sec:design-camera}.

\subsection{Accurate \& Robust WiFi Measurements}\label{sec:design-bearing}

Finally, while existing works use end-to-end optimization, in \name we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for map-building. 
This demands that the bearing measurements made are real-time, robust and accurate.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reasons for inaccuracies in the bearing measurements for indoors are multipath and Non-Line of Sight issues that have been well-studied~\cite{spotfi,arraytrack,ayyalasomayajula2020deep,ma2019wifi,soltanaghaei2018multipath} in the literature. 
It is known that the WiFi signal is broadcasted and at the receiver a combination of all these different paths called `multipath' is measured as shown in Figure~\ref{fig:wifi-meas}.
Additionally, the receiver measures a complex, channel state information (CSI) whose phase values are the accumulation of delays along each individual direction. 
Wherein, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are cause for erroneous bearing estimates.
Additionally, since each antenna is physically at a farther distance, the phase accumulates for the extra distance travelled to each antenna on the access point.

With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna for $n^{th}$ frequency component, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m, n} = \underbrace{\Big[H^{m, n}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m, n}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{arraytrack,spotfi} are vulnerable to aliasing, as there is no distinction between signals coming from opposite sides of the array.
Since we need to resolve this ambiguity in order to estimate the true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. We incorporate this into our CSI model from Eq~\ref{eq:sensor_model1} as:
$$
    H^{m, n}_i = a_i \exp\left({\textstyle -\iota 2 \pi \frac{f_0}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right) \exp \left({\textstyle -\iota 2\pi  \frac{f_n}{c} l_i}\right)
$$
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{spotfi, vasisht2016decimeter}.


Individual CSI measurements are vulnerable to noise and transient multipath, meaning that some of the bearings we measure will be erroneous.
Systems in the past\cite{spotfi} have typically employed a two-stage solution of (i) principle component analysis (PCA) based temporal packet averaging, followed by a\todo{reword} (ii) super-resolution algorithm to deal with multipath accurately and separate the direct path from the reflected paths.
However, these super-resolution algorithms are very compute intensive and thus cannot be deployed in real time in a scalable manner. So, we instead rely just on temporal CSI smoothing to remove this noise from our measured channel. To this end, we observe that reflected paths are much less consistent across packets than the direct path\cite{arraytrack}. So, we combine multiple channel measurements into a matrix $M = \begin{bmatrix}M_0,&M_1,&...\end{bmatrix}$ to estimate the true channel $H$ from the measured channels. Assuming the robot does not move too much in between measurements, the true channel should remain consistent. Additionally, most devices transmitting WiFi signals transmit on multiple antennas, allowing us to make multiple channel measurements per transmission. With these dense measurements, we can now use PCA to estimate the true channel. We assume that noise and multipath is much less correlated across measurements than the direct path. Under this assumption, our distribution of channel measurements has greatest variance along an axis $V$ corresponding to our true channel. In particular, it maximises 
$$
H\approx\argmax_{V}\sum_{i}(|\langle M_i,V \rangle|)^2
$$.
This largest principle component $V$ of the measurement matrix M is commonly known to be the eigenvector corresponding to the largest eigenvalue of $MM^\dag$, where $\dag$ is the conjugate transpose operator. We compute this vector by singular value decomposition of $M$, where $V$ will be the first basis vector in the left subspace. Thus, we have implemented a CSI smoothing method that filters erroneous measurements and attenuates multipath, without using a high-compute super-resolution algorithm. In most cases, this channel will correspond to the direct path, and from here a simple 2D FFT can be used to identify the bearing of the direct path as detailed in ~\cite{ayyalasomayajula2018bloc,xie2019md}.

Thus, \name solves for getting accurate and dense bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

\subsection{Accurate Camera Measurements}\label{sec:design-camera}

In \name we utilize the camera feature extractor and tracker functionalities of the VINS-MONO implementation~\cite{qin2018vins}, wherein they extract the Shi-Tomasi features~\cite{shi1994good} for each frame. 
But as the robot moves some of the older frames and thus the features go out of view.
These out of frame features are replaced by a new set of features identified in the current frame so as to maintain a constant number of detected features in each frame.
This also avoids placing any features behind the camera's FOV and creating chirality issues. \todo{lacks clarity here}
The fixed number of camera points is a tunable parameter and in \name we use \todo{xx} number of features to be detected in each frame as `landmarks' mapped in the environment.
These `landmarks' aid in the local-pose corrections and mapping of the environment as discussed in ~\cref{sec:design-graph2}.

Thus we have seen how the layered approach in bifurcating the tasks between the WiFi and camera sensors to utilize them for what they are best at brings the best of both the sensors. This Visual and WiFi Dual factor graph SLAM solution thus makes \name-SLAM, low-cost, low-compute, accurate and adaptable SLAM system. Thus enabling scalable and deployable robotics using \name-SLAM's design.

==> design/design3.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

We have seen how existing Visual (camera) SLAM algorithms are compute and memory intensive, due to the accumulated drifts of the odometry that needs to be corrected. 
As discussed in ~\cref{sec:back-wifi}, we solve this by designing a dual-layered solution, as demonstrated in Figure~\ref{fig:intro-fig}.
The robot, mounted with WiFi and camera sensors, navigates in the environment, while \name's WiFi layer combines WiFi and odometry measurements to provide for accurate pose estimates that are drift free. 
This design removes the need for compute and memory heavy correlation (`loop-closure') operations. We first describe this drift-free pose generation in ~\cref{sec:design-graph1}.
These drift-free poses are fed to the \name visual layer that consumes these poses via a smart real-time buffer, along with camera frames, which we further detail in ~\cref{sec:design-graph2}.
In ~\cref{sec:design-measure}, we specify \name's methods for integrating these measurements into the \name WiFi and visual layers.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

Firstly, to identify the sensor modality to use within the \name WiFi layer that provides for drift-free pose estimates, we make a few interesting observations:
(i) All robots are equipped with a WiFi transceiver, (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is an inexpensive sensing modality, and (iv) WiFi based localization and tracking~\cite{ma2019wifi} is well studied and can be exploited for global pose estimation. Owing to these reasons, we utilize WiFi as a low-compute and low-memory sensor that can be used to build a SLAM system capable of providing drift-free robot poses to the Visual SLAM system.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}

\noindent\textbf{Angle of Arrival at Robot as WiFi Measurements:}
Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearing measurements are a robust WiFi-based estimation method for indoor localization and tracking.
Inspired from these works, we measure the Angle of Arrival (AoAs) of incoming signals at the robot,  thus not needing collaboration with WiFi access points (APs) in the environment. These are the WiFi measurements to be integrated into \name WiFi layer.
AoA measurements can be estimated at the robot's WiFi device with respect to WiFi transmitters in the environment using the Channel State Information, (CSI) measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi,arraytrack}.

\noindent\textbf{Unknown AP Locations and Robot Poses:}
Most current localization algorithms use AoA measurements with respect to multiple APs to locate the transmitting device. 
Unfortunately, we do not know the locations of these APs in the environment, as in a SLAM scenario we cannot assume any a priori information about the environment.
Thus, we cannot get accurate robot poses using existing localization algorithms~\cite{spotfi,soltanaghaei2018multipath,ayyalasomayajula2020deep,xie2019md}.
There are solutions that use robot pose to estimate the WiFi AP locations~\cite{ayyalasomayajula2020locap}, by tracking AoA measured from an AP across multiple known poses of the robot.
However, the authors of LocAP~\cite{ayyalasomayajula2020locap} need accurate robot poses to do this, which they achieve using a LiDAR based SLAM (Cartographer~\cite{cartographer}). This algorithm is memory and compute inefficient.
So, we need to somehow jointly solve for both the robot poses and the AP locations in the environment with the AoA measurements between them as the only known information.

We observe that GraphSLAM~\cite{gtsam} is capable of jointly solving these multi-variate optimization problems as long as these variables are connected by some measurements. This method uses a graph-based representation of the estimation problem to compute the most likely state of the system (robot poses and landmark locations) given a probabilistic model of the measurements.
So, we define the Wi-Fi facotr graph with odometry readings($z_I^{Odom}$) as measurements connecting two continuous robot poses $p_i,p_{i-1}$, and the Wi-Fi AoA estiamtes ($z_ij^{bearing}$) as measurements connecting the robot's current pose $p_i$ with each AP's position $x_j$ the AoA corresponds to as shown in Figure~\ref{fig:wifi-factor}.
Now that we have defined these variables and measurements, we can compute the most likely robot poses $p_i \forall i\in \{1,2,\cdots,n\}$ where $n$ is the current position of the robot and $n=[1 N]$, where $N$ are the total robot poses in the entirety of time and AP locations $x_j \forall j\in \{1,2,\cdots,N_{ap}\}$, where $N_{ap}$ are the number of APs in the environment.

\noindent\textbf{Building and Optimizing the WiFi-Graph:}
At a high level, the GraphSLAM algorithm defines a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \; \forall i \in [1, N]\}$, where each $\Vec{p}_i$ belongs to the Special Euclidean group ($SE(3)$). 
We can the define the measurement model for the odometry factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$ which would be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion~\cite{diebel2006representing}.
Similarly, one can define the factor graph for the bearing measurements of AP $j$ with AP position $x_j$ as $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$.

Unlike the existing WiFi SLAM architectures~\cite{arun2022p2slam,ferris2007wifi} we do not perform end-to-end optimization, we instead use the incremental smoothing and mapping (iSAM) implementation of the GraphSLAM approach~\cite{gtsam}.
So, once we have defined the measurement models we can estimate the optimized robot poses $S_{opt}^n$ for time instance $n$ by minimizing the total error between our predictions and actual measurements for the subset $I_{sub}$, i.e.
\begin{align}\label{eq:graph-optim-head}
    S_{opt}^n = \argmin_{S} \sum_{i\in I_{sub}} \sum_{j\in I_{sub}}  & \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and AoA measurements respectively. In iSAM, one step of optimization is performed every time a new measurement is added.
Upon a new addition to the graph, we want to optimize $\{p_i \; \forall i \in I_{sub}\}$ for given $I={p_i,x_j: i<n, \forall j \in [1, N_{ap}]}$, where $n$ is the next step of optimization. Only a subset of the factors $I_{sub} \subseteq I$ are optimized, according to the iSAM algorithm, without needing any memory and compute demanding global loop closures. Please refer Appendix~\ref{sec:appendix} for a more formal definitions of each of the variables and understanding the operation of incremental GraphSLAM (iSAM~\cite{gtsam}) which is an open-sourced solver.

\noindent\textbf{Initialization of Factors:} Now that we have defined our graph and the optimization problem, like for any other optimization algorithm we also need to initialize each of the $N$ robot positions and $N_{ap}$ AP positions for the optimizer. 
Like any other SLAM system, we initialize the robot positions using the relative odometry measurements, which have drift accumulated in them. This is the drift we are trying to remove.
Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
While one could naively initialize all known APs in the environment at the origin, some APs may start too far away as to estimate their position at all, as there may be no incoming measurements when the optimizer is started.

Since these APs have no measurements attached to them, the loss associated with them is ill-defined and the optimization problem is unsolvable.
Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this indeterminacy due to poor a poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been study extensively in the bast for localization~\cite{ez}.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's translation $p^t_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maximum among all current robot's poses $p_i \forall i \in [1,n]$ measured at $n^{th}$ time instance, with the intuition that this is where the robot passed closest to the AP.
We can then initialize $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation.
Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
Givem good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/camera_factor.pdf}
    \caption{Shows the details of the implementation of the Camera Factor graph. While a typical camera based SLAM would also correct for the robot poses, but since we do not optimize for robot poses in \name camera SLAM, we can thro these nodes away as shown in the figure.}
    \label{fig:cam-factor}
\end{figure}

\subsection{Camera Factor Graph}\label{sec:design-graph2}

As we described in ~\cref{sec:back-vio}, a Visual-Inertial Odometry based SLAM system needs camera features and odometry measurements. 
To extract, track and map the camera features we utilize  Shi-Tomasi features~\cite{shi1994good} from the VINS-MONO implementation~\cite{qin2018vins}.
These camera features are then mapped onto a unit sphere to get an approximate estimate of the 3D locations of the measured features.
These projections are then projected into the map as `landmarks' in the factor graph for a fixed set of local frames. 
The positions of these `landmarks' and the odometry measurements can now be jointly optimized to correct the robot's trajectory. 
These local corrections ensure accurate 3D mapping of the `landmark' point clouds in the environment as shown in Figure~\ref{fig:cam-factor}.
While a typical camera based SLAM would need to simultaneously correct for the robot poses, in \name, we strongly constrain the robot's poses to discourage optimizing over them, instead estimating them in \name's WiFi SLAM layer.

% We detail on how we extract robust camera measurements in ~\cref{sec:design-camera}, where we go into further details on how we use the feature extraction provided by the VINS-MONO feature extractor and tracker~\cite{qin2018vins}.
In addition to this, these VIO-SLAM systems require global loop closures to cancel the drift accrued in the robot pose estimates provided by the robot's inertial odometry. However, the homogeneity of these visual feature based landmarks demands constant feature matching operations, and requires a large memory cache of all the landmarks.
\name sidesteps this issue by using the global pose estimates provided by the WiFi graph, which do not drift over time, as the robot pose measurements for the camera graph.
Since these WiFi global pose estimates can be made in real time with high-accuracy, we can eliminate the need for global loop closure in these visual feature-based VIO-SLAM systems.

\begin{algorithm}[t]
\caption{Implementation of WiFi pose update buffering to the Visual Odometry graph.}
\label{algo:pose-buffer}
    \SetAlgoLined
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input{Pose threshold $\Delta P$, stability threshold size $N_{thresh}$, max size of circular cache $N_{cache}$}
    initialization circular cache $C_{update} \leftarrow \{\}$;
    Buffer $V_{update} \leftarrow \{\} $;
    Pose Updates $P_{opt}^0\leftarrow \{\} $ \\
    \For{$t \gets 1$ \KwTo $T$}{
        Estimate $P_{opt}^t$ from Eq~\ref{eq:graph-optim-head}
        \begin{flalign}
        P_{filt}^t &= \{p^t - p^{t-1} > \Delta P \;|\; p^t \in P_{opt}^t; p^{t-1} \in P_{opt}^{t-1}\}&&\nonumber\\
                    & \cup \; \{p \;|\; p \in  P_{opt}^t; p \not\in P_{opt}^{t-1}\}&&\nonumber
        \end{flalign}\\
        $N_t \gets |P_{filt}^t|$ \\
        $C_{update} \gets append(C_{update}, N_t)$ \\
        $V_{update} \gets append(V_{update}, P_{filt}^t)$ \\
        \If{$ n < N_{thresh}, \; \forall n \in C_{update} $}{
            Flushes the buffer, $V$ as pose updates
        }
    }
\end{algorithm}

So, these WiFi global pose estimates can be sent to the camera graph as odometry measurements when the WiFi graph updates.

\textbf{Smart Pose Update Buffering:}
However, numerous and large updates to the odometry measurements in the camera graph would trigger frequent graph optimization for large number of camera factors.
These camera factors will keep increasing as the number of robot poses keep increasing, leading to updates in the camera graph which becomes memory intensive.
Thus we cannot naively send each and every WiFi graph's pose updates to the camera graph and observe that these WiFi frames usually are updated at a rate of ~100Hz while camera frames are only fed at ~2-10Hz.
With this observation, \name WiFi graph's pose updates are maintained in a buffer ($V_{update}$) that is continuously updated when there are frequent large updates. A large update to the robot pose is defined with respect to the pose threshold, $\Delta P$ in Algorithm~\ref{algo:pose-buffer}.
This poses in $V_{update}$ are pushed as pose updates to the camera graph only when the WiFi-graph is stable, i.e., when the total number of updates in the past $N_{cache}$ optimization steps is less than $N_{thresh}$.
Effectively, by tuning $N_{cache}$ and $N_{thresh}$, we can define the sensitivity of stability. 
For example, by increasing $N_{cache}$ and decreasing $N_{thresh}$, we wait longer for the WiFi-graph robot poses to stabilize. 
Additionally, by tuning $\Delta P$, we can re-define what we mean by an update to reduce the number of the updates sent to the camera graph. 
By incorporating this smart buffer \name avoids frequent global camera graph optimization avoiding high compute and memory demanding operations. 

Finally, once the camera factor graph receives the pose updates from the WiFi graph, they are used as drift-free pose measurements.
These measurements are used to constrain the camera locations where certain camera features have been detected and mapped.
We utilize VINS-MONO~\cite{qin2018vins} features tracker for feature extraction and feature matching across various frames. 
Once the feature matching across local frames has been performed they are then mapped into the 3D space as point clouds which are then optimized for in tandem with the WiFi global pose updates for optimized mapping and local pose corrections of the robot. 
Thus \name solves for  compute and memory efficient SLAM system using a `Dual-graph' layered approach.

\section{Measurements For factor Graphs}\label{sec:design-measure}
To further demonstrate and deploy \name on COTS devices, we need to estimate accurate measurements for each factor graph.
So in this section, we present our solution for estimating accurate and robust WiFi bearing and camera measurements for the WiFi graph in ~\cref{sec:design-bearing} and camera graph in ~\cref{sec:design-camera}.

\subsection{Accurate \& Robust WiFi Measurements}\label{sec:design-bearing}

Finally, while existing works use end-to-end optimization, in \name we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for map-building. 
This demands that the bearing measurements made are real-time, robust and accurate.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reasons for inaccuracies in the bearing measurements for indoors are multipath and Non-Line of Sight issues that have been well-studied~\cite{spotfi,arraytrack,ayyalasomayajula2020deep,ma2019wifi,soltanaghaei2018multipath} in the literature. 
It is known that the WiFi signal is broadcasted and at the receiver a combination of all these different paths called `multipath' is measured as shown in Figure~\ref{fig:wifi-meas}.
Additionally, the receiver measures a complex, channel state information (CSI) whose phase values are the accumulation of delays along each individual direction. 
Wherein, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are cause for erroneous bearing estimates.
Additionally, since each antenna is physically at a farther distance, the phase accumulates for the extra distance travelled to each antenna on the access point.

With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna for $n^{th}$ frequency component, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m, n} = \underbrace{\Big[H^{m, n}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m, n}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{arraytrack,spotfi} are vulnerable to aliasing, as there is no distinction between signals coming from opposite sides of the array.
Since we need to resolve this ambiguity in order to estimate the true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. We incorporate this into our CSI model from Eq~\ref{eq:sensor_model1} as:
$$
    H^{m, n}_i = a_i \exp\left({\textstyle -\iota 2 \pi \frac{f_0}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right) \exp \left({\textstyle -\iota 2\pi  \frac{f_n}{c} l_i}\right)
$$
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{spotfi, vasisht2016decimeter}.

\todo{connect the english in this paragraph to the channel model build in 2}
Individual CSI measurements are vulnerable to noise and transient multipath, meaning that some of the bearings we measure will be erroneous.
Systems in the past\cite{spotfi} have typically employed a two-stage solution of (i) principle component analysis (PCA) based temporal packet averaging, followed by a (ii) super-resolution algorithm to deal with multipath accurately and separate the direct path from the reflected paths.
However, these super-resolution algorithms are very compute intensive and thus cannot be deployed in real time in a scalable manner. So, we instead rely just on temporal CSI averaging to remove this noise from our measured channel. To this end, we observe that reflected paths are much less consistent across packets than the direct path\cite{arraytrack}. So, we combine multiple channel measurements into a matrix $M = \begin{bmatrix}M_0,&M_1,&...\end{bmatrix}$ to estimate the true channel $H$ from the measured channels. Assuming the robot does not move too much in between measurements, the true channel should remain consistent. Additionally, most devices transmitting WiFi signals transmit on multiple antennas, allowing us to make multiple channel measurements per transmission. With these dense measurements, we can now use PCA to estimate the true channel. We assume that noise and multipath is much less correlated across measurements than the direct path. Under this assumption, our distribution of channel measurements has greatest variance along an axis $V$ corresponding to our true channel, that we call principle component channel or PC-CSI. In particular, it maximises 
$$
H\approx\argmax_{V}\sum_{i}(|\langle M_i,V \rangle|)^2.
$$
This largest principle component $V$ of the measurement matrix M is commonly known to be the eigenvector corresponding to the largest eigenvalue of $MM^\dag$, where $\dag$ is the conjugate transpose operator. We compute this vector by singular value decomposition of $M$, where $V$ will be the first basis vector in the left subspace. Thus, we have implemented a principle component CSI method that filters erroneous measurements and attenuates multipath, without using a high-compute super-resolution algorithm. In most cases, this channel will correspond to the direct path, and from here a simple 2D FFT can be used to identify the bearing of the direct path as detailed in ~\cite{ayyalasomayajula2018bloc,xie2019md}.

Thus, \name solves for getting accurate and dense bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

\subsection{Accurate Camera Measurements}\label{sec:design-camera}

In \name we utilize the camera feature extractor and tracker functionalities of the VINS-MONO implementation~\cite{qin2018vins}, \\wherein they extract the Shi-Tomasi features~\cite{shi1994good} for each frame. 
But as the robot moves some of the older frames and thus the features go out of view.
These out of frame features are replaced by a new set of features identified in the current frame so as to maintain a constant number of detected features in each frame.
This also avoids placing any features behind the camera's FOV and creating chirality issues.
The fixed number of camera points is a tunable parameter and in \name we use 50 number of features to be detected in each frame as `landmarks' mapped in the environment.
These `landmarks' aid in the local-pose corrections and mapping of the environment as discussed in ~\cref{sec:design-graph2}.

Thus we have seen how the layered approach in bifurcating the tasks between the WiFi and camera sensors to utilize them for what they are best at brings the best of both the sensors. This Visual and WiFi Dual factor graph SLAM solution thus makes \name-SLAM, low-memory, low-compute, accurate and adaptable SLAM system. Thus enabling scalable and deployable robotics using \name-SLAM's design.

==> design/design4.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

We have seen how existing Visual (camera) SLAM algorithms are compute and memory intensive, due to the accumulated drifts of the odometry that needs to be corrected. 
As discussed in ~\cref{sec:back-wifi}, we solve this by designing a dual-layered solution, as demonstrated in Figure~\ref{fig:intro-fig}.
The robot, mounted with WiFi and camera sensors, navigates in the environment, while \name's WiFi layer combines WiFi and odometry measurements to provide for accurate pose estimates that are drift free. 
This design removes the need for compute and memory heavy correlation (`loop-closure') operations. We first describe this drift-free pose generation in ~\cref{sec:design-graph1}.
These drift-free poses are fed to the \name visual layer that consumes these poses via a smart real-time buffer, along with camera frames, which we further detail in ~\cref{sec:design-graph2}.
In ~\cref{sec:design-measure}, we specify \name's methods for integrating these measurements into the \name WiFi and visual layers.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

Firstly, to identify the sensor modality to use within the \name WiFi layer that provides for drift-free pose estimates, we make a few interesting observations:
(i) All robots are equipped with a WiFi transceiver, (ii) WiFi is ubiquitously deployed in indoor environments, (iii) WiFi is an inexpensive sensing modality, and (iv) WiFi based localization and tracking~\cite{ma2019wifi} is well studied and can be exploited for global pose estimation. Owing to these reasons, we utilize WiFi as a low-compute and low-memory sensor that can be used to build a SLAM system capable of providing drift-free robot poses to the Visual SLAM system.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}

\noindent\textbf{Angle of Arrival at Robot as WiFi Measurements:}
Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearing measurements are a robust WiFi-based estimation method for indoor localization and tracking.
Inspired from these works, we measure the Angle of Arrival (AoAs) of incoming signals at the robot,  thus not needing collaboration with WiFi access points (APs) in the environment. These are the WiFi measurements to be integrated into \name WiFi layer.
AoA measurements can be estimated at the robot's WiFi device with respect to WiFi transmitters in the environment using the Channel State Information, (CSI) measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi,arraytrack}.

\noindent\textbf{Unknown AP Locations and Robot Poses:}
Most current localization algorithms use AoA measurements with respect to multiple APs to locate the transmitting device. 
Unfortunately, we do not know the locations of these APs in the environment, as in a SLAM scenario we cannot assume any a priori information about the environment.
Thus, we cannot get accurate robot poses using existing localization algorithms~\cite{spotfi,soltanaghaei2018multipath,ayyalasomayajula2020deep,xie2019md}.
There are solutions that use robot pose to estimate the WiFi AP locations~\cite{ayyalasomayajula2020locap}, by tracking AoA measured from an AP across multiple known poses of the robot.
However, the authors of LocAP~\cite{ayyalasomayajula2020locap} need accurate robot poses to do this, which they achieve using a LiDAR based SLAM (Cartographer~\cite{cartographer}). This algorithm is memory and compute inefficient.
So, we need to somehow jointly solve for both the robot poses and the AP locations in the environment with the AoA measurements between them as the only known information.

We observe that GraphSLAM~\cite{gtsam} is capable of jointly solving these multi-variate optimization problems as long as these variables are connected by some measurements. This method uses a graph-based representation of the estimation problem to compute the most likely state of the system (robot poses and landmark locations) given a probabilistic model of the measurements.
So, we define the Wi-Fi facotr graph with odometry readings($z_I^{Odom}$) as measurements connecting two continuous robot poses $p_i,p_{i-1}$, and the Wi-Fi AoA estiamtes ($z_ij^{bearing}$) as measurements connecting the robot's current pose $p_i$ with each AP's position $x_j$ the AoA corresponds to as shown in Figure~\ref{fig:wifi-factor}.
Now that we have defined these variables and measurements, we can compute the most likely robot poses $p_i \forall i\in \{1,2,\cdots,n\}$ where $n$ is the current position of the robot and $n=[1 N]$, where $N$ are the total robot poses in the entirety of time and AP locations $x_j \forall j\in \{1,2,\cdots,N_{ap}\}$, where $N_{ap}$ are the number of APs in the environment.

\noindent\textbf{Building and Optimizing the WiFi-Graph:}
At a high level, the GraphSLAM algorithm defines a state space, $S$, which is a set of robot poses over $N$ time steps in our graph, $S = \{\Vec{p}_i \; \forall i \in [1, N]\}$, where each $\Vec{p}_i$ belongs to the Special Euclidean group ($SE(3)$). 
We can the define the measurement model for the odometry factors between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps $\hat{z}^{odom}(\cdot)$ which would be:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion~\cite{diebel2006representing}.
Similarly, one can define the factor graph for the bearing measurements of AP $j$ with AP position $x_j$ as $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$.

Unlike the existing WiFi SLAM architectures~\cite{arun2022p2slam,ferris2007wifi} we do not perform end-to-end optimization, we instead use the incremental smoothing and mapping (iSAM) implementation of the GraphSLAM approach~\cite{gtsam}.
So, once we have defined the measurement models we can estimate the optimized robot poses $S_{opt}^n$ for time instance $n$ by minimizing the total error between our predictions and actual measurements for the subset $I_{sub}$, i.e.
\begin{align}\label{eq:graph-optim-head}
    S_{opt}^n = \argmin_{S} \sum_{i\in I_{sub}} \sum_{j\in I_{sub}}  & \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and AoA measurements respectively. In iSAM, one step of optimization is performed every time a new measurement is added.
Upon a new addition to the graph, we want to optimize $\{p_i \; \forall i \in I_{sub}\}$ for given $I={p_i,x_j: i<n, \forall j \in [1, N_{ap}]}$, where $n$ is the next step of optimization. Only a subset of the factors $I_{sub} \subseteq I$ are optimized, according to the iSAM algorithm, without needing any memory and compute demanding global loop closures. Please refer Appendix~\ref{sec:appendix} for a more formal definitions of each of the variables and understanding the operation of incremental GraphSLAM (iSAM~\cite{gtsam}) which is an open-sourced solver.

\noindent\textbf{Initialization of Factors:} Now that we have defined our graph and the optimization problem, like for any other optimization algorithm we also need to initialize each of the $N$ robot positions and $N_{ap}$ AP positions for the optimizer. 
Like any other SLAM system, we initialize the robot positions using the relative odometry measurements, which have drift accumulated in them. This is the drift we are trying to remove.
Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
While one could naively initialize all known APs in the environment at the origin, some APs may start too far away as to estimate their position at all, as there may be no incoming measurements when the optimizer is started.

Since these APs have no measurements attached to them, the loss associated with them is ill-defined and the optimization problem is unsolvable.
Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this indeterminacy due to poor a poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been study extensively in the bast for localization~\cite{ez}.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's translation $p^t_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maximum among all current robot's poses $p_i \forall i \in [1,n]$ measured at $n^{th}$ time instance, with the intuition that this is where the robot passed closest to the AP.
We can then initialize $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation.
Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
Given good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.

\subsection{Accurate \& Robust WiFi Measurements}\label{sec:design-bearing}

Finally, while existing works use end-to-end optimization, in \name we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for map-building. 
This demands that the bearing measurements made are real-time, robust and accurate.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reasons for inaccuracies in the bearing measurements for indoors are multipath and Non-Line of Sight issues that have been well-studied~\cite{spotfi,arraytrack,ayyalasomayajula2020deep,ma2019wifi,soltanaghaei2018multipath} in the literature. 
It is known that the WiFi signal is broadcasted and at the receiver a combination of all these different paths called `multipath' is measured as shown in Figure~\ref{fig:wifi-meas}.
Additionally, the receiver measures a complex, channel state information (CSI) whose phase values are the accumulation of delays along each individual direction. 
Wherein, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are cause for erroneous bearing estimates.
Additionally, since each antenna is physically at a farther distance, the phase accumulates for the extra distance travelled to each antenna on the access point.

With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna for $n^{th}$ frequency component, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m, n} = \underbrace{\Big[H^{m, n}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m, n}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{arraytrack,spotfi} are vulnerable to aliasing, as there is no distinction between signals coming from opposite sides of the array.
Since we need to resolve this ambiguity in order to estimate the true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. We incorporate this into our CSI model from Eq~\ref{eq:sensor_model1} as:
$$
    H^{m, n}_i = a_i \exp\left({\textstyle -\iota 2 \pi \frac{f_0}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right) \exp \left({\textstyle -\iota 2\pi  \frac{f_n}{c} l_i}\right)
$$
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{spotfi, vasisht2016decimeter}.

\todo{connect the english in this paragraph to the channel model build in 2}
Individual CSI measurements are vulnerable to noise and transient multipath, meaning that some of the bearings we measure will be erroneous.
Systems in the past\cite{spotfi} have typically employed a two-stage solution of (i) principle component analysis (PCA) based temporal packet averaging, followed by a (ii) super-resolution algorithm to deal with multipath accurately and separate the direct path from the reflected paths.
However, these super-resolution algorithms are very compute intensive and thus cannot be deployed in real time in a scalable manner. So, we instead rely just on temporal CSI averaging to remove this noise from our measured channel. To this end, we observe that reflected paths are much less consistent across packets than the direct path\cite{arraytrack}. So, we combine multiple channel measurements into a matrix $M = \begin{bmatrix}M_0,&M_1,&...\end{bmatrix}$ to estimate the true channel $H$ from the measured channels. Assuming the robot does not move too much in between measurements, the true channel should remain consistent. Additionally, most devices transmitting WiFi signals transmit on multiple antennas, allowing us to make multiple channel measurements per transmission. With these dense measurements, we can now use PCA to estimate the true channel. We assume that noise and multipath is much less correlated across measurements than the direct path. Under this assumption, our distribution of channel measurements has greatest variance along an axis $V$ corresponding to our true channel, that we call principle component channel or PC-CSI. In particular, it maximises 
$$
H\approx\argmax_{V}\sum_{i}(|\langle M_i,V \rangle|)^2.
$$
This largest principle component $V$ of the measurement matrix M is commonly known to be the eigenvector corresponding to the largest eigenvalue of $MM^\dag$, where $\dag$ is the conjugate transpose operator. We compute this vector by singular value decomposition of $M$, where $V$ will be the first basis vector in the left subspace. Thus, we have implemented a principle component CSI method that filters erroneous measurements and attenuates multipath, without using a high-compute super-resolution algorithm. In most cases, this channel will correspond to the direct path, and from here a simple 2D FFT can be used to identify the bearing of the direct path as detailed in ~\cite{ayyalasomayajula2018bloc,xie2019md}.

Thus, \name solves for getting accurate and dense bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

==> design/design5.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

\todo{Start by describing your design... }

We have seen that loop closures can be memory and compute intensive at best or at worst can detrimentally affect the quality of the pose prediction during incorrect keyframe matching. \todo{have you? read your DLOC design intro... }
To circumvent loop-closures entirely, we design a real time \todo{is it just WiFi graph??} Wifi-graph as demonstrated in Figure~\ref{fig:wifi-factor} to take advantage of existing WiFi access points in the environment and provide correction to drift accommodated by Visual-intertial or Lidar-inertial SLAM systems.

The robot, mounted with WiFi and camera (or Lidar) sensors, navigates in the environment. Through local feature matching (or scan matching) and the inertial measurements from IMU (or wheel encoder), the SLAM algorithm provides accurate pose measurements for the robot in real time. These pose updates from the local-odometry are fed into the Wifi-graph which incorporates the bearing of the incoming WiFi signal to track a deployed WiFi access point (AP) in an environment. In effect, the AP is treated as a stationary and unique landmark. Furthermore, since the incoming WiFi signal identifies the access point it originated from, this design removes the need for compute and memory heavy correlation (`loop-closure') operations. 

We first formulate and describe this drift-free pose generation in ~\cref{sec:design-graph1} assuming we have the local-odometry from VIO/LIO.
We then detail on how to get accurate WiFi measurements for the WiFi graph's real-time optimization in ~\cref{sec:design-bearing}. We finally describe how the system is built and optimized along with the Visual-graph in ~\cref{sec:design-camera}.

\subsection{WiFi Factor Graph}\label{sec:design-graph1}

Firstly, to motivate the use of WiFi as the sensor modality to use, we make a few interesting observations:
(i) All robots are equipped with a WiFi transceiver, (ii) It is ubiquitously deployed in indoor environments, (iii) It is an inexpensive sensing modality, and (iv) WiFi based localization and tracking~\cite{ma2019wifi} is well studied and can be exploited for global pose estimation. Owing to these reasons, we utilize WiFi as a low-compute and low-memory sensor that can be used to build a SLAM system capable of providing drift-free robot poses to the Visual (or Lidar) SLAM systems. \todo{make sure you don't under-estimate your contribution to A+B, if WiFi is already low-compute and low-memory what did you do? }

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}

\noindent\textbf{Angle of Arrival at Robot as WiFi Measurements:}
Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearing measurements are a robust WiFi-based estimation method for indoor localization and tracking.
Inspired from these works, we use the bearing of the incoming signals at the robot as our WiFi measurements, thus not needing collaboration with WiFi access points (APs) in the environment.
Bearing measurements can be estimated at the robot's WiFi device with respect to WiFi transmitters in the environment using the Channel State Information, CSI, measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi}.

Unfortunately, we do not know the locations of these APs in the environment a-prioiri, as is typically required~\cite{spotfi}.
So, we need to jointly solve for both the robot poses and the AP locations in the environment with the AoA measurements between them as the only known information.

We observe that GraphSLAM~\cite{gtsam} is capable of jointly solving these multi-variate optimization problems as long as these variables are connected by some measurements. This method uses a graph-based representation of the estimation problem to compute the most likely state of the system (robot poses and landmark locations) given a probabilistic model of the measurements.
So, we define the Wi-Fi factor graph with odometry readings($z_i^{odom}$) as measurements connecting two continuous robot poses $p_i,p_{i+1}$, and the Wi-Fi AoA estimates ($z_{ij}^{Bearing}$) as measurements connecting the robot's current pose $p_i$ with each AP's position $x_j$ as shown in Figure~\ref{fig:wifi-factor} (left).
Here we assume a generic in-between odometry reading, which can be provided by the VIO/LIO \textit{without} their loop-closure modules or a simple wheel encoder.
Now that we have defined these variables and measurements, we can compute the most likely robot poses $p_i \forall i\in \{1,2,\cdots,n\}$ where $n$ is the current position of the robot and $n=[1 N]$, where $N$ are the total robot poses in the entirety of time and AP locations $x_j \forall j\in \{1,2,\cdots,N_{ap}\}$, where $N_{ap}$ are the number of APs in the environment.

\noindent\textbf{Building and Optimizing the WiFi-Graph:}
Unlike prior work~\cite{arun2022p2slam, ferris2007wifi}, we do not use end-end optimization and instead opt to use the incremental smoothing and mapping (iSAM)~\cite{gtsam} to provide real-time pose estimates. At a high level, the state space at time $t$, $S_t$, is a set of robot poses and access point locations over $t$ time steps in our graph, $S_t = \{\Vec{p}_i \; \forall i \in [1, t]\} \cup \{\Vec{x}_j \; \forall j \in [1, N]\}$, with the robot pose, $\Vec{p}_i \in SE(3)$ and the $N$ access points positions observed till time $t$, $x_i \in \mathbb{R}^3$. 
We can the define odometry measurements (from VIO/LIO or wheel encoders) between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps as:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion~\cite{diebel2006representing}.
Similarly, one can define the factor graph for the bearing measurements of AP $j$ with AP position $x_j$ as $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$. \todo{add this factor defn here as well}

So, once we have defined the measurement models we can estimate the optimized robot poses $S^{opt}_t$ for time instance $t$ by minimizing the total error between our predictions and actual measurements,
\begin{align}\label{eq:graph-optim-head}
    S^{opt}_t = \argmin_{S_t} & \sum_{i \leq t} \sum_{j \leq N}  \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and bearing measurements respectively. 

\noindent\textbf{Initialization of Factors:} Next to ensure convergence of our optimization, we need to initialize each of the $t$ robot positions and $N$ AP positions for the optimizer. 
Similar to prioir works~\cite{arun2022p2slam}, the robot positions are initialized using the relative odometry measurements. These poses have accumulated drift over time which we seek to correct.
A naive initialization for the AP's would be to place them at the origin and allow the optimizer to place them appropriately in the environment. Unfortunately, the iSAM optimizer, given the limited number of measurements it has seen up until time $t$, can fail to converge with this naive initialization. 

% Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
% While one could naively initialize all known APs in the environment at the origin, some APs may not be receiving any signals at all as they are actually very far from the robot's origin, thus might be too far away when the optimizer is started.

% Since these faraway APs have no measurements attached to them, the cost associated with them is ill-defined and the optimization problem is unsolvable.
% Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this in-determinancy due to poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been study extensively in the past for localization~\cite{ez}.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's pose $p_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maximum among all current robot's poses $p_i \forall i \in [1,t]$, with the intuition that this is where the robot passed closest to the AP.
We can then initialize the $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation. This random perturbation is added to avoid in-determinancy with the optimizer. 
% Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
% Given good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.

\subsection{Accurate \& Unambiguous WiFi Measurements}\label{sec:design-bearing}

Finally, while existing works use end-to-end optimization, in \name we need to perform real-time global pose estimates as the camera factor graph is consuming these poses in real-times for map-building. 
This demands that the bearing measurements made are real-time, unambiguous and accurate.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reasons for inaccuracies in the bearing measurements for indoors are multipath and Non-Line of Sight issues that have been well-studied~\cite{spotfi,arraytrack,ayyalasomayajula2020deep,ma2019wifi,soltanaghaei2018multipath} in the literature. 
It is known that the WiFi signal is broadcasted and at the receiver a combination of all these different paths called `multipath' is measured as shown in Figure~\ref{fig:wifi-meas}.
Additionally, the receiver measures a complex, channel state information (CSI) whose phase values are the accumulation of delays along each individual direction. 
Wherein, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are cause for erroneous bearing estimates.
Additionally, since each antenna is physically at a farther distance, the phase accumulates for the extra distance travelled to each antenna on the access point.

With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna for $n^{th}$ frequency component, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m, n} = \underbrace{\Big[H^{m, n}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m, n}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/eval_ral/aoa-err-boxplot.pdf}
    \caption{ \todo{complete, }}
    \label{fig:aoa-array}
    \vspace{-0.1in}
\end{figure}


\noindent\textbf{Unambiguous Measurements:} However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{arraytrack,spotfi} can resolve only half-plane of the horizontal plane. Thus these linear arrays are vulnerable to aliasing in the full-horizontal plane, as there is no distinction between signals coming from opposite half-planes of the array. Further, as shown in Figure~\ref{fig:aoa-array}(bottom) the errors in bearing measurements increase as the actual bearings are farther from $0^{\circ}$ for the datasets of $\mathrm{P^2}$SLAM.
Since we need to resolve this ambiguity in order to estimate the accurate and true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. 
This can be further seen from Figure~\ref{fig:aoa-array}(top) for the dataset we have collected with the square array. We can see that a square array can resolve more accurately without ambiguity between $-170^{\circ}$ to $180^{\circ}$.
So, we incorporate this into our CSI model from Eq~\ref{eq:sensor_model1} as:
\begin{align}
    H^{m, n}_i = a_i * & \exp\left({\textstyle -\iota 2 \pi \frac{f_0}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right)  \notag\\ &  * \exp \left({\textstyle -\iota 2\pi  \frac{f_n}{c} l_i}\right)
\end{align}
    
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{spotfi, vasisht2016decimeter}.

\todo{connect the english in this paragraph to the channel model build in 2}

\noindent\textbf{Accurate and Real-time bearing measurements:} In order to identify the direct signal's path among the multiple reflected paths, past Wi-Fi systems\cite{spotfi} have used algorithms that super-resolve the measured signal using principle component analysis (PCA) as well as information across different frequency bins to measure the relative time offset between different signal paths. This allows identification of the direct path, as it must have traveled the least distance of all paths and thus arrives before the other reflections

However, these super-resolution algorithms are very compute intensive, because they need to consider each antenna's CSI at each subcarrier frequency independently, and because they have added another dimension to the search space of signals. So, in \name we employ a sliding-window PCA based algorithm to efficiently combine information across subcarriers to estimate the direct path without having to identify and separate all of the reflected paths present in the signal.

We observe that the direct path signal has a property that the reflected paths typically do not: as it has traveled in a straight line, we can expect its contribution to the measured channel $H$ to be much better described by the model \ref{eq:sensor_model1} than the reflected paths. Intuitively, the direct path channel $H_0$ is relatively simple, while the reflected path channels $H_{1...n}$ to estimate the true channel $H$ from the measured channels. Assuming the robot does not move too much in between measurements, the true channel should remain consistent. Additionally, most devices transmitting WiFi signals transmit on multiple antennas, allowing us to make multiple channel measurements per transmission. With these dense measurements, we can now use PCA to estimate the true channel. We assume that noise and multipath is much less correlated across measurements than the direct path. Under this assumption, our distribution of channel measurements has greatest variance along an axis $V$ corresponding to our true channel, that we call principle component channel or PC-CSI. In particular, it maximises 
$$
H\approx\argmax_{V}\sum_{i}(|\langle M_i,V \rangle|)^2.
$$
This largest principle component $V$ of the measurement matrix M is commonly known to be the eigenvector corresponding to the largest eigenvalue of $MM^\dag$, where $\dag$ is the conjugate transpose operator. We compute this vector by singular value decomposition of $M$, where $V$ will be the first basis vector in the left subspace. Thus, we have implemented a principle component CSI method that filters erroneous measurements and attenuates multipath, without using a high-compute super-resolution algorithm. In most cases, this channel will correspond to the direct path, and from here a simple 2D FFT can be used to identify the bearing of the direct path as detailed in ~\cite{ayyalasomayajula2018bloc,xie2019md}.

\noindent\textbf{RSSI Filtering:} Finally, the measurements averaged across time in PC-FFT might note have direct-path which would lead to the dominant path being the reflected path or a noisy measurement. To avoid this, based on the intuition that the signal without the direct path or a weak direct path has very weak received signal strength (RSSI) we set an empirically verified RSSI threshold of $-65$dBm. This leads to the PC-FFT based bearing measurements are accurate.

Thus, \name solves for getting real-time, unambiguous and accurate bearing measurements to be fed into the WiFi factor graph described in ~\cref{sec:design-graph1}.

\begin{figure*}[pt]
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem-interframetime.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation_no_lc.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/aoa_err.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\textbf{Microbenchmarks}: \textbf{(a) Kimera:} Shows the trade-off between memory consumption(red) and the accuracy(blue) for various interframe rates. \textbf{(b) Cartographer:} Shows the trade-off between compute required(red) and the accuracy(blue) for various scan-matching thresholds. \textbf{(c) Odometry-Graph:} Shows the comparison on how various odometry inputs to the WiFi graph look before optimization.\textbf{(d) Bearing Measurement Algorithms:} Comparison between 2D-FFT from $\mathrm{P^2}$SLAM, PC-2D-FFT and our proposed PC-FFT. \todo{avg cpu: 2dfft: 5.6, pc-2dfft: 4.7, pc-fft: 0.11}}
    \label{fig:micro}
    \vspace{-0.1in}
\end{figure*}

\subsection{Dual Graph Integration}\label{sec:design-camera}
Thus we have seen on how the WiFi graph optimizes for accurate and real-time 3-DoF robot poses without requiring any loop-closures when provided with the odometry measurements.
These Odometry can simply come from a wheel encoder and gyroscope of the wheeled robot but it will not have any visual context to be able to provide any human-readable maps.
In contrast, in \name-SLAM's design, we utilize a dual graph approach, wherein we utilize existing VIO/LIO SLAM systems without their loop closure detection and corrections enabled.
So, while these VIO/LIO systems can correct for local drifts in the wheel encoders or the IMUs, they cannot perform global corrections.
These locally corrected robots 3-DoF poses are used to provide the Odometry measurements for the WiFi-graph that we have built in ~\cref{sec:design-graph1}.

The advantage with turning off the loop closure detection and corrections though is that the rate of memory of consumption and compute required is minimized.
Thus, the `VIO/LIO graph` can map the environment while providing locally corrected odometry measurements to the `WiFi-graph`.
The WiFi-graph thus then performs global corrections without the need of loop-closure detection thus enabling \name-SLAM to be an accurate, real-time robot navigation system that can minimizing the rate of memory consumption and the amount of compute.

==> design/design6.tex <==
% !TEX root = root.tex
\section{\name's Dual layered Design}\label{sec:design}

A robot, mounted with WiFi and camera (or Lidar) sensors, navigates in the environment. Through local feature matching (or scan matching) and the inertial measurements from IMU (or wheel encoder), the SLAM algorithm provides accurate local pose measurements for the robot in real time. These pose updates from the local-odometry are fed into the WiFi-graph (described in ~\cref{sec:design-graph1}) which incorporates the bearing of the incoming WiFi signal (described in ~\cref{sec:design-bearing}) to track a deployed WiFi access point (AP) in an environment. In effect, the AP is treated as a stationary and unique landmark. Furthermore, since the incoming WiFi signal identifies the access point it originated from, this design removes the need for compute and memory heavy correlation (`loop-closure') operations. Finally, it is imperative to initialize our access points optimally to ensure stability of the convergence (described in~\cref{sec:design-init}). 

% We first formulate and describe this drift-free pose generation in ~\cref{sec:design-graph1} assuming we have the local-odometry from VIO/LIO.
% We first detail on how to get accurate WiFi measurements for the WiFi graph's real-time optimization in ~\cref{sec:design-bearing}. 

\subsection{Providing accurate and real-time WiFi measurements}\label{sec:design-bearing}

Firstly, to motivate the use of WiFi as the sensor modality to use, we make a few interesting observations:
(i) All robots are equipped with a WiFi transceiver, (ii) It is ubiquitously deployed in indoor environments, and (iii) WiFi based localization and tracking~\cite{ma2019wifi, spotfi} is well studied and can be exploited for global pose estimation. Owing to these reasons, we utilize WiFi as a promising sensor to build a SLAM system capable of providing drift-free robot poses to the Visual (or Lidar) SLAM systems. 

Recent research into decimeter accurate WiFi localization~\cite{ma2019wifi,spotfi} and accurate WiFi SLAM approaches~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} has shown that bearing measurements are a robust WiFi-based estimation method for indoor localization and tracking.
Inspired from these works, we use the bearing of the incoming signals at the robot as our WiFi measurements (as shown in Figure~\ref{fig:wifi-meas}). This moves away from prior work~\cite{arun2022p2slam} which required bearings to be measured at the access point as well and removes the need to collaborate with WiFi access points (APs) in the environment.
Specifically, these bearing measurements, providing the direction of the WiFi AP's in the environment in the robot's local coordinate frame, can be estimated using the Channel State Information, CSI, measured on reception of a WiFi signal~\cite{arun2022p2slam,spotfi}. But there are important challenges which need to be overcome to ensure these bearing measurements are accurate and unambiguous to allow for real-time global drift corrections.  

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/bearing_measures.pdf}
    \caption{Shows the details of Robust and accurate WiFi bearing measurements made in \name}
    \label{fig:wifi-meas}
\end{figure}

The major reason for inaccuracies in the bearing measurements for indoors is multipath~\cite{spotfi,ayyalasomayajula2020deep,ma2019wifi}. 
A WiFi signal is broadcasted, and multiple reflections of the signal (\textit{mulitpath}) along with the direct path, impinge at the receiver as shown in Figure~\ref{fig:wifi-meas}. Clearly, the `direct-path' (solid-line) is the only path helpful in estimating the bearing to the source and the rest of the `reflected-paths' (dotted lines) are the cause for erroneous bearing estimates. The receiver measures complex-valued channel state information (CSI) describing the phase delay and attenuation between each transmitter-receiver pair.
Since each antenna is at a different location, different phases accumulate between antennas depending on the incoming angle. With this intuition, we can define our WiFi-sensor measurement model at the $m^\mathrm{th}$ antenna, assuming $K$ multipath components as 
\begin{align}\label{eq:sensor_model1}
    H^{m} = \underbrace{\Big[H^{m}_0(\theta_0, l_0)}_\text{Direct Path} + \sum_{i = 1}^K H^{m}_i(\theta_i, l_i)\Big]e^{\textstyle -\iota \phi} 
\end{align}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/eval_ral/aoa-err-boxplot.pdf}
    \caption{Bearing errors are accumulated in steps of $10^\circ$ for the the square antenna array (\textit{Top}) and linear array (\textit{Bottom}).}
    \label{fig:aoa-array}
    \vspace{-0.1in}
\end{figure}

\noindent\textbf{Unambiguous Measurements:} However, the uniform linear arrays used by existing bearing estimation algorithms~\cite{spotfi, arun2022p2slam} are vulnerable to aliasing - they can only measure bearings in a $180^\circ$ range(i.e. the top half plane in Figure~\ref{fig:wifi-meas}) at a time, as there is no distinction between signals coming from opposite sides of the array. Furthermore, as shown in Figure~\ref{fig:aoa-array}(bottom) these arrays have low resolution of signals travelling mostly parallel to the array. The datasets in $\mathrm{P^2}$SLAM utilize a linear array, but since we need to resolve this ambiguity in order to estimate the true direction of arrival, in \name we adapt to a square antenna array, which does not suffer from aliasing. 
This can be further seen from Figure~\ref{fig:aoa-array}(top) for the dataset we have collected with the square array -- \name's finds a good trade-off between resolution and aliasing, able to resolve angles from $-160^{\circ}$ to $160^{\circ}$.
This array allows us to calculate the channel model in Eq~\ref{eq:sensor_model1} as:
\begin{align}
    H^{m}_i (\theta_i, l_i) = a_i \times & \exp\left({\textstyle -\iota 2 \pi \frac{f}{c} \left\langle\begin{bmatrix}\cos{\theta_i}\\\sin{\theta_i}\end{bmatrix},\begin{bmatrix}R_{m,x}\\R_{m,y}\end{bmatrix}\right\rangle}\right)  \notag\\ &  \times \exp \left({\textstyle -\iota 2\pi  \frac{f}{c} l_i}\right)
\end{align}
    
with $a_i$ as the amplitude, $R_{m,x}$ and $R_{m,y}$ as the x and y positions of the $m^{th}$ receiver antenna, and $\theta_i$ and $l_i$ as the angle of arrival and path length of each of the incoming signals. Furthermore, we have an additional phase term, $\phi$, appended to account for random phase offsets that are introduced due to lack of synchronization between the robot and the access points in the environment~\cite{ma2019wifi}.

% \todo{connect the english in this paragraph to the channel model build in 2}

\noindent\textbf{Accurate and Real-time bearing measurements:} In order to identify the direct signal's path among the multiple reflected paths, past Wi-Fi systems\cite{ma2019wifi} have used algorithms that `super-resolve' the measured signal using information across the $N$ different frequency bins to measure the relative time offset between different signal paths. This allows identification of the direct path, as it must have traveled the least distance of all paths and thus arrives before the other reflections.

However, these super-resolution algorithms are very compute intensive because they have added another dimension to the search space of signals. 
So, in \name we employ a sliding-window PCA based algorithm to efficiently combine information across subcarriers to estimate the direct path without identifying all of the reflected paths present in the signal, which we refer to as PCAB (Principle Component Analysis based Bearing). This begs the question, how can we perform adequate bearing estimation despite mulitpath corruption? 

The wireless channel in Eq~\ref{eq:sensor_model1} can be extended to incorporate the $L \geq 1$ transmitters' channel response. $H_f$, an $m\times l$ sub-matrix of the channel values for a particular subcarrier frequency $f$, can be decomposed~\cite{fukushima} by singular value decomposition into
$$H_f=U\Sigma\Bar{V}.$$
The left eigenvectors, $U$, form an orthogonal basis for the signals measured at the receiver, and similarly, the rows of $\bar{V}$ form a basis for signals transmitted from the transmitter. 

We identify a property that the direct path signal has which the others do not: since the direct path has traveled in a straight line, the columns of the direct path channel $H_{0}$ will be very highly correlated over time instances and subcarrier frequencies. However, reflected paths in general are much more susceptible to small changes in transmitter position and frequency, as real-world reflections can take many continuous reflected paths and create complex constructive and destructive interference. Thus, we expect that the strongest principle component of $H$, $U_0$ should correspond to the direct path signal and the multipath can be effectively averaged out.

Specifically, in PCAB, our goal is to get the best estimate of the responses at the receivers ($U_0$). Hence, we treat the channels response for each subcarrier-transmitter pair independently to create a stacked channel matrix at time $i$ as $H_i \in \mathbb{C}^{N \times ML}$, and compute the autocorrelation matrix $H_i\bar{H_i}$. Furthermore, we combine the most recent $T$ matrices across a period of 0.5 seconds and compute $U_0$ as:

% and  instead of working with each receiver-subcarrier pair independently to super-resolve the measured signal, we treat each transmitter-subcarrier pair as a separate transmitter. Thus we can combine the auto-correlation matrices across the $p$ most recent packets and $t$ transmitters to get a very good estimate of $U_0$
$$
U_0 = \boldsymbol{\lambda_0}(\sum_{i= t-T}^t H_{i}\Bar{H}_{i}),
$$
Where $\boldsymbol{\lambda_0}(\cdot)$ denotes the largest eigenvector, which is trivial to compute for our $N \times  N$ autocorrelation matrix. From here, our direct path signal $U_0$ can be mapped to a bearing by a coarse search over the space of possible bearings. This method allows us to achieve similar bearing estimation performance to the standard 2D-FFT algorithm~\cite{arun2022p2slam} at just a fraction of the compute, as PCAB only has to perform a one-dimensional search across possible bearings instead of a 2-dimensional search across bearings and distances.


\noindent\textbf{RSSI Filtering:} One assumption made in the PCAB algorithm is that the direct path is present in the measured channel in the first place. In cases where a large reflector blocks the direct path, no information can be obtained about the direct path's bearing. These non-line-of-sight (NLOS) scenarios are common and need to be handled adequately to avoid instability of the backend optimizer. We observe that in these situations, overall received signal power (RSSI) is typically very low, as the majority of the signal has been blocked. To avoid this, we reject all measurements with RSSI below $-65$dBm, which we empirically observe filters out the vast majority of these obstructed packets. Thus, \name provides real-time, unambiguous and accurate bearing measurements to be fed into the WiFi factor graph, described in ~\cref{sec:design-graph1}.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wifi_factor.pdf}
    \caption{\name's WiFi Graph (a) Shows the various measurements that are made across robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
    \vspace{-1em}
\end{figure}

% \subsection{Dual Graph Integration}\label{sec:design-camera}
% Thus we have seen on how the WiFi graph optimizes for accurate and real-time 3-DoF robot poses without requiring any loop-closures when provided with the odometry measurements.
% These Odometry can simply come from a wheel encoder and gyroscope of the wheeled robot but it will not have any visual context to be able to provide any human-readable maps.
% In contrast, in \name-SLAM's design, we utilize a dual graph approach, wherein we utilize existing VIO/LIO SLAM systems without their loop closure detection and corrections enabled.
% So, while these VIO/LIO systems can correct for local drifts in the wheel encoders or the IMUs, they cannot perform global corrections.
% These locally corrected robots 3-DoF poses are used to provide the Odometry measurements for the WiFi-graph that we have built in ~\cref{sec:design-graph1}.

% The advantage with turning off the loop closure detection and corrections though is that the rate of memory of consumption and compute required is minimized.
% Thus, the `VIO/LIO graph` can map the environment while providing locally corrected odometry measurements to the `WiFi-graph`.
% The WiFi-graph thus then performs global corrections without the need of loop-closure detection thus enabling \name-SLAM to be an accurate, real-time robot navigation system that can minimizing the rate of memory consumption and the amount of compute.

\subsection{Building and Optimizing the WiFi-Graph}\label{sec:design-graph1}

With these WiFi-bearing measurements, the first idea would be to integrate them within the factor graph of an available Visual Factor graph~\cite{rosinol2021kimera}. Unfortunately, discovery and addition of new AP's and global drift corrections made to the graph introduce brief periods of instability (order of few seconds) to the robot's trajectory estimations. These instabilities can introduce large computation overheads as it may demand corrections to the tracked visual landmarks as well. To isolate these periods of instability, we propose a dual graph approach, where the drift-corrected poses from the WiFi graph can be utilized for globally consistent mapping. But unlike prior work~\cite{arun2022p2slam, ferris2007wifi}, we do not use end-end optimization and instead opt to use the incremental smoothing and mapping (iSAM)~\cite{gtsam} to provide real-time pose estimates, which demands a more accurate and realtime bearing estimation as described in Sec.~\ref{sec:design-bearing}. 

At a high level, the state space at time $t$, $S_t$, is a set of robot poses and access point locations over $t$ time steps in our graph, $S_t = \{\Vec{p}_i \; \forall i \in [1, t]\} \cup \{\Vec{x}_j \; \forall j \in [1, N]\}$, with the robot pose, $\Vec{p}_i \in SE(3)$ and the $N$ access points positions observed till time $t$, $x_i \in \mathbb{R}^3$. 
We can the define odometry measurements (from VIO/LIO or wheel encoders, as shown in Fig~\ref{fig:wifi-factor}) between poses $\Vec{p}_i$ and $\Vec{p}_{i+1}$ at two consecutive time steps as:
\begin{align*}
    \hat{z}^{odom}(\Vec{p}_i, \Vec{p}_{i+1}) = \begin{bmatrix} 
                    R(p^q_i)^{-1} (p^t_{i+1} - p^t_{i})^T\\
                    (p^q_{i+1} \ominus p^q_i)_{[1:3]}
                \end{bmatrix} \nonumber 
\end{align*}
where, $R(\cdot) \in SO(3)$ is the rotation matrix corresponding to the given quaternion, $\ominus$ is the relative difference between two quaternions, and $[1:3]$ chooses only the first three elements of the quaternion.
Similarly, the bearing factors AP $j$ at robot position $x_i$ is $\hat{z}^{bot}_{ij}(p_i, x_j) \in \mathbb{R}^2$:
\begin{align}\label{eq:ping-pred}
    &\hat{z}^{bearing}_{ij}(p_i, x_j) = \mathrm{Local}(\mathrm{TransformTo}(x_j, p_i), p_i) \\
                                &= \mathrm{Local}([\cos(\phi)\cos(\theta), \cos(\phi)\sin(\theta), \sin(\phi)]^T, p_i) \nonumber
\end{align}
where, \textit{TransformTo}$(\cdot)$ transforms the coordinates of the AP $x_j$ to the coordinate system provided by the robot at $p_i$, in which the AP subtends an elevation angle of $\phi$ and an azimuth angle of $\theta$. \textit{Local}$(\cdot)$ projects this bearing measurement to the tangent plane defined by the current pose of the robot, $p_i$. 


So, once we have defined the measurement models we can estimate the optimized robot poses $S^{opt}_t$ for time instance $t$ by minimizing the total error between our predictions and actual measurements,
\begin{align}\label{eq:graph-optim-head}
    S^{opt}_t = \argmin_{S_t} & \sum_{i \leq t} \sum_{j \leq N}  \rho\left(\big(e^{bearing}_{ij}\big)^T \Sigma_\mathrm{bearing}^{-1} e^{bearing}_{ij};c\right) \nonumber\\
         & + \sum_{i\in I_{sub}}  \big(e^{odom}_i\big)^T \Sigma_\mathrm{odom}^{-1} e^{odom}_i
\end{align}
where $e^{bearing}_{ij} = z^{bearing}_{ij} - \hat{z}^{bearing}(p_i, x_j)$ is the bearing factor's error between robot and AP poses $i$ and $j$, $e_i^{odom}(p_i, p_{i+1}) = z_i^{odom} - \hat{z}_i^{odom}(p_i, p_{i+1})$ is the odom factor's error, $\rho$ is the Huber cost function with parameter $c$~\cite{zhang1997parameter}. $\Sigma_\mathrm{odom} \in \mathbb{R}^{6 \times 6}$ and $\Sigma_\mathrm{bearing} \in \mathbb{R}^{2 \times 2}$ are diagonal covariance matrices for odometry and bearing measurements respectively. Further note that the bearing measured in Sec.~\ref{sec:design-bearing} measured $\theta$, the azimuth angle in the robot's local frame and we assume that the elevation, $\phi$, of the incoming signal is $0$, hence $z_{ij} = [\cos(\theta) \sin(\theta)]$. We can assume the elevation angle is $0$ despite AP's placed at differing heights as it doesn't affect the azimuth bearing estimation~\cite{arun2022p2slam}. 


\subsection{Initialization of Factors}\label{sec:design-init}
Next, we initialize each of the $t$ robot positions and $N$ AP positions for the optimizer. 
Similar to prioir works~\cite{arun2022p2slam}, the robot positions are initialized using the relative odometry measurements. These poses have accumulated drift over time which we seek to correct.
A naive initialization for the AP's would be to place them at the origin and allow the optimizer to place them appropriately in the environment. Unfortunately, the iSAM optimizer, given the limited number of measurements it has seen up until time $t$, can fail to converge with this naive initialization. 
% Unfortunately, we cannot do so for the AP locations, which we need to identify as well, as they have no priors attached to them whatsoever.
% While one could naively initialize all known APs in the environment at the origin, some APs may not be receiving any signals at all as they are actually very far from the robot's origin, thus might be too far away when the optimizer is started.

% Since these faraway APs have no measurements attached to them, the cost associated with them is ill-defined and the optimization problem is unsolvable.
% Furthermore, APs which have been discovered may not have enough bearing measurements to strongly constrain their locations. This makes the optimization unstable, and the SLAM algorithm can converge to a very poor estimate of the AP location. Thus, we need to initialize the APs in a smart fashion, considering many good bearing measurements, in order to jointly constrain the AP and robot locations.

To solve for this in-determinancy due to poor initialization of the AP's position estimate, we draw from the intuition of WiFi signal propagation characteristics.
WiFi's received signal signal strength indicator (RSSI), has been study extensively in the past for localization.
While RSSI measurements are unreliable to perform accurate localization, they can still provide a general sense of proximity.
Thus, we can identify the robot's pose $p_{ap-j}$ at which the $j^{th}$ AP's RSSI measurements have a local RSSI maximum among all current robot's poses $p_i \forall i \in [1,t]$, with the intuition that this is where the robot passed closest to the AP.
We can then initialize the $j^{th}$ AP's pose $x_j$ as $x_j = p^t_{ap-j} + \Delta$, where $\Delta \in \mathbb{R}^3$ is a small ($\leq 0.1 m$) random perturbation. This random perturbation is added to avoid in-determinancy with the optimizer. Finally, with the real-time, compute-efficient WiFi-bearing in hand, along with a reliable way to integrate these measurements with local odometry measurements, we can proceed with the graph optimization iteratively with each time-step. In the following section we will provide specific implementation details and robustly test \name over a variety of environments. 


% Once all known APs in the environment are detected and initialized in this fashion, the factor graph optimization system is no more indeterminate or ill-defined, and the location of the robot and the APs can be jointly optimized for.
% Given good input bearing measurements, all the challenges for \name's WiFi graph optimization are met, and we can now provide accurate and real-time global pose estimates for the camera graph to consume.



==> evaluation/eval1.tex <==
% !TEX root = root.tex
\section{Results}\label{sec:eval}

Description of the environment. Ground truth data, how it is collected. How is it different from the cartogrpaher real-time and refer to DLoc as one of the examples that also show the same.

Then we show LiDAR and camera baselines with their real-time performances using Cartographer real-time and RTABMap real-time.

\subsection{Pose Estaimtion Accuracy}
We show CDF's of localization accuracy and orientaion accuracy for all of the baselines with \name.

We then show timeseries comparison with cartogrpaher, rtabmpa with \name alone for a couple of environments. highlighting how \name is close to camer and liddar alone.

\subsection{Compute, Latency and Memory}

Accuracy, compute required, latency required, memory required comparison table for all the three.

\subsection{Ablation}

\noindent\textbf{SVD-FFT vs FFT}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/svd_cdf_1.png}
    \caption{(a) Shows the various measurements that are made across various robot poses and AP poses. (b) Shows the details of how these measurements are laid as factors in the implementation of the WiFi Factor graph}
    \label{fig:wifi-factor}
\end{figure}
Individual CSI measurements are vulnerable to noise and transient multipath in the environment. As described above, we extract the underlying signal parameters from multiple CSI measurements across different transmitter antennas using Principle Component Analysis. We evaluate these new smoothed CSI measurement's performance with 2D-FFT.

\noindent\textbf{Square Vs ULA}

\section{Showcase: Autonomous Navigation}\label{sec:showcase}
Using fiduciary markers for labelling various locations in the map. These labels are then used to send commands for the robot to go around from point to point using \name's SLAM implementation.

==> evaluation/eval2.tex <==
% !TEX root = root.tex
\section{Results}\label{sec:eval}

To evaluate \name implemented as mentioned in ~\cref{sec:implementation} we deployed \name's algorithms in one of the environments of the OpenSourced Datasest~\cite{arun2022p2slam} (which will be referred as Env-1). However $\mathrm{P^2}$SLAM dataset uses uniform linear arrays and assume the knowledge of the half-plane the AoA is measured.
Thus to overcome these limitations of their datasets, we collect one more Dataset in a $25m\times40m$ space (which we will be referred Env-2) with the square array we propose in \name's design that removes the half-plane ambiguities.
Additionally, the authors in $\mathrm{P^2}$SLAM use both AoA and AoD measurements of the robot, while in \name we only utilize only AoA and extract only those measurements from the dataset.

Additionally, we benchmark \name's results with two state-of-the-art SLAM systems: RTABMap~\cite{Labb2018RTABMapAA}, a RGB-D camera based SLAM algorithm and Cartographer~\cite{cartographer}, a LiDAR based SLAM algorithm. 
Here we would like to note that while a typical RGB-D and LIDAR sensors have a more denser feature map compared to a monocular camera we use in \name's implementation, the key-features/landmarks that are used for correlation matching are of the same order across monocular, RGB-D and LiDAR sensors.
We test \name's claims of compute and memory efficiency along with \name's SLAM performance.

\subsection{Evaluation Metrics}\label{sec:eval-metrics}

To measure the compute and memory usage we use the widely used open toolbox~\cite{toolbox} which reports \todo{whatever that is.}

\noindent\textbf{Memory Usage:} We use the memory (RAM in MB) usage of the SLAM algorithm as time progresses as the metric to compare \name against state of the art. Where we observe that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.

\noindent\textbf{Compute Usage:} We use the compute memory (MB) usage of the SLAM algorithm as time progresses as the metric to compare \name against state of the art. Where we observe that \name-SLAM reduces the average compute memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.

\noindent\textbf{Pose Estimation:} Since the system reports 4D pose ($(x,y,z,\theta)$) of the robot, which we compare with post-processing optimized cartographer poses as ground truth, as they have shown to have decent performance for indoor robots~\cite{diebel2006representing}. So, we use CDF of RMSE for $(x,y,z)$ and show a median tracking errors of \todo{xx}cm and L1 norm error for $(\theta)$, and a median robots orientation error of \todo{yy$^\circ$} on par with state of the art.

\noindent\textbf{Mapping Accuracy:} Finally, in the dataset we have collected we deploy \todo{xx} camera fiduciaries~\cite{fiducialtechused} across the environment, which are tracked and mapped in the environment by the camera graph.
Thus, the RMSE of the mapped locations of these fiduciaries help us to quantify the accuracy of \name's mapping capabilities.
Where we show that \name's is able to accurately map the environment with a median error of \todo{xx}cm.

\begin{figure*}[ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \caption{Robot Pose errors: (a) Shows the position estimation error of \name and RTABMap in Env-1 and Env-2. (b) Shows the orientation estimation error of \name and RTABMap in Env-1 and Env-2. (c,d) Show the time series tracking error of \name and cartographer and RTABMap in Env-1(c) and Env-2(d). (e,f) Show the time series orientation errors of \name and RTABMap in Env-1(e) and Env-2(f). and (g,h) Shows the top down view of the trajectory of \name compared with cartographer ground truth in Env-1(g) and Env-2(h).}
    \label{fig:tracking-errors}
\end{figure*}

\subsection{Compute and Memory Requirements}\label{sec:eval-compute}

\noindent\textbf{Memory \& Compute usage:}One of the most important contributions of \name's SLAM design is to achieve memory and compute efficient SLAM system without compromise the SLAM tasks. 
Thus we first evaluate the memory and compute usage of \name's overall system when deployed in both Env-1 and Env-2 and compare with two state-of-the-art SLAM systems RTABMap (that uses a RGB-D camera) and Cartographer (that uses a LiDAR).
We plot these memory usage in Figure~\ref{fig:memory-compute}{a} and compute usage in Figure~\ref{fig:memory-compute}{b} over time for each incoming sensor frame for all the three algorithms.
From these plots we can clearly see that \name's SLAM implementation on an average uses only \todo{$xx$} MB of compute memory which is \todo{$x\times$} (\todo{y$\times$}) lower than RTABMap (Cartographer). Additionally we can see that \name uses only \todo{$xx$} MB of memory (RAM) which is \todo{$x\times$} (\todo{y$\times$}) lower than RTABMap (Cartographer), thus demonstrating that \name is both memory and compute efficient by \todo{x$\times$} compared to the state-of-the-art camera and LiDAR based SLAM systems.

\noindent\textbf{Real-time performance of \name:} Additionally, we can also note from both Figure~\ref{fig:memory-compute}{a,b} that while \name's SLAM provides optimized poses and map in real-time and thus the plot ends at \todo{xx}secs when the data collection ends. On the other hand, RTABMap and Cartographer both take \todo{yyy}secs and \todo{zz}secs more to generate a better optimized paths and maps.
This further shows the deployability and scalability of \name due to its real-time performance compared to the existing SLAM systems that take additional time to perform end-to-end bundle adjustments~\cite{semenova2022quantitative} to get more accurate poses and maps.

\noindent\textbf{Ablation for \name's Memory \& Compute usage:} \\
\noindent We further analyze and look into the memory and compute usage of the individual components of \name, that is the individual WiFi and camera grapsh that are running in parallel.
We can see \todo{cool observation here}.

We also, note that for all the time-series plots shown in Figures~\ref{fig:memory-compute} have a series of vertical solid lines which show the AP initialization event happening for each of the individual AP's in the environment as per our smart initialization algorithm discussed in ~\cref{sec:design-graph1}.
We can see that the spikes in the WiFi graph for memory and compute occur at these instances noting that the measurements associated to the specific are laid down at this instant, but even these spikes are much lower than the overall compute and memory requirements of RTABMap and Cartogrpaher.

\begin{figure}[t]
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Map generated by \name for Env-1, (b) Map generated by \name for Env-2, also has the ground truh fiduciaries in blue circles and the predicted locations in red crosses}
    \label{fig:mapping}
\end{figure}

\subsection{Tracking Accuracy}\label{sec:eval-tracking}

\begin{figure*}[ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/svd_cdf_1.png}
        \subcaption{}
    \end{minipage}
    \caption{(a) Real-time tracking errors for \name, cartographer and RTABMap in Env-1, and (b) Real-time tracking errors for \name, cartographer and RTABMap in Env-2 .(c) Tracking errors for pose estimates provided from the WiFi-layer Poses Vs Visual layer for \name's implementation. (d) Shows the comparison of AoA accuracies for FFT Vs SVD-FFT}
    \label{fig:microbencmarks}
\end{figure*}

Now that we have demonstrated memory and compute efficiency of \name, we demonstrate that we achieve these low-compute and low-memory requirements while achieving state-of-the-art accuracies for robot pose estimation first, we will then demonstrate mapping accuracy of \name in ~\cref{sec:eval-mapping}. 

As stated earlier, we benchmark our results with end-to-edn cartographer processed poses as ground truth, against which we compare both \name and RTABMap to show tracking in Figure~\ref{fig:tracking-errors}{a} and orientation errors in Figure~\ref{fig:tracking-errors}{b} across both Env-1 and Env-2.
We can see that name achieves a median tracking error of $xx$cm and a median orientation error of $x^{\circ}$ which is on par with the median tracking error, $xx$cm and orientation error,$x^{\circ}$ of RTABMap. Thus showing that the pose estimation of \name is on par with the state-of-the-art Visual SLAM systems.

Additionally, we also provide the time-series plots of tracking errors across Env-1 and Env-2 in Figures~\ref{fig:tracking-errors}{c,d} and orientation errors in in Figures~\ref{fig:tracking-errors}{e,f} for both \name and RTABMap  showing that \todo{important thing you noticed here, showing that you are on par and providing with a reason why you might be falling short if you are.}

Finally, we also plot the \name's estimated path against the Cartographer's ground truth for both the environments in Figure~\ref{fig:tracking-errors}{g,h} to qualitatively show \name's accurate pose estimation across time.

\subsection{Mapping Accuracy}\label{sec:eval-mapping}

Finally, we evaluate \name's ability to amp features in the environment accurately. While, most of the works only give a qualitative map~\cite{Labb2018RTABMapAA,rosinol2021kimera,mur2015orb,qin2018vins} which also we present in Figure~\ref{fig:mapping}{a,b} for both Env-1 and ENv-2 respectively.
We additionally, place camera fiduciaries in Env-2 dataset that we have collected to measure if the locations of these fiduciaries are mapped accurately in the environment.
These camera fiduciary ground truth are highlighted in Figure~\ref{fig:mapping}{b} as blue circles and \name's mapped location in red crosses.
We compare these locations to provide the mapping errors, which we find has a mean mapping error of ~\todo{xx}cm.
% \todo{the median mapping error for all the fiduciaries is mentioned in text here for Env-2 as Env-2 does not fiduciaries.}



\subsection{Micro-benchmarks}

We have seen that \name demonstrates compute and memory efficient SLAM when deployed in real-world scenarios as seen in the results above. We now present few micro-benchmarks of \name's design to further demonstrate \name's robustness.

\noindent\textbf{Real-time Vs Bundle Adjustment Tracking errors:}\\
Firstly, as we have seen from ~\cref{sec:eval-compute} that while \name performs real-time optimizations, RTABMap and Cartographer post data collection bundle adjustments seen from the more time taken in Figures~\ref{fig:memory-compute}, so in order to perform a fair comparison with \name we look at the real-time poses that are reported when the robot is actually at that location without the pose correction optimizing the past locations and show the time series errors of these pose estimates in Figure~\ref{fig:microbencmarks}{a,b} for tracking and orientation errors respectively.
We can clearly observe from these time-series errors that compared to RTABMap and cartographer \name provide much better instantaneous pose estimates that are at least \todo{$x\times$} less erroneous.

\noindent\textbf{Time taken for each optimization stage on an average:}\\
Secondly, to understand the real-time performance of \name and the existing SLAM systems, we measure the total time taken for each algorithm and divide them by the total sensor frames.
This provides for the average latency for each pose estimation of the algorithms, and we find that while \name achieves real-time performance with a latency of \todo{xx}msec for a frame rate of $xx$fps, RTABMap and cartographer fall behind with \todo{xx}msec (for \todo{y}fps) and \todo{xx}msec (for \todo{y}fps) respectively.

\noindent\textbf{Justifying \name's Dual Layered Approach:}\\
Furthermore, while we have shown the pose estimation results of \name's WiFi graph, the camera graph also performs local pose corrections to these pose estimates while mapping the features in the environment.
So as to develop an insight towards the poses to use, we show the tracking errors for robot locations estimated using \name's WiFi graph and camera graph in Figure~\ref{fig:microbencmarks}{c} from where we can see that owing to its global perspective the WiFi graph provides with much more accurate location estimates than the Camera graph.
This further supports \name's dual graph idea where our intuition stems from the fact that WiFi-SLAM is best for pose estimation and camera-SLAM for mapping the environment.

\noindent\textbf{SVD-FFT vs FFT:}\\
Individual CSI measurements are vulnerable to noise and transient multipath in the environment. As described above, we extract the underlying signal parameters from multiple CSI measurements across different transmitter antennas using Singular Value Decomposition. We evaluate these new SVD CSI measurement's performance with 2D-FFT and show their AoA estimation accuracies as shown in Figure~\ref{fig:microbencmarks}{d}, where we can see that SVD-FFT based AoA estimates reduce the 90$^{th}$ percentile error from \todo{$xx^{\circ}$} to \todo{$yy^{\circ}$}.
We specifically note the 90$^{th}$ percentile errors as these are the corner cases where multipath and NLOS based errors are more prevalent. 
Thus demonstrating the performance improvement from \name's SVD-FFT implementation.
% \todo{table is optional}
% \begin{table}[ht]
%     \centering
%         \begin{tabular}{|l|l|l|l|}
%         \hline
%                      & Overall & Pose Estimation & Mapping   \\\hline \hline
%         ViWiD        &         &                 &           \\\hline
%         RTABMap      &         &                 &         \\\hline
%         Cartographer &         &                 &         \\ \hline
%         \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}



==> evaluation/eval3.tex <==
% !TEX root = root.tex
\section{Results}

\begin{figure*}[ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-rtab-memory.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-rtab-cpu.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-abl-mem.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-abl-cpu.pdf}
        \subcaption{}
    \end{minipage}
    \caption{Memory and Compute: (a) Shows the memory usage (in MB) of \name compared with RTABMap (b) Shows the compute usage (in\% of a single core) of \name compared with RTABMap (c) Shows the memory usage of \name's WiFi and Camera graph, and (d) Shows the compute usage of \name's camera and WiFi graphs}
    \label{fig:memory-compute}
\end{figure*}

\begin{figure*}[ht]
    \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-all-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-all-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-28-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-4-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-28-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-4-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/rviz-3d-plot.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fiducials-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\name's SLAM performance: (a) Shows the position estimation error of \name and RTABMap in Env-1 and Env-2. (b) Shows the orientation estimation error of \name and RTABMap in Env-1 and Env-2. (c,d) Show the time series tracking error of \name and RTABMap in Env-1(c) and Env-2(d). (e,f) Show the time series orientation errors of \name and RTABMap in Env-1(e) and Env-2(f). and (g) Map generated by \name for Env-2 shown along with 3D features mapped in white, the path in red and the APs mapped in green. (h) Map generated by \name for Env-3, also has the ground truth fiducials in blue circles and the predicted locations in red crosses}
    \label{fig:tracking-errors}
\end{figure*}

To evaluate \name implemented as mentioned in ~\cref{sec:implementation} we deployed \name's algorithms over three datasets. We have scenarios covering two different paths driven in a $25 \times 30$ m and a third dataset in which mapping performace of \name is evaluated. Over the three datasets, the robot is driven a cumulative distance of over $1000$ m.
We also note that the authors in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} use AoA measurements at both the bot and the access points, while in \name we only utilize only AoA and extract only those measurements from the dataset.

Additionally, we benchmark \name's results with a state-of-the-art SLAM algorithm, RTABMap~\cite{Labb2018RTABMapAA}, a RGB-D camera based SLAM algorithm.
Additionally, we use the expensive and compute heavy LiDAR based SLAM algorithm, Cartographer~\cite{cartographer}, to compare against for ground truth pose and mapping estaimtes. 
Here we would like to note that while a typical RGB-D and LIDAR sensors have a more denser feature map compared to a monocular camera we use in \name's implementation, the key-features/landmarks that are used for correlation matching are of the same order across monocular, RGB-D and LiDAR sensors.
We test \name's claims of compute and memory efficiency along with \name's SLAM performance.

\subsection{Evaluation Metrics}\label{sec:eval-metrics}

To measure the compute and memory usage we use the widely used open toolbox\footnote{\url{https://github.com/alspitz/cpu_monitor}} which reports the memory used in MB by each individual node running and the compute in percentage of utilization per unit core, so for an 8-core machine, the compute usage can go from 0-800\%.

\noindent\textbf{Memory Usage:} We use the memory (RAM in MB) usage of the SLAM algorithm as time progresses as the metric to compare \name against state of the art. Where we observe that \name-SLAM reduces the average memory utilization to $300$MB which is $3\times$ the Visual SLAM.

\noindent\textbf{Compute Usage:} We use the percentage of a single core used by the SLAM algorithm as time progresses as the metric to compare \name against state of the art. 
That is for an 8-core machine, the compute usage can range from 0\%-800\%
Where we observe that \name-SLAM reduces the average compute memory utilization to $20$\% which is $5\times$ the Visual SLAM.

\noindent\textbf{Pose Estimation:} Since the system reports 4D pose ($(x,y,z,\theta)$) of the robot, which we compare with post-processing optimized cartographer poses as ground truth, as they have shown to have decent performance for indoor robots~\cite{diebel2006representing}. So, we use CDF of RMSE for $(x,y,z)$ and show a median tracking errors of 50cm and L1 norm error for $(\theta)$, and a median robots orientation error of 2$^\circ$ on par with state of the art.

\noindent\textbf{Mapping Accuracy:} Finally, to evaluate mapping performance, we wanted to deploy fiducial markers and get the accuracy by comparing their mapped poses to the ground truth poses. Thus
to evaluate the mapping performance we collect one more Dataset in a $25m\times40m$ space (which we will refer as Env-3). In this dataset we have collected  ArUCo camera fiducials~\cite{garrido2014automatic} across the environment, which are tracked using the OpenCV toolbox available~\cite{opencvaruco} and mapped in the environment by the camera graph.
Thus, the RMSE of the mapped locations of these fiducials help us to quantify the accuracy of \name's mapping capabilities.
Where we show that \name's is able to accurately map the environment with a median error of 105cm.

\subsection{Compute and Memory Requirements}\label{sec:eval-compute}

\noindent\textbf{Memory \& Compute usage:} One of the most important contributions of \name's SLAM design is to achieve memory and compute efficient SLAM system without compromise the SLAM tasks. 
Thus we first evaluate the memory and compute usage of \name's overall system when deployed in both Env-1 and Env-2 and compare with a state-of-the-art SLAM system, RTABMap (that uses a RGB-D camera).
We plot these memory usage in Figure~\ref{fig:memory-compute}{a} and compute usage in Figure~\ref{fig:memory-compute}{b} over time for each incoming sensor frame for bot the algorithms.
From these plots we can clearly see that \name's SLAM implementation on an average uses only $300$ MB of memory which is $3\times$ lower than RTABMap. Additionally we can see that \name uses only $20$\% of compute which is $5\times$ lower than RTABMap, thus demonstrating that \name is both memory and compute efficient by 4$\times$ compared to the state-of-the-art camera SLAM systems.

% \noindent\textbf{Real-time performance of \name:} Additionally, we can also note from both Figure~\ref{fig:memory-compute}{a,b} that while \name's SLAM provides optimized poses and map in real-time and thus the plot ends at \todo{xx}secs when the data collection ends. On the other hand, RTABMap and Cartographer both take \todo{yyy}secs and \todo{zz}secs more to generate a better optimized paths and maps.
% This further shows the deployability and scalability of \name due to its real-time performance compared to the existing SLAM systems that take additional time to perform end-to-end bundle adjustments~\cite{semenova2022quantitative} to get more accurate poses and maps.

\noindent\textbf{Ablation for \name's Memory \& Compute usage:} \\
\noindent We further analyze and look into the memory and compute usage of the individual components of \name, that is the individual WiFi and camera graph that are running in parallel.
We can see most of the  memory and compute usage for \name's algorithm are due to the camera features that are tracked and the \name WiFi layer needs very little compute.

We also, note that for all the time-series plots shown in Figures~\ref{fig:memory-compute} have a series of vertical solid lines which show the AP initialization event happening for each of the individual AP's in the environment as per our smart initialization algorithm discussed in ~\cref{sec:design-graph1}.
We can see that the spikes in the WiFi graph for memory and compute occur at these instances noting that the measurements associated to the specific are laid down at this instant, but even these spikes are much lower than the overall compute and memory requirements of RTABMap.

\begin{figure*}[t]
    \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-top-down-8-28-crop.pdf}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/rtab-top-down-8-28-crop.pdf}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-top-down-8-4-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Shows the top down view of the trajectory of \name compared with cartographer ground truth in Env-1, (b) Shows the top down view of the trajectory of RTABMap compared with cartographer ground truth in Env-1 and (c)hows the top down view of the trajectory of \name compared with cartographer ground truth in Env-2 }
    \label{fig:mapping}
\end{figure*}

\subsection{Tracking Accuracy}\label{sec:eval-tracking}

\begin{figure}[ht]
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-wifi-cam_trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/fft-pca-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Tracking errors for pose estimates provided from the WiFi-layer Poses Vs Visual layer for \name's implementation. (b) Shows the comparison of AoA accuracies for FFT Vs SVD-FFT}
    \label{fig:microbencmarks}
\end{figure}

Now that we have demonstrated memory and compute efficiency of \name, we demonstrate that we achieve these low-compute and low-memory requirements while achieving state-of-the-art accuracies for robot pose estimation first, we will then demonstrate mapping accuracy of \name in ~\cref{sec:eval-mapping}. 

As stated earlier, we benchmark our results with end-to-edn cartographer processed poses as ground truth, against which we compare both \name and RTABMap to show tracking in Figure~\ref{fig:tracking-errors}{a} and orientation errors in Figure~\ref{fig:tracking-errors}{b} across both Env-1 and Env-2.
We can see that name achieves a median tracking error of $50$cm for both Env-1 and Env-2 and a median orientation error of $1^{\circ}$ and $2.8^{\circ}$ for both env-1 and env-2. These are on par with the median tracking errors of $60$cm and $38$cm and median orientation errors, $5^{\circ}$ and $3^{\circ}$ across Env-1 and Env-2 for RTABMap. Thus showing that the pose estimation of \name is on par with the state-of-the-art Visual SLAM systems.

Additionally, we also provide the time-series plots of tracking errors across Env-1 and Env-2 in Figures~\ref{fig:tracking-errors}{c,d} and orientation errors in in Figures~\ref{fig:tracking-errors}{e,f} for both \name and RTABMap  showing that \name performs on par in terms of pose estimations with the RTABMap. We can also see that the high errors in \name are only in the initial stages where it is searching for the APs in the environment and it stabilizes for later stages, showing the robustness of our system. On the other hand, loop-closure dependant SLAM algorithms need a location to be revisted to avoid any drifts.

Finally, we also plot the \name's estimated path against the Cartographer's ground truth for both the environments in Figure~\ref{fig:tracking-errors}{g,h} to qualitatively show \name's accurate pose estimation across time.

\subsection{Mapping Accuracy}\label{sec:eval-mapping}

Finally, we evaluate \name's ability to amp features in the environment accurately. While, most of the works only give a qualitative map~\cite{Labb2018RTABMapAA,rosinol2021kimera,mur2015orb,qin2018vins} which also we present in Figure~\ref{fig:tracking-errors}{g,h} for both Env-1 and Env-3 respectively.
We additionally, place camera fiducials in Env-3 dataset that we have collected to measure if the locations of these fiducials are mapped accurately in the environment.
These camera fiducial ground truth are highlighted in Figure~\ref{fig:tracking-errors}{h} as blue circles and \name's mapped location in red crosses.
We compare these locations to provide the mapping errors, which we find has a mean mapping error of 103cm.


\subsection{Micro-benchmarks}

We have seen that \name demonstrates compute and memory efficient SLAM when deployed in real-world scenarios as seen in the results above. We now present few micro-benchmarks of \name's design to further demonstrate \name's robustness.

% \noindent\textbf{Real-time Vs Bundle Adjustment Tracking errors:}\\
% Firstly, as we have seen from ~\cref{sec:eval-compute} that while \name performs real-time optimizations, RTABMap and Cartographer post data collection bundle adjustments seen from the more time taken in Figures~\ref{fig:memory-compute}, so in order to perform a fair comparison with \name we look at the real-time poses that are reported when the robot is actually at that location without the pose correction optimizing the past locations and show the time series errors of these pose estimates in Figure~\ref{fig:microbencmarks}{a,b} for tracking and orientation errors respectively.
% We can clearly observe from these time-series errors that compared to RTABMap and cartographer \name provide much better instantaneous pose estimates that are at least \todo{$x\times$} less erroneous.

% \noindent\textbf{Time taken for each optimization stage on an average:}\\
% Firstly, to understand the real-time performance of \name and the existing SLAM systems, we measure the total time taken for each algorithm and divide them by the total sensor frames.
% This provides for the average latency for each pose estimation of the algorithms, and we find that while \name achieves real-time performance with a latency of \todo{xx}msec for a frame rate of $xx$fps, RTABMap and cartographer fall behind with \todo{xx}msec (for \todo{y}fps) and \todo{xx}msec (for \todo{y}fps) respectively.

\noindent\textbf{Justifying \name's Dual Layered Approach:}\\
Firstly, while we have shown the pose estimation results of \name's WiFi graph, the camera graph also performs local pose corrections to these pose estimates while mapping the features in the environment.
So as to develop an insight towards the poses to use, we show the tracking errors for robot locations estimated using \name's WiFi graph and camera graph in Figure~\ref{fig:microbencmarks}{c} from where we can see that owing to its global perspective the WiFi graph provides with much more accurate location estimates than the Camera graph.
This further supports \name's dual graph idea where our intuition stems from the fact that WiFi-SLAM is best for pose estimation and camera-SLAM for mapping the environment.

\noindent\textbf{PC-FFT vs FFT:}\\
Additionally, the individual CSI measurements are vulnerable to noise and transient multipath in the environment. As described above, we extract the underlying signal parameters from multiple CSI measurements across different transmitter antennas using Singular Value Decomposition, to identify the principle component of CSI. We evaluate these new SVD CSI measurement's performance with 2D-FFT and show their AoA estimation accuracies as shown in Figure~\ref{fig:microbencmarks}{d}, where we can see that SVD-FFT based AoA estimates reduce the 90$^{th}$ percentile error from $40^{\circ}$ to $25^{\circ}$.
We specifically note the 90$^{th}$ percentile errors as these are the corner cases where multipath based errors are more prevalent. 
Thus demonstrating the performance improvement from \name's PC-FFT implementation.


==> evaluation/eval4.tex <==
% !TEX root = root.tex
\section{Microbenchmarks}~\label{sec:eval-micro}

\subsection{VIO memory vs accuracy}
In this section we describe the details of Kimera~\cite{rosinol2021kimera}, a VIO SLAM system that we utilize as a benchmark comparison.
We also use Kimera as the first-graph 
-- William as of 7/26

\begin{itemize}
    \item Median translation error vs memory and median orientation error vs memory -- \textbf{with and without LCD}
    \item Loop Closure detection frequency vs memory rate 
    \item set a tolerable limit and use that memory requirement and accuracy requirement as a baseline
\end{itemize}

\subsection{Wheel Odom vs VIO without LCD Odom}

Comparison of just the wheel odometery and VIO without LCD odometry to ensure that we are using comparable systems

\subsection{FFT, PC-FFT, MUSIC}
\begin{itemize}
    \item accuracy
    \item compute
\end{itemize}

\begin{figure*}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem-interframetime.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/placeholder.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation_no_lc.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/aoa_err.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\textbf{Microbenchmarks}: \textbf{(a) Kimera:} Shows the trade-off between memory consumption(red) and the accuracy(blue) for various interframe rates. \textbf{(b) Cartographer:} Shows the trade-off between compute required(red) and the accuracy(blue) for various scan-matching thresholds. \textbf{(c) Odometry-Graph:} Shows the comparison on how various odometry inputs to the WiFi graph look before optimization.\textbf{(d) Bearing Measurement Algorithms:} Comparison between 2D-FFT from $\mathrm{P^2}$SLAM, MUSIC and our proposed PC-FFT}
    \label{fig:micro}
    \vspace{-0.1in}
\end{figure*}

\section{Results}\label{sec:eval}

\begin{figure*}
    \begin{minipage}{0.20\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/top-down-kimera.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.20\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/top-down-viofi.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_translation.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_orientation.pdf}    
        \subcaption{}
    \end{minipage}
    
    \caption{\textbf{End-to-end evaluation}: \textbf{(a)} Trajectory estimated by Kimera with loop closures (Orange) and ground truth (dashed-Blue). \textbf{(b)} Trajectory estimated by \name using odometry predictions from Kimera without loop closures (Orange, \textit{WiFi + Kimera w/o LC}) and ground truth (dashed-Blue). \textbf{(c, d)} Time series of translation and orientation error comparing Kimera with loop closure (dashed-Orange) against \name's predictions. \name uses odomtery from Kimera without loop closures (Blue) and just wheel odometry (dashed-Yellow).}
    \label{fig:end-end1}
    \vspace{-0.1in}
\end{figure*}

\begin{figure}[t]
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_orientation.pdf}
    \end{minipage}
    \caption{\textbf{Error analysis:} }
    \label{fig:end-end2}
\end{figure}


\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.42\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem_cpu_w_aoa_ts.pdf}
    \end{minipage}
    \caption{Notes: memory avg slope, Kimera -- 0.56, \name -- 0.2 MB/s}
    \label{fig:mem-cpu}
\end{figure}

To evaluate \name implemented as mentioned in ~\cref{sec:implementation} we deployed \name's algorithms over four datasets. The one presented in the following section was collected in a $25 \times 20$ m environment, with a total distance of $403$ m traversed over a duration of $23$ minutes. The subsequent 3 datasets are the P2SLAM datasets~\cite{arun2022p2slam}. Through these datasets, we have robustly tested \name across 3 distinct environments, 4 different access point placements, and traversed a cumulative distance of $1625$ m with a total travel time of 108 minutes. We also note that the authors in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} use AoA measurements at both the robot and the access points, while in \name we only utilize the AoA at the robot and extract the channels for only those measurements from the dataset.

Additionally, we benchmark \name's results with a state-of-the-art SLAM algorithm, Kimera~\cite{kim2019control}, a stereo-camera based SLAM algorithm. We run Kimera on our dataset with and without loop closures, labelled in the legends as `w/ LC' and `w/o LC' respectively. Additionally, for all the 4 datasets, we run cartographer in real time, with the `global SLAM' and LiDAR scan matching turned off to remove turn off loop closure. This is referred to as `Cartographer w/o LC'. Next, we carefully tune the loop closure parameters to obtain the best quality of loop closures (referred as `Cartographer w/ LC') in real time and benchmark \name against it. To obtain ground truth, we observe that due to compute constraints Cartographer in unable to incorporate all the LiDAR scans in real time, but allowing it to run past the time of data collection allows it to optimize over all the LiDAR scans to provide a near-groundtruth trajectory. The performance of this trajectory was further characterized in DLoc~\cite{ayyalasomayajula2020deep}. 

In the following sections, using the Cartographer ground truth generated, we benchmark \name against Kimera and Cartographer (when run in real-time) and provide results for the translation and orientation errors. We further measure the CPU and memory usage across these SLAM frameworks\footnote{\url{https://github.com/alspitz/cpu_monitor}} and compare the total memory used, the rate of memory increase and the CPU resources used over the entire run of the datasets. 


\subsection{End-to-end evaluation:}

\begin{itemize}
    \item CDFs of translation and orientation errors for \name, Kimera with LCD, WiFi with wheel Odom (real-time)
    \item time-series for of translation and orientation errors for \name, Kimera with LCD, WiFi with wheel Odom (real-time)
    \item overall memory requirements for \name, Kimera, WiFi with wheel Odom
    \item time-series of memory requirement increase for \name, Kimera, WiFi with wheel Odom \todo{extrapolate the time series till 8GB}
\end{itemize}

\subsection{Memory and Accuracy with Various VIO inputs}

understanding how existing VIOs will effect our algorithm

\begin{table*}[ht]
    \centering
    \footnotesize
    \caption{}
    \begin{tabular}{|l|ccc|ccc|ccc|}
    \hline
    \multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{Cart. w/ LC}} & \multicolumn{3}{c|}{\textbf{\name + Cart. w/o LC}} & \multicolumn{3}{c|}{\textbf{\name + Odom}} \\ \cline{2-10} 
     & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \multicolumn{1}{l|}{\textbf{DS 3}} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}Translation \\ Error (cm)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0 \\ (224)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}134.1 \\ (1097)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}23.3\\ (37.4)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}65.9\\ (92.2)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}67.3\\ (182.6)\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}48.6 \\ (114.4)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0\\ (100.2)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}75.5\\ (204.9)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}66.44\\ (234.7)\end{tabular} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}Orientation \\ Error (deg)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{0.8}\\ (4.66)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}5.3\\ (12.6)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.6\\ (1.4)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2.4\\ (4.66)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{2.8}\\ (12)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}1.4\\ (3.3)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1.7\\ (\textbf{2.7})\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.0\\ (\textbf{6.2})\end{tabular}} & \begin{tabular}[c]{@{}c@{}}2.0 \\ (10.3)\end{tabular} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}Total \\ Memory (MB)\end{tabular}} & \multicolumn{1}{c|}{702} & \multicolumn{1}{c|}{658} & 423 & \multicolumn{1}{c|}{613} & \multicolumn{1}{c|}{706} & 356 & \multicolumn{1}{c|}{288} & \multicolumn{1}{c|}{\textbf{252}} & \textbf{163} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}Rate of \\ memory (MB/s)\end{tabular}} & \multicolumn{1}{c|}{0.29} & \multicolumn{1}{c|}{0.33} & 0.38 & \multicolumn{1}{c|}{0.22} & \multicolumn{1}{c|}{0.33} & 0.26 & \multicolumn{1}{c|}{\textbf{0.10}} & \multicolumn{1}{c|}{\textbf{0.11}} & \textbf{0.14} \\ \hline
    \textbf{\begin{tabular}[c]{@{}l@{}}CPU (fraction \\ of cores)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.2\\ (4.2)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.8\\ (4.2)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}1.85\\ (4.4)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.62\\ (2.1)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.85\\ (2.8)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.77\\ (1.1)\end{tabular} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.2\\ (1.6)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.28 \\ (1.7)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.22 \\ (0.5)\end{tabular}} \\ \hline
    \end{tabular}
\end{table*}


\if 0
\begin{figure*}[ht]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-rtab-memory.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-rtab-cpu.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-abl-mem.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-abl-cpu.pdf}
        \subcaption{}
    \end{minipage}
    \caption{Memory and Compute: (a) Shows the memory usage (in MB) of \name compared with RTABMap (b) Shows the compute usage (in\% of a single core) of \name compared with RTABMap (c) Shows the memory usage of \name's WiFi and Camera graph, and (d) Shows the compute usage of \name's camera and WiFi graphs}
    \label{fig:memory-compute}
\end{figure*}

\begin{figure*}[ht]
    \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-all-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-all-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-28-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-4-trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-28-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-main-ts-8-4-ori.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/rviz-3d-plot.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fiducials-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{\name's SLAM performance: (a) Shows the position estimation error of \name and RTABMap in Env-1 and Env-2. (b) Shows the orientation estimation error of \name and RTABMap in Env-1 and Env-2. (c,d) Show the time series tracking error of \name and RTABMap in Env-1(c) and Env-2(d). (e,f) Show the time series orientation errors of \name and RTABMap in Env-1(e) and Env-2(f). and (g) Map generated by \name for Env-2 shown along with 3D features mapped in white, the path in red and the APs mapped in green. (h) Map generated by \name for Env-3, also has the ground truth fiducials in blue circles and the predicted locations in red crosses}
    \label{fig:tracking-errors}
\end{figure*}

\subsection{Evaluation Metrics}\label{sec:eval-metrics}

To measure the compute and memory usage we use the widely used open toolbox\footnote{\url{https://github.com/alspitz/cpu_monitor}} which reports the memory used in MB by each individual node running and the compute in percentage of utilization per unit core, so for an 8-core machine, the compute usage can go from 0-800\%.

\noindent\textbf{Memory Usage:} We use the memory (RAM in MB) usage of the SLAM algorithm as time progresses as the metric to compare \name against state of the art. Where we observe that \name-SLAM reduces the average memory utilization to $300$MB which is $3\times$ the Visual SLAM.

\noindent\textbf{Compute Usage:} We use the percentage of a single core used by the SLAM algorithm as time progresses as the metric to compare \name against state of the art. 
That is for an 8-core machine, the compute usage can range from 0\%-800\%
Where we observe that \name-SLAM reduces the average compute memory utilization to $20$\% which is $5\times$ the Visual SLAM.

\noindent\textbf{Pose Estimation:} Since the system reports 4D pose ($(x,y,z,\theta)$) of the robot, which we compare with post-processing optimized cartographer poses as ground truth, as they have shown to have decent performance for indoor robots~\cite{diebel2006representing}. So, we use CDF of RMSE for $(x,y,z)$ and show a median tracking errors of 50cm and L1 norm error for $(\theta)$, and a median robots orientation error of 2$^\circ$ on par with state of the art.

\noindent\textbf{Mapping Accuracy:} Finally, to evaluate mapping performance, we wanted to deploy fiducial markers and get the accuracy by comparing their mapped poses to the ground truth poses. Thus
to evaluate the mapping performance we collect one more Dataset in a $25m\times40m$ space (which we will refer as Env-3). In this dataset we have collected  ArUCo camera fiducials~\cite{garrido2014automatic} across the environment, which are tracked using the OpenCV toolbox available~\cite{opencvaruco} and mapped in the environment by the camera graph.
Thus, the RMSE of the mapped locations of these fiducials help us to quantify the accuracy of \name's mapping capabilities.
Where we show that \name's is able to accurately map the environment with a median error of 105cm.

\subsection{Compute and Memory Requirements}\label{sec:eval-compute}

\noindent\textbf{Memory \& Compute usage:} One of the most important contributions of \name's SLAM design is to achieve memory and compute efficient SLAM system without compromise the SLAM tasks. 
Thus we first evaluate the memory and compute usage of \name's overall system when deployed in both Env-1 and Env-2 and compare with a state-of-the-art SLAM system, RTABMap (that uses a RGB-D camera).
We plot these memory usage in Figure~\ref{fig:memory-compute}{a} and compute usage in Figure~\ref{fig:memory-compute}{b} over time for each incoming sensor frame for bot the algorithms.
From these plots we can clearly see that \name's SLAM implementation on an average uses only $300$ MB of memory which is $3\times$ lower than RTABMap. Additionally we can see that \name uses only $20$\% of compute which is $5\times$ lower than RTABMap, thus demonstrating that \name is both memory and compute efficient by 4$\times$ compared to the state-of-the-art camera SLAM systems.

% \noindent\textbf{Real-time performance of \name:} Additionally, we can also note from both Figure~\ref{fig:memory-compute}{a,b} that while \name's SLAM provides optimized poses and map in real-time and thus the plot ends at \todo{xx}secs when the data collection ends. On the other hand, RTABMap and Cartographer both take \todo{yyy}secs and \todo{zz}secs more to generate a better optimized paths and maps.
% This further shows the deployability and scalability of \name due to its real-time performance compared to the existing SLAM systems that take additional time to perform end-to-end bundle adjustments~\cite{semenova2022quantitative} to get more accurate poses and maps.

\noindent\textbf{Ablation for \name's Memory \& Compute usage:} \\
\noindent We further analyze and look into the memory and compute usage of the individual components of \name, that is the individual WiFi and camera graph that are running in parallel.
We can see most of the  memory and compute usage for \name's algorithm are due to the camera features that are tracked and the \name WiFi layer needs very little compute.

We also, note that for all the time-series plots shown in Figures~\ref{fig:memory-compute} have a series of vertical solid lines which show the AP initialization event happening for each of the individual AP's in the environment as per our smart initialization algorithm discussed in ~\cref{sec:design-graph1}.
We can see that the spikes in the WiFi graph for memory and compute occur at these instances noting that the measurements associated to the specific are laid down at this instant, but even these spikes are much lower than the overall compute and memory requirements of RTABMap.

\begin{figure*}[t]
    \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-top-down-8-28-crop.pdf}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/rtab-top-down-8-28-crop.pdf}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}{0.28\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-top-down-8-4-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Shows the top down view of the trajectory of \name compared with cartographer ground truth in Env-1, (b) Shows the top down view of the trajectory of RTABMap compared with cartographer ground truth in Env-1 and (c)hows the top down view of the trajectory of \name compared with cartographer ground truth in Env-2 }
    \label{fig:mapping}
\end{figure*}

\subsection{Tracking Accuracy}\label{sec:eval-tracking}

\begin{figure}[ht]
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/viwid-wifi-cam_trans.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{evaluation/figures/fft-pca-crop.pdf}
        \subcaption{}
    \end{minipage}
    \caption{(a) Tracking errors for pose estimates provided from the WiFi-layer Poses Vs Visual layer for \name's implementation. (b) Shows the comparison of AoA accuracies for FFT Vs SVD-FFT}
    \label{fig:microbencmarks}
\end{figure}

Now that we have demonstrated memory and compute efficiency of \name, we demonstrate that we achieve these low-compute and low-memory requirements while achieving state-of-the-art accuracies for robot pose estimation first, we will then demonstrate mapping accuracy of \name in ~\cref{sec:eval-mapping}. 

As stated earlier, we benchmark our results with end-to-edn cartographer processed poses as ground truth, against which we compare both \name and RTABMap to show tracking in Figure~\ref{fig:tracking-errors}{a} and orientation errors in Figure~\ref{fig:tracking-errors}{b} across both Env-1 and Env-2.
We can see that name achieves a median tracking error of $50$cm for both Env-1 and Env-2 and a median orientation error of $1^{\circ}$ and $2.8^{\circ}$ for both env-1 and env-2. These are on par with the median tracking errors of $60$cm and $38$cm and median orientation errors, $5^{\circ}$ and $3^{\circ}$ across Env-1 and Env-2 for RTABMap. Thus showing that the pose estimation of \name is on par with the state-of-the-art Visual SLAM systems.

Additionally, we also provide the time-series plots of tracking errors across Env-1 and Env-2 in Figures~\ref{fig:tracking-errors}{c,d} and orientation errors in in Figures~\ref{fig:tracking-errors}{e,f} for both \name and RTABMap  showing that \name performs on par in terms of pose estimations with the RTABMap. We can also see that the high errors in \name are only in the initial stages where it is searching for the APs in the environment and it stabilizes for later stages, showing the robustness of our system. On the other hand, loop-closure dependant SLAM algorithms need a location to be revisted to avoid any drifts.

Finally, we also plot the \name's estimated path against the Cartographer's ground truth for both the environments in Figure~\ref{fig:tracking-errors}{g,h} to qualitatively show \name's accurate pose estimation across time.

\subsection{Mapping Accuracy}\label{sec:eval-mapping}

Finally, we evaluate \name's ability to amp features in the environment accurately. While, most of the works only give a qualitative map~\cite{Labb2018RTABMapAA,rosinol2021kimera,mur2015orb,qin2018vins} which also we present in Figure~\ref{fig:tracking-errors}{g,h} for both Env-1 and Env-3 respectively.
We additionally, place camera fiducials in Env-3 dataset that we have collected to measure if the locations of these fiducials are mapped accurately in the environment.
These camera fiducial ground truth are highlighted in Figure~\ref{fig:tracking-errors}{h} as blue circles and \name's mapped location in red crosses.
We compare these locations to provide the mapping errors, which we find has a mean mapping error of 103cm.


\subsection{Micro-benchmarks}

We have seen that \name demonstrates compute and memory efficient SLAM when deployed in real-world scenarios as seen in the results above. We now present few micro-benchmarks of \name's design to further demonstrate \name's robustness.

\noindent\textbf{Justifying \name's Dual Layered Approach:}\\
Firstly, while we have shown the pose estimation results of \name's WiFi graph, the camera graph also performs local pose corrections to these pose estimates while mapping the features in the environment.
So as to develop an insight towards the poses to use, we show the tracking errors for robot locations estimated using \name's WiFi graph and camera graph in Figure~\ref{fig:microbencmarks}{c} from where we can see that owing to its global perspective the WiFi graph provides with much more accurate location estimates than the Camera graph.
This further supports \name's dual graph idea where our intuition stems from the fact that WiFi-SLAM is best for pose estimation and camera-SLAM for mapping the environment.

\noindent\textbf{PC-FFT vs FFT:}\\
Additionally, the individual CSI measurements are vulnerable to noise and transient multipath in the environment. As described above, we extract the underlying signal parameters from multiple CSI measurements across different transmitter antennas using Singular Value Decomposition, to identify the principle component of CSI. We evaluate these new SVD CSI measurement's performance with 2D-FFT and show their AoA estimation accuracies as shown in Figure~\ref{fig:microbencmarks}{d}, where we can see that SVD-FFT based AoA estimates reduce the 90$^{th}$ percentile error from $40^{\circ}$ to $25^{\circ}$.
We specifically note the 90$^{th}$ percentile errors as these are the corner cases where multipath based errors are more prevalent. 
Thus demonstrating the performance improvement from \name's PC-FFT implementation.

\fi


==> evaluation/eval5.tex <==
% !TEX root = root.tex
\section{Microbenchmarks}\label{sec:eval-micro}

\begin{figure*}[t]
    \begin{minipage}{0.20\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/top-down-kimera.pdf}
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.20\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/top-down-viofi.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_translation.pdf}    
        \subcaption{}
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_ral/err_ts_orientation.pdf}    
        \subcaption{}
    \end{minipage}
    
    \caption{\textbf{End-to-end evaluation}: \textbf{(a)} Trajectory estimated by Kimera with loop closures (Orange) and ground truth (dashed-Blue). \textbf{(b)} Trajectory estimated by \name using odometry predictions from Kimera without loop closures (Orange, \textit{WiFi + Kimera w/o LC}) and ground truth (dashed-Blue). \textbf{(c, d)} Time series of translation and orientation error comparing Kimera with loop closure (dashed-Orange) against \name's predictions. \name uses odomtery from Kimera without loop closures (Blue) and just wheel odometry (dashed-Yellow).}
    \label{fig:end-end1}
    \vspace{-0.1in}
\end{figure*}


\name-SLAM uses Kimera (for VIO) and cartographer (for LIO) as both benchmarks and also the Odometry inputs for the WiFi-graph defined in ~\cref{sec:design-graph1}. We first analyze how the key parameters in Kimera and Cartographer in ~\cref{sec:micro-vio} and ~\cref{sec:micro-lio} respectively.

\subsection{VIO memory vs accuracy}\label{sec:micro-vio}
To first understand Kimera's performance with various parameters, we have found that the most memory demanding is the interframe time that determines how frequently does Kimera search for a keyframe for loop-closure. That is, lesser the interframe time is the better the loop-closure accuracy and the higher the memory consumption rate. To further understand this trade-off between memory consumption and navigation accuracy, we plotted the average translation error and the total memory consumed for one of the datasets we have collected in Figure~\ref{fig:micro}(a). From this plot, we can clearly see that the best median translation error with reasonably low memory consumption occurs at an interframe time of $1$~sec. Thus in our experiments we utilize the Kimera system with the inteframe rate set to $1$sec as the baseline which we call Kimera with LC (loop-closure). We also utilize the same interframe time for the Odometry given from Kimera without the loop closure detector which we call Kimera w/o LC.

\subsection{LIO compute vs accuracy}\label{sec:micro-lio}
To next understand the performance of Cartographer we first note that single-plane based LIO systems have sparser LiDAR scans. This sparse representation demands extensive scan-matching algorithms~\cite{cartographer} that consume more compute while the scans themselves have lesser memory requirements. Thus to understand and utilize the best tuned cartogrpaher model, we again run the cartogrpaher model with various compute limits enforced onto the system. That is limiting the compute provided to the system, limits the accuracy of scan matching and thus the navigation performance of the system. So, as shown in Figure~\ref{fig:micro}(b) where we plot the median translation accuracy vs the compute consumed for various thresholds, from which we can see \todo{text to come here that will describe the observation and the numbers}.
Thus taking this into account, for all the results we use cartographer both with loop-closure detection (cart w/ LC) and without loop closure detection (cart w/o LC) enabled to run at ~\todo{cxx}compute resources.

\subsection{Wheel Odom vs VIO without LCD Odom}\label{sec:micro-odom}
We showed fine-tuned Kimera and Cartographer systems that perform the best with the practical memory and compute limits. 
Now, let us compare how accurate are their Odometry measurements to the standard odometry provided by a wheeled robots wheel-encoder and see how accurate their navigations are in terms of their translation errors.
The Figure~\ref{fig:micro}(c) shows the comparison from which we can see that the odometry measurements from the Kimera and Cartographer without LC perform better than the odometry from wheel-encoders.
This supports the dual-graph design inuition of \name-SLAM wherein the odometry from VIO/LIO-graph is locally corrected and so is better in local odometry and mapping.

\subsection{2D-FFT, PCA-2DFFT vs PCA-FFT}\label{sec:micro-fft}
Finally, now that we have ensured the accuracy of the odometry measurements from VIO/LIO graph, we also need to understand the accuracy of WiFi bearing measurements that complete the WiFi-graph.
To understand the accuracy and timeliness of the bearings and the need for the design of PCA-FFT described in ~\cref{sec:design-bearing} we compare it with the 2D-FFT defined in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, a 2D-FFT version of the PCA algorithm, and the PCA-FFT algorithm we propose. As shown in Figure~\ref{fig:micro}(d), we can see that the PCA version of the algorithms far outperform in accurate bearing measurements the 2D-FFT from $\mathrm{P^2}$SLAM. On the other hand, while bearing errors for PCA-2D FFT are marginally lower than PCA-FFT, we not that the compute required for PCA-2D FFT is of the orders of \todo{xx} cores, while PCA-FFT only required \todo{xx} cores. Thus we can see that for the sake of both timeliness and accuracy PCA-FFT is a better trade-off.

\section{Results}\label{sec:eval}

\begin{figure}[t]
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_translation.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/err_cdf_orientation.pdf}
    \end{minipage}
    \caption{\textbf{Error analysis:} }
    \label{fig:end-end2}
\end{figure}

To evaluate \name implemented as mentioned in ~\cref{sec:implementation} we deployed \name's algorithms over four datasets. The one presented in ~\cref{sec:eval-kimera} (\name DS) was collected in a $25 \times 20$ m environment, with a total distance of $403$ m traversed over a duration of $23$ minutes. The subsequent 3 datasets (DS 1/2/3) are the P2SLAM datasets~\cite{arun2022p2slam}. Through these datasets, we have robustly tested \name across 3 distinct environments, 4 different access point placements, and traversed a cumulative distance of $1625$ m with a total travel time of $108$ minutes. We note the datasets in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} use AoA measurements at both the robot and the access points, while in \name we only utilize the AoA at the robot and extract the channels for only those measurements from the dataset. Finally, it is important to note that while in DS1/2/3 linear antenna arrays are used, we use square antenna array on the robot in \name DS.

As stated in ~\cref{sec:eval-micro}, we benchmark \name's results with a state-of-the-art SLAM algorithm, Kimera~\cite{rosinol2021kimera}, a stereo-camera based SLAM algorithm. We run Kimera on only \name DS with and without loop closures, labelled in the legends as `w/ LC' and `w/o LC' respectively, since DS1/2/3 lack required IMU measurements. Additionally, for all the 4 datasets, we run Cartographer in real time, with and without the `global SLAM' and LiDAR scan matching, which turn on/off loop closures. These are referred to as `Cart w/LC' and `Cart w/o LC' respectively. As discussed in ~\cref{sec:eval-micro} we have carefully finetuned both Kimera and Cartographer to their best performance as benchmarks. To obtain ground truth, we observe that allowing Cartographer to run past the time of data collection without any compute constraints allows it to provide a near-groundtruth trajectory as characterized in DLoc~\cite{ayyalasomayajula2020deep}. 

In the following sections, using the Cartographer ground truth generated, we benchmark \name against Kimera, Cartographer(when run in real-time), and WiFi graph run with the wheel-encoder odometry (WiFi+Odom) and provide results for the translation and orientation errors. We further measure the CPU and memory usage across these SLAM frameworks\footnote{\url{https://github.com/alspitz/cpu_monitor}} and compare the total memory used, the rate of memory increase and the CPU resources used over the entire run of the datasets.

\subsection{End-to-end evaluation (\name with Kimera):}\label{sec:eval-kimera}

% \begin{table*}[ht]
%     \centering
%     \footnotesize
%     \caption{}
%     \begin{tabular}{|l|cccc|cccc|cccc|}
%     \hline
%     \multirow{2}{*}{} & \multicolumn{4}{c|}{\textbf{Cart. w/ LC}} & \multicolumn{4}{c|}{\textbf{\name + Cart. w/o LC}} & \multicolumn{4}{c|}{\textbf{\name + Odom}} \\ \cline{2-13} 
%      & \multicolumn{1}{l|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3} & \multicolumn{1}{l|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3} & \multicolumn{1}{l|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}} & \multicolumn{1}{c|}{\textbf{DS 2}} & \multicolumn{1}{l|}{\textbf{DS 3}} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}Translation \\ Error (cm)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}88.0\\ (169.4)\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0 \\ (224)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}134.1 \\ (1097)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}23.3\\ (37.4)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}98.5\\ (252.5)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}65.9\\ (92.2)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}67.3\\ (182.6)\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}48.6 \\ (114.4)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}88.1\\ (193)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74.0\\ (100.2)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}75.5\\ (204.9)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}66.44\\ (234.7)\end{tabular} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}Orientation \\ Error (deg)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4.8\\ (7.9)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{0.8}\\ (4.66)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}5.3\\ (12.6)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.6\\ (1.4)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.5\\ (6.9)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2.4\\ (4.66)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{2.8}\\ (12)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}1.4\\ (3.3)\end{tabular} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}1.0\\ (3.7)\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1.7\\ (\textbf{2.7})\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.0\\ (\textbf{6.2})\end{tabular}} & \begin{tabular}[c]{@{}c@{}}2.0 \\ (10.3)\end{tabular} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}Total \\ Memory (MB)\end{tabular}} & \multicolumn{1}{c|}{520} & \multicolumn{1}{c|}{702} & \multicolumn{1}{c|}{658} & 423 & \multicolumn{1}{c|}{486} & \multicolumn{1}{c|}{613} & \multicolumn{1}{c|}{706} & 356 & \multicolumn{1}{c|}{\textbf{270}} & \multicolumn{1}{c|}{\textbf{288}} & \multicolumn{1}{c|}{\textbf{252}} & \textbf{163} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}Rate of \\ memory (MB/s)\end{tabular}} & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{0.29} & \multicolumn{1}{c|}{0.33} & 0.38 & \multicolumn{1}{c|}{0.32} & \multicolumn{1}{c|}{0.22} & \multicolumn{1}{c|}{0.33} & 0.26 & \multicolumn{1}{c|}{\textbf{0.16}} & \multicolumn{1}{c|}{\textbf{0.10}} & \multicolumn{1}{c|}{\textbf{0.11}} & \textbf{0.14} \\ \hline
%     \textbf{\begin{tabular}[c]{@{}l@{}}CPU (fraction \\ of cores)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.8\\ (4.4)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.2\\ (4.2)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3.8\\ (4.2)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}1.85\\ (4.4)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.73\\ (1.90)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.62\\ (2.1)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.85\\ (2.8)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.77\\ (1.1)\end{tabular} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.19\\ (1.4)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.2\\ (1.6)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}0.28 \\ (1.7)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.22 \\ (0.5)\end{tabular}} \\ \hline
%     \end{tabular}
% \end{table*}


\begin{table*}[t]
    \centering
    \footnotesize
    \caption{}
    \label{tab:cart}
    \begin{tabular}{|l||cccc||cccc|}
    \hline
    \multirow{2}{*}{}                   & \multicolumn{4}{c||}{\textbf{Cart. w/ LC}}                                                                                                                    & \multicolumn{4}{c|}{\textbf{\name + Cart. w/o LC}}                                                                                                   \\ \cline{2-9} 
                                        & \multicolumn{1}{c|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}}       & \multicolumn{1}{c|}{\textbf{DS 2}} & \textbf{DS 3}        & \multicolumn{1}{c|}{\textbf{\name DS}} & \multicolumn{1}{c|}{\textbf{DS 1}}        & \multicolumn{1}{c|}{\textbf{DS 2}}         & \textbf{DS 3}      \\ \hline
    \textbf{Translation Error (cm)}     & \multicolumn{1}{c|}{\textbf{88.0 (169.4)}}            & \multicolumn{1}{c|}{74.0 (224)}          & \multicolumn{1}{c|}{134.1 (1097)}  & \textbf{23.3 (37.4)} & \multicolumn{1}{c|}{98.5 (252.5)}                     & \multicolumn{1}{c|}{\textbf{65.9 (92.2)}} & \multicolumn{1}{c|}{\textbf{67.3 (182.6)}} & 48.6 (114.4)       \\ \hline
    \textbf{Orientaion Error ($^\circ$)} & \multicolumn{1}{c|}{4.8 (7.9)}                        & \multicolumn{1}{c|}{\textbf{0.8 (4.66)}} & \multicolumn{1}{c|}{5.3 (12.6)}    & \textbf{0.6 (1.4)}   & \multicolumn{1}{c|}{\textbf{3.5 (6.9)}}               & \multicolumn{1}{c|}{2.4 (4.66)}           & \multicolumn{1}{c|}{\textbf{2.8 (12)}}     & 1.4 (3.3)          \\ \hline
    \textbf{Total Memory (MB)}          & \multicolumn{1}{c|}{520}                              & \multicolumn{1}{c|}{702}                 & \multicolumn{1}{c|}{\textbf{658}}  & 423                  & \multicolumn{1}{c|}{\textbf{486}}                     & \multicolumn{1}{c|}{\textbf{613}}         & \multicolumn{1}{c|}{706}                   & \textbf{356}       \\ \hline
    \textbf{Rate of Memory (MBps)}      & \multicolumn{1}{c|}{\textbf{0.30}}                    & \multicolumn{1}{c|}{0.29}                & \multicolumn{1}{c|}{0.33}          & 0.38                 & \multicolumn{1}{c|}{0.32}                             & \multicolumn{1}{c|}{\textbf{0.22}}        & \multicolumn{1}{c|}{\textbf{0.33}}         & \textbf{0.26}      \\ \hline
    \textbf{CPU (fraction of cores)}    & \multicolumn{1}{c|}{3.8 (4.4)}                        & \multicolumn{1}{c|}{3.2 (4.2)}           & \multicolumn{1}{c|}{3.8 (4.2)}     & 1.85 (4.4)           & \multicolumn{1}{c|}{\textbf{0.73 (1.90)}}             & \multicolumn{1}{c|}{\textbf{0.62 (2.1)}}  & \multicolumn{1}{c|}{\textbf{0.85 (2.8)}}   & \textbf{0.7 (1.1)} \\ \hline
    \end{tabular}
\vspace{-0.1in}
\end{table*}



In this section we demonstrate in depth on how \name-SLAM compares to the state of the art Kimera VIO SLAM on our \name DS.

\noindent\textbf{Navigation Accuracy:} Firstly, we look at the translation and orientation errors of \name-SLAM + Kimera w/o LC and compare it with \name-SLAM+Odom and Kimera w/ LC across Figures~\ref{fig:end-end2},~\ref{fig:end-end1}. Firstly from Figure~\ref{fig:end-end2} we can see that \name-SLAM + Kimera w/o LC has a median ($90^{th}$\%) translation error of $85$cm ($185$cm) and median ($90^{th}$\%) orientation errors of $3^{\circ}$ ($8^{\circ}$). 
We can also see that WiFi+Odom very closely at a median ($90^{th}$\%) translation errors of $90$cm ($205$cm) and median ($90^{th}$\%) orientation errors of $1^{\circ}$ ($4^{\circ}$). While we see that Kimera w/ LC has a median ($90^{th}$\%) translation errors of $105$cm ($300$cm) and median ($90^{th}$\%) orientation errors of $5^{\circ}$ ($20^{\circ}$)showing that  \name-SLAM's WiFi graph implementation out-performs the state-of-the-art Kimera w/ LC, without needing loop-closure detection. Additionally, we can also see that the translation errors and orientation errors for WiFi+Kimera w/o LC are smaller than and on par that for WiFi+Odom respectively, showing how the locally-corrected Odom measurements from Kimera w/o LC aid in better global optimizations.

The understand this further we can see from Figure~\ref{fig:end-end1}(a) where we plot the predicted trajectory for Kimera w/ LC against ground truth where we can see that it looses tracking around the region of $[-5 5] and [-20 -15]$ along $X and Y$ axes, which can be further demonstrated at the $1100$ sec mark in the time series plots shown for the red-dotted line in Figures~\ref{fig:end-end1}(c,d). We can see that after $1100$secs Kimera w/ LC performs incorrect Loop Closure leading to the translation errors shooting up to $~450$cm and orientation errors up to $~25^{\circ}$. In contrast we can see from the blue-solid (green-dotted) line in Figures~\ref{fig:end-end1}(c,d) that \name's WiFi+Kimera w/o LC (WiFi+Odom) closely track the ground truth where it caps at about $~200$cm translation error and $~10^{\circ}$ orientation error.
So we have seen that \name's SLAM navigation is on-par or even more accurate due to its robustness to global corrections than the state-of-the-art VIO, Kimera.

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.42\textwidth}
        \includegraphics[width=\textwidth]{figures/eval_ral/mem_cpu_w_aoa_ts.pdf}
    \end{minipage}
    \caption{Notes: memory avg slope, Kimera -- 0.56, \name -- 0.2 MB/s}
    \label{fig:mem-cpu}
\end{figure}

\noindent\textbf{Memory and Compute:} Next, we run \name-SLAM and Kimera under various settings on \name DS and evaluate the memory and compute consumption of each components of \name SLAM that uses Kimera w/o LC and Kimera w/ LC and plot the time-series as shown in Figure~\ref{fig:mem-cpu}. From the Figure~\ref{fig:mem-cpu}(left) we can see taht Kimera w/ LC has a huge start-up cost of about $2$GB after which we see that it has a memory consumption rate of about $0.56$MBps, in contrast we can see that the memory consumption for \name+Kimera w/o LC has a startup of $0.5$GB, with a consumption rate of only $0.2$MBps. That is given a standard RPi of 8GB RAM, while Kimera w/ LC can only run upto $3$hrs before the robot crashes due to lack of space, \name+Kimera w/o LC can run up to $10$hrs, that is in general \name + Kimera w/o LC has a $3.3\times$ lesser memory consumption rate than the state-of-the-art Kimera system.
To further understand the individual components that lead to this memory consumption we have also plotted the timeseries memory consumption of Kimera w/o LC and WiFi only systems in Figure~\ref{fig:mem-cpu}(left). From which we can see that due to a fix lag local drift correction algorithm that Kimera w/o LC employs it has a constant memory consumption of $0.3$GB. On the other hand, WiFi only has a increasing memory rate of $0.2$MBps because we do not employ a fix-lag filter~\cite{xxxx}, but accumulate all the nodes over all the time. This is not exactly required for the global corrections to occur as these WiFi anchors act as unique self-identifiable landmarks in the environment.

Finally, we can also see from Figure~\ref{fig:mem-cpu}(right) that the compute requirements for \name's WiFi+Kimera w/o LC is upto a $1$ core, while Kimera w/ LC takes up to $1.5$ cores owing to its compute heavy loop closure detection and correction algorithms. Thus \name's design requires about $3.3\times$ less memory and $1.5\times$ less compute than state-of-the-art Kimera system, while achieving about $30\%$ better navigation performance.

\subsection{End-to-end evaluation (\name with Cartographer):}\label{sec:eval-cart}

We further also demonstrate that \name-SLAM can also improve the performance of the state-of-the-art LIO SLAM, Cartographer. So, we compare \name's WiFi+Cart w/o LC against the Cartographer w/ LC when run in real-time. Additionally, since we have the cartographer LiDAR data from the open-sourced $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} datasets, DS 1/2/3 we provide the translation, orientation errors, memory consumption and compte requirements for \name and cartographer in Table~\ref{tab:cart}. From this table we can see that mostly \name's WiFi+Cart w/o LC performs on-par with Cart w/ LC in terms of translation and orientation accuracies. There are two notably different navigation accuracy performances: (a) in DS 2 \name's median ($90^{th}$) translation and orientation errors are $2\times$ ($5\times$) lower for \name's Cart W/o LC than Cart W/ LC. (b) in DS 3 cart. w/ LC has $2\times$ lesser translation and orientation errors than WiFi+cart w/o LC. But we can see that the maximum errors in translation (orientation )are only $114.4$cm (3.3$^\circ$) which are tolerable.

In contrast looking at the memory consumption, both the systems perform almost the same with minor differences. This occurs because unlike Kimera's VIO system where each camera frame consists of dense features, Cartographer's LIO system's each scan has fewer number of features. This limited features in each scan greatly reduces the load on the memory consumption. Instead, having sparser features, LIO systems like Cartographer tend to execute complex scan-matching algorithms for loop closures, which in turn increase the compute requirements of the VIO-SLAM systems. In constrast, since in \name's implementaiton of WiFi+Cart. w/o LC does not require these complex scan matching for loop closures, demands much lesser compute resources. This can be clearly observed in the last row of Table~\ref{tab:cart} which shows the average number of cores used over the entire run of the robot navigation with the maximum number of cores used in parentheses.
Where we can see that \name's WiFi+cart w/o LC requires $4\times$ lesser peak compute than real-time Cartographer implementation across all the 4 datasets.

==> intro/intro-1.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.


Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Since these Visual and LiDAR SLAM systems perform sensor fusion to provide a human-readable map and to reduce the local and global drifts introduced by the odometry sensors.
This mapping and corrections are possible by performing feature identification and feature correlation across current and past frames to re-detect the previously visited location (typically termed as `loop-closure detection'), which leads to two distinct problems: 
(a) The robot needs to have an active memory of all the past features of all the time, making the system limited by the active memory (typically the RAM size). 
(b) Also as time progresses, the search time to find a matching features frame across all the past frames continues to rise.
These issues in the best could lead to the robot just taking longer in state transition, and accidents in the worst owing to inconsistency in the current state and the predicted state, leading to incorrect state-transition decisions.

In this work, so we ask and answer the question what if we can remove these memory intensive and time consuming loop-closures? For which we can see that $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} which performs end-to-end robot navigation optimization without requiring any loop closure detection. Inspired from this observation in this paper, we will present how WiFi can be integrated with visual sensors for real-time autonomous navigation.

\subsection{Literature Review}

Most of the existing Visual and LiDAR SLAM algorithms try to resolve the memory and search-time issues in loop-closure detection and identification by: (a) optimizing on the algorithms for key-frame and key-point detection~\cite{mur2015orb,rosinol2021kimera} to reduce the number of key-frames stored, and (b) using smart representation, like bag-of-words~\cite{rosinol2021kimera} to reduce the search time. While these solutions might extend the run-time of a robot temporarily, it would quickly run into the same issues once it is used for larger or more involved spaces like warehouses.

In a past work~\cite{arun2022p2slam} we demonstrated Radio Frequency(RF) technologies, especially WiFi as a navigation sensor for SLAM robots owing to the ubiquitous deployment of WiFi.
Although $\mathrm{P^{2}}$SLAM performs only end-to-end optimization and cannot translate to real-time navigation of the robot.
There have been other works like WSR~\cite{jadhav2020wsr} that only demonstrates robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi,hashemifar2019augmenting, liu2019collaborative} depend only on WiFi readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

The other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation, like UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi and thus are limited in scalability.
% \footnote{We also want to note that, while we have used WiFi as a sensor in \name, \name's design is modular enough to easily scale to other RF-technologies.}.

Finally, there also exist a few other series of works called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel} that try to reduce the memory usage and processing time by running two different optimizations for mapping and pose-estimation in parallel which tend to drift in real-time while they are corrected post-facto. There are also a few works that perform Decentralized SLAM that off-loads the memory and time intensive loop closure detection and map updates to the cloud~\cite{nandikolla2021navigation,kiss2019gps}. We later demonstrate that even such works can benefit from \name's design and implementation.

\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered SLAM system which overcomes the need of loop-closure detection making it memory efficient and timely.
To build a SLAM system that consumes minimal-memory and performs real-time robot navigation without any delays using the the existing visual and WiFi sensor technologies and architectures have the following limitations:

\noindent\textbf{Noisy WiFi Measurements:} WiFi measurements are not always reliable and are quite noisy for real-time and accurate navigation. While, existing $\mathrm{P^2}$SLAM demonstrates WiFi as a sensor for navigation, it performs retrospective end-to-end optimization and not real-time navigation and optimization. That is while WiFi as a sensor can provide accurate global corrections, for real-time navigation of the robot, WiFi measurements are too noisy, ambiguous and sparse.
    
\noindent \textbf{Naive Sensor Fusion:} One can solve this problem of noisy WiFi measurements by integrating more reliable existing Visual or LiDAR sensors. A naive way to integrate the WiFi and Camera systems are to integrate the WiFi measurements, like the two-way bearing measurements of $\mathrm{P^2}$SLAM into the existing Visual SLAMs as new measurements. This naive integration of bearings into VIO would make the system complex, as the WiFi sensors being more noisier than camera for local pose corrections, that the system might completely neglect WiFi measurements or worse, make incorrect local-corrections.

\subsection{\name SLAM's Solution}

To overcome these the core idea for \name SLAM's design relies on two important aspects (a) Visual sensors are accurate, does not require a lot of memory and are real-time for local drift corrections and feature mapping, and (b) WiFi sensors while sparse and noisy in smaller areas, have accurate global perspective to correct for the global drifts of the robot. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Dual Graph:} The first idea that we propose in \name SLAM is to construct a novel Visual WiFi Dual graph system, where utilizing the the VIO systems like Kimera, ORB-SLAM, or RTABMap that can provide the odometer measurements without performing any global loop closure detection. These local drift corrected odometer measurements are then sent to our WiFi graph, which utilizes these Visual Inertial Odometer (VIO) measurements in tandem with the WiFi measurements made from multiple access points in the environment, whose locations are also not known. These measurements are then combined together in a real-time navigation GraphSLAM optimization backend, for which we use the open-sourced iSAM~\cite{gtsam} toolbox. While, there are visual fiducial markers ~\cite{opencvaruco} that can also act as global constant markers that can help in global corrections with minimal memory overhead. Though, unlike WiFi sensors, visual markers can be easily blocked in a dynamic environment making them less reliable.

\noindent\textbf{(b) Accurate WiFi Measurements:} We have seen from existing works like $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} and WSR~\cite{jadhav2020wsr} that bearing measurements are robust and accurate for WiFi based SLAM algorithms. Unfortunately, the bearing measurement approach detailed in $\mathrm{P^2}$SLAM are not sufficiently accurate and the bearing measurement algorithms of WSR rely on measurements across time limiting the real-time robot navigation performance. 
While some existing bearing measurement algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide real-time AoA measurements at the rate needed for pose estimation.
Thus in \name SLAM we employ a low-compute algorithm, which reduces erroneous measurements by attenuating noisy components in the signal, by combining the WiFi channel measurements across time and finding its principle component which we call PC-CSI. 
The PC-CSI can then be fed to the 2D FFT transform we proposed in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, for more reliable and real-time bearing measurements.

\noindent\textbf{(c) Real-Time Navigation:} Finally, utilizing the locally corrected VIO's `odometer' measurements, and the sparse and more reliable PC-CSI based `bearing' measurements together to construct a factor graph, where the WiFi access point sin the environment are not known as well. So the robot's global drift corrections and the WiFi access points locations are simultaneously using an open-sourced real-time implementation of factor graph optimization backend called iSAM, where we use the VIO's odometer outputs as the measurements for the in-between factors and the robot to WiFi bearings as the WiFi measurements factors as shown in Figure~\ref{fig:wifi-factor}. Thus using these contributions \name SLAM is able to perform real-time and accurate indoor robot navigation with minimal memory requirements.

Finally, with these contributions, we have deployed our \name SLAM robot system on a Turtlebot2 that is equipped with a Hokuyo LiDAR, and Intel 455 RGB-D camera with an inbuilt IMU for deploying cartographer~\cite{cartographer}, RTABMap~\cite{Labb2018RTABMapAA}, and Kimera~\cite{rosinol2021kimera}. We also deploy a 4 antenna WiFi sensor, where the antennas are deployed as a square antennas array to avoid ambiguities, on top of the robot for measuring the bearing to the access points in the environment. We have deployed this robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs along with two of our open-sourced datasets that we use to demonstrate \name's deployability with RTABMap and Cartographer as well. Across these deployments the robot traverses for an overall time of ~\todo{xx}mins covering a distance of ~\todo{xxx} kms across a space of ~\todo{xx} sq. m. where in we show that \name achieves a median translation error of \todo{xx} m and a median orientation error of \todo{$x^{\circ}$}, on par with the state-of-the-art Kimera system with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of ~\todo{xx} MB for a ~\todo{xx} min run, wherein Kimera needs ~\todo{yy} MB. Thus \name SLAM demonstrates accurate, real-time and low-memory SLAM.

==> intro/intro-2.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.


Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Since these Visual and LiDAR SLAM systems perform sensor fusion to provide a human-readable map and to reduce the local and global drifts introduced by the odometry sensors.
This mapping and corrections are possible by performing feature identification and feature correlation across current and past frames to re-detect the previously visited location (typically termed as `loop-closure detection').
Unfortunately, this loop-closure detection needs the SLAM system running on a robot to store all the important features (called `key-frames`) up to the current state.
This implies that the as the robot navigates in increasingly large spaces, the SLAM system running on the robot consumes increasingly more memory.
This increasing memory for SLAM would eventually leaving little for the other applications and processes, which would lead the robot to start malfunctioning or becoming extremely slow.


% the (a) The robot needs to have an active memory of all the past features of all the time, making the system limited by the active memory (typically the RAM size). 
% (b) Also as time progresses, the search time to find a matching features frame across all the past frames continues to rise.
% These issues in the best could lead to the robot just taking longer in state transition, and accidents in the worst owing to inconsistency in the current state and the predicted state, leading to incorrect state-transition decisions.

In this work, so we ask and answer the question what if we can remove these memory intensive loop-closures? 
The first key-insight we make is that the need for loop-closure detection occurs because the individual landmarks or the key-frames identified in the environment are not unique. That is each key-frame does not have a unique ID. If that were possible, it would remove the need for storing each key-frame but only its unique ID.
Whereby we note that through $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, we have demonstrated on how the WiFi routers placed in the environment can act as these unique key-frames that can perform self loop-closure detection.
Inspired from this observation in this paper, we will present our solution that integrates WiFi with visual sensors for real-time autonomous navigation that does not need memory expensive loop-closure detection.

\subsection{Literature Review}

Most of the existing Visual and LiDAR SLAM algorithms try to resolve the memory issues in loop-closure detection and identification by: (a) optimizing on the algorithms for key-frame and key-point detection~\cite{mur2015orb,rosinol2021kimera} to reduce the number of key-frames stored, or by (b) using smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions might lessen the amount of memory required per frame. But the underlying issue of every increasing memory consumption would lead to the same issues once it is used for larger or more involved spaces like warehouses.

As noted earlier, in a past work~\cite{arun2022p2slam} we demonstrated Radio Frequency(RF) technologies, especially WiFi as a navigation sensor for SLAM robots owing to the ubiquitous deployment of WiFi.
In $\mathrm{P^{2}}$SLAM, while we demonstrated accurate WiFi based SLAM, it performs only end-to-end optimization and cannot translate to real-time navigation of the robot.
There have been other works like WSR~\cite{jadhav2020wsr} that only demonstrates robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi,hashemifar2019augmenting, liu2019collaborative} depend only on WiFi readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

The other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation, like UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi and thus are limited in scalability to large spaces or ubiquitous deployment.
% \footnote{We also want to note that, while we have used WiFi as a sensor in \name, \name's design is modular enough to easily scale to other RF-technologies.}.

\todo{Aditya-- can you check the accuracy in technicalities in the following:}
Finally, there also exist a few other series of works called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel} that try to reduce the memory usage and processing time by running two different optimizations for mapping and pose-estimation in parallel which tend to drift in real-time while they are corrected post-facto. There are also a few works that perform Decentralized SLAM that off-loads the memory and time intensive loop closure detection and map updates to the cloud~\cite{nandikolla2021navigation,kiss2019gps}. We later detail on how even such works can benefit from \name's design and implementation.

\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory efficient.
To build a SLAM system that consumes minimal-memory and performs real-time robot navigation without any delays using the the existing visual and WiFi sensor technologies and architectures have the following limitations:

\noindent\textbf{(a) Noisy and sparse WiFi Measurements:} As demonstrated in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} WiFi as a SLAM sensor can provide accurate global corrections without the need of loop closure detection for end-to-end optimization. Although for real-time navigation of the robot, WiFi bearings measured from 2D-FFT are too noisy, ambiguous and sparse.

\noindent\textbf{(b) Unknown WiFi anchors:} Secondly, we do not assume any apriori knowledge of the WiFi access points(APs) in the environments, including their locations. Thus, we need to map the APs accurately, one can initialize the APs at the origin but all the APs do not have measurements with the WiFi radio on the robot leading to ill-defined optimization. Thus, optimal initialization and mapping of the WiFi APs becomes challenging.
    
\noindent \textbf{(c) Naive Sensor Fusion:} One can solve the problem of noisy WiFi measurements by integrating more reliable existing Visual or LiDAR sensors. A naive integration of bearings into existing VIO would make the system complex, as the WiFi sensors are more noisier than camera for local pose corrections, leading to the system to completely neglect WiFi measurements or worse, make incorrect local-corrections.

\subsection{\name SLAM's Solution}

To overcome these the core idea for \name SLAM's design relies on two important aspects (a) Visual sensors are accurate, does not require a lot of memory and are real-time for local drift corrections and feature mapping, and (b) WiFi sensors while sparse and noisy in smaller areas, have accurate global perspective to correct for the global drifts of the robot. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Accurate WiFi Measurements:} We have seen from existing works like $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} and WSR~\cite{jadhav2020wsr} that bearing measurements are robust and accurate for WiFi based SLAM algorithms. Unfortunately, these algorithms have more noisier bearings than are tolerable for real-time robot navigation. 
While some existing bearing measurement algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide real-time AoA measurements at the rate needed for pose estimation.
Thus in \name SLAM we employ a low-compute algorithm, which reduces erroneous measurements by attenuating noisy components in the signal, by combining the WiFi channel measurements across time and finding its principle component which we call PC-CSI. 
The PC-CSI can then be fed to the 2D FFT transform we proposed in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, for more reliable and real-time bearing measurements.

\noindent\textbf{(b) Accurate mapping of WiFi anchors:} For accurate navigation of the robot, the WiFi APs also need to be mapped accurately in the environment. Since, \name-SLAM's accurate navigation without loop closure detection relies on these unique key-frames/landmarks in the WiFi domain, as each AP is uniquely identifiable. The robot while moving around, cannot see all the APs all the time, the number of WiFi APs it can get reasonable data from is limited and thus we have to smartly initialize each AP's location, as the robot connects to one for the first time. Thus, to enable smart mapping of the WiFi APs, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an infection point in the signal strength measured for that AP. Thus, in \name we perform accurate smart AP initialization to map them accurately.

\noindent\textbf{(c) Dual Graph:} The first idea that we propose in \name SLAM is to construct a novel Visual WiFi Dual graph system, where utilizing the the VIO systems like Kimera, ORB-SLAM, or RTABMap that can provide the odometer measurements without performing any global loop closure detection. These local drift corrected odometer measurements are then sent to our WiFi graph, which utilizes these Visual Inertial Odometer (VIO) measurements in tandem with the WiFi measurements made from multiple access points in the environment, whose locations are also not known. These measurements are then combined together in a real-time navigation GraphSLAM optimization backend, for which we use the open-sourced iSAM~\cite{gtsam} toolbox. While, there are visual fiducial markers ~\cite{opencvaruco} that can also act as global constant markers that can help in global corrections with minimal memory overhead. Though, unlike WiFi sensors, visual markers can be easily blocked in a dynamic environment making them less reliable.

% \noindent\textbf{(c) Real-Time Navigation:} Finally, utilizing the locally corrected VIO's `odometer' measurements, and the sparse and more reliable PC-CSI based `bearing' measurements together to construct a factor graph, where the WiFi access point sin the environment are not known as well. So the robot's global drift corrections and the WiFi access points locations are simultaneously using an open-sourced real-time implementation of factor graph optimization backend called iSAM, where we use the VIO's odometer outputs as the measurements for the in-between factors and the robot to WiFi bearings as the WiFi measurements factors as shown in Figure~\ref{fig:wifi-factor}. Thus using these contributions \name SLAM is able to perform real-time and accurate indoor robot navigation with minimal memory requirements.

Finally, with these contributions, we have deployed our \name SLAM robot system on a Turtlebot2 that is equipped with a Hokuyo LiDAR, and Intel d455 RGB-D camera with an in-built IMU for deploying cartographer~\cite{cartographer}, \todo{RTABMap}~\cite{Labb2018RTABMapAA}, and Kimera~\cite{rosinol2021kimera}. We also deploy a 4 antenna WiFi sensor, where the antennas are deployed as a square antennas array to avoid ambiguities, on top of the robot for measuring the bearing to the access points in the environment. We have deployed this robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs along with two of our open-sourced datasets that we use to demonstrate \name's deployability with RTABMap and Cartographer as well. Across these deployments the robot traverses for an overall time of ~\todo{xx}mins covering a distance of ~\todo{xxx} kms across a space of ~\todo{xx} sq. m. where in we show that \name achieves a median translation error of \todo{xx} m and a median orientation error of \todo{$x^{\circ}$}, on par with the state-of-the-art Kimera system with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of ~\todo{xx} MB for a ~\todo{xx} min run, wherein Kimera needs ~\todo{yy} MB. Thus \name SLAM demonstrates accurate, real-time and low-memory SLAM.

==> intro/intro-3.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Diverse indoor applications like inventory management in warehouses, last-mile delivery, and disaster relief~\cite{melenbrink2020site,lastmile} are increasingly interested in deploying autonomous robot systems.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, most current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Since these Visual (VIO) and LiDAR (LIO) SLAM systems utilize the camera frames  or LiDAR scans for sensor fusion to provide a human-readable map and to reduce the local and global drifts that are typically accrued by the odometry sensors.
To perform this, these Visual (LiDAR) sensors identify key-features/landmarks in each camera frame (Lidar scan) and track them across different robot locations.
This landmark mapping and tracking is possible by performing feature correlation across current and past frames (scans) to re-detect the previously visited location (typically termed as `loop-closure detection').

Unfortunately, this loop-closure detection needs the SLAM system running on a robot to store all the important features (called `key-frames`) up to the current state.
This implies to a trade-off as the robot navigates in increasingly large spaces: (a) On one side, the rate of memory consumption of the SLAM system running on the robot would be alarmingly high for systems with dense features (typical VIOs). (b) On the other hand, systems with sparse features, the compute starts to get occupied to enable complex feature matching algorithms (typical single plane LIOs). Additionally, since these features are not uniquely identifiable in bad lighting conditions or monotonous environments~\cite{deng2018feature,zhang2020comparison}, loop-closure detection failure can further detrimentally impact the quality of the SLAM output.

% This trade-off arising from the need of loop-closure detection limits the available memory and/or compute for the other applications and processes, which would lead the robot to start malfunctioning or becoming extremely slow.

In this work, we ask and answer the question what if we can remove these memory and/or compute intensive loop-closures? 
The first key-insight we make is that the need for loop-closure detection occurs because the individual landmarks identified in the environment are not unique. \todo{update the upcoming sentence or this paragraph, it doesn't nor does it deliver punchline...}If that were possible, it would remove the need for storing each key-frame but only its unique ID and circumvent key-frame searches.
Whereby we note that through $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, we have demonstrated on how the WiFi routers placed in the environment can act as these unique landmarks. 
Inspired from these observations, we present our solution that integrates WiFi with visual sensors for real-time autonomous navigation which removes the need for loop-closure detection.

\subsection{Literature Review}
Most of the existing Visual and LiDAR SLAM algorithms try to resolve the memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or by (b) using smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions might lessen the amount of memory required per frame, the underlying issue of ever increasing memory consumption would lead to the same issues once it is used for larger or more involved spaces like warehouses.

As noted earlier, in a past work~\cite{arun2022p2slam} while we demonstrated accurate WiFi based SLAM, it performs only end-to-end optimization and cannot translate to real-time navigation of the robot.
There have been other works like WSR~\cite{jadhav2020wsr} that only demonstrates robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

The other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation, like UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi and thus are limited in scalability to large spaces or ubiquitous deployment.
% \footnote{We also want to note that, while we have used WiFi as a sensor in \name, \name's design is modular enough to easily scale to other RF-technologies.}.

% \todo{Aditya-- can you check the accuracy in technicalities in the following:}
Finally, there also exist a few other series of works called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel} that try to reduce the memory usage and processing time by running two different optimizations for mapping and pose-estimation in parallel which tend to drift in real-time while they are corrected post-facto. There are also a few works that perform Decentralized SLAM that off-loads the memory and time intensive loop closure detection and map updates to the cloud~\cite{nandikolla2021navigation,kiss2019gps}. We later detail on how even such works can benefit from \name's design and implementation.

\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient.

To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Noisy and sparse WiFi Measurements:} As demonstrated in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, WiFi as a SLAM sensor can provide accurate global corrections without the need of loop closure detection for end-to-end optimization. Although for real-time navigation of the robot, WiFi bearings measured from 2D-FFT are too noisy, ambiguous and compute-intensive.

\noindent\textbf{(b) Unknown WiFi anchors:} Secondly, we do not assume any apriori knowledge of the WiFi access points(APs) in the environments, including their locations, and we need to map the APs accurately. One can initialize the APs at the origin but all the APs do not have measurements with the WiFi radio on the robot leading to ill-defined optimization. Thus, optimal initialization of WiFi AP's in imperative for the stability of the SLAM optimization.
    
\noindent \textbf{(c) Naive Sensor Fusion:} One can solve the problem of noisy WiFi measurements by integrating more reliable existing Visual or LiDAR sensors. A naive integration of bearings into existing VIO would make the system complex, as the WiFi sensors are more noisier than camera for local pose corrections, leading to the system to completely neglect WiFi measurements or worse, make incorrect local-corrections.

\subsection{\name SLAM's Solution}
\todo{should we call this statement of contributions?}
To overcome these challenges, the core idea for \name SLAM's design relies on two important aspects (a) Visual sensors are accurate, does not require a lot of memory and are real-time for local drift corrections and feature mapping, and (b) WiFi sensors while sparse and noisy in smaller areas, have accurate global perspective to correct for the global drifts of the robot. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots. \todo{careful to not just call A+B... }

\noindent\textbf{(a) Accurate WiFi Measurements:} We have seen from existing works like $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} and WSR~\cite{jadhav2020wsr} that bearing measurements are robust and accurate for WiFi based SLAM algorithms. Unfortunately, these algorithms have more noisier bearings than are tolerable for real-time robot navigation. 
While some existing bearing measurement algorithms like MUSIC and SpotFi~\cite{spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide real-time AoA measurements at the rate needed for pose estimation.
Thus in \name SLAM we employ a low-compute algorithm, which reduces erroneous measurements by attenuating noisy components in the signal, by combining the WiFi channel measurements across time and finding its principle component which we call PC-CSI. 
The PC-CSI can then be fed to a FFT transform~\cite{arun2022p2slam}, for more reliable and real-time bearing measurements.

\noindent\textbf{(b) Accurate mapping of WiFi anchors:} For accurate navigation of the robot, the WiFi APs also need to be mapped accurately in the environment. As discussed, a naive initialization can lead to an unstable optimization and higher compute. 
Thus, to enable dynamically map of the WiFi APs as they are seen for the first time, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an inflection point in the change of signal strength measured for that AP. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

\noindent\textbf{(c) Dual Graph:} Finally, to make best use of the WiFi and visual sensors, \name proposes to construct a Visual WiFi Dual graph system. We utilize  VIO (or LIO) systems like Kimera~\cite{rosinol2021kimera} (Cartographer~\cite{cartographer}) to provide local odometer measurements without performing any global loop closure detection. These odometer measurements are fused with WiFi measurements from multiple access points in the environment by our WiFi graph, built on open-sourced iSAM~\cite{gtsam} backend. Alternatively, visual fiducial markers ~\cite{opencvaruco} that can also act as global constant markers that can help in global corrections with minimal memory overhead. Though, unlike WiFi sensors, visual markers can be easily blocked in a dynamic environment making them less reliable. \todo{add layering}

Finally, we have deployed our \name SLAM robot system on a Turtlebot2~\cite{turtlebot2} that is equipped with a Hokuyo LiDAR,~\cite{hoku} and Intel d455 RGB-D camera with an in-built IMU for deploying cartographer~\cite{cartographer}, and Kimera~\cite{rosinol2021kimera}. We also deploy a 4 antenna WiFi sensor~\cite{blanco2021accurate}. We have deployed this robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs along with three of our open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of 108 minutes covering a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera system with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of 0.72 GB for a 25 min run, wherein Kimera needs 2.82 GB. Thus \name SLAM demonstrates accurate, real-time and low-memory SLAM. Further note that we disabled visualization on Kimera to only account for the memory consumption by the optimization backend and keyframe storage. 

==> intro/intro-4.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Diverse indoor applications~\cite{melenbrink2020site,lastmile} are increasingly interested in deploying autonomous robot systems.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. Current state-of-the-art SLAM systems\todo{may be connect with robot or SLAM from previous sentence} like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Over time, however, fusing these measurements accrues drift in the robot poses predicted due to sensors errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{xxx} which correlate the current observation with a stored dictionary of past observation.

\todo{may be a sentence claiming loop-closures requires high computational resources and memory resources then the two sentence below explaining that point.}
But as we look towards deploying SLAM systems to larger spaces, performing adequate loop closures demands the storage of a larger dictionary of unique observation made in the environment. Furthermore, the feature matching needed to detect loop closures and performing the adequate corrections over the entire trajectory in real time demands higher computational resources. \todo{may be a connecting sentence communication} Thus, to allow for accurate, scalable and real-time SLAM systems, it is imperative to reduce memory and computational requirements of SLAM systems. Additionally, in monotonous or visually dynamic environment, incorrect feature matching can be detrimental to robot pose prediction. Hence, we ask and answer the question what if we can remove these memory and compute intensive loop-closures? 


% But performing loop closures comes at a trade-off of higher memory and compute consumption. 
% Specifically, the rate of memory consumption of the SLAM system running on the robot would be alarmingly high for systems with dense features (typical VIOs). (b) On the other hand, systems with sparse features, the compute starts to get occupied to enable complex feature matching algorithms (typical single plane LIOs). Additionally, since these features are not uniquely identifiable in bad lighting conditions or monotonous environments~\cite{deng2018feature,zhang2020comparison}, loop-closure detection failure can further detrimentally impact the quality of the SLAM output.

% This trade-off arising from the need of loop-closure detection limits the available memory and/or compute for the other applications and processes, which would lead the robot to start malfunctioning or becoming extremely slow.


\todo{this paragraph is a bit weak and slow... make it more punchy, it is long and un-clear}As the first step, we observe that loop-closures aid in re-identifying previously visited spaces and re-aligns the robot to be consistent with past pose predictions. Alternatively, if the environment could instead inform the robot of it's inconsistency, we could circumvent loop-closures entirely. To allow this, we can incorporate static landmarks in the environment with unique ID's and provide the robot definitive anchors in the environment. Interestingly, these visual landmarks exist~\cite{opencvaruco} and are commonly deployed in environments where loop-closures are insufficient to correct for drifts. Unfortunately, these visual landmarks fail in dynamic conditions, in situations of blockage and can be inconvenient to deploy in some environments. To circumvent these challenges and provide robust unqiue landmarks, we find an alternative in the form of WiFi access points~\cite{arun2022p2slam} and develop \name which integrates WiFi measurements with visual sensors for real-time SLAM. 

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem is that, since the robot must always have memories of everything it has seen on hand, memory consumption is linear in the length of the robot's trajectory, meaning that the even most efficient representations will eventually run out of space given a large or complex enough environment.

As noted earlier, in a past work~\cite{arun2022p2slam} we demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and thus was not suitable for real-time operation on a robot.
There have also been other works like WSR~\cite{jadhav2020wsr} that demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi, meaning they are limited in applicability to deployments without pre-existing localization infrastructure.
% \footnote{We also want to note that, while we have used WiFi as a sensor in \name, \name's design is modular enough to easily scale to other RF-technologies.}.

% \todo{Aditya-- can you check the accuracy in technicalities in the following:}
% Finally, there also exist a few other series of works called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel} that try to reduce the memory usage and processing time by running two different optimizations for mapping and pose-estimation in parallel which tend to drift in real-time while they are corrected post-facto. There are also a few works that perform Decentralized SLAM that off-loads the memory and time intensive loop closure detection and map updates to the cloud~\cite{nandikolla2021navigation,kiss2019gps}. We later detail on how even such works can benefit from \name's design and implementation.

\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient. To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Time-consuming, noisy and sparse WiFi Measurements:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use super-resolution algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain the low-noise bearing measurements needed for online operation. However, because these algorithms require high compute in order to differentiate signal paths, they are not suitable for deployment on devices with low compute capabilities or at large scales.

\todo{justify this instability}
\noindent \textbf{(b) Naive Sensor Fusion:} WiFi-bearings can provide robust corrections to account for global drift. But a naive integration of these WiFi-bearings into existing VIO would make the system difficult to optimize, as the WiFi sensors measurements are more noisier than cameras for local pose corrections.

\noindent\textbf{(c) Unknown WiFi anchors:} Finally, the locations of the AP's are unknown in the environment and need to be dynamically added and mapped during the operation of the robot. A poor initialization of the AP's position estimate can lead to it falling into a local minimum or the estimate becoming numerically unstable or indeterminate.

\subsection{\name's Contributions}
To overcome these challenges, the \name's core design relies on two important aspects: (a) Visual sensors can provide accurate and real-time odometry measurements at a local scale, and (b) WiFi sensors can correct global drifts in odometry, as each measurement comes pre-labeled with a MAC address, meaning no cross-correlation of measurements needs to be done. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots. \todo{careful to not just call A+B... }

\noindent\textbf{(a) Accurate WiFi Measurements:} 
We design a low-compute PCA-based WiFi-bearing estimation algorithm which can estimate the true path a WiFi signal traveled without having to search across all paths or do any super-resolution. 

\noindent\textbf{(b) Dual Graph:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual WiFi Dual graph system. We utilize  VIO~\cite{rosinol2021kimera} or LIO~\cite{cartographer} to provide local odometer measurements (without global loop closure detection). These local odometer measurements are fused with WiFi measurements from access points in the environment by our WiFi graph, built on open-sourced iSAM~\cite{gtsam} backend. We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Accurate mapping of WiFi anchors:} To dynamically map the WiFi APs as they are seen for the first time, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an inflection point in the change of signal strength measured for that AP. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

To verify our claims, we have deployed \name on a Turtlebot2~\cite{turtlebot2} that is equipped with a Hokuyo LiDAR~\cite{hoku} and Intel d455 RGB-D camera~\cite{realsense} with an in-built IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also deploy a 4 antenna WiFi sensor~\cite{blanco2021accurate}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs in addition with three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes covering a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} systems with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB. Additionally, \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name SLAM demonstrates accurate, low-compute and low-memory SLAM. Further note that we disabled visualization on Kimera and Cartographer to only account for the memory and computation by the optimization backend and keyframe storage. 

==> intro/intro-5.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications~\cite{melenbrink2020site,lastmile} are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks for the basis to enable real-time navigation and generate a human-readable map of the robot's environment. \todo{may be connect with robot or SLAM from previous sentence}
And most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Over time, however, fusing these measurements accrues drift in the robot poses predicted due to sensors errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{xxx} which correlate the current observation with a stored dictionary of past observation.

\todo{may be a sentence claiming loop-closures requires high computational resources and memory resources then the two sentence below explaining that point.}

But as we look towards deploying SLAM systems to larger spaces, performing adequate loop closures demands the storage of a larger dictionary of unique observation made in the environment. Furthermore, the feature matching needed to detect loop closures and performing the adequate corrections over the entire trajectory in real time demands higher computational resources.  Thus, to allow for accurate, scalable and real-time SLAM systems, it is imperative to reduce memory and computational requirements of SLAM systems and move away from compute and memory intensive loop closure algorithms~\cite{arshad2021role}. Additionally, in monotonous or visually dynamic environment, incorrect feature matching can be detrimental to robot pose prediction. Hence, we ask and answer the question what if we can remove these memory and compute intensive loop-closures? 


\todo{this paragraph is a bit weak and slow... make it more punchy, it is long and un-clear}

As the first step, we observe that loop-closures aid in re-identifying previously visited spaces and re-aligns the robot to be consistent with past pose predictions. Alternatively, if the environment could instead inform the robot of it's inconsistency, we could circumvent loop-closures entirely. \todo{this statement comes too early:}To allow this, we can incorporate static landmarks in the environment with unique ID's and provide the robot definitive anchors in the environment. Interestingly, these visual landmarks exist~\cite{opencvaruco} and are commonly deployed in environments where loop-closures are insufficient to correct for drifts. Unfortunately, these visual landmarks fail in dynamic conditions, in situations of blockage and can be inconvenient to deploy in some environments. To circumvent these challenges and provide robust unqiue landmarks, we find an alternative in the form of WiFi access points~\cite{arun2022p2slam} and develop \name which integrates WiFi measurements with visual sensors for real-time SLAM. 

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem is that, since the robot must always have memories of everything it has seen on hand, memory consumption is linear in the length of the robot's trajectory, meaning that the even most efficient representations will eventually run out of space given a large or complex enough environment.

As noted earlier, in a past work~\cite{arun2022p2slam} we demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and thus was not suitable for real-time operation on a robot.
There have also been other works like WSR~\cite{jadhav2020wsr} that demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi, meaning they are limited in applicability to deployments without pre-existing localization infrastructure.


\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient. To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Time-consuming, noisy and sparse WiFi Measurements:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use super-resolution algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain the low-noise bearing measurements needed for online operation. However, because these algorithms require high compute in order to differentiate signal paths, they are not suitable for deployment on devices with low compute capabilities or at large scales.

\noindent \textbf{(b) Naive Sensor Fusion:} WiFi-bearings can provide robust corrections to account for global drift. But a naive integration of these WiFi-bearings into existing VIO would make the system difficult to optimize, as the WiFi sensors measurements are more noisier than cameras for local pose corrections. This leads to indeterminancy of the factor graph and higher compute times. 

\noindent\textbf{(c) Unknown WiFi anchors:} Finally, the locations of the AP's are unknown in the environment and need to be dynamically added and mapped during the operation of the robot. A poor initialization of the AP's position estimate can lead to it falling into a local minimum or the estimate becoming numerically unstable or indeterminate.

\subsection{\name's Contributions}
To overcome these challenges, the \name's core design relies on two important aspects: (a) Visual sensors can provide accurate and real-time odometry measurements at a local scale, and (b) WiFi sensors can correct global drifts in odometry, as each measurement comes pre-labeled with a MAC address, meaning no cross-correlation of measurements needs to be done. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots. \todo{careful to not just call A+B... }

\noindent\textbf{(a) Accurate WiFi Measurements:} 
We design a low-compute PCA-based WiFi-bearing estimation algorithm which can estimate the true path a WiFi signal traveled without having to search across all paths or do any super-resolution. 

\noindent\textbf{(b) Dual Graph:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual WiFi Dual graph system. We utilize  VIO~\cite{rosinol2021kimera} or LIO~\cite{cartographer} to provide local odometer measurements (without global loop closure detection). These local odometer measurements are fused with WiFi measurements from access points in the environment by our WiFi graph, built on open-sourced iSAM~\cite{gtsam} backend. We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Accurate mapping of WiFi anchors:} To dynamically map the WiFi APs as they are seen for the first time, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an inflection point in the change of signal strength measured for that AP. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

To verify our claims, we have deployed \name on a Turtlebot2~\cite{turtlebot2} that is equipped with a Hokuyo LiDAR~\cite{hoku} and Intel d455 RGB-D camera~\cite{realsense} with an in-built IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also deploy a 4 antenna WiFi sensor~\cite{blanco2021accurate}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs in addition with three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes covering a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} systems with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB. Additionally, \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name SLAM demonstrates accurate, low-compute and low-memory SLAM. Further note that we disabled visualization on Kimera and Cartographer to only account for the memory and computation by the optimization backend and keyframe storage. 

==> intro/intro-6.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications~\cite{melenbrink2020site} are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks to enable real-time navigation and generate a human-readable map of the robot's environment.
And most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Over time, however, fusing these measurements accrues drift in the robot poses predicted due to sensors errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{arshad2021role} which correlate the current observation with a stored dictionary of past observation.

Unfortunately, these much-needed loop-closures are also the components of SLAM system that increase the memory and compute requirements for these robots.
That is, as we look towards deploying SLAM systems to larger spaces, performing adequate loop closures demands the storage of a larger dictionary of unique observations made during past traversal of the environment (memory usage). Furthermore, the feature matching needed to detect loop closures to perform adequate corrections over the entire trajectory in real time, demands running matching algorithm over a large database of past key points leading to high computational resources (cpu intensive). Thus, to allow for accurate, and easy to  scale real-time SLAM systems, it is imperative to reduce the memory and computational requirements of SLAM systems and possibly move away from compute and memory-intensive loop closure algorithms~\cite{arshad2021role}. Additionally, in a monotonous or visually dynamic environment, incorrect feature matching can be detrimental to robot pose prediction. Hence, we ask and answer the question what if we can remove these memory and compute intensive loop-closures? 
A key observation is that the only purpose of the memory and compute intense loop-closures is to aid in re-identifying previously visited spaces and re-align the robot to be consistent with past pose predictions. So, we tackle this issue in \name by developing a system that can smartly overcome the need for these loop-closures and mitigate the mo.
One way to do this is to incorporate static landmarks in the environment with unique ID's and provide the robot definitive anchors in the environment. Interestingly, these visual landmarks exist~\cite{opencvaruco} and are commonly deployed in environments where loop-closures are insufficient to correct for drifts. Unfortunately, these visual landmarks fail in dynamic conditions, in situations of blockage and can be inconvenient to deploy in some environments. To circumvent these challenges and provide robust unique landmarks, we find an alternative in WiFi-sensors measurements and develop \name which integrates them with visual sensors for accurate and real-time SLAM. 

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem is that, since the robot must always have memories of everything it has seen on hand, memory consumption is linear in the length of the robot's trajectory, meaning that the even most efficient representations will eventually run out of space given a large or complex enough environment.

As noted earlier, in a past work~\cite{arun2022p2slam} we demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and thus was not suitable for real-time operation on a robot.
There have also been other works like WSR~\cite{jadhav2020wsr} that demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi, meaning they are limited in applicability to deployments without pre-existing localization infrastructure.


\subsection{Problem Statement}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient. To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Time-consuming, noisy and sparse WiFi Measurements:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use super-resolution algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain the low-noise bearing measurements needed for online operation. However, because these algorithms require high compute in order to differentiate signal paths, they are not suitable for deployment on devices with low compute capabilities or at large scales.

\noindent \textbf{(b) Naive Sensor Fusion:} WiFi-bearings provide robust corrections to account for global drift. But a naive fusion of these bearings into existing VIO~\cite{rosinol2021kimera} would make the system difficult to optimize, as the WiFi sensors measurements are more noisier than cameras', for local pose corrections. This may lead to higher compute or an indeterminant factor graph. 

\noindent\textbf{(c) Unknown WiFi anchors:} Finally, the locations of the AP's are unknown in the environment and need to be dynamically added and mapped during the operation of the robot. A poor initialization of the AP's position estimate can lead to it falling into a local minimum or the estimate becoming numerically unstable or indeterminate.

\subsection{\name's Contributions}
To overcome these challenges, the \name's core design relies on two modules to function appropriately: (a) a Visual sensor module that can provide accurate and real-time odometry measurements at a local scale, and (b) and a WiFi sensor module that can in real-time correct global drifts in odometry. While $\mathrm{P^2}$SLAM shows that as each WiFi measurement comes pre-labeled with a MAC address, no cross-correlation of measurements needs to be done but it cannot perform real-time navigation~\cite{arun2022p2slam} and so cannot be deployed. Using these insights, \name SLAM makes following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Accurate WiFi Measurements:} 
We design a low-compute PCA-based WiFi-bearing estimation algorithm which can estimate the true path a WiFi signal traveled without having to search across all paths or do any super-resolution. 

\noindent\textbf{(b) Dual Graph:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual-WiFi Dual graph system. We utilize  VIO~\cite{rosinol2021kimera} or LIO~\cite{cartographer} to provide local odometer measurements (without global loop closure detection). These local odometer measurements are fused with WiFi measurements from access points in the environment by our WiFi graph, built on open-sourced iSAM~\cite{gtsam} backend. We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Accurate mapping of WiFi anchors:} To dynamically map the WiFi APs as they are seen for the first time, we track the signal strength of WiFi measurement to that AP and initialize the APs location to the bot's current location where we see an inflection point in the change of signal strength measured for that AP. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

To verify our claims, we have deployed \name on a ground robot Turtlebot2 platform that is equipped with a Hokuyo LiDAR and Intel d455 RGB-D camera with a built-in IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also deploy a 4 antenna WiFi channel sensor~\cite{nexmon:project}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs (with loop-closures turned off) in addition with three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes and a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} systems with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB. Additionally, \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average, showing \name can perform accurate, low-compute and low-memory SLAM. Further note that we disabled visualization tools on Kimera and Cartographer to only account for the memory and computate used by the optimization backend and keyframe storage.

==> intro/intro7.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks to enable real-time navigation and generate a human-readable map of the robot's environment.
To enable these applications, most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Over time, however, fusing these measurements accrues drift in the robot poses predicted due to sensors errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{arshad2021role} which correlate the current observation with a stored dictionary of past observations to ensure consistency of the robot's trajectory over long periods of time.

Unfortunately, these much-needed loop-closures are also weakest links in SLAM systems and increase the memory requirements and are compute intensive as they are not robust.
In a monotonous or visually dynamic environment, many false-positive loop closures can be detrimental to robot pose predictions. Furthermore, as we look towards deploying SLAM systems to larger spaces, performing loop closures demands the storage of an ever-larger dictionary of unique observations made during past traversal of the environment, demanding higher memory usage. Additionally, the feature matching needed to discover loop closures in real time demands running a cross-correlation algorithm over a large database of past key points leading to high compute requirements. Thus, to allow for accurate and scalable real-time SLAM systems, it is imperative to reduce their memory and compute requirements, and ideally move away from compute and memory-intensive loop closure algorithms~\cite{arshad2021role}.  Hence, we explore if these loop closures can be entirely removed while maintaining SLAM accuracy. 
% \todo{maybe saying "how to remove loop-closures while maintaining accuracies" might sound better?}
% \todo{should we make these two purpose eliminate loop closure and help monotonous envrionments?}

% \todo{From the how question above, maybe you can relate to saying that, "to be able to remove we first understand that loop-closures are only used for...". Then the WiFi part becomes more of a key observation in terms of robustly removing loop-closures.}
To develop a SLAM system without loop closures, we need to find an alternative method to re-identify previously visited spaces and make the current pose estimate consistent with past estimates in that space.
Incorporating static and \textit{uniquely identifiable} landmarks in the environment aids in re-identifying previously visited spaces. Furthermore, \textit{accurately mapping} their positions allows the robot to leverage these landmarks to anchor itself to the environment and hence circumvent loop closures. Various static landmarks which are identifiable by cameras~\cite{olson2011apriltag} or LiDARs~\cite{huang2021lidartag} have been deployed where loop closures are insufficient to correct for drifts.  
Unfortunately, these visual landmarks can fail in dynamic conditions, in situations of blockage, or in dynamic lighting conditions and are inconvenient or impossible to deploy in some environments. 

\todo{reword the following as Problem statement:}
\noindent\textbf{Problem Statement:} To circumvent these challenges in providing unique landmarks, in this work, we demonstrate that WiFi access points are a robust replacement to these visual landmarks and can aid in removing `loop-closures'. 
% To circumvent these challenges in providing unique landmarks, we find a better alternative in WiFi access points as these landmarks by making a key observation -- WiFi measurements are robust to the environmental changes which detrimentally affect these specialized landmarks. 
Hence, to capitalize on these WiFi sensors, we develop \name which integrates them with visual sensors for accurate and resource-efficient SLAM without relying on loop closures.

% \todo{tie it back to loop closures?}. 

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem is that, since the robot must always have memories of everything it has seen on hand, memory consumption is linear in the length of the robot's trajectory, meaning that the even most efficient representations will eventually run out of space given a large or complex enough environment.

In a past work~\cite{arun2022p2slam},   demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and thus was not suitable for real-time operation on a robot.
There have also been other works like WSR~\cite{jadhav2020wsr} that demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most of the other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are known to be unreliable in dynamic indoor scenarios~\cite{ma2019wifi}.

Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi, meaning they are limited in applicability to deployments without pre-existing localization infrastructure.


\subsection{Challenges}
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph (\name) SLAM", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it memory and compute efficient. To build \name, we need to surmount the following challenges:

\noindent\textbf{(a) Tradeoff between WiFi Measurement accuracy and compute:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use super-resolution algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain the low-noise bearing measurements needed for online operation. However, because these algorithms require high compute in order to differentiate signal paths, they are not suitable for deployment on devices with low compute capabilities or at large scales.

\todo{call it scalability? Compatibility? Bring out how we are actually not only solving loop-closures but also aiding the existing VIO/LIO systems to remove their `loop-closures' making existing works accurate with low-compute and memory.}
\noindent \textbf{(b) Naive Sensor Fusion:} Utilizing WiFi access points as landmarks provide robust corrections to account for global drift. But a naive fusion of these WiFi measurements into existing VIO~\cite{rosinol2021kimera} would make the system difficult to optimize, as they are more noisier than cameras' feature tracking for local pose corrections. This may lead to higher compute or an indeterminant factor graph. 

\todo{Strengthen the following: The AP location are not known, and adding them without a good prior would make the system instable needing heavy compute and worse making the system indeterminate.}
\noindent\textbf{(c) Unknown WiFi anchors:} Finally, the locations of the AP's are unknown in the environment and need to be dynamically added and mapped during the operation of the robot. A poor initialization of the AP's position estimate can lead to it falling into a local minimum or the estimate becoming numerically unstable or indeterminate.

\subsection{\name's Contributions}
To overcome these challenges, \name's core design relies on two modules to function appropriately: (a) a Visual sensor module that can provide accurate and real-time odometry measurements at a local scale, and (b) and a WiFi sensor module that can in real-time correct global drifts in odometry. 
Using these insights, we make the following contributions to enable accurate, real-time indoor navigation for robots.

% While $\mathrm{P^2}$SLAM shows that as each WiFi measurement comes pre-labeled with a MAC address, no cross-correlation of measurements needs to be done but it cannot perform real-time navigation~\cite{arun2022p2slam} and so cannot be deployed. 


\noindent\textbf{(a) Accurate WiFi Measurements:} 
We design a low-compute PCA-based WiFi-bearing estimation algorithm which can estimate the true path a WiFi signal traveled without having to search across all paths or do any super-resolution. 

\noindent\textbf{(b) Dual Graph:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual-WiFi Dual graph system. We utilize local odometry measurements (without global loop closure detection) extracted via inertial sensors and visual feature tracking. These local odometer measurements are then fused with WiFi measurements to tracking the WiFi landmarks in the environment by our WiFi graph. We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Accurate initialization of WiFi landmarks:} Finally, to dynamically map these WiFi landmarks as they are seen for the first time, we track the signal strength of WiFi measurement to that AP. Next, we initialize the APs location to the robot's current location when we see an inflection point in the change of signal strength measured. This allows us to initialize the AP at the closest point to it's true location and improves the convergence of the SLAM backend. 

To verify our claims, we have deployed \name on a ground robot Turtlebot2 platform that is equipped with a Hokuyo LiDAR and Intel d455 RGB-D camera with an in-built IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also deploy a 4 antenna WiFi sensor~\cite{nexmon:project}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs (with loop-closures turned off) in addition with three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes and a distance of $1625$ m. We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer} systems with loop-closures. While achieving the similar pose estimation accuracy \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB. Additionally, \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name SLAM demonstrates accurate, low-compute and low-memory SLAM. Further note that we disabled visualization on Kimera and Cartographer to only account for the memory and computation by the optimization backend and keyframe storage. 

==> intro/intro9.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

\todo{summarize loop closures quickly, talk about real-timeliness and working with existing works; combine 1st and 3rd para; talk abut making more systems work of smaller computers }
Diverse indoor applications are increasingly interested in deploying autonomous indoor robots.
These robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks to enable real-time navigation and to generate a human-readable map of the robot's environment.
To enable these applications, most state-of-the-art SLAM systems~\cite{Labb2018RTABMapAA, rosinol2021kimera, cartographer, mur2015orb} use visual (monocular or RGB-D cameras) and/or LiDAR sensors in tandem with odometry measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. 
Despite this fusion, error in the predicted trajectory increases over time due to accumulation of sensor errors. Fortunately, these drifts can be corrected with `loop closures'~\cite{arshad2021role} which correlate the current observation with a dictionary of past observations, ensuring self-consistency of the robot's estimated trajectory on a global scale.

Unfortunately, these much-needed loop-closures are also the weakest links in SLAM systems, as they increase the memory requirements, are compute intensive, and are not robust~\cite{arshad2021role}.
In particular, false-positive loop closures, common in monotonous or visually dynamic environments, are highly detrimental to robot pose predictions. Furthermore, as we scale to larger spaces, performing loop closures demands the storage of an ever-larger dictionary of unique observations, demanding higher memory usage. Consequently, the feature matching needed to discover loop closures in large spaces requires extensive search, leading to high compute requirements. Thus, for real-time SLAM systems to be both accurate and scalable, it is imperative they are resource-efficient. Hence, we explore if these resource consuming loop closures can be entirely removed while maintaining SLAM accuracy.

\todo{we don't technically do re-identification}
To develop a SLAM system without loop closures, we need to find an alternative method to re-identify previously visited spaces and make the current pose estimate consistent with past estimates in that space.
Incorporating static and \textit{uniquely identifiable} landmarks in the environment aids in re-identifying previously visited spaces. Furthermore, \textit{accurately mapping} their poses allows the robot to leverage these landmarks to anchor its estimate to the environment and circumvent loop closures. Accordingly, various static landmarks which are identifiable by cameras~\cite{olson2011apriltag} or LiDARs~\cite{huang2021lidartag} have been deployed where loop closures are insufficient to correct for drifts.  
Unfortunately, these visual landmarks can fail in situations of blockage or dynamic lighting conditions. Their deployment further scales poorly to large environments. 

\noindent\textbf{Goal:} Clearly, to deliver a resource-efficient and real-time SLAM system, we need to incorporate `uniquely identifiable' and `mappable' landmarks in our environments. These landmarks need to be robust in dynamic environments and easily scalable to large spaces.  

To achieve this goal, we demonstrate that WiFi access points are a robust replacement to these visual landmarks and can aid in removing `loop-closures'. We develop \name which integrates them with visual sensors for accurate and resource-efficient SLAM without relying on loop closures. \name is also readily scalable, as WiFi access points are already ubiquitously deployed in indoor environments making them a natural choice for a landmark.

\subsection{Literature Review}
Most existing Visual and LiDAR SLAM algorithms try to resolve memory issues in loop-closure detection and identification by: (a) optimizing key-frame and key-point detection~\cite{mur2015orb} to reduce the number of key-frames stored, or (b) using a smart representation, like bag-of-words~\cite{rosinol2021kimera} for efficient storage and retrieval. While these solutions reduce the amount of memory required per step, the underlying problem of the memory consumption being linear in the length of the robot's trajectory remains. This implies that even the most efficient representations will eventually run out of memory given a large or complex enough environment.

\todo{this takes away novelty here, don't force loop closure as much, but the timeliness}
Past work~\cite{arun2022p2slam} demonstrated accurate WiFi based SLAM, which has no need for loop closures as its WiFi measurements exist in a globally consistent reference frame, even if the positions of the anchors are unknown beforehand. However, it performed only an a-posteriori fusion of wheel odometry and WiFi measurements and cannot perform online robot operation.
There are also works like WSR~\cite{jadhav2020wsr}, which demonstrate robot reconnaissance using WiFi and not global indoor navigation. Most other existing WiFi-based SLAM systems~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi} depend only on WiFi RSSI readings which are unreliable in dynamic indoor scenarios~\cite{ma2019wifi} and require a-priori fingerprinting data for navigation.

\todo{this is deviating, maybe move it above after the goal para?} Other RF-sensor technologies that are used for localization which are shown to extend to robotic navigation include UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot}. However, these RF-sensors are \textbf{(a)} not as ubiquitously deployed limiting wider adoption or \textbf{(b)} have shorter ranges compared to WiFi limiting their scalability to large spaces. 

\subsection{Challenges}
\todo{convert to problem/solution format }
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual-graph", a dual-layered real-time SLAM system which overcomes the need of loop-closure detection making it resource efficient. To build \name, we surmount the following challenges:

\noindent\textbf{(a) Tradeoff between WiFi measurement accuracy and compute:} We have seen from existing works~\cite{arun2022p2slam, jadhav2020wsr, zhang2020robot} that bearing measurements extracted from the WiFi Channel-state estimate (CSI) are viable for WiFi based SLAM algorithms. These systems use \textit{super-resolution} algorithms like MUSIC and SpotFi~\cite{spotfi} to obtain low-noise bearing measurements needed for online operation. However, this accuracy comes at the cost of computation, and are not suitable for realt-time deployment on devices with low compute capabilities.

% \todo{call it scalability? Compatibility? Bring out how we are actually not only solving loop-closures but also aiding the existing VIO/LIO systems to remove their `loop-closures' making existing works accurate with low-compute and memory.}
\todo{single factor graph does not make sense, why is multiple bad?}
\noindent \textbf{(b) Infeasible sensor fusion via a single factor graph:} Most sensor-fusion techniques rely on incorporating measurements within factor graphs~\cite{gtsam} to optimally solve for the SLAM problem. Unfortunately, WiFi is subject to outlier measurements due to transient reflections, so immediate incorporation of every measurement can hurt the local state estimate. Hence, a simple integration of WiFi landmarks into the same framework as a Visual/LiDAR sensor~\cite{rosinol2021kimera} can lead to a poor estimate of the recent robot poses due to local inconsistency in WiFi measurements.
% Utilizing WiFi access points as landmarks provide robust corrections to account for global drift. But a naive fusion of these WiFi measurements into existing VIO~\cite{rosinol2021kimera} would make the system difficult to optimize, as they are more noisier than cameras' feature tracking for local pose corrections. This may lead to higher compute or an indeterminant factor graph. 

% \todo{Strengthen the following: The AP location are not known, and adding them without a good prior would make the system instable needing heavy compute and worse making the system indeterminate.}
\noindent\textbf{(c) Initialization of Unknown WiFi anchors:} As new landmarks, visual or WiFi-based, are discovered, they need to be accurately placed in the map to ensure stable convergence of the factor graph. 
This task is easy in the case of visual markers'~\cite{olson2011apriltag, huang2021lidartag} owing to the pixel-scale accuracy of cameras and LiDARs. Unfortunately, the poorer resolution offered by WiFi measurements makes initialization of the AP's position estimate in the environment nontrivial. A poor initialization can lead to the non-optimal state estimate or worse, an indeterminacy in the solution. 

\subsection{\name's Contributions}
\todo{mention what VIO contains, the sensors it utilizes}
To overcome these challenges, \name deploys a bifurcated design: (a) a third-party visual-inertial odometry (VIO) module that can provide accurate and real-time odometry measurements at a local scale, and (b) and a WiFi sensor module that can plugs into an existing VIO system and performs online correction of global drifts.
Using these insights, we make the following contributions to enable accurate, real-time indoor navigation for robots.

\noindent\textbf{(a) Accurate and compute-efficient WiFi Measurements:} 
\name breaks away from the accuracy-compute tradeoff by designing a PCA-based WiFi Bearing (PCAB) estimation algorithm. By adequately combining WiFi measurements over time to suppress noise, PCAB circumvents compute intensive super resolution algorithms whilst delivering accurate and real-time bearing estimates.

\noindent\textbf{(b) Extensible dual graph optimization:} To make best use of the WiFi and visual sensors, \name proposes to construct a Visual-WiFi Dual graph system. We utilize local odometry measurements (without global loop closure detection) extracted via inertial sensors and visual feature tracking. These local odometry measurements are then fused with WiFi measurements to track the WiFi landmarks in the environment by our WiFi graph. This dual-graph approach further allows robots to plug-and-play \name into the existing Visual/LiDAR SLAM systems whilst reducing their compute and memory consumption. 
% We further note that this dual layered approach allows for further independent development of these Visual and WiFi-based SLAM algorithms.

\noindent\textbf{(c) Smart initialization of WiFi landmarks:} Finally, to dynamically map these WiFi landmarks when they are first observed, the robot tracks the strength of the WiFi signal from the access point (AP). Next, we initialize the APs location close to the robot's current location when we see an inflection point in the change of signal strength measured. This allows us to initialize the AP close to its true location, which improves the convergence of the factor graph. 

\todo{too many details and no takeaway, bring in abstract}
\todo{add some system level contributions; like cartographer could not be run on rpi; increases the run time of kimera on rpi due to memory savings etc.}
To verify our claims, we have deployed \name on a ground robot TurtleBot2 platform that is equipped with a Hokuyo LiDAR and Intel Realsense D455 RGB-D camera with a built-in IMU for deploying cartographer~\cite{cartographer} and Kimera~\cite{rosinol2021kimera} respectively. We also equip it with a 4 antenna WiFi radio~\cite{nexmon:project}. We deploy the robot in one large environment to collect data for demonstrating \name's compatibility with Kimera's VIO outputs (with loop-closures turned off), \textit{in addition} to three open-sourced datasets~\cite{arun2022p2slam} that we use to demonstrate \name's deployability with LiDAR-inertial odometry (LIO) from Cartographer. Across these deployments the robot traverses for an overall time of $108$ minutes and a distance of $1625$ m. 
\todo{show that this works on COTS devices, does not come out}
We show that \name achieves a median translation error of $70.8$ cm and a median orientation error of $2.6^{\circ}$, on par with the state-of-the-art Kimera~\cite{rosinol2021kimera} and Cartographer~\cite{cartographer}. While achieving a similar navigation accuracy: (a) \name only needs a total of $0.72$ GB for a $25$ minute run, wherein Kimera needs $2.82$ GB, (b) \name utilizes on average $0.72$ fraction of single core of CPU whereas Cartographer utilizes over $3.2$ cores of the CPU on average. Thus \name demonstrates accurate, low-compute and low-memory SLAM.  


==> intro/intros_old/intro1.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

A strong need for automation in various industries spanning hospitality to security has led to an increased adoption of robots capable of autonomous, reliable and safe indoor navigation. The trend kick-started by the early adoption of automated vacuum cleaners has grown many-fold to use these robots for monitoring security in office spaces, serving patrons at restaurants and moving large equipment in hospitals. The autonomy, reliability and safety these robots boast is owed to the suite of sensors they use. Most autonomous robots can be commonly spotted sporting 
1. a LiDAR at the top to provide a 360-degree view, 
2. a stereo/RGBD camera facing forward to provide a detailed 3D-map, 
3. bumper sensors to avoid catastrophic collisions,
4. odometry sensors (wheel encoder and IMU) to provide high-resolution odometry data, and
5. GPS/GNSS to aid in locating the robot (outdoor only) in a global frame. 
The data from these sensors are expertly fused taking into consideration each sensors reliability within a back-end optimization framework to generate an accurate estimate of the robot's location and its relation to the environment around it. The fusion of these different sensing modalities provides a very robust solution for autonomous navigation for robots.

% let's see how good sensor fusion works; explain landmarks, features, loop closure in few sentences...
To achieve autonomous navigation, the first key step is for the robot to build a map of it's environment and localize itself within this map in real time. 
Furthermore, this map should consist of rich contextual data -- labels of room numbers, descriptions of spaces, markings for various exits and entrances of buildings. 
This problem is commonly called Simultaneous Localization and Mapping (SLAM). 
In a two-step process, which involves first extracting and tracking the characteristic features from visual sensors, and second, combining the data from these sensors with odometry, the robot can build an accurate map and localize itself within this map. The characteristic features (\textit{landmarks}) extracted generally include corners or edges in Camera images or LiDAR scans. Tracking these features provides corrections to errors accumulated by odometry sensors, and saving some of the salient features helps the robot recognize and create additional constraints (\textit{loop-closures}) with previously visited places. Through this two-step process, robots can effectively navigate the strengths and weaknesses of individual sensors to solve the SLAM problem.

% but this fails in monotonous envs ...\todo{because of the same reasons we have mentioned in P2SLAM}
Unfortunately, in indoor environments we observe gaps left behind this common suite of sensors generally employed on robots. LiDAR's, although great in providing an accurate point cloud of an environment, fail in environments with little structural features, like long corridors or spaces larger than the field of view of the LiDAR. Furthermore, they are expensive, bulky and power hungry. Stereo or RGBD cameras offer an advantage over LiDAR's in that they allow for finer feature detection. For example, a long corridor adorned with posters and paintings provide robust and recognizable features to track against. Unfortunately, motion blur, dynamic lighting conditions and monotonous visual environments can all lead to feature tracking failure and even false positive loop closure hypothesis.
Furthermore, viable distances to obtain accurate depth from RGBD/Stereo sensor range from \todo{xx} m - \todo{xx} m, making them unusable in large spaces. 
Discounting the LiDAR's and cameras in these challenging environments leaves us with two remaining sensors -- odometry sensors and GPS. A combination of wheel encoders and IMU's provide accurate change in position over \todo{a local region and time}
% a period of few minutes. 
Unfortunately, lacking the \todo{global} correction provided by visual sensors, these odometry sensors can accrue large drifts, in the order of many tens of meters, when traversing large distances of hundreds of meters. In outdoor environments, we have the advantage of falling back on GPS location information, accurate to a few meters, to correct for these large drifts in odometry \todo{at a global scale}. Unfortunately, this is not the case in indoor environments, where GPS information is scantly available. This leaves an open problem for autonomous navigation for indoor robotics -- what is the best sensor we could incorporate to fill in the gaps left by these multitude of sensors? 

% bring up and kill other sensors, distill to wifi, rebuff it after a better lit review ...
To answer this pressing question, we can in fact take inspiration from GPS. Using a network of satellites, GPS can position a GPS-capable device to within a few meters with a global frame of reference. This can help to correct for drifts accumulated due to odometry and incorrect measurements from visual sensors \todo{within the local frames}. In this vein, we observe that an alternative signal is abundant indoors -- RF-signals like Bluetooth, Ultrawide-band (UWB) or WiFi. RF-based sensing can provide, in a loose sense, replace GPS and many recent works have proposed the use RF-based sensing to fill the gaps left by visual sensors. VIRAL SLAM~\cite{nguyen2021viral} uses UWB based ranging in conjunction with LiDAR's, cameras and IMU's to develop a tightly coupled and robust 3D drone based localization and mapping. \todo{not strong enough: Unfortunately, the deployment of various UWB anchors in the environment limits the adoption of this solution}. \todo{kill radar: Why?} The systems proposed in \cite{sato2019rapid, jadidi2018radio} use range information extracted from BLE's received signal strength to correct for drifts accrued by the onboard IMU. Unfortunately, RSSI-based systems have been proven to be inadequate to changing environment conditions and hence act as a poor proxy to range. RFly~\cite{ma2017drone} takes advantage of  RFID tags attached in the environment as robust landmarks, and in conjunction with RFID readers deployed in the environment, jointly estimates the location of a drone and these RFID tags. In a similar vein, Rover~\cite{zhang2020robot} uses WiFi backscatter tags placed in the environment to jointly estimate the location of the robot and tags. Unfortunately, these tags have small range and these systems would require a dense deployment of tags to work, scaling poorly to large environments and requiring a high cost of deployment. The final RF based sensing briefly touched upon before is WiFi. It provides inherent advantages due to its long range and ubiquitous deployment both in the environment and on most robots. 

% WiFi alone cannot give us the map of the environment or a physical representation of a map or context
Keeping these advantages in mind, many systems have been proposed incorporating WiFi sensors within SLAM, ranging from aiding loop closure~\cite{hashemifar2019augmenting, liu2019collaborative} or incorporating them as range~\cite{huang2011efficient,ferris2007wifi} and bearing sensor~\cite{xxx}. Unfortunately, the systems in \cite{hashemifar2019augmenting, liu2019collaborative} and \cite{ huang2011efficient,ferris2007wifi} utilize RSSI for fingerprinting or as a proxy for range respectively and hence lack robustness in dynamic environments. While, P2SLAM~\cite{xxx}, incorporating bearings extracted from CSI~\cite{ayyalasomayajula2018bloc}, is more robust to dynamic environments, it does not tightly fuse with visual sensors, and hence its locations lack contextual information with respect to a map. \name seeks to solve this problem by showcasing a system which tightly couples visual landmarks from a monocular camera and readily deploys in any unknown environment. The key deliverable for \name is to provide an end-to-end sensing solution (WiFi + monocular camera, in conjunction with odometry sensors), which furnishes context-rich location information in real-time without requiring any prior information about the environment. \name achieves this by incorporating WiFi as a bearing sensor~\cite{xxx}, employing the feature tracker from VINS-MONO~\cite{qin2018vins} and fusing odometry from a combination of a wheel encoder and IMU with an open-sourced GraphSLAM framework~\cite{gtsam}. Furthermore, we showcase our system with a simple application which builds a map labelled with room numbers and autonomously navigates to a given room number to deliver a package. 

% but there are problems to implementing this...
But there are three key problems which \name seeks to solve to enable dense \underline{V}isual \underline{I}nertial \underline{O}dometry with Wi\underline{Fi} possible. 
\begin{itemize}
    \item \textbf{Accurate AoA measurements:} Movement of the robot and limited knowledge of antenna placements on the access points (AP) deployed in the environment reduces the accuracy of the angle of arrival measured at the robot. \name observes that for each frequency and packet, extracting the strongest principal component helps to reduce non-idealities introduced by the robots velocity and vibration and accurate average across multiple transmit antenna. In this vein, \name uses an SVD-FFT algorithm to accurate estimate the angle of arrival on the robot (Sec.~\ref{sec:xxx}).
    \item \textbf{2.5D:} AP's are generally deployed higher than the robot's WiFi receiver. This implies we need to estimate both the azimuth and polar angle of arrival (3D-AoA). Unfortunately, with four or fewer antennas~\footnote{Most commercially available WiFi receivers come with only four or fewer antennas~\cite{quantenna, halperin2011tool, gringoli2019free}}, measuring 3D-AoA is very difficult due to reduced resolution. \name overcomes this by observing that the measured angle of arrival of a signal impinging from a higher elevation lies on the inclined plane connecting the AP and the robot, oriented according the heading of the robot. This observation allows \name to extract a single inclined-AoA from a linear antenna array and incorporate these measurements within GraphSLAM~\cite{gtsam} by defining a new measurement factor (Sec.~\cite{xxx}).
    \item \textbf{Half-plane Ambiguity:} Using a linear antenna array creates an ambiguity in the incline-AoA measured in the $360^\circ$ search-space. Using MH-iSAM2\cite{hsiao2019mh}, \name elegantly resolves this ambiguity by incorporating the multiple hypothesis within GraphSLAM and prunes the incorrect hypothesis in the future when more measurements are available (Sec.~\cite{xxx}).
\end{itemize}

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publically available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry. 

% we make this solution possible by ... efficiently fusing WiFi and camera for their strong suits, where our system relies on WiFi majorly for it's localization and tracking purposes and camera for it's map building and optimal and safe navigation purposes


% with \name, we implement and observe the following ...solutions which make realizing low-cost, robust indoor navigation robots a reality



% \subsection{Storyline}
% WiFi+camera with simplistic sensors, and plug them for the robot
% Monocular cameras are not sufficient within themselves
% So people have moved to stereo-vision and LiDAR
% Under 50\$ we can give you context based mapping with robust localization.

==> intro/intros_old/intro10.tex <==


% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholder.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features
%Thus, existing Visual SLAM systems are not light-weight and require extensive compute and memory resources to operate in real time, 
hindering their deployment in the real world~\cite{semenova2022quantitative}. 
However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous `Localization' and `Mapping' that is compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm which is memory and compute efficient and scalable. \name SLAM's  key insight is to eliminate memory intensive storage and computationally expensive correlation operations over the past measurement. \name system/robot consists of a WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. These pose estimates are then fed to \name's visual layer as shown in Figure~\ref{fig:intro-fig}, used by \name visual layer to label visual data with a pose.  
Since Wi-Fi pose measurements do not accrue drift over time, unlike standard visual SLAM algorithms, \name visual SLAM does not need to cross-correlate measurements across time to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.
While \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method generalizes to other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or next gen 5G femto-cell implementations~\cite{5g}. 
% call out real-time


Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with a clear interface of sharing of pose estimation from WiFi layer, to enable visual layers for the environment mapping. Such layering would bring the advantages of networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled, it would enable researchers in wireless sensing and visual SLAM domain to improve the individual algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm. 
%each layer can improved by themselves and such improvement would improve overall performance    
%above paragraph: emphasize no AP priors

% This abstraction of the complementary pose estimation WiFi SLAM, and the environment mapping Visual SLAM layers has advantages as in networking layer abstractions~\cite{session1994it5}.
% That is both the pose estimation layer and the mapping layer can be optimized within themselves without effecting the other layer's performance.
% For example, while we use WiFi-sensor for \name's implementation due to its widespread deployment in indoors, other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative sensors depending on the use case.

% figure: robot, rf layer -> visual layer
%Design ideas behind dual-graph (bring up performance), can use more than just Wi-Fi.

However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi localization solutions and feeding them into existing Visual SLAM algorithms.
We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free pose estimates from the Wi-Fi layer to be robust and real-time. To get these pose estimates from the Wi-Fi-layer, we employ Angle of Arrival (AoA) based localization~\cite{spotfi,jadhav2020wsr,arun2022p2slam,ayyalasomayajula2018bloc}, due to its widespread use.
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these systems use compute intensive super-resolution algorithms, which cannot provide AoA measurements at the rate needed for real time pose estimation.
%I would be cautious about bragging too much about svdfft, it is not a new algorithm.
To solve this, in \name we employ a [] algorithm, borrowing intuition from MUSIC~\cite{schmidtmusic,spotfi}, which both smooths erroneous measurements and attenuates multipath components in the signal. This smoothed CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. We use this method to measure AoA between the robot and Wi-Fi access points in the environment. However, this alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we cannot assume access point locations are known a priori.

\noindent\textbf{Unknown Wi-Fi Access Point Locations:} GraphSLAM~\cite{gtsam} is well known to jointly solve for multi-variate optimization as long as these variable are connected by some measurements.
So we define the Wi-Fi graph with the Odometry measurements connecting two continuous robot poses, and the Wi-Fi AoA measurements connecting the robot's current pose with each AP's position the AoA corresponds to. 
Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, we need to provide initial values to variables in question. 
While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. 
To overcome this issue, a naive solution can be to initialize all the AP locations at the origin. 
This is not an issue when the AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. 
However, when few measurements constrain the AP's pose, as is the case when the robot first traverses the environment for the real time, the optimizer is poorly conditioned. 
To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) proximity sensing~\cite{ez,zee}.
That is we initialize the location of the Wi-Fi AP at the time instance when the RSSI measured for a given access point is a local maxima along the path taken.

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Finally, the optimized robot poses generated by the Wi-Fi graph need to update the robot poses in the camera graph in real-time.
Unfortunately, if the already traversed robot poses are getting large corrections very frequently, it would result in large and frequent feature map corrections in the camera graph as well, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made.
These accumulated corrections are only pushed to the Camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.


These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We extract widely used Shi-Tomasi features~\cite{shi1994good} for the camera sensor using the opensourced VINS-MONO feature tracker~\cite{qin2018vins}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> intro/intros_old/intro11.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholder.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment, it would construct a 'loop closure'.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features.
%Thus, existing Visual SLAM systems are not light-weight and require extensive compute and memory resources to operate in real time, 
hindering their deployment in the real world~\cite{semenova2022quantitative}. However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous `Localization' and `Mapping' that is compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm which is memory and compute efficient and scalable. \name's SLAM key insight is to eliminate  memory intensive storage and computationally expensive correlation over the past measurement, essentialy develop a loop-closure free SLAM. \name system/robot consists of has WiFi radio, which is fed to a Wi-Fi sensing layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. These pose estimates are then fed to \name's visual layer as shown in Figure~\ref{fig:intro-fig}, used by visual layer to label visual data with a pose.  
Since Wi-Fi pose measurements do not accrue drift over time, unlike standard visual SLAM algorithms, \name visual SLAM does not need to cross-correlate measurements across time to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.
While \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method generalizes to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance}. 

Additionally, \name presents a layered abstraction for both WiFi layaer and Visual SLAM layer, with a clear interface of sharing of pose estimation from WiFi layer, to enable visual layers for the environment mapping. Such layering would bring the advantages of networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled, it would enable researchers in wireless sensing and visual SLAM domain to improve the individual algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm. %each layer can improved by themselves and such improvement would improve overall performance    
%above paragraph: emphasize no AP priors

% This abstraction of the complementary pose estimation WiFi SLAM, and the environment mapping Visual SLAM layers has advantages as in networking layer abstractions~\cite{session1994it5}.
% That is both the pose estimation layer and the mapping layer can be optimized within themselves without effecting the other layer's performance.
% For example, while we use WiFi-sensor for \name's implementation due to its widespread deployment in indoors, other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative sensors depending on the use case.

% figure: robot, rf layer -> visual layer
%Design ideas behind dual-graph (bring up performance), can use more than just Wi-Fi.

However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi sensing solutions and feeding them into existing Visual SLAM algorithms.
We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free robot pose estimates from the Wi-Fi layer to be robust and real-time. To get these pose estimates from the Wi-Fi-layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve WiFi-layer pose. %Extracting angle-of-arrival has been studied extensively in literature, due to use of those in WiFi localization~\cite{spotfi,jadhav2020wsr,arun2022p2slam,ayyalasomayajula2018bloc}. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use compute intensive super-resolution algorithms, which cannot provide compute efficient AoA measurements at the rate needed for real time pose estimation.
%I would be cautious about bragging too much about svdfft, it is not a new algorithm.
To solve this, in \name we employ a low-compute algorithm, which both smooths erroneous measurements and attenuates multipath components in the signal, by combining the CSI across time. The smoothed CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points. 

\noindent\textbf{Unknown Wi-Fi Access Point Locations:}
An obvious idea would be to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization, which includes WiFi-AP locations. Specifically, we define the Wi-Fi graph with the robot side AoA measurements from different APs and concurrent odometry measurements, with robot pose and AP's location as variables. %connecting two continuous robot poses, and the Wi-Fi AoA measurements connecting the robot's current pose with each AP's position the AoA corresponds to. 
Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, initial values to variables are extreme importance to lead the optimizer in a trajectory to solve the problem. 
While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. Furthermore, arbitrary initializing AP's locations would work only when AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. 
However, to be compute efficient with a few measurements and constrain the AP's pose, as is the case when the robot in real-time maps the environment, the optimizer is poorly conditioned for AP's location. 
To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) as proximity sensing~\cite{ez,zee} to initialize the location of WiFi AP. The location of the Wi-Fi AP is initialized with robot pose at the time instance when the RSSI measured for a given access point is a local maxima along the path taken. 

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Finally, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As robot moves, the WiFi graph continues to optimize its previous robot poses. A continuous updates of already traversed robot poses to the camera graph, would trigger large corrections and those too very frequently, and result in large and frequent feature map corrections, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made. The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.


These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We extract widely used Shi-Tomasi features~\cite{shi1994good} for the camera sensor using the opensourced VINS-MONO feature tracker~\cite{qin2018vins}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> intro/intros_old/intro12.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholder.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features, hindering their deployment in the real world~\cite{semenova2022quantitative}. 
However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous `Localization' and `Mapping' that is compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm which is memory and compute efficient and scalable. \name SLAM's  key insight is to eliminate memory intensive storage and computationally expensive correlation operations over the past measurement. \name system/robot consists of a WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. These pose estimates are then fed to \name's visual layer as shown in Figure~\ref{fig:intro-fig}, used by \name visual layer to label visual data with a pose.  
Since Wi-Fi pose measurements do not accrue drift over time, unlike standard visual SLAM algorithms, \name visual SLAM does not need to cross-correlate measurements across time to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with a clear interface of sharing of pose estimation from WiFi layer, to enable visual layers for the environment mapping. Such layering would bring the advantages of networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled.
It would enable researchers in wireless sensing and visual SLAM domain to improve the independent algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm.
For example, while \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 

However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi sensing solutions and feeding them into existing Visual SLAM algorithms.
We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free,robust and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduce erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 

\noindent\textbf{Unknown Wi-Fi Access Point Locations:}
An obvious idea would be to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization, which includes WiFi-AP locations. Specifically, we define the Wi-Fi graph with the robot side AoA measurements from different APs and concurrent odometry measurements, with robot pose and AP's location as variables. 
Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, initial values to variables are extreme importance to lead the optimizer in a trajectory to solve the problem. 
While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. Furthermore, arbitrary initializing AP's locations would work only when AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. 
However, to be compute efficient with few AoA measurements that constrain the AP's pose, as is the case when the robot in real-time maps the environment, the optimizer is poorly conditioned for AP's location. 
To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) based proximity sensing~\cite{ez,zee} to initialize the location of WiFi AP. The location of the Wi-Fi AP is initialized to the robot pose at the time instance when the RSSI measured for a given access point is a local maxima along a path taken. 

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Finally, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As robot moves, the WiFi graph continues to optimize its previous robot poses. A continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.


These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> intro/intros_old/intro13.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/viwid_intro-crop.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement units) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements requires the SLAM system to be both memory and compute intensive.~\cite{semenova2022quantitative}.
The way these Visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory through its environment, because when the robot returns to a previous location, it will observe the same features.
The drawback of this method is that as new features are observed, they must constantly be correlated with past observed features, to check if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observes more new features. This hinders their deployment in the real world~\cite{semenova2022quantitative}. 
However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous Localization and Mapping system that is compute and memory efficient, to make autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm which is memory and compute efficient, and scalable. \name SLAM's  key insight is a method to eliminate memory intensive storage and computationally expensive correlation operations over past measurements. \name system/robot consists of a WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. These pose estimates are then fed to \name's visual layer as shown in Figure~\ref{fig:intro-fig}, used by \name visual layer to label visual data with a pose.  
\name's key observation is that Wi-Fi pose measurements do not accrue drift over time, as they are derived from fixed WiFi anchors in the environment. Therefore, unlike standard visual SLAM algorithms, \name visual SLAM can leverage drift free robot pose as input, and thus, do not require the SLAM algorithms to cross-correlate measurements across time to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with a interface of sharing of robot poses from WiFi layer, to enable the visual layer to map the environment without any correlation. Such layering would bring the advantages similar to networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled.
It would enable researchers in wireless sensing and visual SLAM domain to improve the independent algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm.
For example, while \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 


% WiFi graph

\noindent\textbf{WiFi Graph:}
A natural question is can we use large work on WiFi sensing to develop the WiFi layer/graph which can construct the robot poses (location and orientation). Without the location knowledge of the access points in the environment eliminates ability to leverage large body of research in WiFi Localization. Furthermore, recent works~\cite{ayyalasomayajula2020locap,xxx} leverages an autonomous visual SLAM robot to map the WiFi access, which requires the visual SLAM to have converged, leading to similar compute and memory challenges. In \name, we design a computational efficient WiFi-graph, which in real-time enables the robot to provide poses (location and orientation), without knowledge of WiFi APs location. \name key insight is to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization to solve for both the robot pose and AP's location as variables. Specifically, \name deploys multi-antenna radio at the robot to achieve robot side AoA measurements from different APs in the environment and simultaneous odometry measurements forms an input to graphSLAM. Furthermore, \name develops many optimizations for WiFi graph to make it compute efficient, to output robot poses over time. Intutively, graphSLAM combines the inputs from odometry and AoA's over time to backpropogate and refine the robot pose estimate and WiFi AP position over time. 

% Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, initial values to variables are extreme importance to lead the optimizer in a trajectory to solve the problem. While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. Furthermore, arbitrary initializing AP's locations would work only when AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. However, to be compute efficient with few AoA measurements that constrain the AP's pose, as is the case when the robot in real-time maps the environment, the optimizer is poorly conditioned for AP's location. To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) based proximity sensing~\cite{ez,zee} to initialize the location of WiFi AP. The location of the Wi-Fi AP is initialized to the robot pose at the time instance when the RSSI measured for a given access point is a local maxima along a path taken. 

% 
% However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi sensing solutions and feeding them into existing Visual SLAM algorithms.
% We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Next, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As robot moves, the WiFi graph continues to optimize its previous robot poses via back-propagation. A continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free,robust and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduce erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 

These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiducial markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> intro/intros_old/intro13_ag.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and generating human readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/viwid_intro-crop.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features, hindering their deployment in the real world~\cite{semenova2022quantitative}. 
% However, visual sensors are still necessary for building a contextual map of the robot's environment, so, there is a need for a robust Simultaneous `Localization' and `Mapping' that is compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM system which is low-cost\footnote{requires only Camera as a visual sensor, doesn't require LiDAR}, memory, compute efficient and scalable. \name SLAM's  key insight is to eliminate memory intensive storing of past measurements and computationally expensive correlation operations over the past measurement. 
\name system/robot consists of a multi-antenna WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of robot, without assuming the knowledge of Wi-Fi access point locations in map. 
These pose estimates are then fed to \name's visual layer to label visual data with a prior pose (as shown in Figure~\ref{fig:intro-fig}). 
\name's key observation is that WiFi layers robot pose measurements do not accrue drift over time, as they are derived from fixed WiFi anchors in the environment. 
Therefore, unlike standard visual SLAM algorithms, \name visual SLAM can leverage drift free robot pose as input, and thus, does not require the SLAM algorithms to cross-correlate across past measurement to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Visual layer (needs only camera).

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with a interface of sharing of robot poses from WiFi layer, to enable the visual layer to map the environment without any correlation. Such layering would bring the advantages similar to networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in WiFi layer and Visual layer are completely decoupled.
It would enable researchers in wireless sensing and visual SLAM domain to improve the independent algorithms, \name's architecture could leverage those improvement to build a more accurate SLAM algorithm.
For example, while \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 


% WiFi graph

\noindent\textbf{WiFi Graph:}
A natural question is can we simply use the work on WiFi sensing to develop the WiFi layer which can construct the robot poses (location and orientation). Turns out, most state of the art in WiFi sensing assume knowledge of access point to localize \cite{}. However, ideally no prior knowledge of environment is desirable as it leads to ease of deployment~\cite{ayyalasomayajula2020locap}. Thus, not assuming the WiFi AP location hinders the ability to simply piggyback on using existing prior works in WiFi sensing to deploy the WiFi layer. 
% Furthermore, recent work~\cite{ayyalasomayajula2020locap} pose an inverse problem with WiFi sensing, where they leverage an autonomous visual SLAM robot to map the WiFi access points to make the WiFi sensing deploy-able.
% This however, requires the visual SLAM to have converged, leading to similar compute and memory challenges to map the WiFi access points themselves. 
Bypassing these issues entirely, in \name, we design a computational efficient WiFi-graph, which in real-time enables the robot to provide poses (location and orientation), without knowledge of WiFi APs location. \name key insight is to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization; for example, solve for both the robot pose and AP's location variables. 
The idea here is to do a coarse initialization of WiFi access points, based on their RSSI measurements, and the GraphSLAM framework would use the WiFi measurements and Odometry measurement to optimize for access point locations implicitly, and robot poses explicitly. Intuitively, it combines measurements of wifi-sensor, odometry across a trajectory (time-series of multiple location) to obtain accurate robot poses.  

% Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, initial values to variables are extreme importance to lead the optimizer in a trajectory to solve the problem. While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. Furthermore, arbitrary initializing AP's locations would work only when AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. However, to be compute efficient with few AoA measurements that constrain the AP's pose, as is the case when the robot in real-time maps the environment, the optimizer is poorly conditioned for AP's location. To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) based proximity sensing~\cite{ez,zee} to initialize the location of WiFi AP. The location of the Wi-Fi AP is initialized to the robot pose at the time instance when the RSSI measured for a given access point is a local maxima along a path taken. 

% 
% However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi sensing solutions and feeding them into existing Visual SLAM algorithms.
% We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:


\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:}
Naturally, the graphSLAM would require high-quality, real-time input to achieve robust robot poses as well implicit locations of the AP, which do not accrue drift. 
% Specifically, \name deploys multi-antenna radio at the robot to achieve robot side AoA measurements from different APs in the environment and simultaneous odometry measurements forms an input to graphSLAM. 
% Furthermore, \name develops many optimizations for WiFi graph to make it compute efficient, to output robot poses over time. 
% Intutively, graphSLAM combines the inputs from odometry and AoA's over time to backpropogate and refine the robot pose estimate and WiFi AP position over time. 
In order to accurately estimate the map, the visual layer requires drift-free, robust and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose from the fixed APs located at implict positions optimized by the SLAM framework. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduce erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 


\noindent\textbf{Efficient Pose Updates to Camera Graph:} Next, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As robot moves, the WiFi graph continues to optimize its previous robot poses via back-propagation. A continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.



These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We evaluate \name over two environments of the publicly available dataset~\cite{arun2022p2slam}.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We benchmark our results against the state-of-the-art Visual SLAM system, RTABMap~\cite{Labb2018RTABMapAA}, and we use the high compute and expensive LiDAR sensor readings reported in the Datasets~\cite{arun2022p2slam} to estimate thee ground truth for our measurements.
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} the Visual SLAM.
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$}the Visual (LiDAR).
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.



==> intro/intros_old/intro14.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and generating a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/viwid_intro-crop.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}


Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory and compute-intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observes more new features, hindering their deployment in the real world~\cite{semenova2022quantitative}. 


In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM system which is low-cost\footnote{requires only Camera as a visual sensor, doesn't require LiDAR}, memory, compute efficient and scalable. \name SLAM's key insight is to eliminate memory-intensive storing of past measurements and computationally expensive correlation operations over the past measurement. 
\name system/robot consists of a multi-antenna WiFi radio, which is fed to \name's Wi-Fi layer to provide pose (position and orientation) estimates of the robot, without assuming the knowledge of Wi-Fi access point locations in a map. 
These pose estimates are then fed to \name's visual layer to label visual data with a prior pose (as shown in Figure~\ref{fig:intro-fig}). 
\name's key observation is that WiFi layers robot pose measurements do not accrue drift over time, as they are derived from fixed WiFi anchors in the environment. 
Therefore, unlike standard visual SLAM algorithms, \name visual SLAM can leverage drift-free robot pose as input, and thus, does not require the SLAM algorithms to cross-correlate across past measurement to correct for these drifts, thereby eliminating excessive storage and compute requirements.
Thus, \name enables compute and memory-efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Visual layer (needs only camera).

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with an interface of sharing of the robot poses from WiFi layer, to enable the visual layer to map the environment without any correlation. Such layering would bring advantages similar to networking layer abstractions~\cite{session1994it5} to the SLAM research. Specifically, a powerful implication of our layered architecture, is that innovations in the WiFi layer and Visual layer are completely decoupled.
It would enable researchers in wireless sensing and visual SLAM domain to improve the independent algorithms, \name's architecture could leverage that improvement to build a more accurate SLAM algorithm.
For example, while \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 


\noindent\textbf{WiFi Graph:}
A natural question is can we simply use the work on WiFi sensing to develop the WiFi layer which can construct the robot poses (location and orientation). Turns out, most state-of-the-art in WiFi sensing assume knowledge of access points to localize \cite{arraytrack,spotfi}. However, ideally, no prior knowledge of the environment is desirable as it leads to ease of deployment~\cite{ayyalasomayajula2020locap}. Thus, not assuming the WiFi AP location hinders the ability to simply piggyback on using existing prior works in WiFi sensing to deploy the WiFi layer. 
Bypassing these issues entirely, in \name, we design a computational efficient WiFi-graph, which in real-time enables the robot to provide poses (location and orientation), without knowledge of WiFi APs location. \name key insight is to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization; for example, solve for both the robot pose and AP's location variables. 
The idea here is to do a coarse initialization of WiFi access points, based on their RSSI measurements, and the GraphSLAM framework would use the WiFi measurements and Odometry measurement to optimize for access point locations implicitly, and robot poses explicitly. Intuitively, it combines measurements of wifi-sensor, odometry across a trajectory (time-series of multiple locations) to obtain accurate robot poses.  


\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:}
Naturally, the graphSLAM would require high-quality, real-time input to achieve robust robot poses as well implicit locations of the AP, which do not accrue drift. 
To accurately estimate the map, the visual layer requires drift-free, robust, and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose from the fixed APs located at implicit positions optimized by the SLAM framework. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real-time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduces erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 


\noindent\textbf{Efficient Pose Updates to Camera Graph:} Next, the optimized robot poses generated by the Wi-Fi graph need are fed to update the robot poses in the camera graph in real-time. As the robot moves, the WiFi graph continues to optimize its previous robot poses via back-propagation. Continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute-intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made to the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates make the camera graph optimization efficient by avoiding any possible memory or compute-intensive stages.



These effective solutions surmount the key challenges to integrating Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We evaluate \name over two different where  we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
In addition to this, we also collect one more dataset in a $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot-driven cumulative distance of over $1000$ m across these two environments. 
We benchmark our results against the state-of-the-art Visual SLAM system, RTABMap~\cite{Labb2018RTABMapAA}, and we use the high compute and expensive LiDAR sensor readings to estimate the ground truth for our measurements.
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to $20\%$ of cores which is $5\times$ better than current Visual SLAM.
    \item We also show that \name-SLAM reduces the average memory utilization to $300$MB which is $3\times$ the Visual (LiDAR).
    \item We show a pose estimation performance with 50cm median location estimation error and $2^{\circ}$ median orientation estimation error on par with the state-of-the-art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiducial markers placed in the environment to within 105cm of error.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in the layered SLAM domain for sensor fusion approaches.



==> intro/intros_old/intro15.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}


Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) frameworks, which enable real-time navigation and generate a human-readable map of the robot's environment. This is crucial for many tasks expected of an indoor robot. However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/viwid_intro-crop.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}


Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Kimera~\cite{rosinol2021kimera}, ORB-SLAM~\cite{mur2015orb}, or Cartographer~\cite{cartographer} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, and also when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM algorithms are memory intensive, as the robot must keep all features it has seen in memory. 
Furthermore, they spend increasing compute time looking them up and comparing them as it observes more new features, hindering their deployment in the real world~\cite{semenova2022quantitative}. 


In this paper, we present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM system which is a memory+compute efficient, scalable and low-cost\footnote{requires only a monocular camera as a visual sensor, does not require LiDAR}. 
\name SLAM's key insight is to eliminate memory-intensive storing of past measurements and computationally expensive correlation operations while maintaining drift free robot trajectory to ensure accurate SLAM. 
\name system/robot consists of a multi-antenna WiFi radio, which is fed to \name's Wi-Fi layer to provide 3D-pose (position and orientation) estimates of the robot, without assuming the knowledge of Wi-Fi access point locations in a map. 
These pose estimates are then fed to \name's visual layer to label visual data with a prior pose (as shown in Figure~\ref{fig:intro-fig}). 
\todo{Causes confusion for Reviewer 3: does this mean you're replacing standard odometry?}
\name's key observation is that WiFi layers robot pose measurements do not accrue drift over time, as they are derived from fixed WiFi anchors in the environment. 
Therefore, unlike standard visual SLAM algorithms, \name's visual SLAM can leverage drift-free robot pose as input, effectively circumventing the memory+compute intensive cross-correlation across past measurements.
Thus, \name enables compute and memory-efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Visual layer (needs only camera).

Additionally, \name presents a layered abstraction for both WiFi layer and Visual SLAM layer, with an interface of sharing of the robot poses from WiFi layer, to enable the visual layer to map the environment without any correlation operations. 
Such layering would bring advantages similar to networking layer abstractions~\cite{session1994it5} to the SLAM research. 
Specifically, a powerful implication of our layered architecture is that innovations in the WiFi layer and Visual layer are completely decoupled.
This decoupling would enable researchers in wireless sensing and visual SLAM domain to independently improve algorithms, and allow \name's architecture to easily leverage these improvement to build a more accurate SLAM algorithm.
For example, while \name's Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method can generalize to other RF-sensors like BLE~\cite{toasa2021experimental,ayyalasomayajula2018bloc}, UWB~\cite{zhao2021uloc} or next gen 5G femto-cell implementations~\cite{menta2019performance,chaloupka2017technology}. 


\noindent\textbf{WiFi Graph:}
A natural question is can we simply use the work on WiFi sensing to develop the WiFi layer which can construct the robot poses (location and orientation). Turns out, most state-of-the-art in WiFi sensing assume knowledge of access points to localize \cite{arraytrack,spotfi}. However, ideally, for ease of deployment, no prior knowledge of the environment is desirable~\cite{ayyalasomayajula2020locap}. Thus, not assuming the WiFi AP location hinders the ability to simply piggyback on using existing prior works in WiFi sensing to deploy the WiFi layer. 
Bypassing these issues entirely, in \name, we design a computational efficient WiFi-graph, which in real-time enables the robot to provide poses (location and orientation), without knowledge of WiFi APs location. 
\name's key insight is to leverage the GraphSLAM~\cite{gtsam} as it is well known to jointly solve for multi-variate optimization; specifically in the case of the WiFi-graph, solve for both the robot's pose and AP's location variables. 
The idea here is to first coarsely initialize the WiFi access points as new access points are discovered prior to optimization. 
Next, the GraphSLAM framework would use the WiFi measurements and Odometry measurements to optimize for access point locations implicitly, and robot poses explicitly. 
Intuitively, it combines measurements of wifi-sensor, odometry across a trajectory (time-series of multiple locations) to obtain accurate robot poses.  


\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:}
% Naturally, the graphSLAM would require high-quality, real-time input to achieve robust robot poses as well as implicit locations of the AP, which do not accrue drift. 
To accurately estimate the map, the visual layer requires drift-free, robust, and real-time robot pose estimates from the Wi-Fi layer. To get these pose estimates from the \name's Wi-Fi layer, we employ a multi-antenna radio at the robot, which is used to extract Angle of Arrival (AoA) information, which we leverage to achieve drift-free pose from the fixed APs located at implicit positions optimized by the SLAM framework. 
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these algorithms use super-resolution, which cannot provide compute efficient AoA measurements at the rate needed for real-time pose estimation.
To solve this, in \name we employ a low-compute algorithm, which reduces erroneous measurements by attenuating multipath components in the signal, by combining the CSI across time and finding its principle component of the CSI (PC-CSI). 
The PC-CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. 
We use this method to measure AoA at the robot from Wi-Fi access points in the environment. 
However, the AoA alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we do not wish to assume access point locations are known apriori. 
This is primarily why WiFi localization cannot be used as they assume knowledge of access points~\cite{ayyalasomayajula2020locap,arraytrack,spotfi}. 


\noindent\textbf{Efficient Pose Updates to Camera Graph:} Next, the optimized robot poses generated by the Wi-Fi graph are fed to update the robot poses in the camera graph in real-time. 
As the robot moves, the WiFi graph continues to optimize its previous robot poses via \todo{back-propagation (not the best term)}. 
Continuous updates of already traversed robot poses to the camera graph, would trigger large and frequent corrections.
This results in large and frequent feature map corrections, making the system compute-intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made to the Wi-Fi pose estimations and accumulates all the corrections to be made. 
The robot poses are only pushed to the camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates make the camera graph optimization efficient by avoiding any possible memory or compute-intensive stages.

These effective solutions surmount the key challenges to integrating Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM2~\cite{gtsam}.
We evaluate \name over two different paths driven in a $25 \times 30$ m. 
In addition to this, we also collect one more dataset in the $25 \times 30$ m environment to evaluate the mapping capabilities of \name.
\name is robustly tested with the robot-driven cumulative distance of over $1000$ m across these three datasets. 
We benchmark our results against the state-of-the-art Visual SLAM system, RTABMap~\cite{Labb2018RTABMapAA}, and we use the high compute and expensive LiDAR sensor readings to estimate the ground truth for our measurements.
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to $20\%$ of cores which is $5\times$ better than current Visual SLAM.
    \item We also show that \name-SLAM reduces the average memory utilization to $300$MB which is $3\times$ less than Visual-SLAM.
    \item We show a pose estimation performance with $50$ cm median location estimation error and $2^{\circ}$ median orientation estimation error, performing on par with the state-of-the-art systems.
    \item We also show the \name's real-time mapping accuracy by mapping the camera fiducial markers placed in the environment to within $105$ cm of error using a monocular camera.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the datasets we have collected, to enable further research and development in the layered SLAM domain for sensor fusion approaches.



==> intro/intros_old/intro2.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

A strong need for automation in various industries spanning hospitality to security has led to an increased adoption of robots capable of autonomous, reliable and safe indoor navigation. The trend kick-started by the early adoption of automated vacuum cleaners has grown many-fold to use these robots for monitoring security in office spaces, serving patrons at restaurants and moving large equipment in hospitals. The autonomy, reliability and safety these robots boast is owed to the suite of sensors they use. Most autonomous robots can be commonly spotted sporting 
1. a LiDAR at the top to provide a 360-degree view, 
2. a camera facing forward to provide a feature-rich map, 
3. bumper sensors to avoid catastrophic collisions, and
4. odometry sensors (wheel encoder and IMU) to provide high-resolution odometry data.
The data from these sensors are expertly fused taking into consideration each sensors reliability within a back-end optimization framework to generate an accurate estimate of the robot's location and its relation to the environment around it. The fusion of these different sensing modalities provides a very robust solution for autonomous navigation of robots.

% let's see how good sensor fusion works; explain landmarks, features, loop closure in few sentences...
To achieve autonomous navigation, the first key step is for the robot to build a map of its environment and localize itself within this map in real time. 
Furthermore, this map should consist of rich contextual data -- labels of room numbers, descriptions of spaces, markings for various exits and entrances of buildings. 
This problem is commonly called Simultaneous Localization and Mapping (SLAM). 
In a two-step process, which involves first extracting and tracking the characteristic features from visual sensors, and second, combining the data from these sensors with odometry, the robot can build an accurate map and localize itself within this map. The characteristic features (\textit{landmarks}) extracted generally include corners or edges in Camera images or LiDAR scans. Tracking these features provides corrections to errors accumulated by odometry sensors, and saving some of the salient features helps the robot recognize and create additional constraints (\textit{loop-closures}) with previously visited places. Through this two-step process, robots can effectively navigate the strengths and weaknesses of individual sensors to solve the SLAM problem.

% but this fails in monotonous envs ...\todo{because of the same reasons we have mentioned in P2SLAM}
Unfortunately, in indoor environments, we observe gaps left behind this common suite of sensors generally employed on robots. LiDAR's, although great in providing an accurate point cloud of an environment, fail in environments with little structural features, like long corridors or spaces larger than the field of view of the LiDAR. Furthermore, they are expensive, bulky and power hungry. To combat these weaknesses of LiDARs or to develop robots at lower cost-points, cameras (monocular, stereo or RGBD) are employed. Cameras offer an advantage over LiDAR's in that they allow for finer feature detection. For example, a long corridor adorned with posters and paintings provide robust and recognizable features to track against. Unfortunately, motion blur, dynamic lighting conditions and monotonous visual environments can all lead to feature tracking failure and even false positive loop closure hypothesis.
% Furthermore, viable distances to obtain accurate depth from RGBD/Stereo sensor range from \todo{xx} m - \todo{xx} m, making them unusable in large spaces. 
Discounting LiDAR's or cameras in these challenging environments leaves us with odometry sensors. A combination of wheel encoders and IMU's provide accurate change in position over a local region and a period of few minutes. 
Unfortunately, lacking the global correction provided by visual sensors via loop-closures, these odometry sensors can accrue large drifts, in the order of many tens of meters, when traversing large distances of hundreds of meters. This leaves an open problem for autonomous navigation for indoor robotics -- what is the best sensor we could incorporate to fill in the gaps left by these multitude of sensors? 

% bring up and kill other sensors, distill to wifi, rebuff it after a better lit review ...
To answer this pressing question, we can in fact take inspiration from GPS. Using a network of satellites, GPS can position a GPS-capable device to within a few meters with a global frame of reference. This can help to correct for large drifts accumulated due to odometry and incorrect tracking from visual sensors. But, GPS signals are scantly available in indoor scenarios to provide the necessary corrections. Fortunately, we observe that an alternative, RF-signals, like Bluetooth, Ultrawide-band (UWB) or WiFi, are abundant indoors. RF-based sensing can, in a loose sense, replace GPS and many recent works have proposed the use RF-based sensing to fill the gaps left by visual sensors. As expanded in Section~\ref{sec:related}, implementations based on UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot} exist. Unfortunately, these systems are limitedly employed due to high deployment cost or poor scalability. Fortunately, as compared to UWB and BLE, WiFi is more ubiquitously deployed (reducing deployment cost) and provides a larger range than RFID or other backscatter devices (making it scalable). Keeping these advantages in mind, many systems have been proposed incorporating WiFi sensors within SLAM, for aiding loop closures~\cite{hashemifar2019augmenting, liu2019collaborative} or incorporating them as range~\cite{huang2011efficient,ferris2007wifi} or bearing sensors~\cite{xxx}. Unfortunately, the systems in \cite{hashemifar2019augmenting, liu2019collaborative} and \cite{ huang2011efficient,ferris2007wifi} utilize RSSI for fingerprinting or as a proxy for range respectively and hence lack robustness in dynamic environments. While, P2SLAM~\cite{xxx}, incorporating bearings extracted from CSI~\cite{ayyalasomayajula2018bloc}, is more robust to dynamic environments, it does not tightly fuse with visual sensors, and hence its locations lack contextual information with respect to a map. 

\name seeks to solve this problem by showcasing a system which tightly couples visual landmarks from a monocular camera and readily deploys in any unknown environment. The key deliverable for \name is to provide an end-to-end sensing solution (WiFi + monocular camera, in conjunction with odometry sensors), which furnishes context-rich location information in real-time without requiring any prior information about the environment. \name achieves this by incorporating WiFi as a bearing sensor~\cite{xxx}, employing the feature tracker from VINS-MONO~\cite{qin2018vins} and fusing odometry from a combination of a wheel encoder and IMU with an open-sourced GraphSLAM framework~\cite{gtsam}. Furthermore, we showcase our system with a simple application which builds a map labelled with room numbers and autonomously navigates to a given room number to deliver a package. 

% but there are problems to implementing this...
But there are three key problems which \name seeks to solve to enable dense \underline{V}isual \underline{I}nertial \underline{O}dometry with Wi\underline{Fi} possible. 
\begin{itemize}
    \item \textbf{Accurate AoA measurements:} Movement of the robot and limited knowledge of antenna placements on the access points (AP) deployed in the environment reduces the accuracy of the angle of arrival measured at the robot. \name observes that for each frequency and packet, extracting the strongest principal component helps to reduce non-idealities introduced by the robots velocity and vibration and accurate average across multiple transmit antenna. In this vein, \name uses an SVD-FFT algorithm to accurate estimate the angle of arrival on the robot (Sec.~\ref{sec:xxx}).
    \item \textbf{2.5D:} AP's are generally deployed higher than the robot's WiFi receiver. This implies we need to estimate both the azimuth and polar angle of arrival (3D-AoA). Unfortunately, with four or fewer antennas~\footnote{Most commercially available WiFi receivers come with only four or fewer antennas~\cite{quantenna, halperin2011tool, gringoli2019free}}, measuring 3D-AoA is very difficult due to reduced resolution. \name overcomes this by observing that the measured angle of arrival of a signal impinging from a higher elevation lies on the inclined plane connecting the AP and the robot, oriented according the heading of the robot. This observation allows \name to extract a single inclined-AoA from a linear antenna array and incorporate these measurements within GraphSLAM~\cite{gtsam} by defining a new measurement factor (Sec.~\cite{xxx}).
    \item \textbf{Half-plane Ambiguity:} Using a linear antenna array creates an ambiguity in the incline-AoA measured in the $360^\circ$ search-space. Using MH-iSAM2\cite{hsiao2019mh}, \name elegantly resolves this ambiguity by incorporating the multiple hypothesis within GraphSLAM and prunes the incorrect hypothesis in the future when more measurements are available (Sec.~\cite{xxx}).
\end{itemize}

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publically available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry. 

% we make this solution possible by ... efficiently fusing WiFi and camera for their strong suits, where our system relies on WiFi majorly for it's localization and tracking purposes and camera for it's map building and optimal and safe navigation purposes


% with \name, we implement and observe the following ...solutions which make realizing low-cost, robust indoor navigation robots a reality



% \subsection{Storyline}
% WiFi+camera with simplistic sensors, and plug them for the robot
% Monocular cameras are not sufficient within themselves
% So people have moved to stereo-vision and LiDAR
% Under 50\$ we can give you context based mapping with robust localization.

==> intro/intros_old/intro3.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Increasing research into autonomous robots for indoors, have spun a myriad of applications and use cases like in equipment and inventory management ranging from hospitals~\cite{hospital,tracking,robots} to warehouses~\cite{warehouse,management,robots} in addition to the usual indoor navigation~\cite{indoor,navigation,robots} and exploration robots~\cite{distaster,zone,exploration,robots}. 
Most of these applications like inventory management and delivery in the critical cases like hospitals demands a fleet of robust, secure and autonomous robots.
While, there has been an effort in deploying a fleet of robots for last-mile delivery in the recent past~\cite{last,mile,delivery,papers}, the technology has not scaled up due to high cost to return value in deploying these robots.
The expensive costs, both in terms of price and compute come from the usage of suite of sensors on these robots~\cite{last,mile,ecomically,inefficient}.
Most algorithms~\cite{visual,slam,algorithms} on these autonomous robots can be commonly spotted utilizing the sensor data from a LiDAR, RGBD or monocular camera in tandem with odometry sensors (wheel encoder and IMU) to provide high-resolution simultaneous mapping and localization.
These pool of sensors, especially LiDAR and RGBD sensors, become expensive in terms of compute and price as the robustness requirement for the autonomous deployment increases.
Unfortunately, this cost ultimately limits these autonomous systems from scaling to deployment. 
Thus, to be able to realize these applications, the Simultaneous Localization and Mapping (SLAM) algorithms to be deployed on these fleet of autonomous robots need to be (a) low-cost, (b) low-compute, and (c) capable of understanding its surroundings.


A majority of current SLAM algorithms on these robots utilize visual (monocular/RGBD cameras)~\cite{camera,slam,algorithms} and LiDAR~\cite{lidar,slam,algorithms} sensors.
While these LiDAR and visual sensors provide the context of the surroundings to the robot, they have extensive compute and memory requirements, and are very expensive, which limit them to scale towards these low-cost, context aware autonomous robots.
So, in this paper, we first ask the question on how we can reduce the cost/expense of these autonomous robots?
In the recent past, there has been a lot of research towards Radio Frequency (RF) sensors as the low-cost, low-compute sensors for robust SLAM algorithms~\cite{wifi,uwb,ble,p2slam,papers}.
While the RF-sensors enable low-power and low-compute SLAM algorithms, these SLAM algorithms fall short in two categories, firstly most of these algorithms~\cite{rf,fingerprinting,slam,algos} utilize these RF-measurements as landmarks, which require labour intensive fingerprinting. 
Secondly, the other algorithms~\cite{p2slam,other,similar,papers} that utilize only RF-sensors and integrate them completely into the SLAM algorithms lack the understanding of their surroundings, which becomes important when deployed in real-world.
Thus, there is a lack of a SLAM algorithm that uses low-cost, low-compute sensor and still be able to get an understanding or context of the environment around the robot.
% inexpensive semantic mapping

In this paper, we thus present \name, a low-cost, low-compute SLAM algorithm that has an awareness of the surrounding environment. 
To achieve this \name implements first of its kind integration of low-cost, low-compute RF sensor with a simple monocular camera
\todo{ temporary copy paste from the previous iteration of the intro:}
in real-time without requiring any prior information about the environment. \name achieves this by incorporating WiFi as a bearing sensor~\cite{xxx}, employing the feature tracker from VINS-MONO~\cite{qin2018vins} and fusing odometry from a combination of a wheel encoder and a gyroscope with an open-sourced GraphSLAM framework~\cite{gtsam}. 
While, \name's implementation is demonstrated using WiFi owing to its widescale deployment one of the major advantages \name is that it abstracts bearing as the RF-sensor measurement.
Thus any RF-sensor that can report their bearings like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as altnerative RF-sensors.
Furthermore, we showcase our system with a simple application which builds a map labelled with room numbers and autonomously navigates to a given room number to deliver a package. 

% but there are problems to implementing this...
But there are three key problems which \name seeks to solve to enable dense \underline{V}isual \underline{I}nertial \underline{O}dometry with Wi\underline{Fi} possible. 
\begin{itemize}
    \item \textbf{Accurate AoA measurements:} Movement of the robot and limited knowledge of antenna placements on the access points (AP) deployed in the environment reduces the accuracy of the angle of arrival measured at the robot. \name observes that for each frequency and packet, extracting the strongest principal component helps to reduce non-idealities introduced by the robots velocity and vibration and accurate average across multiple transmit antenna. In this vein, \name uses an SVD-FFT algorithm to accurate estimate the angle of arrival on the robot (Sec.~\ref{sec:xxx}).
    \item \textbf{2.5D:} AP's are generally deployed higher than the robot's WiFi receiver. This implies we need to estimate both the azimuth and polar angle of arrival (3D-AoA). Unfortunately, with four or fewer antennas~\footnote{Most commercially available WiFi receivers come with only four or fewer antennas~\cite{quantenna, halperin2011tool, gringoli2019free}}, measuring 3D-AoA is very difficult due to reduced resolution. \name overcomes this by observing that the measured angle of arrival of a signal impinging from a higher elevation lies on the inclined plane connecting the AP and the robot, oriented according the heading of the robot. This observation allows \name to extract a single inclined-AoA from a linear antenna array and incorporate these measurements within GraphSLAM~\cite{gtsam} by defining a new measurement factor (Sec.~\cite{xxx}).
    \item \textbf{Half-plane Ambiguity:} Using a linear antenna array creates an ambiguity in the incline-AoA measured in the $360^\circ$ search-space. Using MH-iSAM2\cite{hsiao2019mh}, \name elegantly resolves this ambiguity by incorporating the multiple hypothesis within GraphSLAM and prunes the incorrect hypothesis in the future when more measurements are available (Sec.~\cite{xxx}).
\end{itemize}

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publically available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.

==> intro/intros_old/intro4.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Recent time has seen a rise in demand for autonomous robots and drones for various applications ranging from inventory management in warehouses, hospitals, construction sites~\cite{hosptials,warehoueses,construction,sites} in addition to the navigation~\cite{navigation,robots} and exploration robots~\cite{exploration,robots} for last-mile delivery~\cite{last,mile,delivery}, mapping~\cite{Labb2018RTABMapAA}, and disaster relief~\cite{disaster,relief,jadhav2020wsr}. 
This increasing demand has led the researchers towards deploying fleets of robots to increase the efficiency for these applications, in for example last-mile delivery~\cite{last,mile,delivery} or collaborative robots for indoor explorations~\cite{collab,bots}.
These applications brings forth some important requirements for the current SLAM algorithms to be scalable and deployable:
(a) they should be `low-compute', as they need to run most of the times on a compute-limited platforms, (b) they should be `low-cost', so as to be able to deploy them widely, and (c) they should be `adaptable' to different environmental changes, like dynamic-visibility conditions and/or obstacles in the path.


There exist a lot of powerful tools for autonomous robot systems~\cite{Labb2018RTABMapAA,cartographer,orbslam}, these are far from being scalable to a fleet of robots.
Most of these existing works in SLAM use either IMU/odometry to get the poses of the robot. 
These pose measurements in tandem with camera/LiDAR visual sensors are used to jointly optimize for absolute poses by correcting for the drifts of the IMU/odometry measurements and also to map the environment. 
Firstly, these LiDAR sensors are very expensive, making the LiDAR based SLAM algorithms hard to deploy.
Secondly, while the camera sensors are cheap the joint optimization for optimal Visual SLAM has three distinct operations: (1) feature extraction and tracking, (2) local feature matching and mapping, and (3) global loop-closures. 
While the first two components are not compute intensive, the global loop-closure algorithms are very compute hungry and increase the latency of the system in a compute-restrained scenario~\cite{semenova2022quantitative}.
% 

In contrast, there is a couple of decades of research in RF-based localization and tracking that uses existing RF deployment architectures in the environment, like WiFi, to locate and track various devices in the environment.
As most of the current robots are connected to these internet, they have access to WiFi connectivity which has led the researchers to delve into using WiFi for SLAM implementations~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
These algorithms have been shown to not need global loop-closures making them `low-cost' and 'low-compute' systems~\cite{arun2022p2slam,zhang2020robot}.
Although, unfortunately due to the low-wavelength of RF-signals, these algorithms suffer from lack of context or a map of their surroundings. 
Thus making them non-adaptable to various environmental changes that require awareness of the surroundings/map.

% Current research in Visual SLAM and RF-sensing have thus completely bifurcated from each other. 
% Although as stated above, it is apparent that if we can appropriately integrate the `low-cost', `low-compute' RF sensor with a simple monocular camera that can provide context/map(`adaptable') we can achieve a deployable and scalable SLAM algorithm.
% One might assume

To solve these issues, in this paper we present \name (\underline{V}isual \underline{I}nertial \underline{O}dometry with Wi-\underline{Fi}), that amalgamates the best of both RF and camera worlds. 
While there exist few current works that try to incorporate RF-signals into existing Visual SLAM algorithms~\cite{hashemifar2019augmenting, liu2019collaborative,nguyen2021viral,jadhav2020wsr}, but these systems only try to use the RF signals to aid in the `global loop closures' ~\cite{hashemifar2019augmenting, liu2019collaborative} or depend on the Visual SLAM system to provide the pose of the RF sensor on board~\cite{nguyen2021viral,jadhav2020wsr} making them compute hungry.
In contrast, \name is a first of its kind integration that maintains the `low-cost' and `low-compute' of RF sensor, and simultaneously utilizes a simple monocular camera that can provide context/map(`adaptable') making it a scalable and deployable SLAM system.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/placeholder.pdf}
    \caption{\name's layered approach: WiFi bearings and IMU/Odomtry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time.}
    \label{fig:intro_fig}
\end{figure}


To perform this optimal integration in \name's design, we make a simple yet key observation that both the RF-sensors and the camera-sensors have two independent tasks that can be easily layered to make the system truly scalable.
To be more precise, a camera sensor is the best possible solution to provide real-time current context to the robot regarding its surrounding environment, but it cannot directly help towards estimating the robots absolute pose.
% This has led the researchers in the past to develop complex and compute hungry global loop-closures based optimization for accurate SLAM.
If only these robots could have access to an `Oracle' that could provide these absolute pose measurements they could obtain an optimized map by just performing low-compute feature extraction and local feature matching.
On the other hand, if the existing RF based SLAM approaches could somehow get context awareness and adaptability while maintaining low-cost and low-compute demand. 
We solve both of these problems in \name using the inspiration from network layering/abstraction principals, where in each layer has distinct functionalities and clear boundaries as shown in Figure~\ref{fig:intro_fig}. 
Wherein we firstly use RF measurements and fusing odometry from a combination of a wheel encoder and IMU with an open-sourced GraphSLAM framework~\cite{gtsam} to obtain the optimized poses of the robot.
These global poses are then fed into the the camera feature tracker of one of the widely used VINS-MONO~\cite{qin2018vins} as the `Oracle' camera locations to perform just the low-compute optimization stages of: (1) feature extraction and tracking, and (2) local feature matching and mapping. 
Thus achieving the best of both worlds and making \name's implementation low-cost, low-power and adaptable.

To achieve robust and stable performance with this key insight, we firstly identify that amongst the existing RF sensors, WiFi is the most ubiquitously deployed in the related application scenarios. 
While few of the past works have tried to integrate RSSI measurements~\cite{bruno2011wislam,ferris2007wifi} it is well known that these RSSI measurements are very fickle for indoor scenarios. 
Further, in recent past, researchers have shown reliable performance with bearing/angle of arrival(AoA) to or from the WiFi sensor on the robot~\cite{arun2022p2slam,jadhav2020wsr} to the Access Points in the environment as the WiFi feature measurement.
So, \name utilizes the WiFi sensor on the robot to measure the bearing/AoA to the Access Point.
% \footnote{Thus any RF-sensor that can report their bearings like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative RF-sensors.}.
% Additionally one can also use the bearing measurement from the Access Point to the WiFi sensor on-board~\cite{jadhav2020wsr,arun2022p2slam}, which would require the Access Points' infrastructure to collaborate with the robot.
We only use the bearing measurements from the Access Point to the robot's WiFi sensor, since the toherway around would require the Access Points to report their measurements to the robot which is not always feasible.
% This collaboration is not always possible and so to ease \name's deployment we just use an on-board WiFi sensor that can report the AoA from the Access Point to the robot's WiFi sensor.

These bearing measurements need to be optimized over multiple poses of the bot in real-time and have to backpropogate any errors in these two-way bearing measurements to optimize for the overall bot and AP poses in real-time. 
To this extent, \name utilizes open-sourced GraphSLAM library's real-time implementation of iSAM~\cite{gtsam} by laying down these additional bearing measurements incrementally as and when they come in along with the relative-pose measurement within a factor graph.
At a high level, the presence of bearings measured at the robot allows for accurate mapping of the WiFi access points in the environment and also simultaneously locate itself with respect to these global landmarks.
Thus, \name does not also need to assume the location of the WiFi access points in the environment, making it independent from the WiFi infrastructure.

Since, \name is not performing end-to-end optimization, the bearing measurements being added to the iSAM factor graph cannot be sparse, noisy or ambiguous to avoid ill-defined factor graph optimization. Unfortunately WiFi signals go though heavy multipath and Non Line of Sight(NLoS) Scenarios in the indoor environment making these bearing measurements more noisier than tolerable. 
To overcome this issue, 
% previous works use packet averaging based techniques in tandem with complex MUSIC algorithms that are time consuming, increasing the latency of the bearing measurement fed into the factor graph for optimization. This in turn would delay the updates in the camera feature tracker, which could lead to disastrous performance in mapping and environment awareness. 
in \name we use novel SVD-FFT based averaging algorithm that performs temporal averaging and measure the accurate bearing measurements in real-time.
Additionally most of the solutions for WiFi bearing measurements assume uniform linear arrays~\cite{ayyalasomayajula2020deep,spotfi,arraytrack,soltanaghaei2018multipath} which can only solve half space, providing an ambiguous aliased peak in the other half plane. To avoid this, in \name we utilize a 4-antenna square array with a side length of $3\lambda/8$, where $\lambda$ is the wavelength of the WiFi signal received. This removes the half-plane ambiguities in our system, thus providing reliable, continuous and unambiguous WiFi bearing measurements in real-time to the iSAM factor graph for real-time pose estimation.

Finally, once the optimized robot poses are generated, these are then sent to the camera factor graph that is using the camera features to track and map the environment. To perform this environment mapping, \name uses the camera feature tracker of one of the widely used VINS-MONO~\cite{qin2018vins} implementations, which uses the WiFi factor graph provided robot poses as the camera's pose initialization with a strong confidence. 
The camera factor graph is also implemented as an iSAM factor graph, using the open-sourced real time GraphSLAM framework~\cite{gtsam}. 
This camera factor graph takes the camera features in tandem with robot poses to them track the features and map the environment without the need for any compute heavy global loop closures. 
Thus \name designs first of its kind layered (dual-graph) approach by bringing the best of both (camera and WiFi) sensors together to solve for a low-cost, low-compute and adaptable SLAM system.

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publically available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.
Furthermore, we showcase our system with a simple application which builds a map labelled with room numbers and autonomously navigates to a given room number to deliver a package. 

==> intro/intros_old/intro5.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Recent time has seen a rise in demand for autonomous robots and drones for various applications ranging from inventory management in warehouses, hospitals, construction sites~\cite{hosptials,warehoueses,construction,sites} in addition to the navigation~\cite{navigation,robots} and exploration robots~\cite{exploration,robots} for last-mile delivery~\cite{last,mile,delivery}, mapping~\cite{Labb2018RTABMapAA}, and disaster relief~\cite{disaster,relief,jadhav2020wsr}. 
This increasing demand has led the researchers towards deploying fleets of robots to increase the efficiency for these applications, for example in last-mile delivery~\cite{last,mile,delivery} or collaborative robots for indoor explorations~\cite{collab,bots}.
These applications brings forth some important requirements for the current SLAM algorithms to be real-time, scalable and deployable:
(a) they should be `low-compute', as they need to run in real-time and sometimes in a memory and compute-limited scenario, (b) they should be `low-cost', so as to be able to deploy them widely, and (c) they should be `adaptable' to different environmental changes, like dynamic-visibility conditions and/or obstacles in the path.


There exist a lot of powerful tools for autonomous robot systems~\cite{Labb2018RTABMapAA,cartographer,orbslam} but these are far from being scalable.
Most of these existing works in SLAM use either IMU/odometry to get the poses of the robot. 
These pose measurements in tandem with camera/LiDAR visual sensors are used to jointly optimize for absolute poses by correcting for the drifts of the IMU/odometry measurements and also to map the environment. 
Firstly, the LiDAR sensors are very expensive, making the LiDAR based SLAM algorithms too costly to deploy.
Secondly, while the camera sensors are low-cost they are compute intensive. 
The joint optimization for optimal Visual SLAM has three distinct operations: (1) feature extraction and tracking, (2) local feature matching and mapping, and (3) global loop-closures. 
While the first two components are not compute intensive but only useful for local pose estimation and mapping, and the global loop-closure algorithms are very compute intensive, memory consuming, time consuming~\cite{semenova2022quantitative} but are required for global corrections, robot poses and map generation.


In contrast, there is a couple of decades of research in RF-based localization and tracking that uses existing RF deployment architectures in the environment, like WiFi, to locate and track various devices in the environment.
As most of the current robots are connected to WiFi and owing to wide-spread deployment of WiFi, researchers have explored towards using WiFi for SLAM implementations~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
These algorithms have been shown to not need global loop-closures making them `low-cost' and 'low-compute' systems~\cite{arun2022p2slam,zhang2020robot}.
\todo{kill p2slam with real-time and zhang et al with range and }
Although, due to the low-wavelength of the WiFi-signals, these algorithms suffer from lack of context or a map of their surroundings. 
Thus making them non-adaptable to various environmental changes that require awareness of the surroundings/map.


To solve these issues, in this paper we present \name-SLAM (\underline{Vi}sual \underline{Wi}Fi \underline{D}ual graph SLAM), that amalgamates the best of both WiFi and camera worlds. 
While there exist few current works that try to incorporate WiFi-signals into existing Visual SLAM algorithms~\cite{hashemifar2019augmenting, liu2019collaborative,nguyen2021viral,jadhav2020wsr}, but these systems only try to use the WiFi signals to aid in the `global loop closures' ~\cite{hashemifar2019augmenting, liu2019collaborative} or depend on the Visual SLAM system to provide the pose of the WiFi sensor on board~\cite{nguyen2021viral,jadhav2020wsr} making them compute and memory hungry, and time consuming.
In contrast, \name is a first of its kind integration that maintains the `low-cost' and `low-compute' of RF sensor, and simultaneously utilizes a simple monocular camera that can provide context/map(`adaptable') making it a scalable and deployable SLAM system.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/placeholder.pdf}
    \caption{\name's layered approach: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time.}
    \label{fig:intro_fig}
\end{figure}


To perform this optimal integration in \name's design, we make two key observations with respect to the existing camera and Visual SLAM systems.
Firstly, while a camera sensor is the best possible solution to provide real-time and low-compute local robot pose and local map, it needs heavy memory and compute resources to perform global robot pose estimation and optimization.
So, if these camera SLAM systems could have access to an `Oracle' that could provide these global robot pose estimates they can just perform the low-compute feature extraction and local feature matching to obtain a final optimized map with global optimized robot poses.
On the other hand, we observe that while the existing WiFi based SLAM approaches provide optimized global robot poses with low-memory and compute demands. So, all these WiFi SLAM systems need are local context/map which could provided by the visual SLAM approaches.
From these observations, \name is designed using the inspiration from network layering/abstraction principals, where in each layer has distinct functionalities and clear boundaries as shown in Figure~\ref{fig:intro_fig}. 
Wherein we firstly use WiFi measurements along with odometry from a combination of a wheel encoder and IMU with an open-sourced GraphSLAM framework~\cite{gtsam} to obtain the optimized global pose estimates of the robot in real-time.
These global pose estimates are then fed as the `Oracle' camera locations into the the camera feature tracker in real-time.
We use one of the widely used VINS-MONO~\cite{qin2018vins} to perform just the low-compute optimization stages of: (1) feature extraction and tracking, and (2) local feature matching and mapping. 
Thus using the best of both sensors and making \name a real-time, scalable and deployable SLAM.

To start with the WiFi factor graph, while a few of the past works have tried to integrate RSSI measurements~\cite{bruno2011wislam,ferris2007wifi} it is well known that these RSSI measurements are very fickle for indoor scenarios. 
Further, in recent past, researchers have shown reliable performance with bearing/angle of arrival(AoA) to or from the WiFi sensor on the robot~\cite{arun2022p2slam,jadhav2020wsr} to the Access Points in the environment as the WiFi feature measurement.
So, \name utilizes the WiFi sensor on the robot to measure the bearing/AoA to the Access Point.
We only use the bearing measurements from the Access Point to the robot's WiFi sensor, since the other way around would require the Access Points to report their measurements to the robot which is not always feasible.
These WiFi bearing measurements are fed to the graph in tandem with IMU/Odometer over multiple poses of the bot in real-time for optimization. This optimization is done over all the robot poses till date in the graph by backpropogating any errors to optimize for the overall bot and AP poses in real-time. 
To this extent, \name utilizes open-sourced GraphSLAM library's real-time implementation of iSAM~\cite{gtsam} by laying down these additional bearing measurements and relative-IMU/Odometer measurements incrementally as and when they come within a factor graph.
At a high level, the presence of bearings measured at the robot allows for accurate mapping of the WiFi access points in the environment and also simultaneously locate itself with respect to these global landmarks.
Thus, \name's WiFi factor graph does not also need to assume the location of the WiFi access points in the environment, making it independent from the WiFi infrastructure.

Additionally, \name's WiFi graph needs to be optimized in real-time as these optimized global pose estimates are fed into the camera graph for real-time local estimates. This real-time WiFi graph optimization poses many challenges to WiFi bearing estimation:

\noindent \textbf{(i) Real-Time Bearing measurements:} Real-time WiFi factor graph optimization in turn demands that the bearing measurements have to be done with minimum latency. While there exist  simple FFT based approaches~\cite{ayyalasomayajula2018bloc} are too inaccurate and provide noisy bearing measurements.

\noindent \textbf{(ii) Accurate Bearing measurements:} Additionally moving WiFi sensors, especially in indoor settings lead to dynamic multipath and Non Line of Sight(NLoS) scenarios making the bearing measurements erroneous and sparse. While, accurate bearing measurement algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} that utilize packet averaging across time, they involve high-latency computations.

\noindent \textbf{(iii) Ambiguous Half-Plane measurements:} Finally most of the solutions for WiFi bearing measurements assume uniform linear arrays~\cite{ayyalasomayajula2020deep,spotfi,arraytrack,soltanaghaei2018multipath} that only solve half space, providing an ambiguous aliased peak in the other half space. 

\name uses a novel SVD-FFT based averaging algorithm that performs real-time temporal averaging by actually identifying the strongest direction component across all the packets.
This leads to reduced noise in the WiFi measurements enabling measurement of accurate bearings in real-time, solving for the first two issues together.
Finally, to avoid the ambiguous peaks problem, in \name we deploy a 4-antenna square array with a side length of $3\lambda/8$ on the robot, where $\lambda$ is the wavelength of the WiFi signal received. 
This removes the half-plane ambiguities in our system, thus providing reliable, continuous and unambiguous WiFi bearing measurements in real-time to the iSAM factor graph for real-time pose estimation.


Secondly for the camera factor graph, the optimized robot poses generated from the WiFi graph are fed to the camera factor graph in real-time.
The camera's local feature tracker and mapping operations are then initialized with these global robot pose estimates with a strong confidence and are optimized using using the open-sourced real time GraphSLAM framework~\cite{gtsam}, iSAM.
For these local pose corrections and mapping, \name uses the camera feature tracker of one of the widely used VINS-MONO~\cite{qin2018vins} implementations.
Since, the camera factor graph utilizes the pre-optimized global pose estimates, it does not need the compute and memory heavy global loop-closure operation.
Thus \name designs first of its kind layered (dual-graph) approach by bringing the best of both (camera and WiFi) sensors together to solve for a low-cost, low-compute and adaptable SLAM system.

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publicly available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.
Furthermore, we showcase \name with a simple application that maps with labelled room numbers and autonomously navigates to a given room number to deliver a package. 

==> intro/intros_old/intro6.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

Recent times have seen a rise in demand for autonomous robots and drones for various applications ranging from inventory management in warehouses, hospitals and construction sites~\cite{hosptials,warehoueses,construction,sites} to the navigation~\cite{navigation,robots} and exploration robots~\cite{exploration,robots} for last-mile delivery~\cite{last,mile,delivery}, mapping~\cite{Labb2018RTABMapAA}, and disaster relief~\cite{disaster,relief,jadhav2020wsr}. 
Furthermore, many of these applications demand a fleet of coordinated robots to perform tasks efficiently. 
To deliver on these applications, Simultaneous Localization and Mapping (SLAM) algorithms need to be (a) `low-compute', to ensure real-time operation on memory and compute constrained machines, (b) `low-cost', to ensure wide deployment, and (c) `context-aware' of environmental changes, which requires a map/context of the environment the robot is exploring.

There exist many powerful tools for autonomous robot systems,~\cite{Labb2018RTABMapAA,cartographer,orbslam} but these are far from being scalable.
Most of these existing works in SLAM use either an IMU or wheel-encoder to get the relative poses of the robot over time. 
These relative pose measurements in tandem with camera/LiDAR visual sensors are used to jointly optimize for absolute robot poses and simultaneously map the environment by correcting for the drifts in the IMU/odometry measurements. Unfortunately, introducing these camera/LiDAR sensors make the SLAM problem very compute and memory intensive.

Joint optimization for optimal Visual SLAM has three distinct operations: (1) feature extraction and tracking, (2) local feature matching and mapping, and (3) global loop-closures. 
The first two components aid in local pose estimation of the robot and mapping of the environment and are generally computationally light. Unfortunately, over time, these pose estimates accrue drifts and when robots revisit previously mapped areas, their current pose estimate disagrees with the map. The third component, performing global loop-closures, corrects for these erroneous drifts and builds coherent maps. Unfortunately, this is very compute and memory intensive and time consuming. 
% While the first two components are not compute intensive but only useful for local pose estimation and mapping, global loop-closure algorithms are very compute intensive, memory consuming, time consuming~\cite{semenova2022quantitative} but are required for global corrections, robot poses and map generation.
Furthermore, LiDAR-sensor based SLAM systems~\cite{cartographer} also utilize a similar three component structure, and the component performing global loop-closures is the most compute and memory intensive. 
% There are also LiDAR sensor based SLAM systems~\cite{cartographer} which also uses global loop closures, and are additionally very expensive, making LiDAR based SLAM algorithms too expensive and high-compute to deploy. 
%will: I moved the lidar sentence to the end of this paragraph since it was stuck in the middle of explaining why camera SLAM is bad

In contrast, there are a couple of decades of research in RF-based localization and tracking~\cite{ayyalasomayajula2018bloc,spotfi,uwb,bacscatter,rfid} that uses existing RF deployment architectures in the environment, like WiFi, to locate and track various devices in the environment.
As most of the current robots are connected to WiFi and owing to wide-spread deployment of WiFi, researchers have explored developing WiFi radios as sensor for SLAM implementations~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
These algorithms have been shown to not need global loop-closures making them `low-cost' and 'low-compute' systems~\cite{arun2022p2slam,zhang2020robot}.
However, \cite{zhang2020robot} uses WiFi backscatter that has very limited range and needs very extensive deployment of backscatter tags making them an expensive deployment.
On the other hand, in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, the authors employ an end-to-end optimization, sidestepping the challenges which arise when real-time pose estimates are needed.
Additionally, WiFi cannot map the space leading to lack of `context-awareness' for both the systems~\cite{arun2022p2slam,zhang2020robot}.


To solve these issues, in this paper we present \name, that amalgamates the best of both WiFi and camera worlds. 
While there exist few current works that try to incorporate WiFi-signals into existing Visual SLAM algorithms~\cite{hashemifar2019augmenting, liu2019collaborative,nguyen2021viral,jadhav2020wsr}, these systems only try to use the WiFi signals to aid in `global loop closures' ~\cite{hashemifar2019augmenting, liu2019collaborative} or depend on the Visual SLAM system to provide the pose of the WiFi sensor on board~\cite{nguyen2021viral,jadhav2020wsr} making them compute and memory hungry, and time consuming.
In contrast, \name is a first of its kind integration that maintains the `low-cost' and `low-compute' of RF sensor, and simultaneously utilizes a simple monocular camera that can provide `context-awareness' through mapping making it a scalable and deployable SLAM system.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/placeholder.pdf}
    \caption{\name's layered approach: WiFi bearings and IMU/Odometry measurements provide for optimized global poses for the robot in real-time using the WiFi factor graph. These optimized poses are then fed to the camera factor graph that then generates the context/map in real-time.}
    \label{fig:intro_fig}
\end{figure}


Two key observations that inspires this scalable \name's design are that firstly, the existing camera based SLAM systems are the best possible solutions to provide a real-time and low-compute local map.
But these camera systems need heavy memory and compute resources to perform global robot pose estimations and optimization. 
So, if these camera SLAM systems could have access to an `Oracle' that could provide these global robot pose estimates, absent of any drifts, they can avoid compute heavy global loop-closures. 
Secondly, the existing WiFi based SLAM approaches provide optimized global robot poses with low-memory and compute demands but do not have context of the map or local surroundings.
Thus, these WiFi SLAM systems can provide for the global optimized poses to the camera SLAM systems which can then be fed as `Oracle' measurements to avoid global loop-closures.
With this intuition and the well established concepts of network layering/abstraction principals, we design a Dual-graph solution for WiFi and Visual SLAM nodes.
Wherein the first WiFi SLAM layer is defined with iSAM, an open-sourced GraphSLAM framework~\cite{gtsam} to obtain the optimized global pose estimates of the robot in real-time.
These global pose estimates are then fed in real-time as the `Oracle' camera locations (or odometry measurements) to the Visual SLAM layer that performs just the low-compute optimization stages of: 
(i) feature extraction and tracking using VINS-MONO~\cite{qin2018vins} algorithm, and 
(ii) local feature mapping and robot pose optimization  using a second `Camera graph' defined in iSAM.
This layered approach make the best use of the individual strengths of each sensing modality allowing \name-SLAM to be a real-time, scalable and deployable SLAM solution.


This \underline{Vi}sual \underline{Wi}Fi \underline{D}ual graph SLAM solution of \name-SLAM leads to the following set of challenges,

\noindent\textbf{Robust WiFi Measurements:} To define the measurements to be used in the WiFi factor graph, few of the past works have tried to integrate RSSI measurements~\cite{bruno2011wislam,ferris2007wifi}. Unfortunately, it is well known that these RSSI measurements are very fickle for indoor scenarios. 
So in recent past, researchers have shown reliable performance with using angle-of-arrivals measured to or from the WiFi sensor on the robot~\cite{arun2022p2slam,jadhav2020wsr} to the Access Points in the environment as the WiFi feature measurement.
Thus, in \name we utilize these robust bearing measurements in tandem with IMU/Odometer over multiple poses of the robot in real-time for optimization.

\noindent\textbf{Real-time and accurate WiFi pose estimates:} Real-time WiFi factor graph optimization in turn demands that the bearing measurements have to be furnished with minimum latency. 
While there exist simple FFT based approaches~\cite{ayyalasomayajula2018bloc} which are low-latency, they can be very inaccurate in estimating the bearing due to dynamic multipath and non-line of sight (NLoS) scenarios. 
While this is currently solved by temporal averaging in MUSIC and SpotFi~\cite{arraytrack,spotfi}, these algorithms are very time-consuming.
But, these algorithms demonstrate that since direct path is the only consistent path over time, temporal averaging would increase the signal strength recieved for direct path over all the reflected paths.
Thus, \name uses SVD-FFT that takes the advantage of packet averaging ideas from the MUSIC and SpotFi~\cite{arraytrack,spotfi} while maintaining the latency of the order of FFT based approaches~\cite{ayyalasomayajula2018bloc}.
These real-time accurate WiFi bearing measurements are then fed to the WiFi graph in tandem with IMU/Odometer measurements over multiple poses of the robot for optimization defined by the iSAM's factor graph~\cite{gtsam}. 

\noindent\textbf{Access Point Initialization:} \name's WiFi real-time iSAM GraphSLAM implementation does not assume the location of the WiFi access points in the environment as most of the existing WiFi SLAM algorithms~\cite{ferris2007wifi,arun2022p2slam}. 
Although unlike the existing works~\cite{arun2022p2slam} that perform end-to-end optimization, \name does real-time pose estimates using incremental pose-graph optimization using iSAM.
This leads to the optimization becoming indeterminate or ill-conditioned in the WiFi graph optimization if the APs are all initialized at the origin.
Thus to overcome this ill-defined optimization issues, in \name we smartly initialize the location of the WiFi AP at the time instance when the signal strength measured for the access point is a local maxima along the path taken.
This further implies that all the bearing factors measured to that AP are also fed into the factor graph at the instance the AP is placed, thus avoiding any ill-conditioned factor graph optimizations.
% This optimization is done over all the robot poses to date in the graph by backpropagating any errors to optimize for the overall bot and AP poses in real-time. \todo{this is not right?} 
% At a high level, the presence of bearings measured at the robot allows for accurate mapping of the WiFi access points in the environment and also simultaneously locate itself with respect to these global landmarks.
% Thus, \name's WiFi factor graph does not also need to assume the location of the WiFi access points in the environment, making it independent from the WiFi infrastructure.

\noindent\textbf{Judicious Pose updates to Camera Graph:} Finally, these optimized robot poses generated from the WiFi graph need to be updated to the camera factor graph defined with iSAM in real-time.
Unfortunately, this is not as straightforward as obtaining real-time pose updates to all the existing odometry pose factors of the camera graph.
As too frequent pose updates that are significantly large for the past Odometer readings would trigger frequent end-to-end graph optimization and updates in the camera graph which becomes memory intensive as the number of robot poses keep increasing.
To avoid this, \name's WiFi graph's pose updates are maintained in a buffer that is continuously updated when there are frequent large updates.
This buffer of pose-updates are pushed as odometer updates to the camera graph only when these global pose updates are lesser than a threshold, which is empirically determined.
This buffer-based updates avoids frequent global camera graph optimization avoiding high compute and memory demanding operations.
% While this buffered-updates creates lag in the camera graph's updates with respect to the WiFi graph.
% Fortunately though, the WiFi Graph optimization is triggered at 100s of Hz that this delay due to buffer-based camera pose updates are not observable for practical robot's real-time mapping and pose-estimation that is performed at 1-10Hz.

With these solutions \name overcomes the challenges of designing first of its kind layered (dual-graph) approach to solve for a low-cost, low-compute and context-aware SLAM system.
% Thus \name designs first of its kind layered (dual-graph) approach by bringing the best out of both the camera and the WiFi sensors to solve for a low-cost, low-compute and adaptable SLAM system.


These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publicly available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.
% Furthermore, we showcase \name with a simple application that maps with labelled room numbers and autonomously navigates to a given room number to deliver a package. 

==> intro/intros_old/intro7.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/placeholder.pdf}
    \caption{\name Deployed in a real world environment with the WiFi SLAM providing accurate global pose estimates and the camera graph providing accurate map of the environment}
    \label{fig:intro_fig}
\end{figure}

Recent times have seen a rise in demand for autonomous robots and drones for various applications ranging from inventory management in warehouses, hospitals and construction sites~\cite{hosptials,warehoueses,construction,sites} to the navigation~\cite{navigation,robots} and exploration robots~\cite{exploration,robots} for last-mile delivery~\cite{last,mile,delivery}, mapping~\cite{Labb2018RTABMapAA}, and disaster relief~\cite{disaster,relief,jadhav2020wsr}. 
Furthermore, many of these applications demand a fleet of coordinated robots to perform tasks efficiently. 
To deliver on these applications, Simultaneous Localization and Mapping (SLAM) algorithms need to be (a) `low-compute', to ensure real-time operation on memory and compute constrained machines, (b) `low-cost', to ensure wide deployment, and (c) `context-aware' to be able to react to environmental changes, which requires a map of the environment the robot is exploring.

There exist many powerful tools for autonomous robot systems,~\cite{Labb2018RTABMapAA,cartographer,orbslam} but these are far from being scalable.
Most of these existing works in SLAM use either an IMU or wheel-encoder to get the relative poses of the robot over time. 
These relative pose measurements in tandem with Visual/LiDAR sensors are used to jointly optimize for absolute robot poses and simultaneously map the environment by correcting for the drifts in the IMU/odometry measurements. 
Unfortunately, introducing these Visual/LiDAR sensors make the SLAM problem very compute and memory intensive.

Joint optimization for optimal Visual SLAM has three distinct operations: (1) feature extraction and tracking, (2) local feature matching and mapping, and (3) global loop closures. 
The first two components aid in local pose estimation of the robot and mapping of the environment and are generally computationally light. Unfortunately, over time, these pose estimates accrue drifts and when robots revisit previously mapped areas, their current pose estimate disagrees with the map. The third component, performing global loop closures, corrects for these erroneous drifts and builds coherent maps. Unfortunately, this is very compute and memory intensive and time consuming. 
Furthermore, LiDAR-sensor based SLAM systems~\cite{cartographer} also utilize a similar three component structure, and the component performing global loop closures is the most compute and memory intensive. 

In contrast, there are a couple of decades of research in RF-based localization and tracking~\cite{ayyalasomayajula2018bloc,spotfi,uwb,bacscatter,rfid,ma2019wifi} that uses existing RF deployment architectures in the environment, like WiFi, to locate and track various devices in the environment.
As most of the current robots are connected to WiFi and owing to wide-spread deployment of WiFi, researchers have explored developing WiFi radios as sensor for SLAM implementations~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
These algorithms have been shown to not need global loop closures making them `low-cost' and 'low-compute' systems~\cite{arun2022p2slam,zhang2020robot}.
However, \cite{zhang2020robot} uses WiFi backscatter that has very limited range and needs very extensive deployment of backscatter tags making them an expensive deployment.
On the other hand, in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}, the authors employ an end-to-end optimization, sidestepping the challenges which arise when real-time pose estimates are needed.
Additionally, WiFi cannot map the space leading to lack of `context-awareness' for both the systems~\cite{arun2022p2slam,zhang2020robot}.


To solve these issues, in this paper we present \name, that amalgamates the best of both WiFi and camera worlds and provides for accurate pose estimations and low-compute, low-power mapping as demonstrated in Figure~\ref{fig:intro_fig}.
While there exist few current works that try to incorporate WiFi-signals into existing Visual SLAM algorithms~\cite{hashemifar2019augmenting, liu2019collaborative,jadhav2020wsr}, these systems only try to use the WiFi signals to aid in `global loop closures' ~\cite{hashemifar2019augmenting, liu2019collaborative} or depend on the Visual SLAM system to provide the pose of the WiFi sensor on board~\cite{jadhav2020wsr} making them compute and memory hungry, and time consuming.
In contrast, \name is a first of its kind integration that maintains the `low-cost' and `low-compute' of RF sensor, and simultaneously utilizes a simple monocular camera that can provide `context-awareness' through mapping making it a scalable and deployable SLAM system.


Two key observations that inspires this scalable \name's design are that firstly, the existing camera based SLAM systems are the best possible solutions to provide a real-time and low-compute local map.
But these camera systems need heavy memory and compute resources to perform global robot pose estimations and optimization~\cite{semenova2022quantitative}. 
So, if these camera SLAM systems could have access to an `Oracle' that could provide these global robot pose estimates, absent of any drifts, they can avoid compute heavy global loop closures. 
Secondly, the existing WiFi based SLAM approaches provide optimized global robot poses with low-memory and compute demands~\cite{arun2022p2slam,jadhav2020wsr} but do not have context of the map or local surroundings.
Thus, these WiFi SLAM systems can provide for the global optimized poses to the camera SLAM systems which can then be fed as `Oracle' measurements to avoid global loop closures.
With this intuition and the well established concepts of network layering/abstraction principals~\cite{session1994it5}, we design a Dual-graph solution for WiFi and Visual SLAM nodes.
Wherein the first WiFi SLAM layer obtains the optimized global pose estimates of the robot in real-time.
These global pose estimates are then fed in real-time as the `Oracle' camera locations (or odometry measurements) to the Visual SLAM layer.
This Visual SLAM system not needing global loop-closures only performs just the low-compute optimization stages (1 and 2 from above) providing local pose corrections and environment mapping. Thus making \name's design scalable.


This \underline{Vi}sual \underline{Wi}Fi \underline{D}ual graph SLAM solution of \name-SLAM leads to the following set of challenges:

\noindent\textbf{(a) Robust WiFi Measurements:} To define the measurements to be used in the WiFi factor graph, few of the past works have tried to integrate RSSI measurements~\cite{bruno2011wislam,ferris2007wifi}. 
Unfortunately, it is well known that these RSSI measurements are very fickle for indoor scenarios. 
So in recent past, researchers have shown reliable performance with using angle-of-arrivals measured to or from the WiFi sensor on the robot~\cite{arun2022p2slam,jadhav2020wsr} to the Access Points in the environment as the WiFi feature measurement.
Thus in \name, we utilize these robust bearing measurements in tandem with IMU/Odometer over multiple poses of the robot in real-time for optimization.

While most of these bearing measurements are done taking the advantage of Uniform Linear arrays~\cite{arraytrack, spotfi}, but these linear arrays can only solve for half-planes thus providing for ambiguity whether the robot is in front or at the back of the AP. Thus in \name we avoid this issue by adapting to a square antenna array with appropriate antenna spacing to avoid any ambiguities.

\noindent\textbf{(b) Real-time \& accurate WiFi Bearing estimates:} Real-time WiFi factor graph optimization in turn demands that the bearing measurements have to be furnished with minimum latency. 
While there exist simple FFT based approaches~\cite{ayyalasomayajula2018bloc} which are low-latency, they can be very inaccurate in estimating the bearing due to dynamic multipath and non-line of sight (NLoS) scenarios. 
While this is currently solved by temporal averaging in MUSIC and SpotFi~\cite{arraytrack,spotfi}, these algorithms are very time-consuming.
But, these algorithms demonstrate that since direct path is the only consistent path over time, temporal averaging would strengthen the signal received for direct path over all the reflected paths.

\name uses novel SVD-FFT algorithm that takes the advantage of packet averaging ideas from the MUSIC and SpotFi~\cite{arraytrack,spotfi} while maintaining the latency of the order of FFT based approaches~\cite{ayyalasomayajula2018bloc}.
These real-time accurate WiFi bearing measurements are then fed to the WiFi graph in tandem with IMU/Odometer measurements over multiple poses of the robot for optimization defined in iSAM~\cite{gtsam}. 

\noindent\textbf{(c) Access Point Initialization:} \name's WiFi real-time iSAM GraphSLAM implementation does not assume the location of the WiFi access points in the environment as most of the existing WiFi SLAM algorithms~\cite{ferris2007wifi,arun2022p2slam}. 
Although unlike the existing works~\cite{arun2022p2slam} that perform end-to-end optimization, \name does real-time pose estimates using incremental pose-graph optimization using iSAM.
This leads to the optimization to be ill-conditioned in the WiFi graph optimization if the APs are all initialized at the origin.

To overcome this ill-defined optimization issues, in \name we initialize the location of the WiFi AP at the time instance when the signal strength measured for the access point is a local maxima along the path taken.
This further implies that all the bearing factors measured to that AP are also fed into the factor graph at the instance the AP is placed, thus avoiding any ill-conditioned factor graph optimizations.


\noindent\textbf{(d) Judicious Pose updates to Camera Graph:} Finally, the optimized robot poses generated by the WiFi graph update the robot poses in the camera factor graph in real-time.
A straightforward way to update these robot poses would be for the WiFi graph to push all the updates and trigger an end-to-end optimization of the camera graph to fix all pose drifts accumulated. 
Unfortunately, frequent, numerous and large pose updates which trigger end-to-end graph optimization in the camera graph becomes memory intensive. 

To keep the memory usage low and provide accurate pose updates to camera graph, \name's WiFi graph's updates are buffered when frequent and large corrections are made. 
Finally, once the large corrections to the WiFi graph are completed, which spans a period of few seconds, this buffer of pose corrections is pushed as `Oracle' updates to the camera graph. This buffer-based updates avoids frequent global camera graph optimization avoiding high compute and memory demanding operations.

% \noindent\textbf{Easy Integration of All Sensing Modalities:}  \todo{Add final system level contribution of enabling easy integration of any sensing modality with wifi graph.}

With these solutions \name overcomes the challenges of designing first of its kind layered (dual-graph) approach to solve for a low-cost, low-compute and context-aware SLAM system. 
Additionally, this layered approach of \name enables the same advantages as it did for communication layers, in that each layer could be independently used as a plug and play model.
That is, although we have demonstrated \name using WiFi owing to its wide-scale deployment one of the major advantages \name is that it abstracts bearing as the sensor measurement input, and global pose updates as the output.
Thus any RF-sensor that can report their bearings like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative RF-sensors.
These sensors like WiFi sensors would also provide the global pose estimates that can be plugged into the camera graph. Similarly, the camera graph is not limited to either the VINS-MONO feature extractor or on camera itself, we can easily replace it with LiDAR and its corresponding sensor to get the similar mapping results from the global pose estimates received from the RF-Graph.

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over publicly available different datasets with three different scenarios. These scenarios have data across two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested by driving a robot a cumulative distance of over $1225$ m in these two environments. We show an improvement of at least $xx \times$ over purely relying on visual odometry. Furthermore, testing in visually-challenging scenarios shown \name perform at least $xx \times$ as compared to visual odometry.

==> intro/intros_old/intro8.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/visual_drawbacks-crop.pdf}
    \caption{Drawbacks of Visual SLAM systems: (a) Local loop-closures are scalable (b) Global loop-closures and corrections make these systems memory and compute intensive.}
    \label{fig:visual-bad}
\end{figure}
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
The advantage of these robots, apart from being autonomous, is that they can be deployed without any prior knowledge of the environment and the robots can explore and navigate within the environment.
This is because these robots utilize a Simultaneous Localization and Mapping (SLAM) framework, where they can simultaneously locate themselves and map the environment around them.
Despite these advantages, the current SLAM based robot systems are not yet widely deployed for these indoor applications.


The majority of current SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometer measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment.
These visual and LiDAR sensors that grant the system mapping and localization capabilities also make the system both memory and compute intensive~\cite{semenova2022quantitative}.
This is mainly because of the `loop-closures' happening as shown in Figure~\ref{fig:visual-bad}b.

Conceptually these Visual sensors are identifying key features (f1-f10k) in the environment called `landmarks'.
These landmarks are mapped and in turn the robot locating itself with respect to how these landmarks are changing from one instance to the other, thus performing SLAM.
However, as seen the robot can quickly accrue drift due to Odometer readings and needs correction which happens by matching current landmarks with old ones.
While this is not memory or compute intensive for local corrections as shown in Figure~\ref{fig:visual-bad}a which requires smaller search space of `landmarks' and fewer pose corrections.
But global `loop-closure' as shown in Figure~\ref{fig:visual-bad}b would need active memory of all the 10k landmarks and corrections backpropagated over many poses, making the system memory and compute intensive.
In order to make these SLAM robotic systems scalable we need a SLAM system design that achieves compute and memory efficiency without compromising on the robot pose estimation and environment mapping.
Consequently, identifying a sensor to use in the SLAM systems that can alleviate these limitations of Visual and LiDAR sensors is required.
WiFi based SLAM systems are an attractive sensor modality which have shown to be memory and compute efficient~\cite{arun2022p2slam,bruno2011wislam,zhang2020robot}.
So the idea of the dual-layered SLAM is that the first WiFi SLAM layer obtains the optimized global pose estimates of the robot in real-time, which are then sent over to the camera SLAM.
Unfortunately though, since they utilize WiFi as the only sensor neglecting the already widely deployed cameras on the robots which in turn disable them from getting the map of the environment compromising the intent of SLAM.

To that end, we propose \name's key idea of a Dual-layered solution for WiFi and Visual (camera) SLAM nodes, or rather ViWiD-SLAM (\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered SLAM) that is inspired from the network layering/abstraction principals~\cite{session1994it5}. 
A key intuition that motivates this dual-layered design of \name, is that for the camera SLAM can be made compute and power efficient if the robot had accurate pose estimates from an `Oracle'.
Since, this knowledge of accurate pose estimates, would not lead to the accrued drift on a global scale as shown in Figure~\ref{fig:visual-bad}b.
This avoids the need for compute and memory intensive global loop closures, while still being able to map the environment using local mapping.
Thus, the Visual SLAM system can utilize the global poses from WiFi layer as `Oracle' measurements and can track the landmarks from the monocular camera and optimize for local pose corrections and provide a map of the environment.
Thus, this Dual-layered WiFi and Visual SLAM systems enable compute and memory efficient SLAM system that can provide accurate global pose estimations and map.

This abstraction of the complementary pose estimation WiFi SLAM, and the environment mapping Visual SLAM layers has advantages as in networking layer abstractions~\cite{session1994it5}.
That is both the pose estimation layer and the mapping layer can be optimized within themselves without effecting the other layer's performance.
For example, while we use WiFi-sensor for \name's implementation due to its widespread deployment in indoors, other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or the next gen 5G femto-cell implementations~\cite{5g} can be used as alternative sensors depending on the use case.

To implement \name, we have deployed both the WiFi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
This GraphSLAM framework utilizes the measurements from the sensors as factors to tie the mapped environment to the robot poses and optimize for both robot poses and the map simultaneously.
So, we need to first identify the measurements for both WiFi and the Visual camera sensors that can be used to define the graph for the GraphSLAM optimization framework.
To this extent, we use the widely used Shi-Tomasi features~\cite{shi1994good} for the camera sensor and extract them using the opensourced VINS-MONO feature tracker~\cite{qin2018vins}.
For the WiFi sensor features, it has been extensively shown that the angle of arrival(AoA) measurements  based localization~\cite{spotfi,arraytrack} and SLAM~\cite{arun2022p2slam,jadhav2020wsr,zhang2020robot} are more robust.
Thus in \name, we utilize these AoA measurements in tandem with IMU/Odometer over multiple poses of the robot in real-time for optimization of the WiFi SLAM layer.


In the WiFi SLAM layer, to provide the `Oracle' global pose estimates to the Camera graph, we need to be able to perform real-time WiFi graph optimization. 
This in turn demands real-time and robust AoA measurements from the WiFi readings.
While the  existing AoA prediction algorithm like MUSIC and SpotFi~\cite{arraytrack,spotfi} provide robust measurements using temporal averaging and super-resolution, they are very time-consuming.
But, these algorithms demonstrate that since direct path is the only consistent path over time, temporal averaging would strengthen the signal received for direct path over all the reflected paths.
With this intuition, in \name we create a novel real-time and robust AoA estimation algorithm we call \textit{SVD-FFT}.
This algorithm takes the advantage of packet averaging ideas from the MUSIC and SpotFi~\cite{arraytrack,spotfi} while maintaining the latency of the order of 2D-FFT based approaches~\cite{ayyalasomayajula2018bloc,xie2019md}.
These real-time accurate WiFi bearing measurements are then fed to the WiFi graph in tandem with IMU/Odometer measurements over multiple poses of the robot for optimization defined in iSAM~\cite{gtsam}. 


Additionally, as with any SLAM system \name's WiFi SLAM layer does not assume apriori information about the environment which includes the location of the WiFi access points to which robot measures its AoA. 
This lack of knowledge of WiFi access points do not lead to any inconsistencies when the WiFi graph is optimized end-to-end in post-factum to data collection as demonstrated in $\mathrm{P^2}$SLAM~\cite{arun2022p2slam}.
Unlike $\mathrm{P^2}$SLAM, \name does real-time pose estimates using incremental pose-graph optimization using iSAM that lays down the WiFi AoA measurements incrementally.
This would lead to many of the APs have which not yet been discovered in the environment or are not effected by the current incoming bearing measurements, thus making the optimization problem ill-defined.
To overcome this ill-defined optimization issues, in \name we take advantage of the WiFi received signal strength (RSSI) proximity sensing~\cite{ez,zee}.
That is we initialize the location of the WiFi AP at the time instance when the RSSI measured for a given access point is a local maxima along the path taken.
This further implies that all the AoA measurements to that AP are also fed into the graph optimization at the instance the AP is placed, thus avoiding any ill-conditioned optimization definitions.


Finally, the optimized robot poses generated by the WiFi graph update the robot poses in the camera graph in real-time.
Unfortunately, frequent, numerous and large pose updates which trigger end-to-end graph optimization in the camera graph becomes memory and compute intensive. 
While, we can naively add simple timed buffer to lag the camera graph behind the WiFi graph this would be inefficient as these numerous and large pose updates do not always occur.
Instead, in \name's design we buffer the WiFi graph's updates only when frequent and large corrections to the past poses are made. 
Once the large corrections to the WiFi graph are completed, this buffer of pose corrections is pushed as `Oracle' updates to the camera graph. 
This smart buffer-based updates avoids frequent global camera graph optimization avoiding high compute and memory demanding camera optimization operations.

These effective solutions surmount the key challenges to integrate WiFi sensing readily into a SLAM framework. We evaluate \name over a publicly available dataset~\cite{arun2022p2slam} and also a more complete dataset we have collected. Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment. \name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} cpu cores which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item Finally, we show that this low-compute and low-memory does not compromise \name's SLAM performance. Where we show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error which are on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Additionally, we would also open-source the dataset that we have collected to enable further research and development in this layered SLAM domain for sensor fusion approaches.



==> intro/intros_old/intro9.tex <==
% !TEX root = root.tex
\section{Introduction}\label{sec:intro}

%Paragraph establishes SLAM, why we need SLAM
Diverse indoor applications like inventory management in warehouses, hospitals and construction sites~\cite{melenbrink2020site}, last-mile delivery~\cite{lastmile}, and disaster relief~\cite{jadhav2020wsr} are increasingly interested in deploying autonomous robot systems~\cite{stewart2021unmanned,marketlastmile}.
Indoor robots are typically equipped with Simultaneous Localization and Mapping (SLAM) framework, enabling real-time navigation and mapping of the robot's environment. This is crucial for many tasks expected of an indoor robot.
However, limitations in current SLAM frameworks limit the uptake of indoor robotics in real-world applications.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/placeholder.pdf}
    \caption{\name's Design: \name is deployed in a Dual Layered approach. The first layer that uses Wi-Fi sensor reports the robot poses to the \name camera layer which maps the environment making \name compute and memory efficient.}
    \label{fig:intro-fig}
\end{figure}
%Why visual SLAM is bad(high level)

Current state-of-the-art SLAM systems like RTABMap~\cite{Labb2018RTABMapAA}, Cartographer~\cite{cartographer}, Kimera~\cite{rosinol2021kimera}, or ORB-SLAM~\cite{mur2015orb} use visual (monocular or RGB-D cameras) or LiDAR sensors in tandem with odometry (dead-reckoning) measurements reported from IMUs (inertial measurement unit) or wheel-encoders to locate themselves and map the environment. These different sensors are typically combined with a sensor-fusion algorithm in a technique known as Graph SLAM~\cite{grisetti2010tutorial}.
However, fusing these measurements makes the SLAM system both memory and compute intensive~\cite{semenova2022quantitative}.
The way these visual SLAM systems work is by correlating sensor observations of the environment across frames to estimate the robot's motion, while simultaneously inserting these observations into a map.
These correlations can be used to correct for drifts in the robot's estimated trajectory, as when the robot returns to a previous location, it will observe the same features in its environment.
The drawback of this method is that as new features are observed, they must constantly be correlated with all past observed features, to see if the robot has been to its current location before.
Thus, current Visual SLAM systems are memory and compute intensive, as the robot must keep all features it has seen in memory, and spend increasing compute time looking them up and comparing them as it observers more new features.
Thus, existing Visual SLAM systems are not light-weight and require extensive compute and memory resources to operate in real time, hindering their deployment in the real world~\cite{semenova2022quantitative}. However, visual sensors are still necessary for building a contextual map of the robot's environment. So, there is a need for a robust Simultaneous `Localization' and `Mapping' solution that is also compute and memory efficient to make these autonomous indoor robots scalable.


%Put Wi-Fi->visual dual layers right after first sentence
%get rid of 'visual slam' emphasize that we don't use loop closures
%high level design
%We feed probabilistic path from Wi-Fi layer to visual layer which now doesn't need to
We present \name, "\underline{Vi}sual \underline{Wi}Fi \underline{D}ual layered (\name) SLAM", a dual-layered SLAM algorithm, which uses a Wi-Fi sensing based layer to provide pose (position and orientation) estimations, without assuming the Wi-Fi access point locations, to \name's visual layer as shown in Figure~\ref{fig:intro-fig}.
Since Wi-Fi pose measurements do not accrue drift over time, unlike standard visual SLAM algorithms, \name does not need to cross-correlate measurements across time to correct for these drifts.
Thus, using the \name Wi-Fi layer's pose estimations the map can be estimated by the \name visual layer in a compute and memory efficient manner.
Thus, \name enables compute and memory efficient SLAM that can provide accurate robot pose estimations provided by the \name Wi-Fi layer and a map of the environment provided by the \name Camera layer.
While \name Wi-Fi layer uses a Wi-Fi sensor due to its widespread deployment in indoor scenarios, our method generalizes to other RF-sensors like BLE~\cite{ble}, UWB~\cite{uwb} or next gen 5G femto-cell implementations~\cite{5g}. 
Additionally, this abstraction of the complementary pose estimation WiFi layer, and the environment mapping \name Visual layers will bring the advantages of networking layer abstractions~\cite{session1994it5} to the research in SLAM.
%above paragraph: emphasize no AP priors

% figure: robot, rf layer -> visual layer
%Design ideas behind dual-graph (bring up performance), can use more than just Wi-Fi.

However, this visual-Wi-Fi integration cannot be accomplished by simply using existing Wi-Fi localization solutions and feeding them into existing Visual SLAM algorithms.
We identify three key challenges presented by integrating Wi-Fi-based sensors with visual SLAM:

\noindent\textbf{Accurate, Real-time Wi-Fi-layer Pose estimation:} In order to accurately estimate the map, the visual layer requires drift-free pose estimates from the Wi-Fi layer to be robust and real-time. To get these pose estimates from the Wi-Fi-layer, we employ Angle of Arrival (AoA) based localization~\cite{spotfi,jadhav2020wsr,arun2022p2slam,ayyalasomayajula2018bloc}, due to its widespread use.
However, it is well known that the Wi-Fi sensors are vulnerable to erroneous AoA measurements~\cite{arraytrack,spotfi}, due to reflectors in the environment (multipath).
While standard AoA-based algorithms like MUSIC and SpotFi~\cite{arraytrack,spotfi} have tackled this issue, these systems use compute intensive super-resolution algorithms, which cannot provide AoA measurements at the rate needed for real time pose estimation.
%I would be cautious about bragging too much about svdfft, it is not a new algorithm.
To solve this, in \name we employ a CSI de-noising algorithm, borrowing intuition from MUSIC~\cite{schmidtmusic,spotfi}, which both smooths erroneous measurements and attenuates multipath components in the signal. This smoothed CSI can then be fed to a 2D-FFT transform~\cite{ayyalasomayajula2018bloc,xie2019md}, for accurate and low-compute real-time AoA measurements. We use this method to measure AoA between the robot and Wi-Fi access points in the environment. However, this alone cannot provide accurate robot pose estimates, as for a generalizable SLAM system, we cannot assume access point locations are known a priori.

\noindent\textbf{Unknown Wi-Fi Access Point Locations:} GraphSLAM~\cite{gtsam} is well known to jointly solve for multi-variate optimization as long as these variable are connected by some measurements.
So we define the Wi-Fi graph with the Odometry measurements connecting two continuous robot poses, and the Wi-Fi AoA measurements connecting the robot's current pose with each AP's position the AoA corresponds to. 
Now to be able to jointly-optimize for the Wi-Fi graph, and as with all optimizers, we need to provide initial values to variables in question. 
While we can initiate the Robot's pose to Odometer's readings, locations of Wi-Fi APs have no priors. 
To overcome this issue, a naive solution can be to initialize all the AP locations at the origin. 
This is not an issue when the AP's are strongly constrained with multiple AoA measurements to multiple robot poses after all the data has been collected~\cite{arun2022p2slam}. 
However, when few measurements constrain the AP's pose, as is the case when the robot first traverses the environment for the real time, the optimizer is poorly conditioned. 
To overcome this poorly conditioned optimization, in \name we take advantage of the Wi-Fi received signal strength (RSSI) proximity sensing~\cite{ez,zee}.
That is we initialize the location of the Wi-Fi AP at the time instance when the RSSI measured for a given access point is a local maxima along the path taken.

\noindent\textbf{Efficient Pose Updates to Camera Graph:} Finally, the optimized robot poses generated by the Wi-Fi graph need to update the robot poses in the camera graph in real-time.
Unfortunately, if the already traversed robot poses are getting large corrections very frequently, it would result in large and frequent feature map corrections in the camera graph as well, making the system compute intensive.
To resolve this, \name uses a smart buffer that continuously monitors the pose corrections being made the Wi-Fi pose estimations and accumulates all the corrections to be made.
These accumulated corrections are only pushed to the Camera graph when the buffer detects that large pose corrections are no longer detected. 
Thus the smart buffer-based updates makes the camera graph optimization efficient by avoiding any possible memory or compute intensive stages.


These effective solutions surmount the key challenges to integrate Wi-Fi sensing readily into a SLAM framework.
To implement \name, we have deployed both the Wi-Fi SLAM system and the Visual SLAM system using the widely used real-time GraphSLAM framework of iSAM~\cite{gtsam}.
We extract widely used Shi-Tomasi features~\cite{shi1994good} for the camera sensor using the opensourced VINS-MONO feature tracker~\cite{qin2018vins}.
We evaluate \name over a publicly available dataset~\cite{arun2022p2slam} and also a more complete dataset we have collected.
Over these datasets, we have scenarios covering two different paths driven in a $25 \times 30$ m and another path driven in a $50 \times 40$ environment.
\name is robustly tested with the robot driven cumulative distance of over $1225$ m across these two environments. 
We demonstrate the following key results to verify the low-compute and low-memory design of \name's SLAM:
\begin{itemize}[leftmargin=*]
    \item Firstly, we show that \name reduces the average compute utilization to \todo{$xx$} CPU memory which is \todo{$xx\times$} (\todo{$y\times$}) the Visual SLAM (LiDAR SLAM).
    \item We also show that \name-SLAM reduces the average memory utilization to \todo{$xx$}MB which is \todo{$xx\times$} (\todo{$y\times$}) the Visual (LiDAR) SLAM.
    \item We show a pose estimation performance with \todo{xx}cm median location estimation error and\todo{$yy^{\circ}$} median orientation estimation error on par with the state-of-the art systems.
    \item We also show the \name's mapping accuracy by mapping the camera fiduciary markers accurate to within \todo{$xx$}cm of error, on par with the state of the art as well.
\end{itemize}
Finally, we would open-source \name's code for the dual-graph framework and the dataset we have collected, to enable further research and development in layered SLAM domain for sensor fusion approaches.

==> related_work/related.tex <==
% !TEX root = root.tex
\section{Related Work}\label{sec:related}

\name's design motivation is to develop a context enabled SLAM algorithm that is low-cost, low-compute and solves for the problems plaguing many existing works. 
These existing works span the fields of visual sensor based SLAM, RF-sensors in SLAM and RF-sensor based localization, mapping, and tracking algorithms.

\noindent\textbf{Visual SLAM:} SLAM for Indoor navigation has been actively pursued by the robotics community for the past decade that led to a myriad of SLAM algorithms~\cite{Labb2018RTABMapAA,mur2015orb,qin2018vins,cartographer}. Most of these algorithms extensively rely on LiDAR~\cite{cartographer} and/or cameras (both monocular or RGBD)~\cite{Labb2018RTABMapAA, mur2015orb}. While these algorithms achieve cm-accurate localization and feature-rich mapping of the environment, they tend to fail under poor-lighting conditions, feature-degenerate conditions. These algorithms also rely on `loop closures' and `re-localization' for larger spaces that require heavy compute on edge making them difficult to scale. In contrast, \name is designed to rely on WiFi for localization and camera for context/mapping thus removing the need for loop closures for the compute intensive camera features. This design ensures that it does not rely on loop closures as the WiFi APs are a constant landmarks known to the robot making it low-compute  and still providing the context of the map.

\noindent\textbf{Dual Layered SLAM:} There are other dual layered SLAM body of works that just use Visual sensors for both the pose estimation and the mapping, called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel}. 
While, these works try to minimize the calls but still use loop-closures loop-closures and bundle adjustments making them less memory and compute efficient compared to \name's design.
On the other hand, there are some Decentralized SLAM works that off-load the memory intensive loop-closure and map updates~\cite{cieslewski2018data,ahmad2020carmap} to the cloud to minimize the memory and compute on the device deployed on the robot. Even these works can benefit from \name's implementation to make systems more efficient even at the cloud.
Finally, there are some outdoor navigation works that utilize GPS as an additional sensor for outdoor autonomous driving assistance systems~\cite{nandikolla2021navigation,kiss2019gps} but are still limited to using loop-closures to correct for the car's pose in the long run owing to GPS's poor resolution.

\noindent\textbf{RF-sensors for SLAM:} Many RF-technology based SLAM implementations based on UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot} exist. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi. 
We note that, extension of \name's WiFi implementation to other RF-sensors is trivial, as we abstract bearing as the measurement feature of the WiFi sensor's measurement. 
Thus, as long as they are able to measure bearings~\cite{uloc} to and/or from the robot to fixed access points in the environment any RF system can make use of \name's implementation.


\noindent\textbf{WiFi-SLAM:} There are a few existing works~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi,hashemifar2019augmenting, liu2019collaborative} that try to utilize WiFi sensor readings to improve SLAM algorithms. Unfortunately, most of these works utilize RSSI as the features metric which needs intense mapping of the space and are known to vary drastically in dynamic indoor scenarios~\cite{ma2019wifi}, making them unsuitable metrics for WiFi signals.
While there are recent works~\cite{jadhav2020wsr,arun2022p2slam} that utilize bearing measurements for their SLAM implementations, WSR~\cite{jadhav2020wsr} does not perform localization but just robot reconnaissance. On the other hand, $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} does not provide any context of the surroundings and performs an end-to-end optimization which does not help in making real-time context aware decisions for the robots. In contrast, \name uses camera features for providing real-time context to in-tandem WiFi bearing measurements that are enabling accurate localization of the robot.

\noindent\textbf{RF Localization:} Past two decades of research in RF-based localization, does not SLAM but only localization and tracking~\cite{spotfi,arraytrack,soltanaghaei2018multipath,ayyalasomayajula2020deep, ma2019wifi} of either the source or the receiving sensor. In contrast, \name integrates WiFi with camera to Simultaneously Locate the bot and Map the environment, without assuming any prior information about locations in the environment.


\iffalse
\name's concept and design overlap with a myriad of fields ranging from SLAM for robotics to RF-sensors based localization, tracking and navigation systems
% Visual sensors -- Camera/Lidar based

\noindent\textbf{Visual Sensors:} Indoor navigation has been actively pursued by the robotics community in the past decades. There is extensive work relying on LIDAR's~\cite{} and cameras~\cite{} which allow for cm-accurate navigation estimates in feature-rich and well-lit environments. Unfortunately, as discussed above, these assumptions may not be valid in a large number of environments. 

Radar Based 

Audio/Ultrasonic

RFID based

UWB/Bluetooth based

WiFi Based sensing
1. Cover existing localization work -- spotfi, arraytrack, ubilocate etc.
  Work poorly in Low density scenario

k poorly in Low density scenario
  Show only stationary device results
  Do not demonstrate real-time localization requirements
  Do not identify poor packets and provide confidence metrics
2. RSSI-based SLAM
3. Loop closure assistance using RSSI
4. CSI-AoA methods

VIRAL SLAM~\cite{nguyen2021viral} uses UWB based ranging in conjunction with LiDAR's, cameras and IMU's to develop a tightly coupled and robust 3D drone based localization and mapping. \todo{not strong enough: Unfortunately, the deployment of various UWB anchors in the environment limits the adoption of this solution}. \todo{kill radar: Why?} The systems proposed in \cite{sato2019rapid, jadidi2018radio} use range information extracted from BLE's received signal strength to correct for drifts accrued by the onboard IMU. Unfortunately, RSSI-based systems have been proven to be inadequate to changing environment conditions and hence act as a poor proxy to range. RFly~\cite{ma2017drone} takes advantage of  RFID tags attached in the environment as robust landmarks, and in conjunction with RFID readers deployed in the environment, jointly estimates the location of a drone and these RFID tags. In a similar vein, Rover~\cite{zhang2020robot} uses WiFi backscatter tags placed in the environment to jointly estimate the location of the robot and tags. Unfortunately, these tags have small range and these systems would require a dense deployment of tags to work, scaling poorly to large environments and requiring a high cost of deployment. The final RF based sensing briefly touched upon before is WiFi. It provides inherent advantages due to its long range and ubiquitous deployment both in the environment and on most robots. 
\fi

==> related_work/related2.tex <==
% !TEX root = root.tex
\section{Related Work}\label{sec:related}

\name's design motivation is to develop a context enabled SLAM algorithm that is low-cost, low-compute and solves for the problems plaguing many existing works. 
These existing works span the fields of visual sensor based SLAM, RF-sensors in SLAM and RF-sensor based localization, mapping, and tracking algorithms.

\noindent\textbf{Visual SLAM:} SLAM for Indoor navigation has been actively pursued by the robotics community for the past decade that led to a myriad of SLAM algorithms~\cite{Labb2018RTABMapAA,mur2015orb,qin2018vins,cartographer}. Most of these algorithms extensively rely on LiDAR~\cite{cartographer} and/or cameras (both monocular or RGBD)~\cite{Labb2018RTABMapAA, mur2015orb}. While these algorithms achieve cm-accurate localization and feature-rich mapping of the environment, they tend to fail under poor-lighting conditions, feature-degenerate conditions. These algorithms also rely on `loop closures' and `bundle-adjustments' for larger spaces that require heavy compute on edge making them difficult to scale. In contrast, \name does not need loop closures or `bundle adjustments'  to provide accurate pose estimations and human readable maps.

\noindent\textbf{Dual Layered SLAM:} There are other dual layered SLAM body of works that just use Visual sensors for both the pose estimation and the mapping, called Parallel Tracking and Mapping (PTAM)~\cite{pire2017s,forster2014svo,klein2007parallel}. 
While, these works try to minimize the calls but still use loop-closures loop-closures and bundle adjustments making them less memory and compute efficient compared to \name's design.
On the other hand, there are some Decentralized SLAM works that off-load the memory intensive loop-closure and map updates~\cite{cieslewski2018data,ahmad2020carmap} to the cloud to minimize the memory and compute on the device deployed on the robot. Even these works can benefit from \name's implementation to make systems compute and memory efficient even at the cloud, owing to \name's light-weight design.
Finally, there are some outdoor navigation works that utilize GPS as an additional sensor for outdoor autonomous driving assistance systems~\cite{nandikolla2021navigation,kiss2019gps} but are still limited to using compute and memory intensive loop-closures to correct for the car's pose in the long run owing to GPS's poor resolution.

\noindent\textbf{RF-sensors for SLAM:} Many RF-technology based SLAM implementations based on UWB~\cite{nguyen2021viral}, BLE~\cite{sato2019rapid, jadidi2018radio}, RFID~\cite{ma2017drone}, or backscatter devices~\cite{zhang2020robot} exist. However, these RF technologies are not as ubiquitously deployed and have limited ranges compared to WiFi. 
We note that, extension of \name's WiFi implementation to other RF-sensors is trivial, as we abstract bearing as the measurement feature of the WiFi sensor's measurement. 
Thus, as long as they are able to measure AoAs~\cite{zhao2021uloc} to and/or from the robot to fixed access points in the environment any RF system can make use of \name's implementation.


\noindent\textbf{WiFi-SLAM:} There are a few existing works~\cite{hashemifar2019augmenting, liu2019collaborative,huang2011efficient,ferris2007wifi,hashemifar2019augmenting, liu2019collaborative} that try to utilize WiFi sensor readings to improve SLAM algorithms. Unfortunately, most of these works utilize RSSI as the features metric which needs intense mapping of the space and are known to vary drastically in dynamic indoor scenarios~\cite{ma2019wifi}, making them unsuitable metrics for WiFi signals.
While there are recent works~\cite{jadhav2020wsr,arun2022p2slam} that utilize bearing measurements for their SLAM implementations, WSR~\cite{jadhav2020wsr} does not perform localization but just robot reconnaissance. On the other hand, $\mathrm{P^2}$SLAM~\cite{arun2022p2slam} does not provide any maps of the surroundings and performs an end-to-end optimization which does not help in making real-time awareness to the robots for example to avoid crashes into other robots or humans. In contrast, \name uses camera features for providing real-time context to in-tandem WiFi bearing measurements that are enabling accurate localization of the robot.

% \noindent\textbf{RF Localization:} Past two decades of research in RF-based localization, does not SLAM but only localization and tracking~\cite{spotfi,arraytrack,soltanaghaei2018multipath,ayyalasomayajula2020deep, ma2019wifi} of either the source or the receiving sensor. In contrast, \name integrates WiFi with camera to Simultaneously Locate the bot and Map the environment, without assuming any prior information about locations in the environment.
